Accessible fragments of generalized probabilistic theories, cone equivalence, and applications to witnessing nonclassicality

The formalism of generalized probabilistic theories (GPTs) was originally developed as a way to characterize the landscape of conceivable physical theories. Thus, the GPT describing a given physical theory necessarily includes all physically possible processes. We here consider the question of how to provide a GPT-like characterization of a particular experimental setup within a given physical theory. We show that the resulting characterization is not generally a GPT in and of itself-rather, it is described by a more general mathematical object that we introduce and term an accessible GPT fragment. We then introduce an equivalence relation, termed cone equivalence, between accessible GPT fragments (and, as a special case, between standard GPTs). We give a number of examples of experimental scenarios that are best described using accessible GPT fragments, and where moreover cone-equivalence arises naturally. We then prove that an accessible GPT fragment admits of a classical explanation if and only if every other fragment that is cone-equivalent to it also admits of a classical explanation. Finally, we leverage this result to prove several fundamental results regarding the experimental requirements for witnessing the failure of generalized noncontextuality. In particular, we prove that neither incompatibility among measurements nor the assumption of freedom of choice is necessary for witnessing failures of generalized noncontextuality, and, moreover, that such failures can be witnessed even using arbitrarily inefficient detectors.

==> Diagrams/vectorP.tex <==
\begin{tikzpicture}
	\begin{pgfonlayer}{nodelayer}
		\node [style=none] (5) at (0, 0.5) {};
		\node [style=point] (6) at (0, -0.75) {$s$};
		\node [style=right label] (14) at (0, 0.25) {$S|P$};
	\end{pgfonlayer}
	\begin{pgfonlayer}{edgelayer}
		\draw [qWire] (6) to (5.center);
	\end{pgfonlayer}
\end{tikzpicture}


==> defs.tex <==
\newcommand\nuclear{\omding\char195\xspace}
\newcommand\goodskull{\omding\char194\xspace}

%\newcommand{\C}{\ensuremath{\mathbb{C}}}

\newcommand{\smallsum}{\textstyle{\sum\limits_i}}
\newcommand{\smallsumi}[1]{\textstyle{\sum\limits_{#1}}}

\newcommand{\emptydiag}{\,\tikz{\node[style=empty diagram] (x) {};}\,}
\newcommand{\scalar}[1]{\,\tikz{\node[style=scalar] (x) {$#1$};}\,}
\newcommand{\dscalar}[1]{\,\tikz{\node[style=scalar, doubled] (x) {$#1$};}\,}
\newcommand{\boxmap}[1]{\,\tikz{\node[style=small box] (x) {$#1$};\draw(0,-1)--(x)--(0,1);}\,}
\newcommand{\tboxmap}[3]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=small box] (0) at (0, 0) {$#1$};
    \node [style=none] (1) at (0, -0.5) {};
    \node [style=none] (2) at (0, -1.25) {};
    \node [style=none] (3) at (0, 1.25) {};
    \node [style=none] (4) at (0, 0.5) {};
    \node [style=right label] (5) at (0.25, -1) {$#2$};
    \node [style=right label] (6) at (0.25, 1) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (2.center) to (1.center);
    \draw (4.center) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}}
\newcommand{\boxstate}[1]{\,\tikz{\node[style=small box] (x) {$#1$};\draw(x)--(0,1);}\,}
\newcommand{\boxeffect}[1]{\,\tikz{\node[style=small box] (x) {$#1$};\draw(0,-1)--(x);}\,}
\newcommand{\boxmapTWOtoONE}[1]{\,\tikz{\node[style=small box] (x) {$#1$};\draw(-0.8,-1)--(x)--(0,1);\draw (0.8,-1)--(x);}\,}
\newcommand{\boxmapONEtoTWO}[1]{\,\tikz{\node[style=small box] (x) {$#1$};\draw(0,-1)--(x)--(-1,1);\draw (x)--(1,1);}\,}

\newcommand{\doubleop}{\ensuremath{\textsf{double}}\xspace}

\newcommand{\kscalar}[1]{\,\tikz{\node[style=kscalar] (x) {$#1$};}\,}
\newcommand{\kscalarconj}[1]{\,\tikz{\node[style=kscalarconj] (x) {$#1$};}\,}

\newcommand{\dmap}[1]{\,\tikz{\node[style=dmap] (x) {$#1$};\draw[boldedge] (0,-1.3)--(x)--(0,1.3);}\,}
\newcommand{\dmapdag}[1]{\,\tikz{\node[style=dmapdag] (x) {$#1$};\draw[boldedge] (0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\map}[1]{\,\tikz{\node[style=map] (x) {$#1$};\draw(0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\mapdag}[1]{\,\tikz{\node[style=mapdag] (x) {$#1$};\draw(0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\maptrans}[1]{\,\tikz{\node[style=maptrans] (x) {$#1$};\draw(0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\mapconj}[1]{\,\tikz{\node[style=mapconj] (x) {$#1$};\draw(0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\mapONEtoTWO}[1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=map] (0) at (0, 0) {$#1$};
    \node [style=none] (1) at (0, -0.5) {};
    \node [style=none] (2) at (-0.75, 0.5) {};
    \node [style=none] (3) at (-0.75, 1.25) {};
    \node [style=none] (4) at (0, -1.25) {};
    \node [style=none] (5) at (0.75, 0.5) {};
    \node [style=none] (6) at (0.75, 1.25) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (4.center) to (1.center);
    \draw (2.center) to (3.center);
    \draw (5.center) to (6.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\pointmap}[style=point][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,-0.3) {$#1$};\node [style=none] (3) at (0, 1.0) {};\node [style=none] (3) at (0, -1.0) {};\draw (x)--(0,0.7);}\,}
\newcommand{\graypointmap}[1]{\pointmap[style=gray point]{#1}}

\newcommand{\dpointmap}[1]{\,\tikz{\node[style=point,doubled] (x) at (0,-0.3) {$#1$};\draw[boldedge] (x)--(0,0.7);}\,}
\newcommand{\dcopointmap}[1]{\,\tikz{\node[style=copoint, doubled] (x) at (0,0.3) {$#1$};\draw[boldedge] (x)--(0,-0.7);}\,}

\newcommand{\dpoint}[1]{\,\tikz{\node[style=point,doubled] (x) at (0,-0.3) {$#1$};\draw[boldedge] (x)--(0,0.7);}\,}
\newcommand{\dcopoint}[1]{\,\tikz{\node[style=copoint, doubled] (x) at (0,0.3) {$#1$};\draw[boldedge] (x)--(0,-0.7);}\,}

\newcommand{\kpoint}[1]{\,\tikz{\node[style=kpoint] (x) at (0,-0.05) {$#1$};\draw (x)--(0,0.9);}\,}
\newcommand{\kpointconj}[1]{\,\tikz{\node[style=kpoint conjugate] (x) at (0,-0.05) {$#1$};\draw (x)--(0,0.9);}\,}

\newcommand{\kpointdag}[1]{\,\tikz{\node[style=kpoint adjoint] (x) at (0,0.05) {$#1$};\draw (x)--(0,-0.9);}\,}
\newcommand{\kpointadj}[1]{\kpointdag{#1}}
\newcommand{\kpointtrans}[1]{\,\tikz{\node[style=kpoint transpose] (x) at (0,0.05) {$#1$};\draw (x)--(0,-0.9);}\,}

\newkeycommand{\typedkpoint}[style=kpoint,edgestyle=][2]{%
\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, 1) {};
    \node [style=\commandkey{style}] (1) at (0, -0.75) {$#2$};
    \node [style=right label] (2) at (0.25, 0.5) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [\commandkey{edgestyle}] (1) to (0.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\typedkpointdag}[style=kpoint adjoint,edgestyle=][2]{%
\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1) {};
    \node [style=\commandkey{style}] (1) at (0, 0.75) {$#2$};
    \node [style=right label] (2) at (0.25, -0.5) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [\commandkey{edgestyle}] (0.center) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\typedpoint}[2]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, 1) {};
    \node [style=point] (1) at (0, -0.5) {$#2$};
    \node [style=right label] (2) at (0.25, 0.5) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (1) to (0.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\bistate}[1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=kpoint, minimum width=1 cm, inner sep=2pt] (0) at (0, -0.25) {$#1$};
    \node [style=none] (1) at (-0.75, 0) {};
    \node [style=none] (2) at (0.75, 0) {};
    \node [style=none] (3) at (-0.75, 0.75) {};
    \node [style=none] (4) at (0.75, 0.75) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (1.center) to (3.center);
    \draw (2.center) to (4.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\bistateadj}[1]{\,\begin{tikzpicture}[yshift=-3mm]
  \begin{pgfonlayer}{nodelayer}
    \node [style=kpointadj, minimum width=1 cm, inner sep=2pt] (0) at (0, 0.5) {$\psi$};
    \node [style=none] (1) at (-0.75, 0.25) {};
    \node [style=none] (2) at (0.75, 0.25) {};
    \node [style=none] (3) at (-0.75, -0.5) {};
    \node [style=none] (4) at (0.75, -0.5) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (1.center) to (3.center);
    \draw (2.center) to (4.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\bistatebraket}[2]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=kpoint, minimum width=1 cm, inner sep=2pt] (0) at (0, -0.75) {$#1$};
    \node [style=none] (1) at (-0.75, -0.5) {};
    \node [style=none] (2) at (0.75, -0.5) {};
    \node [style=none] (3) at (-0.75, 0.5) {};
    \node [style=none] (4) at (0.75, 0.5) {};
    \node [style=kpointadj, minimum width=1 cm, inner sep=2pt] (5) at (0, 0.75) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (1.center) to (3.center);
    \draw (2.center) to (4.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\binop}[2]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0.75, -1.25) {};
    \node [style=right label, xshift=1 mm] (1) at (0.75, -1) {$#1$};
    \node [style=none] (2) at (0, 1.25) {};
    \node [style=white dot] (3) at (0, 0) {$#2$};
    \node [style=none] (4) at (-0.75, -1.25) {};
    \node [style=right label] (5) at (-0.5, -1) {$#1$};
    \node [style=right label] (6) at (0.25, 1) {$#1$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [bend right=15, looseness=1.00] (0.center) to (3);
    \draw [bend left=15, looseness=1.00] (4.center) to (3);
    \draw (3) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\dkpoint}[1]{\,\tikz{\node[style=dkpoint] (x) at (0,-0.1) {$#1$};\draw[boldedge] (x)--(0,1);}\,}
\newcommand{\dkpointadj}[1]{\,\tikz{\node[style=dkpointadj] (x) at (0,0.1) {$#1$};\draw[boldedge] (x)--(0,-1);}\,}

\newcommand{\trace}{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -0.75) {};
    \node [style=upground] (1) at (0, 0.75) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw [style=boldedge] (0.center) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

%\newcommand{\namedeq}[1]{%
%\ensuremath{\overset{\,(#1)}{\vphantom{X}=}}\xspace}
%\newcommand{\scalareq}{%
%\ensuremath{\overset{\diamond}{=}}\xspace}

\newkeycommand{\pointketbra}[style1=copoint,style2=point][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.5) {};
    \node [style=\commandkey{style1}] (1) at (0, -0.75) {$#1$};
    \node [style=\commandkey{style2}] (2) at (0, 0.75) {$#2$};
    \node [style=none] (3) at (0, 1.5) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (1);
    \draw (2) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\twocopointketbra}[style1=copoint,style2=copoint,style3=point][3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (-0.75, -1.5) {};
    \node [style=none] (1) at (0.75, -1.5) {};
    \node [style=\commandkey{style1}] (2) at (-0.75, -0.75) {$#1$};
    \node [style=\commandkey{style2}] (3) at (0.75, -0.75) {$#2$};
    \node [style=\commandkey{style3}] (4) at (0, 0.75) {$#3$};
    \node [style=none] (5) at (0, 1.5) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (2);
    \draw (1.center) to (3);
    \draw (4) to (5.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\graytwocopointketbra}{\twocopointketbra[style1=gray copoint,style2=gray copoint,style3=gray point]}

\newkeycommand{\twopointketbra}[style1=copoint,style2=point,style3=point][3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.5) {};
    \node [style=none] (1) at (-0.75, 1.5) {};
    \node [style=\commandkey{style1}] (2) at (0, -0.75) {$#1$};
    \node [style=\commandkey{style2}] (3) at (-0.75, 0.75) {$#2$};
    \node [style=\commandkey{style3}] (4) at (0.75, 0.75) {$#3$};
    \node [style=none] (5) at (0.75, 1.5) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (2);
    \draw (1.center) to (3);
    \draw (4) to (5.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\graytwopointketbra}{\twopointketbra[style1=gray copoint,style2=gray point,style3=gray point]}

\newcommand{\idwire}{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.5) {};
    \node [style=none] (3) at (0, 1.5) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\shortidwire}{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -0.8) {};
    \node [style=none] (3) at (0, 0.8) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\pointbraket}[style1=point,style2=copoint][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -0.5) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0.5) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\graypointbraket}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=gray point] (0) at (0, -0.5) {$#1$};
    \node [style=gray copoint] (1) at (0, 0.5) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\kpointbraket}[style1=kpoint,style2=kpoint adjoint][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -0.75) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0.75) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\kpointbraketconj}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=kpoint conjugate] (0) at (0, -0.75) {$#1$};
    \node [style=kpoint transpose] (1) at (0, 0.75) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\kpointketbra}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -2) {};
    \node [style=kpointdag] (1) at (0, -1) {$#1$};
    \node [style=kpoint] (2) at (0, 1) {$#2$};
    \node [style=none] (3) at (0, 2) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (1);
    \draw (2) to (3.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\boxpointmap}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1.25) {$#1$};
    \node [style=map] (1) at (0, 0) {$#2$};
    \node [style=none] (2) at (0, 1.25) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newcommand{\boxtranspointmap}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1.25) {$#1$};
    \node [style=maptrans] (1) at (0, 0) {$#2$};
    \node [style=none] (2) at (0, 1.25) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newkeycommand{\kpointmap}[style1=kpoint,style2=map][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -1.1) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 0.2) {$#2$};
    \node [style=none] (2) at (0, 1.5) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newcommand{\boxpointmapdag}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1.25) {$#1$};
    \node [style=mapdag] (1) at (0, 0) {$#2$};
    \node [style=none] (2) at (0, 1.25) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2.center);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newcommand{\boxcopointmap}[2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=none] (0) at (0, -1.25) {};
    \node [style=map] (1) at (0, 0) {$#1$};
    \node [style=copoint] (2) at (0, 1.25) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0.center) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
\,}

\newcommand{\sandwichmap}[3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1.25) {$#1$};
    \node [style=map] (1) at (0, 0) {$#2$};
    \node [style=copoint] (2) at (0, 1.25) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newcommand{\kpointsandwichmap}[3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=kpoint] (0) at (0, -1.5) {$#1$};
    \node [style=map] (1) at (0, 0) {$#2$};
    \node [style=kpointdag] (2) at (0, 1.5) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newcommand{\kpointsandwichmapdag}[3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=kpoint] (0) at (0, -1.5) {$#1$};
    \node [style=mapdag] (1) at (0, 0) {$#2$};
    \node [style=kpointdag] (2) at (0, 1.5) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newcommand{\sandwichmapdag}[3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1.25) {$#1$};
    \node [style=mapdag] (1) at (0, 0) {$#2$};
    \node [style=copoint] (2) at (0, 1.25) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newcommand{\sandwichmaptrans}[3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1.25) {$#1$};
    \node [style=maptrans] (1) at (0, 0) {$#2$};
    \node [style=copoint] (2) at (0, 1.25) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newcommand{\sandwichmapconj}[3]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=point] (0) at (0, -1.25) {$#1$};
    \node [style=mapconj] (1) at (0, 0) {$#2$};
    \node [style=copoint] (2) at (0, 1.25) {$#3$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
    \draw (1) to (2);
  \end{pgfonlayer}
\end{tikzpicture}%
}

\newkeycommand{\sandwichtwo}[style1=point,style2=map,style3=map,style4=copoint][4]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style2}] (0) at (0, -0.75) {$#2$};
    \node [style=\commandkey{style3}] (1) at (0, 0.75) {$#3$};
    \node [style=\commandkey{style1}] (2) at (0, -2) {$#1$};
    \node [style=\commandkey{style4}] (3) at (0, 2) {$#4$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (2) to (0);
    \draw (0) to (1);
    \draw (1) to (3);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\longbraket}[style1=point,style2=copoint][2]{\,%
\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=\commandkey{style1}] (0) at (0, -2) {$#1$};
    \node [style=\commandkey{style2}] (1) at (0, 2) {$#2$};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newkeycommand{\onb}[style=point]{\ensuremath{\left\{\tikz{\node[style=\commandkey{style}] (x) at (0,-0.3) {$j$};\draw (x)--(0,0.7);}\right\}}\xspace}

\newcommand{\whiteonb}{\onb[style=point]}

\newcommand{\grayonb}{\onb[style=gray point]}

\newcommand{\redonb}{\onb[style=red point]}

\newcommand{\greenonb}{\onb[style=green point]}


\newkeycommand{\copointmap}[style=copoint][1]{\,\tikz{\node[style=\commandkey{style}] (x) at (0,0.3) {$#1$};\draw (x)--(0,-0.7);}\,}

\newcommand{\redpointmap}[1]{\,\tikz{\node[style=red point] (x) at (0,-0.3) {$#1$};\draw (x)--(0,0.7);}\,}

\newcommand{\redcopointmap}[1]{\,\tikz{\node[style=red copoint] (x) at (0,0.3) {$#1$};\draw (x)--(0,-0.7);}\,}

\newcommand{\greenpointmap}[1]{\,\tikz{\node[style=green point] (x) at (0,-0.3) {$#1$};\draw (x)--(0,0.7);}\,}

\newcommand{\greencopointmap}[1]{\,\tikz{\node[style=green copoint] (x) at (0,0.3) {$#1$};\draw (x)--(0,-0.7);}\,}

% \newkeycommand{\comult}[style=white dot]{\,\begin{tikzpicture}
%   \begin{pgfonlayer}{nodelayer}
%     \node [style=none] (0) at (0, -1) {};
%     \node [style=none] (1) at (-0.75, 1) {};
%     \node [style=\commandkey{style}] (2) at (0, 0) {};
%     \node [style=none] (3) at (0.75, 1) {};
%   \end{pgfonlayer}
%   \begin{pgfonlayer}{edgelayer}
%     \draw [bend left=15, looseness=1.00] (2) to (1.center);
%     \draw (0.center) to (2);
%     \draw [bend right=15, looseness=1.00] (2) to (3.center);
%   \end{pgfonlayer}
% \end{tikzpicture}\,\xspace}

% \newkeycommand{\mult}[style=white dot]{\,\begin{tikzpicture}
%   \begin{pgfonlayer}{nodelayer}
%     \node [style=none] (0) at (0, 1) {};
%     \node [style=none] (1) at (-0.75, -1) {};
%     \node [style=\commandkey{style}] (2) at (0, 0) {};
%     \node [style=none] (3) at (0.75, -1) {};
%   \end{pgfonlayer}
%   \begin{pgfonlayer}{edgelayer}
%     \draw [bend right=15, looseness=1.00] (2) to (1.center);
%     \draw (0.center) to (2);
%     \draw [bend left=15, looseness=1.00] (2) to (3.center);
%   \end{pgfonlayer}
% \end{tikzpicture}\,\xspace}


\newcommand{\grayphasepoint}[1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=grey phase dot] (0) at (0, -0.5) {$#1$};
    \node [style=none] (1) at (0, 1) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\graysquarepoint}[1]{\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=gray square point] (0) at (0, -0.5) {};
        \node [style=none] (1) at (0, 0.75) {};
        \node [style=none] (2) at (0.75, -0.5) {$#1$};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw (0) to (1.center);
    \end{pgfonlayer}
\end{tikzpicture}}

\newcommand{\phase}[2]{\,\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=none] (0) at (0, 1) {};
        \node [style=#1] (2) at (0, -0) {$#2$};
        \node [style=none] (3) at (0, -1) {};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw (2) to (0.center);
        \draw (3.center) to (2);
    \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\dphase}[2]{\,\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=none] (0) at (0, 1) {};
        \node [style=#1] (2) at (0, -0) {$#2$};
        \node [style=none] (3) at (0, -1) {};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw [doubled] (2) to (0.center);
        \draw [doubled] (3.center) to (2);
    \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\measure}[1]{\,\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=none] (0) at (0, 0.5) {};
        \node [style=#1] (2) at (0, -0) {};
        \node [style=none] (3) at (0, -0.5) {};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw (2) to (0.center);
        \draw[doubled] (3.center) to (2);
    \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\prepare}[1]{\,\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=none] (0) at (0, 0.5) {};
        \node [style=#1] (2) at (0, -0) {};
        \node [style=none] (3) at (0, -0.5) {};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw[doubled] (2) to (0.center);
        \draw (3.center) to (2);
    \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\whitephase}[1]{\phase{white phase dot}{#1}}
\newcommand{\whitedphase}[1]{\dphase{white phase ddot}{#1}}
\newcommand{\greyphase}[1]{\phase{grey phase dot}{#1}}
\newcommand{\greydphase}[1]{\dphase{grey phase ddot}{#1}}

\newcommand{\whitephasepoint}[1]{\,\begin{tikzpicture}
  \begin{pgfonlayer}{nodelayer}
    \node [style=white phase dot] (0) at (0, -0.5) {$#1$};
    \node [style=none] (1) at (0, 1) {};
  \end{pgfonlayer}
  \begin{pgfonlayer}{edgelayer}
    \draw (0) to (1.center);
  \end{pgfonlayer}
\end{tikzpicture}\,}

\newcommand{\pointcopointmap}[2]{\,\tikz{
  \node[style=copoint] (x) at (0,-0.7) {$#2$};\draw (x)--(0,-1.5);
  \node[style=point] (y) at (0,0.7) {$#1$};\draw (0,1.5)--(y);
}\,}

\newcommand{\innerprodmap}[2]{\,\tikz{
\node[style=copoint] (y) at (0,0.5) {$#1$};
\node[style=point] (x) at (0,-0.5) {$#2$};
\draw (x)--(y);}\,}

\newcommand{\wginnerprodmap}[2]{\,\begin{tikzpicture}
    \begin{pgfonlayer}{nodelayer}
        \node [style=point] (0) at (0, -0.75) {$#2$};
        \node [style=gray copoint] (1) at (0, 0.75) {$#1$};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
        \draw (0) to (1);
    \end{pgfonlayer}
\end{tikzpicture}\,}

\def\alpvec{[\vec{\alpha}]}
\def\alpprevec{\vec{\alpha}}
\def\betvec{[\vec{\beta}_j]}
\def\betprevec{\vec{\beta}_j}

\def\blackmu{\mu_{\smallblackdot}}
\def\graymu {\mu_{\smallgraydot}}
\def\whitemu{\mu_{\smallwhitedot}}

\def\blacketa{\eta_{\smallblackdot}}
\def\grayeta {\eta_{\smallgraydot}}
\def\whiteeta{\eta_{\smallwhitedot}}

\def\blackdelta{\delta_{\smallblackdot}}
\def\graydelta {\delta_{\smallgraydot}}
\def\whitedelta{\delta_{\smallwhitedot}}

\def\blackepsilon{\epsilon_{\smallblackdot}}
\def\grayepsilon {\epsilon_{\smallgraydot}}
\def\whiteepsilon{\epsilon_{\smallwhitedot}}

% \def\whiteeta{\eta_{\!\smallwhitedot}}
% \def\whitevarepsilon{\varepsilon_{\!\smallwhitedot}}

\def\whitePhi{\Phi_{\!\smallwhitedot}}
\def\graymeas{m_{\!\smallgraydot}}

\newcommand{\Owg}{\ensuremath{{\cal O}_{\!\smallwhitedot\!,\!\smallgraydot}}}
\newcommand{\whiteK}{\ensuremath{{\cal  K}_{\!\smallwhitedot}}}
\newcommand{\grayK}{\ensuremath{{\cal  K}_{\!\smallgraydot}}}




% CATEGORY VARIABLES
\newcommand{\catC}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\catCop}{\ensuremath{\mathcal{C}^{\mathrm{op}}}\xspace}
\newcommand{\catD}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\catDop}{\ensuremath{\mathcal{D}^{\mathrm{op}}}\xspace}


% STANDARD CATEGORIES
\newcommand{\catSet}{\ensuremath{\textrm{\bf Set}}\xspace}
\newcommand{\catRel}{\ensuremath{\textrm{\bf Rel}}\xspace}
\newcommand{\catFRel}{\ensuremath{\textrm{\bf FRel}}\xspace}
\newcommand{\catVect}{\ensuremath{\textrm{\bf Vect}}\xspace}
\newcommand{\catFVect}{\ensuremath{\textrm{\bf FVect}}\xspace}
\newcommand{\catFHilb}{\ensuremath{\textrm{\bf FHilb}}\xspace}
\newcommand{\catHilb}{\ensuremath{\textrm{\bf Hilb}}\xspace}
\newcommand{\catSuperHilb}{\ensuremath{\textrm{\bf SuperHilb}}\xspace}
\newcommand{\catAb}{\ensuremath{\textrm{\bf Ab}}\xspace}
\newcommand{\catTop}{\ensuremath{\textrm{\bf Top}}\xspace}
\newcommand{\catCHaus}{\ensuremath{\textrm{\bf CHaus}}\xspace}
\newcommand{\catHaus}{\ensuremath{\textrm{\bf Haus}}\xspace}
\newcommand{\catGraph}{\ensuremath{\textrm{\bf Graph}}\xspace}
\newcommand{\catMat}{\ensuremath{\textrm{\bf Mat}}\xspace}
\newcommand{\catGr}{\ensuremath{\textrm{\bf Gr}}\xspace}
\newcommand{\catSpek}{\ensuremath{\textrm{\bf Spek}}\xspace}




% ========================
% = COMMUTATIVE DIAGRAMS =
% ========================

\tikzstyle{cdiag}=[matrix of math nodes, row sep=3em, column sep=3em, text height=1.5ex, text depth=0.25ex,inner sep=0.5em]
\tikzstyle{arrow above}=[transform canvas={yshift=0.5ex}]
\tikzstyle{arrow below}=[transform canvas={yshift=-0.5ex}]

\newcommand{\csquare}[8]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2);
\end{tikzpicture}
}

% commands for putting pushout/pullback brackets on commutative diags
\newcommand{\NWbracket}[1]{%
\draw #1 +(-0.25,0.5) -- +(-0.5,0.5) -- +(-0.5,0.25);}
\newcommand{\NEbracket}[1]{%
\draw #1 +(0.25,0.5) -- +(0.5,0.5) -- +(0.5,0.25);}
\newcommand{\SWbracket}[1]{%
\draw #1 +(-0.25,-0.5) -- +(-0.5,-0.5) -- +(-0.5,-0.25);}
\newcommand{\SEbracket}[1]{%
\draw #1 +(0.25,-0.5) -- +(0.5,-0.5) -- +(0.5,-0.25);}
\newcommand{\THETAbracket}[2]{%
\draw [rotate=#1] #2 +(0.25,0.5) -- +(0.5,0.5) -- +(0.5,0.25);}

\newcommand{\posquare}[8]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node [swap] {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2);
    \NWbracket{(m-2-2)}
\end{tikzpicture}
}

\newcommand{\pbsquare}[8]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node [swap] {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2);
  \SEbracket{(m-1-1)}
\end{tikzpicture}
}

\newcommand{\ctri}[6]{
    \begin{tikzpicture}[-latex]
        \matrix (m) [cdiag,ampersand replacement=\&] { #1 \& #2 \\ #3 \& \\ };
        \path [arrs] (m-1-1) edge node {$#4$} (m-1-2)
              (m-1-1) edge node [swap] {$#5$} (m-2-1)
              (m-2-1) edge node [swap] {$#6$} (m-1-2);
    \end{tikzpicture}
}

% \newcommand{\crun}[5]{
% \ensuremath{#1 \overset{#2}{\longrightarrow} #3 \overset{#4}{\longrightarrow} #5}
% }

\newcommand{\carr}[3]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #3 \\};
    \path [arrs] (m-1-1) edge node {$#2$} (m-1-2);
\end{tikzpicture}
}

\newcommand{\crun}[5]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #3 \& #5 \\};
    \path [arrs] (m-1-1) edge node {$#2$} (m-1-2)
                 (m-1-2) edge node {$#4$} (m-1-3);
\end{tikzpicture}
}

\newcommand{\cspan}[5]{
\ensuremath{#1 \overset{#2}{\longleftarrow} #3
               \overset{#4}{\longrightarrow} #5}
}

\newcommand{\ccospan}[5]{
\ensuremath{#1 \overset{#2}{\longrightarrow} #3
               \overset{#4}{\longleftarrow} #5}
}

\newcommand{\cpair}[4]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\};
    \path [arrs] (m-1-1.20) edge node {$#3$} (m-1-2.160)
                 (m-1-1.-20) edge node [swap] {$#4$} (m-1-2.-160);
\end{tikzpicture}
}

\newcommand{\csquareslant}[9]{
\begin{tikzpicture}[-latex]
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2)
                 (m-1-2) edge node [swap] {$#9$} (m-2-1);
\end{tikzpicture}
}




==> mab2bib/myfile.tex <==
@control{REVTEX42Control,
}
@control{apsrev42Control,
	title        = {{0}},
	year         = 1,
	pages        = {0},
	editor       = {0}
}
@misc{lami2018non,
	title        = {Non-classical correlations in quantum mechanics and beyond},
	author       = {Lami, Ludovico},
	year         = 2018,
	publisher    = {arXiv},
	doi          = {10.48550/ARXIV.1803.02902},
	url          = {https://arxiv.org/abs/1803.02902},
	copyright    = {arXiv.org perpetual, non-exclusive license},
}
@misc{selby2022open,
	title        = {An open-source linear program for testing nonclassicality},
	author       = {Selby, John H. and Wolfe, Elie and Schmid, David and Sainz, Ana Belén},
	year         = 2022,
	publisher    = {arXiv},
	doi          = {10.48550/ARXIV.2204.11905},
	url          = {https://arxiv.org/abs/2204.11905},
	copyright    = {arXiv.org perpetual, non-exclusive license}
}
@book{hartkamper1974foundations,
	title        = {{Foundations of quantum mechanics and ordered linear spaces}},
	author       = {Hartk{\"a}mper, Alois and Neumann, Hans},
	year         = 1974,
	volume       = 29
}
@article{aubrun2021entangleability,
	title        = {{Entangleability of cones}},
	author       = {Aubrun, Guillaume and Lami, Ludovico and Palazuelos, Carlos and Pl{\'a}vala, Martin},
	year         = 2021,
	journal      = {Geometric and Functional Analysis},
	publisher    = {Springer},
	volume       = 31,
	number       = 2,
	pages        = {181--205}
}
@article{muller2021probabilistic,
	title        = {{Probabilistic theories and reconstructions of quantum theory}},
	author       = {M{\"u}ller, Markus},
	year         = 2021,
	journal      = {SciPost Physics Lecture Notes},
	pages        = {028}
}
@misc{mueller2021testing,
	title        = {Testing quantum theory with generalized noncontextuality},
	author       = {M{\"u}ller, Markus P. and Garner, Andrew J. P.},
	year         = 2021,
	publisher    = {arXiv},
	doi          = {10.48550/ARXIV.2112.09719},
	url          = {https://arxiv.org/abs/2112.09719},
	copyright    = {arXiv.org perpetual, non-exclusive license}
}
@misc{garner2020characterization,
	title        = {{Characterization of the probabilistic models that can be embedded in quantum theory}},
	author       = {Andrew J. P. Garner and Markus P. M{\"u}ller},
	year         = 2020,
	eprint       = {2004.06136},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@misc{grabowecky2021experimentally,
	title        = {{Experimentally bounding deviations from quantum theory for a photonic three-level system using theory-agnostic tomography}},
	author       = {Michael Grabowecky and Christopher Pollack and Andrew Cameron and Robert Spekkens and Kevin Resch},
	year         = 2021,
	eprint       = {2108.05864},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@misc{daley2021experimentally,
	title        = {{Experimentally adjudicating between different causal accounts of Bell inequality violations via statistical model selection}},
	author       = {Patrick J. Daley and Kevin J. Resch and Robert W. Spekkens},
	year         = 2021,
	eprint       = {2108.00053},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{dariano2014determinism,
	title        = {{Determinism without causality}},
	author       = {D'Ariano, GM and Manessi, Franco and Perinotti, Paolo},
	year         = 2014,
	journal      = {Physica Scripta},
	publisher    = {IOP Publishing},
	volume       = 2014,
	number       = {T163},
	pages        = {014013},
	url          = {https://iopscience.iop.org/article/10.1088/0031-8949/2014/T163/014013}
}
@article{HMZ16,
	title        = {{An invitation to quantum incompatibility}},
	author       = {Heinosaari, Teiko and Miyadera, Takayuki and Ziman, M{\'a}rio},
	year         = 2016,
	journal      = {J. Phys. A},
	publisher    = {IOP Publishing},
	volume       = 49,
	number       = 12,
	pages        = 123001,
	doi          = {10.1088/1751-8113/49/12/123001},
	url          = {https://doi.org/10.1088/1751-8113/49/12/123001}
}
@incollection{wiseman2017causarum,
	title        = {{Causarum Investigatio and the two Bell’s theorems of John Bell}},
	author       = {Wiseman, Howard M and Cavalcanti, Eric G},
	year         = 2017,
	booktitle    = {Quantum [Un] Speakables II},
	publisher    = {Springer},
	pages        = {119--142},
	url          = {https://doi.org/10.1007/978-3-319-38987-5_6}
}
@article{pusey2019contextuality,
	title        = {{Contextuality without access to a tomographically complete set}},
	author       = {Pusey, Matthew F and Del Rio, Lidia and Meyer, Bettina},
	year         = 2019,
	journal      = {arXiv:1904.08699},
	url          = {https://arxiv.org/abs/1904.08699}
}
@misc{simplex_forthcoming,
	author       = {John H. Selby and David Schmid and Elie Wolfe and Ana Belén Sainz and Ravi Kunjwal and Robert W. Spekkens},
	note         = {Forthcoming}
}
@misc{selby2021incompatibility,
	title        = {{Contextuality without incompatibility}},
	author       = {John H. Selby and David Schmid and Elie Wolfe and Ana Belén Sainz and Ravi Kunjwal and Robert W. Spekkens},
	year         = 2021,
	eprint       = {2106.09045},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{plavala2016all,
	title        = {{All measurements in a probabilistic theory are compatible if and only if the state space is a simplex}},
	author       = {Pl{\'a}vala, Martin},
	year         = 2016,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 94,
	number       = 4,
	pages        = {042108},
	doi          = {10.1103/PhysRevA.94.042108},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.94.042108}
}
@misc{plavala2021general,
	title        = {{General probabilistic theories: An introduction}},
	author       = {Pl{\'a}vala, Martin},
	year         = 2021,
	eprint       = {2103.07469},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{sainz2018almost,
	title        = {{Almost-quantum correlations violate the no-restriction hypothesis}},
	author       = {Sainz, Ana Bel{\'e}n and Guryanova, Yelena and Ac{\'\i}n, Antonio and Navascu{\'e}s, Miguel},
	year         = 2018,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 120,
	number       = 20,
	pages        = 200402,
	doi          = {10.1103/PhysRevLett.120.200402},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.120.200402}
}
@misc{singh2021revealing,
	title        = {{Revealing quantum contextuality using a single measurement device by generalizing measurement non-contextuality}},
	author       = {Jaskaran Singh and Arvind},
	year         = 2021,
	eprint       = {2102.00410},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{navascues2015almost,
	title        = {{Almost quantum correlations}},
	author       = {Navascu{\'e}s, Miguel and Guryanova, Yelena and Hoban, Matty J and Ac{\'\i}n, Antonio},
	year         = 2015,
	journal      = {Nature communications},
	publisher    = {Nature Publishing Group},
	volume       = 6,
	number       = 1,
	pages        = {1--7},
	url          = {https://www.nature.com/articles/ncomms7288}
}
@article{baldijao2021noncontextuality,
	title        = {{Emergence of Noncontextuality under Quantum Darwinism}},
	author       = {Baldij\~ao, Roberto D. and Wagner, Rafael and Duarte, Cristhiano and Amaral, B\'arbara and Cunha, Marcelo Terra},
	year         = 2021,
	month        = {Sep},
	journal      = {PRX Quantum},
	publisher    = {American Physical Society},
	volume       = 2,
	pages        = {030351},
	doi          = {10.1103/PRXQuantum.2.030351},
	url          = {https://link.aps.org/doi/10.1103/PRXQuantum.2.030351},
	issue        = 3,
	numpages     = 17
}
@article{contextmetrology,
	title        = {{Certifying Quantum Signatures in Thermodynamics and Metrology via Contextuality of Quantum Linear Response}},
	author       = {Lostaglio, Matteo},
	year         = 2020,
	month        = {Dec},
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 125,
	pages        = 230603,
	doi          = {10.1103/PhysRevLett.125.230603},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.125.230603},
	issue        = 23,
	numpages     = 6
}
@misc{wright2020general,
	title        = {{General Probabilistic Theories with a Gleason-type Theorem}},
	author       = {Wright, Victoria J and Weigert, Stefan},
	year         = 2021,
	month        = nov,
	journal      = {{Quantum}},
	publisher    = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
	volume       = 5,
	pages        = 588,
	doi          = {10.22331/q-2021-11-25-588},
	issn         = {2521-327X},
	url          = {https://doi.org/10.22331/q-2021-11-25-588}
}
@article{filippov2020operational,
	title        = {{Operational restrictions in general probabilistic theories}},
	author       = {Filippov, Sergey N and Gudder, Stan and Heinosaari, Teiko and Lepp{\"a}j{\"a}rvi, Leevi},
	year         = 2020,
	journal      = {Found. Phys.},
	publisher    = {Springer},
	pages        = {1--27},
	doi          = {10.1007/s10701-020-00352-6}
}
@incollection{sep-category-mistakes,
	title        = {{Category Mistakes}},
	author       = {Magidor, Ofra},
	year         = 2019,
	booktitle    = {The Stanford Encyclopedia of Philosophy},
	publisher    = {Metaphysics Research Lab, Stanford University},
	url          = {https://plato.stanford.edu/archives/fall2019/entries/category-mistakes/},
	editor.hide  = {Edward N. Zalta},
	howpublished = {\url{https://plato.stanford.edu/entries/category-mistakes}},
	edition.hide = {Fall 2019}
}
@misc{BarnumLami,
	title        = {{Classical embeddability of general probabilistic theories}},
	author       = {Barnum, Howard and Lami, Ludovico},
	howpublished = {Forthcoming.}
}
@article{cabello1998proposed,
	title        = {{Proposed Experimental Tests of the Bell-Kochen-Specker Theorem}},
	author       = {Cabello, Ad\'an and Garc\'{\i}a-Alcaine, Guillermo},
	year         = 1998,
	month        = mar,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 80,
	pages        = {1797--1799},
	doi          = {10.1103/PhysRevLett.80.1797},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.80.1797},
	issue        = 9,
	numpages     = {0}
}
@article{cabello2000kochen,
	title        = {{Kochen--Specker theorem and experimental test on hidden variables}},
	author       = {Cabello, Ad{\'a}n},
	year         = 2000,
	journal      = {Int. J. Mod. Phys. A},
	publisher    = {World Scientific},
	volume       = 15,
	number       = 18,
	pages        = {2813--2820},
	doi          = {10.1142/S0217751X00002020}
}
@misc{Woods2020,
	title        = {{Solvable Criterion for the Contextuality of any Prepare-and-Measure Scenario}},
	author       = {Victor Gitton and Mischa P. Woods},
	year         = 2021,
	eprint       = {2003.06426},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{simon2000feasible,
	title        = {{Feasible ``Kochen-Specker'' Experiment with Single Particles}},
	author       = {Simon, Christoph and \ifmmode \dot{Z}\else \.{Z}\fi{}ukowski, Marek and Weinfurter, Harald and Zeilinger, Anton},
	year         = 2000,
	month        = aug,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 85,
	pages        = {1783--1786},
	doi          = {10.1103/PhysRevLett.85.1783},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.85.1783},
	issue        = 9,
	numpages     = {0}
}
@article{simon2001hidden,
	title        = {{Hidden-Variable Theorems for Real Experiments}},
	author       = {Simon, Christoph and Brukner, \ifmmode \check{C}\else \v{C}\fi{}aslav and Zeilinger, Anton},
	year         = 2001,
	month        = may,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 86,
	pages        = {4427--4430},
	doi          = {10.1103/PhysRevLett.86.4427},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.86.4427},
	issue        = 20,
	numpages     = {0}
}
@article{larsson2002kochen,
	title        = {{A Kochen-Specker inequality}},
	author       = {Jan-{\AA}ke Larsson},
	year         = 2002,
	month        = jun,
	journal      = {Europhys. Lett.},
	publisher    = {{IOP} Publishing},
	volume       = 58,
	number       = 6,
	pages        = {799--805},
	doi          = {10.1209/epl/i2002-00444-0},
	url          = {https://doi.org/10.1209/epl/i2002-00444-0}
}
@article{cabello2008proposed,
	title        = {{Proposed Experiment for Testing Quantum Contextuality with Neutrons}},
	author       = {Cabello, Ad\'an and Filipp, Stefan and Rauch, Helmut and Hasegawa, Yuji},
	year         = 2008,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 100,
	pages        = 130404,
	doi          = {10.1103/PhysRevLett.100.130404},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.100.130404},
	issue        = 13,
	numpages     = 4
}
@article{PuseydelRio,
	title        = {{Contextuality without access to a tomographically complete set}},
	author       = {{Pusey}, Matthew F. and {del Rio}, L{\'\i}dia and {Meyer}, Bettina},
	year         = 2019,
	month        = apr,
	journal      = {arXiv:1904.08699},
	url          = {https://arxiv.org/abs/1904.08699},
	eid.hide     = {arXiv:1904.08699},
	pages.hide   = {arXiv:1904.08699},
	archiveprefix = {arXiv},
	eprint.hide  = {1904.08699},
	primaryclass = {quant-ph},
	adsurl       = {https://ui.adsabs.harvard.edu/abs/2019arXiv190408699P},
	adsnote      = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{POM,
	title        = {{Preparation Contextuality Powers Parity-Oblivious Multiplexing}},
	author       = {Spekkens, Robert W. and Buzacott, D. H. and Keehn, A. J. and Toner, Ben and Pryde, G. J.},
	year         = 2009,
	month        = jan,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 102,
	pages        = {010401},
	doi          = {10.1103/PhysRevLett.102.010401},
	url          = {http://link.aps.org/doi/10.1103/PhysRevLett.102.010401},
	issue        = 1,
	numpages     = 4
}
@article{PBRexp,
	title        = {{Measurements on the reality of the wavefunction}},
	author       = {Ringbauer, M. and Duffus, B. and Branciard, C. and Cavalcanti, E. G. and White, A. G. and Fedrizzi, A.},
	year         = 2015,
	month        = mar,
	journal      = {Nat Phys},
	publisher    = {Nature Publishing Group},
	volume       = 11,
	number       = 3,
	pages        = {249--254},
	issn         = {1745-2473},
	url          = {http://dx.doi.org/10.1038/nphys3233},
	note         = {Article}
}
@article{Bellreview,
	title        = {{Bell nonlocality}},
	author       = {Brunner, Nicolas and Cavalcanti, Daniel and Pironio, Stefano and Scarani, Valerio and Wehner, Stephanie},
	year         = 2014,
	month        = apr,
	journal      = {Rev. Mod. Phys.},
	publisher    = {American Physical Society},
	volume       = 86,
	pages        = {419--478},
	doi          = {10.1103/RevModPhys.86.419},
	url          = {https://link.aps.org/doi/10.1103/RevModPhys.86.419},
	issue        = 2,
	numpages     = 60
}
@inbook{epistricted,
	title        = {{Quasi-Quantization: Classical Statistical Theories with an Epistemic Restriction}},
	author       = {Spekkens, Robert W.},
	year         = 2016,
	booktitle    = {{Quantum Theory: Informational Foundations and Foils}},
	publisher    = {Springer Netherlands},
	address      = {Dordrecht},
	pages        = {83--135},
	doi          = {10.1007/978-94-017-7303-4_4},
	isbn         = {978-94-017-7303-4},
	editor       = {Chiribella, Giulio and Spekkens, Robert W.}
}
@article{Bell2,
	title        = {{On the Problem of Hidden Variables in Quantum Mechanics}},
	author       = {Bell, John S.},
	year         = 1966,
	month        = jul,
	journal      = {Rev. Mod. Phys.},
	publisher    = {American Physical Society},
	volume       = 38,
	pages        = {447--452},
	doi          = {10.1103/RevModPhys.38.447},
	url          = {http://link.aps.org/doi/10.1103/RevModPhys.38.447},
	issue        = 3,
	numpages     = {0}
}
@article{Chaves,
	title        = {{Polynomial Bell Inequalities}},
	author       = {Chaves, Rafael},
	year         = 2016,
	month        = jan,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 116,
	pages        = {010402},
	doi          = {10.1103/PhysRevLett.116.010402},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.116.010402},
	issue        = 1,
	numpages     = 6
}
@article{Budroni2012,
	title        = {{Bell inequalities from variable-elimination methods}},
	author       = {Costantino Budroni and Adan Cabello},
	year         = 2012,
	journal      = {J. Phys. A},
	volume       = 45,
	number       = 38,
	pages        = 385304,
	url          = {http://stacks.iop.org/1751-8121/45/i=38/a=385304}
}
@article{parable,
	title        = {{Specker's parable of the overprotective seer: A road to contextuality, nonlocality and complementarity}},
	author       = {Yeong-Cherng Liang and Robert W. Spekkens and Howard M. Wiseman},
	year         = 2011,
	journal      = {Physics Reports},
	volume       = 506,
	number       = 1,
	pages        = {1--39},
	issn         = {0370-1573},
	url          = {http://www.sciencedirect.com/science/article/pii/S0370157311001517},
	note         = {},
	doi.hide     = {10.1016/j.physrep.2011.05.001}
}
@article{AFLS,
	title        = {{A Combinatorial Approach to Nonlocality and Contextuality}},
	author       = {Ac{\'i}n, Antonio and Fritz, Tobias and Leverrier, Anthony and Sainz, Ana Bel{\'e}n},
	year         = 2015,
	journal      = {Comm. Mathe. Phys.},
	volume       = 334,
	number       = 2,
	pages        = {533--628},
	doi          = {10.1007/s00220-014-2260-1},
	issn         = {1432-0916},
	url          = {http://dx.doi.org/10.1007/s00220-014-2260-1}
}
@article{CSW,
	title        = {{Graph-Theoretic Approach to Quantum Correlations}},
	author       = {Cabello, Ad\'an and Severini, Simone and Winter, Andreas},
	year         = 2014,
	month        = jan,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 112,
	pages        = {040401},
	doi          = {10.1103/PhysRevLett.112.040401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.112.040401},
	issue        = 4,
	numpages     = 5
}
@article{merminsquare,
	title        = {{Deriving robust noncontextuality inequalities from algebraic proofs of the Kochen-Specker theorem: the Peres-Mermin square}},
	author       = {{Krishna}, A. and {Spekkens}, R.~W. and {Wolfe}, E.},
	year         = 2017,
	month        = apr,
	journal      = {arXiv:1704.01153},
	url          = {http://arxiv.org/abs/1704.01153},
	archiveprefix = {arXiv},
	eprint.hide  = {1704.01153},
	primaryclass = {quant-ph},
	adsnote      = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{ChavesGrossLuft,
	title        = {{Causal structures from entropic information: geometry and novel scenarios}},
	author       = {Rafael Chaves and Lukas Luft and David Gross},
	year         = 2014,
	journal      = {New J. Phys.},
	volume       = 16,
	number       = 4,
	pages        = {043001},
	url          = {http://stacks.iop.org/1367-2630/16/i=4/a=043001}
}
@article{browne,
	title        = {{Computational Power of Correlations}},
	author       = {Anders, Janet and Browne, Dan E.},
	year         = 2009,
	month        = feb,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 102,
	pages        = {050502},
	doi          = {10.1103/PhysRevLett.102.050502},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.102.050502},
	issue        = 5,
	numpages     = 4
}
@mastersthesis{Anirudh,
	title        = {{Experimentally Testable Noncontextuality Inequalities Via Fourier-Motzkin Elimination}},
	author       = {{Krishna, Anirudh}},
	year         = 2015,
	publisher    = {UWSpace},
	url          = {http://hdl.handle.net/10012/9752},
	school       = {University of Waterloo}
}
@article{inflation,
	title        = {{The Inflation Technique for Causal Inference with Latent Variables}},
	author       = {Elie Wolfe and Robert W. Spekkens and Tobias Fritz},
	year         = 2016,
	month        = sep,
	journal      = {arXiv:1609.00672},
	url          = {http://arxiv.org/abs/1609.00672}
}
@article{KS,
	title        = {{The problem of hidden variables in quantum mechanics}},
	author       = {Simon Kochen and Ernst Specker},
	year         = 1967,
	journal      = {J. Math. \& Mech.},
	volume       = 17,
	pages        = {59--87},
	doi          = {10.1007/978-94-010-1795-4\_17},
	issn         = {0022-2518},
	note         = {Also available from the \href[pdfnewwindow]{http://www.iumj.indiana.edu/IUMJ/fulltext.php?year=1968\&volume=17\&artid=17004}{Indiana Univ. Math. J.}},
	coden        = {IUMJAB}
}
@article{LeeSpekkens,
	title        = {{Causal inference via algebraic geometry: feasibility tests for functional causal structures with two binary observed variables}},
	author       = {CiarÃ¡n M. Lee and Robert W. Spekkens},
	year         = 2015,
	month        = jun,
	journal      = {arXiv:1506.03880},
	url          = {http://arxiv.org/abs/1506.03880}
}
@article{Bennett,
	title        = {{Quantum cryptography using any two nonorthogonal states}},
	author       = {Bennett, Charles H.},
	year         = 1992,
	month        = may,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 68,
	pages        = {3121--3124},
	doi          = {10.1103/PhysRevA.59.1070},
	url          = {http://link.aps.org/doi/10.1103/PhysRevLett.68.3121},
	issue        = 21,
	numpages     = {0},
	doi.hide     = {10.1103/PhysRevLett.68.3121}
}
@article{randomness,
	title        = {{Certified randomness in quantum physics}},
	author       = {Acin, Antonio and Masanes, Llu{\'\i}s},
	year         = 2016,
	month        = dec,
	day          = {08},
	journal      = {Nature},
	publisher    = {Macmillan Publishers Limited, part of Springer Nature. All rights reserved.},
	volume       = 540,
	number       = 7632,
	pages        = {213--219},
	doi          = {10.1038/nature20119},
	issn         = {0028-0836}
}
@article{Harrigan,
	title        = {{Einstein, Incompleteness, and the Epistemic View of quantum states}},
	author       = {Harrigan, Nicholas and Spekkens, Robert W.},
	year         = 2010,
	journal      = {Found. Phys.},
	volume       = 40,
	number       = 2,
	pages        = {125--157},
	doi          = {10.1007/s10701-009-9347-0},
	issn         = {1572-9516}
}
@article{comm,
	title        = {{Nonlocality and communication complexity}},
	author       = {Buhrman, Harry and Cleve, Richard and Massar, Serge and de Wolf, Ronald},
	year         = 2010,
	month        = mar,
	journal      = {Rev. Mod. Phys.},
	publisher    = {American Physical Society},
	volume       = 82,
	pages        = {665--698},
	doi          = {10.1103/RevModPhys.82.665},
	url          = {http://link.aps.org/doi/10.1103/RevModPhys.82.665},
	issue        = 1,
	numpages     = {0}
}
@article{Maroney,
	title        = {{How statistical are quantum states?}},
	author       = {O. J. E. Maroney},
	year         = 2012,
	month        = jul,
	journal      = {arXiv:1207.6906},
	url          = {http://arxiv.org/abs/1207.6906}
}
@article{Leifer,
	title        = {{Maximally Epistemic Interpretations of the Quantum State and Contextuality}},
	author       = {Leifer, M. S. and Maroney, O. J. E.},
	year         = 2013,
	month        = mar,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 110,
	pages        = 120401,
	url          = {http://link.aps.org/doi/10.1103/PhysRevLett.110.120401},
	issue        = 12,
	numpages     = 5,
	doi.hide     = {10.1103/PhysRevLett.110.120401}
}
@article{DIQKD,
	title        = {{No Signaling and Quantum Key Distribution}},
	author       = {Barrett, Jonathan and Hardy, Lucien and Kent, Adrian},
	year         = 2005,
	month        = jun,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 95,
	pages        = {010503},
	url          = {http://link.aps.org/doi/10.1103/PhysRevLett.95.010503},
	issue        = 1,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.95.010503}
}
@article{zeroerror,
	title        = {{Improving Zero-Error Classical Communication with Entanglement}},
	author       = {Cubitt, Toby S. and Leung, Debbie and Matthews, William and Winter, Andreas},
	year         = 2010,
	month        = jun,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 104,
	pages        = 230503,
	url          = {http://link.aps.org/doi/10.1103/PhysRevLett.104.230503},
	issue        = 23,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.104.230503}
}
@article{Barrett2,
	title        = {{No $\ensuremath\psi$-Epistemic Model Can Fully Explain the Indistinguishability of Quantum States}},
	author       = {Barrett, Jonathan and Cavalcanti, Eric G. and Lal, Raymond and Maroney, Owen J. E.},
	year         = 2014,
	month        = jun,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 112,
	pages        = 250403,
	url          = {http://link.aps.org/doi/10.1103/PhysRevLett.112.250403},
	issue        = 25,
	numpages     = 6,
	doi.hide     = {10.1103/PhysRevLett.112.250403}
}
@article{gencontext,
	title        = {{Contextuality for preparations, transformations, and unsharp measurements}},
	author       = {Spekkens, R. W.},
	year         = 2005,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 71,
	pages        = {052108},
	url          = {http://link.aps.org/doi/10.1103/PhysRevA.71.052108},
	issue        = 5,
	numpages     = 17,
	doi.hide     = {10.1103/PhysRevA.71.052108}
}
@article{CHSH,
	title        = {{Proposed Experiment to Test Local Hidden-Variable Theories}},
	author       = {Clauser, John F. and Horne, Michael A. and Shimony, Abner and Holt, Richard A.},
	year         = 1969,
	month        = oct,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 23,
	pages        = {880--884},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.23.880},
	issue        = 15,
	numpages     = {0},
	doi.hide     = {10.1103/PhysRevLett.23.880}
}
@article{Bell,
	title        = {{On the Einstein Podolsky Rosen paradox}},
	author       = {Bell, J. S.},
	year         = 1964,
	month        = nov,
	journal      = {Physics},
	publisher    = {American Physical Society},
	volume       = 1,
	pages        = {195--200},
	doi          = {10.1103/PhysicsPhysiqueFizika.1.195},
	url          = {https://link.aps.org/doi/10.1103/PhysicsPhysiqueFizika.1.195},
	issue        = 3,
	numpages     = 6
}
@article{negativity,
	title        = {{Negativity and Contextuality are Equivalent Notions of Nonclassicality}},
	author       = {Spekkens, Robert W.},
	year         = 2008,
	month        = jul,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 101,
	pages        = {020401},
	url          = {http://link.aps.org/doi/10.1103/PhysRevLett.101.020401},
	issue        = 2,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.101.020401}
}
@article{Beltrametti_1995,
	title        = {{A classical extension of quantum mechanics}},
	author       = {E G Beltrametti and S Bugajski},
	year         = 1995,
	month        = jun,
	journal      = {J. Phys. A},
	publisher    = {{IOP} Publishing},
	volume       = 28,
	number       = 12,
	pages        = {3329--3343},
	doi          = {10.1088/0305-4470/28/12/007},
	url          = {https://doi.org/10.1088%2F0305-4470%2F28%2F12%2F007}
}
@article{Ferrie_2008,
	title        = {{Frame representations of quantum mechanics and the necessity of negativity in quasi-probability representations}},
	author       = {Christopher Ferrie and Joseph Emerson},
	year         = 2008,
	month        = jul,
	journal      = {J. Phys. A},
	publisher    = {{IOP} Publishing},
	volume       = 41,
	number       = 35,
	pages        = 352001,
	doi          = {10.1088/1751-8113/41/35/352001},
	url          = {https://doi.org/10.1088%2F1751-8113%2F41%2F35%2F352001}
}
@article{Bohm,
	title        = {{A Suggested Interpretation of the Quantum Theory in Terms of "Hidden" Variables. I}},
	author       = {Bohm, David},
	year         = 1952,
	month        = jan,
	journal      = {Phys. Rev.},
	booktitle    = {The {Stanford} Encyclopedia of Philosophy},
	publisher    = {American Physical Society},
	volume       = 85,
	pages        = {166--179},
	doi          = {10.1103/PhysRev.85.166},
	url          = {https://link.aps.org/doi/10.1103/PhysRev.85.166},
	issue        = 2,
	numpages     = {0},
	editor       = {Edward N. Zalta},
	edition      = {Summer 2017}
}
@misc{Leibniz,
	title        = {{The ontological identity of empirical indiscernibles: Leibniz's methodological principle and its significance in the work of Einstein}},
	author       = {{Spekkens}, Robert W.},
	year         = 2019,
	eprint       = {1909.04628},
	archiveprefix = {arXiv},
	primaryclass = {physics.hist-ph}
}
}
@article{AWV,
	title        = {{Anomalous Weak Values Are Proofs of Contextuality}},
	author       = {Pusey, Matthew F.},
	year         = 2014,
	month        = nov,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 113,
	pages        = 200401,
	url          = {http://link.aps.org/doi/10.1103/PhysRevLett.113.200401},
	issue        = 20,
	numpages     = 5,
	doi.hide     = {10.1103/PhysRevLett.113.200401}
}
@article{janotta2013generalized,
	title        = {{Generalized probabilistic theories without the no-restriction hypothesis}},
	author       = {Janotta, Peter and Lal, Raymond},
	year         = 2013,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 87,
	number       = 5,
	pages        = {052131},
	doi          = {10.1103/PhysRevA.87.052131},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.87.052131},
	issue        = 5,
	numpages     = 14
}
@article{spekkens2007evidence,
	title        = {{Evidence for the epistemic view of quantum states: A toy theory}},
	author       = {Spekkens, Robert W.},
	year         = 2007,
	month        = mar,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 75,
	number       = 3,
	pages        = {032110},
	url          = {http://link.aps.org/doi/10.1103/PhysRevA.75.032110},
	issue        = 3,
	numpages     = 30,
	doi.hide     = {10.1103/PhysRevA.75.032110}
}
@article{NPA,
	title        = {{A convergent hierarchy of semidefinite programs characterizing the set of quantum correlations}},
	author       = {Miguel Navascues and Stefano Pironio and Antonio Acin},
	year         = 2008,
	journal      = {New J. Phys.},
	volume       = 10,
	number       = 7,
	pages        = {073013},
	url          = {http://stacks.iop.org/1367-2630/10/i=7/a=073013}
}
@article{RAC,
	title        = {{Optimal bounds for parity-oblivious random access codes}},
	author       = {Chailloux, Andre and Kerenidis, Iordanis  and Kundu, Srijita  and Sikora, Jamie},
	year         = 2016,
	journal      = {New J. Phys.},
	volume       = 18,
	number       = 4,
	pages        = {045003},
	url          = {http://stacks.iop.org/1367-2630/18/i=4/a=045003}
}
@article{Saha_2019,
	title        = {{State independent contextuality advances one-way communication}},
	author       = {Debashis Saha and Pawe{\l} Horodecki and Marcin Paw{\l}owski},
	year         = 2019,
	month        = sep,
	journal      = {New J. Phys.},
	publisher    = {{IOP} Publishing},
	volume       = 21,
	number       = 9,
	pages        = {093057},
	doi          = {10.1088/1367-2630/ab4149},
	url          = {https://doi.org/10.1088/2F1367-2630/2Fab4149}
}
@article{GPT_Barrett,
	title        = {{Information processing in generalized probabilistic theories}},
	author       = {Barrett, Jonathan},
	year         = 2007,
	month        = {Mar},
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 75,
	pages        = {032304},
	doi          = {10.1103/PhysRevA.75.032304},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.75.032304},
	issue        = 3,
	numpages     = 21
}
@article{barnum2011information,
	title        = {{Information Processing in Convex Operational Theories}},
	author       = {Howard Barnum and Alexander Wilce},
	year         = 2011,
	month        = feb,
	journal      = {Elec. Notes Theo. Comp. Sci.},
	publisher    = {Elsevier {BV}},
	volume       = 270,
	number       = 1,
	pages        = {3--15},
	doi          = {10.1016/j.entcs.2011.01.002},
	url          = {https://doi.org/10.1016/j.entcs.2011.01.002}
}
@article{hardy2011reformulating,
	title        = {{Reformulating and reconstructing quantum theory}},
	author       = {Hardy, Lucien},
	year         = 2011,
	journal      = {arXiv:1104.2066},
	url          = {https://arxiv.org/abs/1104.2066}
}
@article{Pirsa_nc,
	title        = {{Noncontextuality: how we should define it, why it is natural, and what to do about its failure}},
	author       = {Spekkens, R. W.},
	year         = 2017,
	journal      = {{PIRSA:17070035}},
	url          = {http://pirsa.org/17070035}
}
@article{magic,
	title        = {{Contextuality supplies the `magic' for quantum computation}},
	author       = {Howard, Mark and Wallman, Joel and Veitch, Victor and Emerson, Joseph},
	year         = 2014,
	month        = jun,
	day          = 19,
	journal      = {Nature},
	volume       = 510,
	number       = 7505,
	pages        = {351--355},
	doi          = {10.1038/nature13460},
	issn         = {0028-0836}
}
@article{cloningcontext,
	title        = {{Contextual advantage for state-dependent cloning}},
	author       = {Matteo Lostaglio and Gabriel Senno},
	year         = 2020,
	month        = apr,
	journal      = {Quantum},
	publisher    = {Verein zur Forderung des Open Access Publizierens in den Quantenwissenschaften},
	volume       = 4,
	pages        = 258,
	doi          = {10.22331/q-2020-04-27-258},
	url          = {https://doi.org/10.22331/q-2020-04-27-258}
}
@article{comp1,
	title        = {{Contextuality in measurement-based quantum computation}},
	author       = {Raussendorf, Robert},
	year         = 2013,
	month        = aug,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 88,
	pages        = {022322},
	url          = {http://link.aps.org/doi/10.1103/PhysRevA.88.022322},
	issue        = 2,
	numpages     = 7,
	doi.hide     = {10.1103/PhysRevA.88.022322}
}
@article{comp2,
	title        = {{Non-adaptive measurement-based quantum computation and multi-party Bell inequalities}},
	author       = {Hoban, Matty J and Campbell, Earl T and Loukopoulos, Klearchos and Browne, Dan E},
	year         = 2011,
	journal      = {New J. Phys.},
	volume       = 13,
	number       = 2,
	pages        = {023014},
	url          = {http://stacks.iop.org/1367-2630/13/i=2/a=023014}
}
@article{Schmid2018,
	title        = {{All the noncontextuality inequalities for arbitrary prepare-and-measure experiments with respect to any fixed set of operational equivalences}},
	author       = {Schmid, David and Spekkens, Robert W. and Wolfe, Elie},
	year         = 2018,
	month        = jun,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 97,
	pages        = {062103},
	doi          = {10.1103/PhysRevA.97.062103},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.97.062103},
	issue        = 6,
	numpages     = 12
}
@article{Helstrom,
	title        = {{Quantum detection and estimation theory}},
	author       = {Helstrom, Carl W.},
	year         = 1969,
	journal      = {J. Stat. Phys.},
	volume       = 1,
	number       = 2,
	pages        = {231--252},
	doi          = {10.1007/BF01007479},
	issn         = {1572-9613},
	url          = {http://dx.doi.org/10.1007/BF01007479}
}
@article{twothms,
	title        = {{Hidden variables and the two theorems of John Bell}},
	author       = {Mermin, N. David},
	year         = 1993,
	month        = jul,
	journal      = {Rev. Mod. Phys.},
	publisher    = {American Physical Society},
	volume       = 65,
	pages        = {803--815},
	url          = {http://link.aps.org/doi/10.1103/RevModPhys.65.803},
	issue        = 3,
	numpages     = {0},
	doi.hide     = {10.1103/RevModPhys.65.803}
}
@article{operationalks,
	title        = {{From the Kochen-Specker Theorem to Noncontextuality Inequalities without Assuming Determinism}},
	author       = {Kunjwal, Ravi and Spekkens, Robert W.},
	year         = 2015,
	month        = sep,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 115,
	pages        = 110403,
	doi          = {10.1103/PhysRevLett.115.110403},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.115.110403},
	issue        = 11,
	numpages     = 5
}
@article{robust,
	title        = {{The robust noncontextuality inequalities in the simplest scenario}},
	author       = {Matthew F. Pusey},
	year         = 2015,
	month        = jun,
	journal      = {arXiv:1506.04178},
	url          = {https://arxiv.org/abs/1506.04178}
}
@article{PP1,
	title        = {{Pre- and Post-Selection Paradoxes and Contextuality in Quantum Mechanics}},
	author       = {Leifer, M. S. and Spekkens, Robert W.},
	year         = 2005,
	month        = nov,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 95,
	pages        = 200405,
	url          = {http://link.aps.org/doi/10.1103/PhysRevLett.95.200405},
	issue        = 20,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.95.200405}
}
@inproceedings{PP2,
	title        = {{Logical pre- and post-selection paradoxes are proofs of contextuality}},
	author       = {Matthew F. Pusey and Matthew S. Leifer},
	year         = 2015,
	publisher    = {EPTCS},
	volume       = 195,
	pages        = {295--306},
	doi          = {10.4204/EPTCS.195.22},
	howpublished.hide = {EPTCS 195, 2015, pp. 295-306}
}
@article{NCFraction,
	title        = {{Contextual Fraction as a Measure of Contextuality}},
	author       = {Abramsky, Samson and Barbosa, Rui Soares and Mansfield, Shane},
	year         = 2017,
	month        = aug,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 119,
	pages        = {050504},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.119.050504},
	issue        = 5,
	numpages     = 6,
	doi.hide     = {10.1103/PhysRevLett.119.050504}
}
@article{Bastrakov2015,
	title        = {{Fast method for verifying Chernikov rules in Fourier-Motzkin elimination}},
	author       = {Bastrakov, S. I. and Zolotykh, N. Yu.},
	year         = 2015,
	journal      = {Comp. Mat. and Math. Phys.},
	volume       = 55,
	number       = 1,
	pages        = {160--167},
	doi          = {10.1134/S0965542515010042},
	issn         = {1555-6662},
	url          = {http://dx.doi.org/10.1134/S0965542515010042}
}
@article{DantzigEaves,
	title        = {{Fourier-Motzkin elimination and its dual}},
	author       = {George B Dantzig and B Curtis Eaves},
	year         = 1973,
	journal      = {J. Combin. Th. A},
	volume       = 14,
	number       = 3,
	pages        = {288--297},
	issn         = {0097-3165},
	url          = {http://www.sciencedirect.com/science/article/pii/0097316573900046},
	doi.hide     = {10.1016/0097-3165(73)90004-6}
}
@article{BalasProjectionCone,
	title        = {{Projection with a Minimal System of Inequalities}},
	author       = {Balas, Egon},
	year         = 1998,
	journal      = {Comp. Optimiz. Applic.},
	volume       = 10,
	number       = 2,
	pages        = {189--193},
	doi          = {10.1023/A:1018368920203},
	issn         = {1573-2894},
	\\url        = {http://dx.doi.org/10.1023/A:1018368920203}
}
@article{barber1996quickhull,
	title        = {{The quickhull algorithm for convex hulls}},
	author       = {Barber, C Bradford and Dobkin, David P and Huhdanpaa, Hannu},
	year         = 1996,
	journal      = {ACM Trans. Math. Soft.},
	publisher    = {ACM},
	volume       = 22,
	number       = 4,
	pages        = {469--483},
	doi          = {10.1145/235815.235821}
}
@article{Zolotykh2012,
	title        = {{New modification of the double description method for constructing the skeleton of a polyhedral cone}},
	author       = {N. Yu. Zolotykh},
	year         = 2012,
	month        = jan,
	journal      = {Comp. Math. and Math. Phys.},
	publisher    = {Pleiades Publishing Ltd},
	volume       = 52,
	number       = 1,
	pages        = {146--156},
	doi          = {10.1134/s0965542512010162},
	url          = {https://doi.org/10.1134/s0965542512010162}
}
@article{Fukuda1996,
	title        = {{Double description method revisited}},
	author       = {Fukuda, Komei and Prodon, Alain},
	year         = 1996,
	journal      = {Comb. Comp. Sci.},
	publisher    = {Springer Berlin Heidelberg},
	address      = {Berlin, Heidelberg},
	pages        = {91--111},
	doi          = {10.1007/3-540-61576-8_77},
	isbn         = {978-3-540-70627-4},
	editor       = {Deza, Michel and Euler, Reinhardt and Manoussakis, Ioannis}
}
@article{avis_convexhull_2015,
	title        = {{How good are convex hull algorithms?}},
	author       = {David Avis and David Bremner and Raimund Seidel},
	year         = 1997,
	journal      = {Comp. Geom.},
	volume       = 7,
	number       = 56,
	pages        = {265--301},
	doi          = {10.1016/S0925-7721(96)00023-5},
	issn         = {0925-7721},
	url          = {http://www.sciencedirect.com/science/article/pii/S0925772196000235}
}
@article{Shapot2012,
	title        = {{Solution Building for Arbitrary System of Linear Inequalities in an Explicit Form}},
	author       = {Demetrius V. Shapot and Alexander M. Lukatskii},
	year         = 2012,
	journal      = {Am. J. Comp. Math.},
	publisher    = {Scientific Research Publishing,  Inc,},
	volume       = {02},
	number       = {01},
	pages        = {1--11},
	doi          = {10.4236/ajcm.2012.21001},
	\\url        = {http://dx.doi.org/10.4236/ajcm.2012.21001}
}
@incollection{Avis2000lrs,
	title        = {{A Revised Implementation of the Reverse Search Vertex Enumeration Algorithm}},
	author       = {Avis, David},
	year         = 2000,
	booktitle    = {Polytopes --- Combinatorics and Computation},
	publisher    = {Birkh{\"a}user Basel},
	series       = {DMV Seminar},
	volume       = 29,
	pages        = {177--198},
	url          = {http://link.springer.com/chapter/10.1007/978-3-0348-8438-9_9},
	\\editor     = {Kalai, Gil and Ziegler, G{\"u}nter M.}
}
@phdthesis{JonesThesis2005,
	title        = {{Polyhedral Tools for Control}},
	author       = {Jones, Colin},
	year         = 2005,
	publisher    = {University of Cambridge},
	url          = {http://infoscience.epfl.ch/record/169769/files/cued_control_980.pdf},
	details      = {http://infoscience.epfl.ch/record/169769},
	documenturl  = {http://infoscience.epfl.ch/record/169769/files/cued_control_980.pdf},
	oai-id       = {oai:infoscience.epfl.ch:169769},
	oai-set      = {driver},
	status       = {PUBLISHED},
	submitter    = 207237,
	unit         = {LA},
	school       = {University of Cambridge}
}
@techreport{jones2004equality,
	title        = {{Equality Set Projection: A new algorithm for the projection of polytopes in halfspace representation}},
	author       = {Jones, Colin and Kerrigan, Eric C and Maciejowski, Jan},
	year         = 2004,
	url          = {http://infoscience.epfl.ch/record/169768/files/resp_mar_04_15.pdf},
	institution  = {Cambridge University Engineering Dept},
	details      = {http://infoscience.epfl.ch/record/169768}
}
@article{Jones2008,
	title        = {{On Polyhedral Projection and Parametric Programming}},
	author       = {Jones, C. N. and Kerrigan, E. C. and Maciejowski, J. M.},
	year         = 2008,
	journal      = {J. Optimiz. Theo. Applic.},
	volume       = 138,
	number       = 2,
	pages        = {207--220},
	doi          = {10.1007/s10957-008-9384-4},
	issn         = {1573-2878},
	\\url        = {http://dx.doi.org/10.1007/s10957-008-9384-4}
}
@article{Schurmann2013,
	title        = {{Exploiting Symmetries in Polyhedral Computations}},
	author       = {Schrmann, Achill},
	year         = 2013,
	journal      = {Disc. Geom. Optim.},
	publisher    = {Springer International},
	pages        = {265--278},
	doi          = {10.1007/978-3-319-00200-2_15},
	isbn         = {978-3-319-00200-2},
	editor       = {Bezdek, Karoly and Deza, Antoine and Ye, Yinyu},
	\\address.hide = {Heidelberg},
	\\url        = {http://dx.doi.org/10.1007/978-3-319-00200-2_15}
}
@incollection{bremner_symmetries_2009,
	title        = {{Polyhedral representation conversion up to symmetries}},
	author       = {Bremner, David and Dutour Sikiric, Mathieu and Sch{\"u}rmann, Achill},
	year         = 2009,
	booktitle    = {Polyhedral computation},
	publisher    = {Amer. Math. Soc.},
	series       = {CRM Proc. Lecture Notes},
	volume       = 48,
	pages        = {45--71},
	isbn         = 9780821873328,
	url          = {https://books.google.ca/books?id=uuzf-Fy1Cj8C},
	note         = {\href{https://arxiv.org/abs/math/0702239}{arXiv:math/0702239}},
	lccn         = 2008054354
}
@article{panda_2015,
	title        = {{PANDA: a software for polyhedral transformations}},
	author       = {L{\"o}rwald, Stefan and Reinelt, Gerhard},
	year         = 2015,
	journal      = {Euro. J. Comp. Optim.},
	publisher    = {Springer Berlin Heidelberg},
	pages        = {1--12},
	doi          = {10.1007/s13675-015-0040-0},
	issn         = {2192-4406},
	\\url        = {http://dx.doi.org/10.1007/s13675-015-0040-0}
}
@article{infeasibilitycertificates,
	title        = {{Certificates of Primal or Dual Infeasibility in Linear Programming}},
	author       = {Andersen, Erling D.},
	year         = 2001,
	journal      = {Comp. Optim. Applic.},
	volume       = 20,
	number       = 2,
	pages        = {171--183},
	doi          = {10.1023/A:1011259103627},
	issn         = {1573-2894},
	\\url        = {http://dx.doi.org/10.1023/A:1011259103627}
}
@article{KLP19,
	title        = {{Anomalous weak values and contextuality: Robustness, tightness, and imaginary parts}},
	author       = {Kunjwal, Ravi and Lostaglio, Matteo and Pusey, Matthew F.},
	year         = 2019,
	month        = oct,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 100,
	pages        = {042116},
	doi          = {10.1103/PhysRevA.100.042116},
	url          = {https://doi.org/10.1103/PhysRevA.100.042116},
	issue        = 4,
	numpages     = 19
}
@article{Kunjwal19,
	title        = {{Beyond the Cabello-Severini-Winter framework: Making sense of contextuality without sharpness of measurements}},
	author       = {Kunjwal, Ravi},
	year         = 2019,
	month        = sep,
	journal      = {{Quantum}},
	publisher    = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
	volume       = 3,
	pages        = 184,
	doi          = {10.22331/q-2019-09-09-184},
	issn         = {2521-327X},
	url          = {https://doi.org/10.22331/q-2019-09-09-184}
}
@article{Kunjwal20,
	title        = {{Hypergraph framework for irreducible noncontextuality inequalities from logical proofs of the Kochen-Specker theorem}},
	author       = {Kunjwal, Ravi},
	year         = 2020,
	month        = jan,
	journal      = {{Quantum}},
	publisher    = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
	volume       = 4,
	pages        = 219,
	doi          = {10.22331/q-2020-01-10-219},
	issn         = {2521-327X},
	url          = {https://doi.org/10.22331/q-2020-01-10-219}
}
@article{Kunjwal16,
	title        = {{Contextuality beyond the Kochen-Specker theorem}},
	author       = {Kunjwal, Ravi},
	year         = 2016,
	journal      = {arXiv:1612.07250},
	url          = {https://arxiv.org/abs/1612.07250}
}
@misc{YK20,
	title        = {{Contextuality in entanglement-assisted one-shot classical communication}},
	author       = {Shiv Akshar Yadavalli and Ravi Kunjwal},
	year         = 2021,
	eprint       = {2006.00469},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@misc{faacets,
	title        = {{Faacets}},
	howpublished = {\url{http://www.faacets.com}}
}
@article{Sikora,
	title        = {{Lower Bounds for Quantum Oblivious Transfer}},
	author       = {Chailloux, Andr{\'e} and Kerenidis, Iordanis and Sikora, Jamie},
	year         = 2013,
	month        = jan,
	journal      = {Quantum Info. Comput.},
	publisher    = {Rinton Press, Incorporated},
	address      = {Paramus, NJ},
	volume       = 13,
	number       = {1-2},
	pages        = {158--177},
	issn         = {1533-7146},
	url          = {http://dl.acm.org/citation.cfm?id=2481591.2481600},
	issue_date   = {January 2013},
	numpages     = 20,
	acmid        = 2481600
}
@article{LoChauBC,
	title        = {{Is Quantum Bit Commitment Really Possible?}},
	author       = {Lo, Hoi-Kwong and Chau, H. F.},
	year         = 1997,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 78,
	pages        = {3410--3413},
	doi          = {10.1103/PhysRevLett.78.3410},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.78.3410},
	issue        = 17,
	numpages     = {0}
}
@article{AmbainisCF,
	title        = {{A new protocol and lower bounds for quantum coin flipping}},
	author       = {Andris Ambainis},
	year         = 2004,
	journal      = {Journal of Computer and System Sciences},
	volume       = 68,
	number       = 2,
	pages        = {398--416},
	doi          = {https://doi.org/10.1016/j.jcss.2003.07.010},
	issn         = {0022-0000},
	url          = {http://www.sciencedirect.com/science/article/pii/S0022000003001417},
	note         = {Special Issue on STOC 2001}
}
@article{RudolphSpekkensBC,
	title        = {{Degrees of concealment and bindingness in quantum bit commitment protocols}},
	author       = {Spekkens, R. W. and Rudolph, T.},
	year         = 2001,
	month        = dec,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 65,
	pages        = {012310},
	doi          = {10.1103/PhysRevA.65.012310},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.65.012310},
	issue        = 1,
	numpages     = 10
}
@article{cointossing,
	title        = {{Quantum cryptography: Public key distribution and coin tossing}},
	author       = {Charles H. Bennett and Gilles Brassard},
	year         = 2014,
	journal      = {Theoretical Computer Science},
	volume       = 560,
	number       = {},
	pages        = {7--11},
	doi          = {http://dx.doi.org/10.1016/j.tcs.2014.05.025},
	issn         = {0304-3975},
	url          = {http://www.sciencedirect.com/science/article/pii/S0304397514004241},
	note         = {Theoretical Aspects of Quantum Cryptography: celebrating 30 years of BB84}
}
@article{bitcommit,
	title        = {{Unconditionally Secure Quantum Bit Commitment is Impossible}},
	author       = {Mayers, Dominic},
	year         = 1997,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 78,
	pages        = {3414--3417},
	doi          = {10.1103/PhysRevLett.78.3414},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.78.3414},
	issue        = 17,
	numpages     = {0}
}
@article{Hardy,
	title        = {{Quantum Theory From Five Reasonable Axioms}},
	author       = {{Hardy}, L.},
	year         = 2001,
	month        = jan,
	journal      = {arXiv:quant-ph/0101012},
	url          = {https://arxiv.org/abs/quant-ph/0101012},
	eprint.hide  = {quant-ph/0101012},
	adsurl       = {http://adsabs.harvard.edu/abs/2001quant.ph..1012H},
	adsnote      = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{cab4,
	title        = {{Experimentally Testable State-Independent Quantum Contextuality}},
	author       = {Cabello, Ad\'an},
	year         = 2008,
	month        = nov,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 101,
	pages        = 210401,
	doi          = {10.1103/PhysRevLett.101.210401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.101.210401},
	issue        = 21,
	numpages     = 4
}
@article{cab5,
	title        = {{Simple Test for Hidden Variables in Spin-1 Systems}},
	author       = {Klyachko, Alexander A. and Can, M. Ali and Binicio\ifmmode \breve{g}\else \u{g}\fi{}lu, Sinem and Shumovsky, Alexander S.},
	year         = 2008,
	month        = jul,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 101,
	pages        = {020403},
	doi          = {10.1103/PhysRevLett.101.020403},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.101.020403},
	issue        = 2,
	numpages     = 4
}
@article{specker,
	title        = {{Fine's theorem, noncontextuality, and correlations in Specker's scenario}},
	author       = {Kunjwal, Ravi},
	year         = 2015,
	month        = feb,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 91,
	pages        = {022108},
	doi          = {10.1103/PhysRevA.91.022108},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.91.022108},
	issue        = 2,
	numpages     = 11
}
@article{determinism,
	title        = {{The Status of Determinism in Proofs of the Impossibility of a Noncontextual Model of Quantum Theory}},
	author       = {Spekkens, Robert W.},
	year         = 2014,
	month        = nov,
	day          = {01},
	journal      = {Foundations of Physics},
	volume       = 44,
	number       = 11,
	pages        = {1125--1155},
	doi          = {10.1007/s10701-014-9833-x},
	issn         = {1572-9516},
	url          = {https://doi.org/10.1007/s10701-014-9833-x}
}
@article{Fine,
	title        = {{Hidden Variables, Joint Probability, and the Bell Inequalities}},
	author       = {Fine, Arthur},
	year         = 1982,
	month        = feb,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 48,
	pages        = {291--295},
	doi          = {10.1103/PhysRevLett.48.291},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.48.291},
	issue        = 5,
	numpages     = {0}
}
@book{Pitowsky,
	title        = {{Quantum Probability â?? Quantum Logic}},
	author       = {Pitowsky, I.},
	year         = 2014,
	publisher    = {Springer Berlin Heidelberg},
	series       = {Lecture Notes in Physics},
	isbn         = 9783662137345,
	url          = {https://books.google.ca/books?id=BhEeswEACAAJ}
}
@article{ncycle,
	title        = {{All noncontextuality inequalities for the $n$-cycle scenario}},
	author       = {Ara\'ujo, Mateus and Quintino, Marco T\'ulio and Budroni, Costantino and Cunha, Marcelo Terra and Cabello, Ad\'an},
	year         = 2013,
	month        = aug,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 88,
	pages        = {022118},
	doi          = {10.1103/PhysRevA.88.022118},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.88.022118},
	issue        = 2,
	numpages     = 7
}
@article{posquasi,
	title        = {{Quasi-probability representations of quantum theory with applications to quantum information science}},
	author       = {Christopher Ferrie},
	year         = 2011,
	journal      = {Reports on Progress in Physics},
	volume       = 74,
	number       = 11,
	pages        = 116001,
	url          = {http://stacks.iop.org/0034-4885/74/i=11/a=116001}
}
@article{NPAprl,
	title        = {{Bounding the Set of Quantum Correlations}},
	author       = {Navascu\'es, Miguel and Pironio, Stefano and Ac\'{\i}n, Antonio},
	year         = 2007,
	month        = jan,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 98,
	pages        = {010401},
	doi          = {10.1103/PhysRevLett.98.010401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.98.010401},
	issue        = 1,
	numpages     = 4
}
@article{deba1,
	title        = {{State independent contextuality advances one-way communication}},
	author       = {{Saha}, D. and {Horodecki}, P. and {Paw{\l}owski}, M.},
	year         = 2017,
	month        = aug,
	journal      = {ArXiv e-prints},
	archiveprefix = {arXiv},
	eprint       = {1708.04751},
	primaryclass = {quant-ph},
	adsurl       = {http://adsabs.harvard.edu/abs/2017arXiv170804751S},
	adsnote      = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{deba2,
	title        = {{Reformulating noncontextuality inequalities in an operational approach}},
	author       = {{Xu}, Z.-P. and {Saha}, D. and {Su}, H.-Y. and {Paw{\l}owski}, M. and {Chen}, J.-L.},
	year         = 2016,
	month        = dec,
	journal      = {PRA},
	volume       = 94,
	number       = 6,
	pages        = {062103},
	doi          = {10.1103/PhysRevA.94.062103},
	archiveprefix = {arXiv},
	eprint       = {1509.06027},
	primaryclass = {quant-ph},
	eid          = {062103},
	adsurl       = {http://adsabs.harvard.edu/abs/2016PhRvA..94f2103X},
	adsnote      = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{DIQKD2,
	title        = {{From Bell's Theorem to Secure Quantum Key Distribution}},
	author       = {Ac\'{\i}n, Antonio and Gisin, Nicolas and Masanes, Llu{\'\i}s},
	year         = 2006,
	month        = sep,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 97,
	pages        = 120405,
	doi          = {10.1103/PhysRevLett.97.120405},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.97.120405},
	issue        = 12,
	numpages     = 4
}
@inbook{DantzigLP,
	title        = {{Duality and Theorems of the Alternatives}},
	year         = 2003,
	booktitle    = {Linear Programming: 2: Theory and Extensions},
	publisher    = {Springer New York},
	address      = {New York, NY},
	pages        = {43--65},
	doi          = {10.1007/0-387-21569-7_2},
	isbn         = {978-0-387-21569-3},
	url          = {https://doi.org/10.1007/0-387-21569-7_2}
}
@inbook{YinyuYe2016LP,
	title        = {{Duality and Complementarity}},
	author       = {Luenberger, David G. and Ye, Yinyu},
	year         = 2016,
	booktitle    = {Linear and Nonlinear Programming},
	publisher    = {Springer International Publishing},
	address      = {Cham},
	pages        = {83--114},
	doi          = {10.1007/978-3-319-18842-3_4},
	isbn         = {978-3-319-18842-3},
	url          = {https://doi.org/10.1007/978-3-319-18842-3_4}
}
@article{Fritz2013Marginal,
	title        = {{Entropic Inequalities and Marginal Problems}},
	author       = {Tobias Fritz and Rafael Chaves},
	year         = 2013,
	month        = feb,
	journal      = {{IEEE} Trans. Info. Theo.},
	publisher    = {Institute of Electrical and Electronics Engineers ({IEEE})},
	volume       = 59,
	number       = 2,
	pages        = {803--817},
	doi          = {10.1109/tit.2012.2222863},
	url          = {https://doi.org/10.1109/tit.2012.2222863}
}
@article{FritzBeyondBellI,
	title        = {{Beyond Bell's theorem: correlation scenarios}},
	author       = {Tobias Fritz},
	year         = 2012,
	journal      = {New J. Physics},
	volume       = 14,
	number       = 10,
	pages        = 103001,
	url          = {http://stacks.iop.org/1367-2630/14/i=10/a=103001}
}
@article{Chaves2015InfoTheo,
	title        = {{Information\textendashtheoretic implications of quantum causal structures}},
	author       = {Rafael Chaves and Christian Majenz and David Gross},
	year         = 2015,
	month        = jan,
	journal      = {Nat. Comm.},
	publisher    = {Springer Nature},
	volume       = 6,
	pages        = 5766,
	doi          = {10.1038/ncomms6766},
	url          = {https://doi.org/10.1038/ncomms6766}
}
@article{scarani2011extremaltripartite,
	title        = {{Extremal correlations of the tripartite no-signaling polytope}},
	author       = {Stefano Pironio and Jean-Daniel Bancal and Valerio Scarani},
	year         = 2011,
	journal      = {J. Phys. A},
	volume       = 44,
	number       = 6,
	pages        = {065303},
	url          = {http://stacks.iop.org/1751-8121/44/i=6/a=065303}
}
@article{bancal2010symmetric,
	title        = {{Looking for symmetric Bell inequalities}},
	author       = {Jean-Daniel Bancal and Nicolas Gisin and Stefano Pironio},
	year         = 2010,
	journal      = {J. Phys. A},
	volume       = 43,
	number       = 38,
	pages        = 385303,
	url          = {http://stacks.iop.org/1751-8121/43/i=38/a=385303}
}
@article{Brunner2008,
	title        = {{Partial list of bipartite Bell inequalities with four binary settings}},
	author       = {Nicolas Brunner and Nicolas Gisin},
	year         = 2008,
	month        = apr,
	journal      = {Phys. Lett. A},
	publisher    = {Elsevier {BV}},
	volume       = 372,
	number       = 18,
	pages        = {3162--3167},
	doi          = {10.1016/j.physleta.2008.01.052},
	url          = {https://doi.org/10.1016/j.physleta.2008.01.052}
}
@article{Collins2004,
	title        = {{A relevant two qubit Bell inequality inequivalent to the CHSH inequality}},
	author       = {Daniel Collins and Nicolas Gisin},
	year         = 2004,
	journal      = {J. Phys. A},
	volume       = 37,
	number       = 5,
	pages        = 1775,
	url          = {http://stacks.iop.org/0305-4470/37/i=5/a=021}
}
@article{Basoalto2001,
	title        = {{A general computer program for the Bell detection loophole}},
	author       = {Roberto M. Basoalto and Ian C. Percival},
	year         = 2001,
	journal      = {Physics Letters A},
	volume       = 280,
	number       = 1,
	pages        = {1--6},
	doi          = {https://doi.org/10.1016/S0375-9601(01)00035-4},
	issn         = {0375-9601},
	url          = {http://www.sciencedirect.com/science/article/pii/S0375960101000354}
}
@article{Elliot2009,
	title        = {{A linear program for testing local realism}},
	author       = {Matthew B. Elliott},
	year         = 2009,
	journal      = {arXiv:0905.2950},
	url          = {https://arxiv.org/abs/0905.2950}
}
@article{Zukowski1999,
	title        = {{Strengthening the Bell Theorem: conditions to falsify local realism in an experiment}},
	author       = {{Zukowski}, M. and {Kaszlikowski}, D. and {Baturo}, A. and {Larsson}, J.-A.},
	year         = 1999,
	journal      = {arXiv:quant-ph/9910058},
	url          = {https://arxiv.org/abs/quant-ph/9910058}
}
@article{farinholt2014ideal,
	title        = {{An ideal characterization of the Clifford operators}},
	author       = {Farinholt, JM},
	year         = 2014,
	journal      = {J. Phys. A: Math. Theor.},
	publisher    = {IOP Publishing},
	volume       = 47,
	number       = 30,
	pages        = 305303
}
@article{aharonov2003simple,
	title        = {{A simple proof that Toffoli and Hadamard are quantum universal}},
	author       = {Aharonov, Dorit},
	year         = 2003,
	journal      = {quant-ph/0301040}
}
@unpublished{van2017quantum,
	title        = {{Quantum theory is a quasi-stochastic process theory}},
	author       = {van de Wetering, John},
	year         = 2017,
	eprint       = {1704.08525},
	archiveprefix = {arXiv}
}
@article{lee2015computation,
	title        = {{Computation in generalised probabilisitic theories}},
	author       = {Lee, Ciar{\'a}n M and Barrett, Jonathan},
	year         = 2015,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 17,
	number       = 8,
	pages        = {083001},
	url          = {https://iopscience.iop.org/article/10.1088/1367-2630/17/8/083001/meta}
}
@article{barrett2019computational,
	title        = {The computational landscape of general physical theories},
	author       = {Jonathan Barrett and Niel de Beaudrap and Matty J. Hoban and Ciar{\'{a}}n M. Lee},
	year         = 2019,
	month        = {may},
	journal      = {npj Quantum Information},
	publisher    = {Springer Science and Business Media {LLC}},
	volume       = 5,
	number       = 1,
	doi          = {10.1038/s41534-019-0156-9},
	url          = {https://doi.org/10.1038%2Fs41534-019-0156-9}
}
@article{barnum2018oracles,
	title        = {{Oracles and query lower bounds in generalised probabilistic theories}},
	author       = {Barnum, Howard and Lee, Ciar{\'a}n M and Selby, John H},
	year         = 2018,
	journal      = {Foundations of physics},
	publisher    = {Springer},
	volume       = 48,
	number       = 8,
	pages        = {954--981},
	url          = {https://link.springer.com/article/10.1007/s10701-018-0198-4}
}
@article{gibbons2004discrete,
	title        = {{Discrete phase space based on finite fields}},
	author       = {Gibbons, Kathleen S and Hoffman, Matthew J and Wootters, William K},
	year         = 2004,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 70,
	number       = 6,
	pages        = {062101},
	url          = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.70.062101}
}
@article{krumm2019quantum,
	title        = {{Quantum computation is the unique reversible circuit model for which bits are balls}},
	author       = {Krumm, Marius and M{\"u}ller, Markus P},
	year         = 2019,
	journal      = {npj Quantum Information},
	publisher    = {Nature Publishing Group},
	volume       = 5,
	number       = 1,
	pages        = {1--8},
	url          = {https://www.nature.com/articles/s41534-018-0123-x}
}
@article{garner2018interferometric,
	title        = {{Interferometric computation beyond quantum theory}},
	author       = {Garner, Andrew JP},
	year         = 2018,
	journal      = {Foundations of Physics},
	publisher    = {Springer},
	volume       = 48,
	number       = 8,
	pages        = {886--909},
	url          = {https://link.springer.com/article/10.1007/s10701-018-0142-7}
}
@article{campbell2012magic,
	title        = {{Magic-state distillation in all prime dimensions using quantum reed-muller codes}},
	author       = {Campbell, Earl T and Anwar, Hussain and Browne, Dan E},
	year         = 2012,
	journal      = {Phys. Rev. X},
	publisher    = {APS},
	volume       = 2,
	number       = 4,
	pages        = {041021},
	url          = {https://journals.aps.org/prx/pdf/10.1103/PhysRevX.2.041021}
}
@article{eastin2009restrictions,
	title        = {{Restrictions on transversal encoded quantum gate sets}},
	author       = {Eastin, Bryan and Knill, Emanuel},
	year         = 2009,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 102,
	number       = 11,
	pages        = 110502,
	url          = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.102.110502}
}
@article{gross2006hudson,
	title        = {{Hudson's theorem for finite-dimensional quantum systems}},
	author       = {Gross, David},
	year         = 2006,
	journal      = {J. Math. Phys.},
	publisher    = {American Institute of Physics},
	volume       = 47,
	number       = 12,
	pages        = 122107,
	url          = {https://aip.scitation.org/doi/10.1063/1.2393152}
}
@article{PhysRevLett.81.5672,
	title        = {{Power of One Bit of Quantum Information}},
	author       = {Knill, E. and Laflamme, R.},
	year         = 1998,
	month        = dec,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 81,
	pages        = {5672--5675},
	doi          = {10.1103/PhysRevLett.81.5672},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.81.5672},
	issue        = 25,
	numpages     = {0}
}
@article{PhysRevLett.91.147902,
	title        = {{Efficient Classical Simulation of Slightly Entangled Quantum Computations}},
	author       = {Vidal, Guifr\'e},
	year         = 2003,
	month        = oct,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 91,
	pages        = 147902,
	doi          = {10.1103/PhysRevLett.91.147902},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.91.147902},
	issue        = 14,
	numpages     = 4
}
@article{PhysRevA.72.042316,
	title        = {{Entanglement and the power of one qubit}},
	author       = {Datta, Animesh and Flammia, Steven T. and Caves, Carlton M.},
	year         = 2005,
	month        = oct,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 72,
	pages        = {042316},
	doi          = {10.1103/PhysRevA.72.042316},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.72.042316},
	issue        = 4,
	numpages     = 14
}
@book{anygatemakesStabUniversal,
	title        = {{Self-dual codes and invariant theory}},
	author       = {Nebe, Gabriele and Rains, Eric M and Sloane, Neil James Alexander},
	year         = 2006,
	publisher    = {Springer},
	volume       = 17,
	url          = {https://www.springer.com/gp/book/9783540307297}
}
@article{generatorsForCliffordGroup,
	title        = {{Full length article}},
	author       = {Gottesman, Daniel},
	year         = 1999,
	journal      = {Chaos, Solitons \& Fractals},
	volume       = 10,
	number       = 10,
	pages        = {1749--1758},
	doi          = {https://doi.org/10.1016/S0960-0779(98)00218-5},
	issn         = {0960-0779},
	url          = {http://www.sciencedirect.com/science/article/pii/S0960077998002185}
}
@article{PhysRevA.83.032310,
	title        = {{Noise thresholds for higher-dimensional systems using the discrete Wigner function}},
	author       = {van Dam, Wim and Howard, Mark},
	year         = 2011,
	month        = mar,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 83,
	pages        = {032310},
	doi          = {10.1103/PhysRevA.83.032310},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.83.032310},
	issue        = 3,
	numpages     = 13
}
@article{CSC,
	title        = {{Mathematical Foundations for a Compositional Distributional Model of Meaning}},
	author       = {{Coecke}, Bob and {Sadrzadeh}, Mehrnoosh and {Clark}, Stephen},
	year         = 2010,
	month        = mar,
	url          = {https://ui.adsabs.harvard.edu/abs/2010arXiv1003.4394C},
	archiveprefix = {arXiv},
	eprint       = {1003.4394},
	primaryclass = {cs.CL},
	adsnote      = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{bankova2016graded,
	title        = {{Graded entailment for compositional distributional semantics}},
	author       = {Bankova, Desislava and Coecke, Bob and Lewis, Martha and Marsden, Daniel},
	year         = 2016,
	journal      = {arXiv:1601.04908},
	url          = {https://arxiv.org/abs/1601.04908}
}
@article{coecke2016mathematical,
	title        = {{A mathematical theory of resources}},
	author       = {Coecke, Bob and Fritz, Tobias and Spekkens, Robert W},
	year         = 2016,
	month        = oct,
	journal      = {Info. Comp.},
	publisher    = {Elsevier},
	volume       = 250,
	pages        = {59--86},
	doi          = {10.1016/j.ic.2016.02.008}
}
@inproceedings{MarthaC,
	title        = {{A compositional explanation of the `Pet Fish' phenomenon}},
	author       = {Coecke, Bob and Lewis, Martha},
	year         = 2015,
	booktitle    = {International Symposium on Quantum Interaction},
	pages        = {179--192},
	url          = {https://link.springer.com/chapter/10.1007/978-3-319-28675-4_14},
	organization = {Springer}
}
@article{TriangleGisin,
	title        = {{Genuine Quantum Nonlocality in the Triangle Network}},
	author       = {Renou, Marc-Olivier and Baumer, Elisa and Boreiri, Sadra and Brunner, Nicolas and Gisin, Nicolas and Beigi, Salman},
	year         = 2019,
	month        = sep,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 123,
	pages        = 140401,
	doi          = {10.1103/PhysRevLett.123.140401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.123.140401},
	issue        = 14,
	numpages     = 5
}
@inbook{Putnam1969,
	title        = {{Is Logic Empirical?}},
	author       = {Putnam, Hilary},
	year         = 1969,
	booktitle    = {Boston Studies in the Philosophy of Science: Proceedings of the Boston Colloquium for the Philosophy of Science 1966/1968},
	publisher    = {Springer Netherlands},
	address      = {Dordrecht},
	pages        = {216--241},
	doi          = {10.1007/978-94-010-3381-7_5},
	isbn         = {978-94-010-3381-7},
	url          = {https://doi.org/10.1007/978-94-010-3381-7_5},
	editor       = {Cohen, Robert S. and Wartofsky, Marx W.}
}
@article{VanHimbeeck2019quantumviolationsin,
	title        = {{Quantum violations in the Instrumental scenario and their relations to the Bell scenario}},
	author       = {Van Himbeeck, Thomas and Bohr Brask, Jonatan and Pironio, Stefano and Ramanathan, Ravishankar and Sainz, Ana Bel{\'{e}}n and Wolfe, Elie},
	year         = 2019,
	month        = sep,
	journal      = {{Quantum}},
	publisher    = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
	volume       = 3,
	pages        = 186,
	doi          = {10.22331/q-2019-09-16-186},
	issn         = {2521-327X},
	url          = {https://doi.org/10.22331/q-2019-09-16-186}
}
@article{pusey2012reality,
	title        = {{On the reality of the quantum state}},
	author       = {Pusey, Matthew F and Barrett, Jonathan and Rudolph, Terry},
	year         = 2012,
	journal      = {Nature Physics},
	publisher    = {Nature Publishing Group},
	volume       = 8,
	number       = 6,
	pages        = {475--478},
	url          = {https://www.nature.com/articles/nphys2309}
}
@unpublished{gottesman1997stabilizer,
	title        = {{Stabilizer codes and quantum error correction}},
	author       = {Gottesman, Daniel},
	year         = 1997,
	url          = {https://thesis.library.caltech.edu/2900/},
	note         = {arXiv Preprint quant-ph/9705052}
}
@unpublished{gottesman1998heisenberg,
	title        = {{The Heisenberg representation of quantum computers}},
	author       = {Gottesman, Daniel},
	year         = 1998,
	url          = {https://arxiv.org/abs/quant-ph/9807006},
	note         = {arxiv Preprint quant-ph/9807006}
}
@article{PhysRevA.71.042302,
	title        = {{Discrete Wigner functions and quantum computational speedup}},
	author       = {Galv\~ao, Ernesto F.},
	year         = 2005,
	month        = apr,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 71,
	pages        = {042302},
	doi          = {10.1103/PhysRevA.71.042302},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.71.042302},
	issue        = 4,
	numpages     = 6
}
@article{anwar2012qutrit,
	title        = {{Qutrit magic state distillation}},
	author       = {Anwar, Hussain and Campbell, Earl T and Browne, Dan E},
	year         = 2012,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 14,
	number       = 6,
	pages        = {063006},
	url          = {https://iopscience.iop.org/article/10.1088/1367-2630/14/6/063006}
}
@article{PhysRevLett.109.230503,
	title        = {{Positive Wigner Functions Render Classical Simulation of Quantum Computation Efficient}},
	author       = {Mari, A. and Eisert, J.},
	year         = 2012,
	month        = dec,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 109,
	pages        = 230503,
	doi          = {10.1103/PhysRevLett.109.230503},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.109.230503},
	issue        = 23,
	numpages     = 5
}
@article{PhysRevX.5.021003,
	title        = {{Wigner Function Negativity and Contextuality in Quantum Computation on Rebits}},
	author       = {Delfosse, Nicolas and Allard Guerin, Philippe and Bian, Jacob and Raussendorf, Robert},
	year         = 2015,
	month        = apr,
	journal      = {Phys. Rev. X},
	publisher    = {American Physical Society},
	volume       = 5,
	pages        = {021003},
	doi          = {10.1103/PhysRevX.5.021003},
	url          = {https://link.aps.org/doi/10.1103/PhysRevX.5.021003},
	issue        = 2,
	numpages     = 23
}
@article{PhysRevA.95.052334,
	title        = {{Contextuality and Wigner-function negativity in qubit quantum computation}},
	author       = {Raussendorf, Robert and Browne, Dan E. and Delfosse, Nicolas and Okay, Cihan and Bermejo-Vega, Juan},
	year         = 2017,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 95,
	pages        = {052334},
	doi          = {10.1103/PhysRevA.95.052334},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.95.052334},
	issue        = 5,
	numpages     = 22
}
@article{bravyi2005universal,
	title        = {{Universal quantum computation with ideal Clifford gates and noisy ancillas}},
	author       = {Bravyi, Sergey and Kitaev, Alexei},
	year         = 2005,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 71,
	number       = 2,
	pages        = {022316},
	url          = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.71.022316}
}
@book{Ladyman2007,
	title        = {{Every Thing Must Go: Metaphysics Naturalized}},
	author       = {James Ladyman and Don Ross},
	year         = 2007,
	publisher    = {Oxford University Press},
	url          = {https://global.oup.com/academic/product/every-thing-must-go-9780199276196?cc=pl&lang=en&}
}
@article{montina2008exponential,
	title        = {{Exponential complexity and ontological theories of quantum mechanics}},
	author       = {Montina, Alberto},
	year         = 2008,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 77,
	number       = 2,
	pages        = {022104},
	url          = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.77.022104}
}
@article{catani2020mathematical,
	title        = {{A mathematical framework for operational fine tunings}},
	author       = {Catani, Lorenzo and Leifer, Matthew},
	year         = 2020,
	journal      = {arXiv:2003.10050},
	url          = {https://arxiv.org/abs/2003.10050}
}
@article{bartlett2007reference,
	title        = {{Reference frames, superselection rules, and quantum information}},
	author       = {Bartlett, Stephen D and Rudolph, Terry and Spekkens, Robert W},
	year         = 2007,
	journal      = {Reviews of Modern Physics},
	publisher    = {APS},
	volume       = 79,
	number       = 2,
	pages        = 555,
	url          = {https://journals.aps.org/rmp/abstract/10.1103/RevModPhys.79.555}
}
@article{selby2019compositional,
	title        = {{Compositional resource theories of coherence}},
	author       = {Selby, John H and Lee, Ciar{\'a}n M},
	year         = 2019,
	journal      = {arXiv:1911.04513},
	url          = {https://arxiv.org/abs/1911.04513}
}
@article{cho2017disintegration,
	title        = {{Disintegration and Bayesian inversion, both abstractly and concretely}},
	author       = {Cho, Kenta and Jacobs, Bart},
	year         = 2017,
	journal      = {arxiv org/abs/1709.00322},
	url          = {https://www.cs.ru.nl/K.Cho/papers/disintegration.pdf}
}
@article{Deba2019,
	title        = {{Quantum prescriptions are more ontologically distinct than they are operationally distinguishable}},
	author       = {{Chaturvedi}, Anubhav and {Saha}, Debashis},
	year         = 2019,
	month        = sep,
	archiveprefix = {arXiv},
	eprint       = {1909.07293},
	adsurl       = {https://ui.adsabs.harvard.edu/abs/2019arXiv190907293C}
}
@misc{Leiferpersonalcomm,
	author       = {Leifer, Matt},
	howpublished = {personal communication}
}
@article{saha2019preparation,
	title        = {{Preparation contextuality as an essential feature underlying quantum communication advantage}},
	author       = {Saha, Debashis and Chaturvedi, Anubhav},
	year         = 2019,
	month        = aug,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 100,
	pages        = {022108},
	doi          = {10.1103/PhysRevA.100.022108},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.100.022108},
	issue        = 2,
	numpages     = 13
}
@article{fritz2016beyond,
	title        = {{Beyond Bell's theorem II: Scenarios with arbitrary causal structure}},
	author       = {Fritz, Tobias},
	year         = 2016,
	journal      = {Communications in Mathematical Physics},
	publisher    = {Springer},
	volume       = 341,
	number       = 2,
	pages        = {391--434},
	url          = {https://link.springer.com/article/10.1007%2Fs00220-015-2495-5}
}
@article{fritz2012beyond,
	title        = {{Beyond Bell's theorem: correlation scenarios}},
	author       = {Fritz, Tobias},
	year         = 2012,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 14,
	number       = 10,
	pages        = 103001,
	url          = {https://iopscience.iop.org/article/10.1088/1367-2630/14/10/103001/meta}
}
@article{henson2014theory,
	title        = {{Theory-independent limits on correlations from generalized Bayesian networks}},
	author       = {Henson, Joe and Lal, Raymond and Pusey, Matthew F},
	year         = 2014,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 16,
	number       = 11,
	pages        = 113043,
	url          = {https://iopscience.iop.org/article/10.1088/1367-2630/16/11/113043/meta}
}
@article{selby2017leaks,
	title        = {{Leaks: quantum, classical, intermediate and more}},
	author       = {Selby, John and Coecke, Bob},
	year         = 2017,
	journal      = {Entropy},
	publisher    = {Multidisciplinary Digital Publishing Institute},
	volume       = 19,
	number       = 4,
	pages        = 174,
	url          = {https://www.mdpi.com/1099-4300/19/4/174}
}
@article{peres2002unspeakable,
	title        = {{Unspeakable quantum information. eprint}},
	author       = {Peres, A and Scudo, PF},
	year         = 2002,
	journal      = {quantph/0201017},
	url          = {https://arxiv.org/abs/0201017}
}
@misc{marvian2020inaccessible,
	title        = {{Inaccessible information in probabilistic models of quantum systems, non-contextuality inequalities and noise thresholds for contextuality}},
	author       = {Iman Marvian},
	year         = 2020,
	eprint       = {2003.05984},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{van2018effect,
	title        = {{An effect-theoretic reconstruction of quantum theory}},
	author       = {John van de Wetering},
	year         = 2019,
	month        = dec,
	journal      = {Compositionality},
	publisher    = {Compositionality},
	volume       = 1,
	pages        = 1,
	doi          = {10.32408/compositionality-1-1},
	url          = {https://doi.org/10.32408/compositionality-1-1}
}
@article{tull2018categorical,
	title        = {{A Categorical Reconstruction of Quantum Theory}},
	author       = {Tull,  Sean},
	year         = 2020,
	journal      = {Logical Methods in Computer Science ; Volume 16},
	publisher    = {episciences.org},
	pages        = {Issue 1 ; 1860--5974},
	doi          = {10.23638/LMCS-16(1:4)2020},
	url          = {https://lmcs.episciences.org/6035},
	language     = {en}
}
@inproceedings{abramsky2019comonadic,
	title        = {{A comonadic view of simulation and quantum resources}},
	author       = {Abramsky, Samson and Barbosa, Rui Soares and Karvonen, Martti and Mansfield, Shane},
	year         = 2019,
	booktitle    = {2019 34th Annual ACM/IEEE Symposium on Logic in Computer Science (LICS)},
	pages        = {1--12},
	url          = {https://ieeexplore.ieee.org/document/8785677},
	organization = {IEEE}
}
@article{coecke2014terminality,
	title        = {{Terminality implies non-signalling}},
	author       = {Coecke, Bob},
	year         = 2014,
	journal      = {arXiv:1405.3681},
	url          = {https://arxiv.org/abs/1405.3681}
}
@article{kissinger2017equivalence,
	title        = {{Equivalence of relativistic causal structure and process terminality}},
	author       = {Kissinger, Aleks and Hoban, Matty and Coecke, Bob},
	year         = 2017,
	journal      = {arXiv:1708.04118},
	url          = {https://arxiv.org/abs/1708.04118}
}
@article{karvonen2018categories,
	title        = {{Categories of empirical models}},
	author       = {Karvonen, Martti},
	year         = 2018,
	journal      = {arXiv:1804.01514},
	url          = {https://arxiv.org/abs/1804.01514}
}
@article{mansfield2018quantum,
	title        = {{Quantum advantage from sequential-transformation contextuality}},
	author       = {Mansfield, Shane and Kashefi, Elham},
	year         = 2018,
	journal      = {Physical review letters},
	publisher    = {APS},
	volume       = 121,
	number       = 23,
	pages        = 230401,
	url          = {https://dx.doi.org/10.1103/PhysRevLett.121.230401}
}
@article{gheorghiu2019ontological,
	title        = {{Ontological models for quantum theory as functors}},
	author       = {Gheorghiu, Alexandru and Heunen, Chris},
	year         = 2019,
	journal      = {arXiv:1905.09055},
	url          = {https://arxiv.org/abs/1905.09055}
}
@article{penrose1971applications,
	title        = {{Applications of negative dimensional tensors}},
	author       = {Penrose, Roger},
	year         = 1971,
	journal      = {Combinatorial mathematics and its applications},
	volume       = 1,
	pages        = {221--244},
	url          = {https://www.mscs.dal.ca/~selinger/papers/graphical-bib/public/Penrose-applications-of-negative-dimensional-tensors.pdf}
}
@incollection{kelly1972many,
	title        = {{Many-variable functorial calculus. I.}},
	author       = {Kelly, G Maxwell},
	year         = 1972,
	booktitle    = {Coherence in categories},
	publisher    = {Springer},
	pages        = {66--105},
	url          = {https://link.springer.com/chapter/10.1007/BFb0059556}
}
@inproceedings{abramsky2004categorical,
	title        = {{A categorical semantics of quantum protocols}},
	author       = {Abramsky, Samson and Coecke, Bob},
	year         = 2004,
	booktitle    = {Proceedings of the 19th Annual IEEE Symposium on Logic in Computer Science, 2004.},
	pages        = {415--425},
	url          = {https://ieeexplore.ieee.org/document/1319636},
	organization = {IEEE}
}
@article{hefford2020hyper,
	title        = {{Hyper-decoherence in Density Hypercubes}},
	author       = {Hefford, James and Gogioso, Stefano},
	year         = 2020,
	journal      = {arXiv:2003.08318},
	url          = {https://arxiv.org/abs/2003.08318}
}
@article{gogioso2018quantum,
	title        = {{Quantum field theory in categorical quantum mechanics}},
	author       = {Gogioso, Stefano and Genovese, Fabrizio},
	year         = 2018,
	journal      = {arXiv:1805.12087},
	url          = {https://arxiv.org/abs/1805.12087}
}
@article{gogioso2016infinite,
	title        = {{Infinite-dimensional categorical quantum mechanics}},
	author       = {Gogioso, Stefano and Genovese, Fabrizio},
	year         = 2016,
	journal      = {arXiv:1605.04305},
	url          = {https://arxiv.org/abs/1605.04305}
}
@article{gogioso2017fantastic,
	title        = {{Fantastic quantum theories and where to find them}},
	author       = {Gogioso, Stefano},
	year         = 2017,
	journal      = {arXiv:1703.10576},
	url          = {https://arxiv.org/abs/1703.10576}
}
@article{wilce2018shortcut,
	title        = {{A shortcut from categorical quantum theory to convex operational theories}},
	author       = {Wilce, Alexander},
	year         = 2018,
	journal      = {arXiv:1803.00707},
	url          = {https://arxiv.org/abs/1803.00707}
}
@article{gogioso2017categorical,
	title        = {{Categorical probabilistic theories}},
	author       = {Gogioso, Stefano and Scandolo, Carlo Maria},
	year         = 2017,
	journal      = {arXiv:1701.08075},
	url          = {https://arxiv.org/abs/1701.08075}
}
@book{d2017quantum,
	title        = {{Quantum theory from first principles: an informational approach}},
	author       = {D'Ariano, Giacomo Mauro and Chiribella, Giulio and Perinotti, Paolo},
	year         = 2017,
	publisher    = {Cambridge University Press},
	url          = {https://www.cambridge.org/core/books/quantum-theory-from-first-principles/4B583F61C12E168F55FBCC2664ADB750}
}
@article{hardy2010formalism,
	title        = {{A formalism-local framework for general probabilistic theories including quantum theory}},
	author       = {Hardy, Lucien},
	year         = 2010,
	journal      = {arXiv:1005.5164},
	url          = {https://arxiv.org/abs/1005.5164}
}
@article{coecke2010quantum,
	title        = {{Quantum picturalism}},
	author       = {Coecke, Bob},
	year         = 2010,
	journal      = {Contemporary physics},
	publisher    = {Taylor \& Francis},
	volume       = 51,
	number       = 1,
	pages        = {59--83},
	url          = {https://arxiv.org/abs/0908.1787}
}
@book{coecke2018picturing,
	title        = {{Picturing Quantum Processes: A First Course in Quantum Theory and Diagrammatic Reasoning}},
	author       = {Coecke, Bob and Kissinger, Aleks},
	year         = 2017,
	publisher    = {Cambridge University Press},
	doi          = {10.1017/9781316219317},
	place        = {Cambridge}
}
@article{coecke2004logic,
	title        = {{The logic of entanglement}},
	author       = {Coecke, Bob},
	year         = 2004,
	journal      = {0402014},
	url          = {https://arxiv.org/abs/0402014}
}
@inproceedings{mellies2006functorial,
	title        = {{Functorial boxes in string diagrams}},
	author       = {Melli{\`e}s, Paul-Andr{\'e}},
	year         = 2006,
	booktitle    = {International Workshop on Computer Science Logic},
	pages        = {1--30},
	url          = {https://link.springer.com/chapter/10.1007/11874683_1},
	organization = {Springer}
}
@incollection{selinger2010survey,
	title        = {{A survey of graphical languages for monoidal categories}},
	author       = {Selinger, Peter},
	year         = 2010,
	booktitle    = {New structures for physics},
	publisher    = {Springer},
	pages        = {289--355},
	url          = {https://link.springer.com/chapter/10.1007%2F978-3-642-12821-9_4}
}
@article{myers2016string,
	title        = {{String Diagrams For Double Categories and Equipments}},
	author       = {Myers, David Jaz},
	year         = 2016,
	journal      = {arXiv:1612.02762},
	url          = {https://arxiv.org/abs/1612.02762}
}
@article{fritz2018bimonoidal,
	title        = {{Bimonoidal structure of probability monads}},
	author       = {Fritz, Tobias and Perrone, Paolo},
	year         = 2018,
	journal      = {Electronic Notes in Theoretical Computer Science},
	publisher    = {Elsevier},
	volume       = 341,
	pages        = {121--149},
	url          = {https://www.sciencedirect.com/science/article/pii/S1571066118300872}
}
@article{joyal1991geometry,
	title        = {{The geometry of tensor calculus, I}},
	author       = {Joyal, Andr{\'e} and Street, Ross},
	year         = 1991,
	journal      = {Advances in mathematics},
	publisher    = {Academic Press},
	volume       = 88,
	number       = 1,
	pages        = {55--112},
	url          = {https://www.sciencedirect.com/science/article/pii/000187089190003P}
}
@book{spirtes2000causation,
	title        = {{Causation, prediction, and search}},
	author       = {Spirtes, Peter and Glymour, Clark N and Scheines, Richard and Heckerman, David},
	year         = 2000,
	publisher    = {MIT press},
	url          = {https://mitpress.mit.edu/books/causation-prediction-and-search-second-edition}
}
@article{perrone2019notes,
	title        = {{Notes on Category Theory with examples from basic mathematics}},
	author       = {Perrone, Paolo},
	year         = 2019,
	journal      = {arXiv:1912.10642},
	url          = {https://arxiv.org/abs/1912.10642}
}
@article{selby2018reconstructing,
	title        = {{Reconstructing quantum theory from diagrammatic postulates}},
	author       = {Selby, John H and Scandolo, Carlo Maria and Coecke, Bob},
	year         = 2018,
	journal      = {arXiv:1802.00367},
	url          = {https://arxiv.org/abs/1802.00367}
}
@article{LeiferSpekkens,
	title        = {{Towards a formulation of quantum theory as a causally neutral theory of Bayesian inference}},
	author       = {Leifer, M. S. and Spekkens, Robert W.},
	year         = 2013,
	month        = nov,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 88,
	pages        = {052130},
	doi          = {10.1103/PhysRevA.88.052130},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.88.052130},
	issue        = 5,
	numpages     = 38
}
@article{Chuang1997,
	title        = {{Prescription for Experimental Determination of the Dynamics of a Quantum Black Box}},
	author       = {Chuang, Isaac L. and Nielsen, M. A.},
	year         = 1997,
	month        = nov,
	journal      = {Journal of Modern Optics},
	volume       = 44,
	number       = {11-12},
	pages        = {2455--2467},
	doi          = {10.1080/09500349708231894},
	issn         = {0950-0340}
}
@article{Schmidcausal,
	title        = {{Why initial system-environment correlations do not imply the failure of complete positivity: A causal perspective}},
	author       = {Schmid, David and Ried, Katja and Spekkens, Robert W.},
	year         = 2019,
	month        = aug,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 100,
	pages        = {022112},
	doi          = {10.1103/PhysRevA.100.022112},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.100.022112},
	issue        = 2,
	numpages     = 26
}
@incollection{hardy2013theory,
	title        = {{On the theory of composition in physics}},
	author       = {Hardy, Lucien},
	year         = 2013,
	booktitle    = {Computation, Logic, Games, and Quantum Foundations. The Many Facets of Samson Abramsky},
	publisher    = {Springer},
	pages        = {83--106},
	url          = {https://link.springer.com/chapter/10.1007/978-3-642-38164-5_7}
}
@article{allen2017quantum,
	title        = {{Quantum Common Causes and Quantum Causal Models}},
	author       = {Allen, John-Mark A. and Barrett, Jonathan and Horsman, Dominic C. and Lee, Ciar\'an M. and Spekkens, Robert W.},
	year         = 2017,
	month        = jul,
	journal      = {Phys. Rev. X},
	publisher    = {American Physical Society},
	volume       = 7,
	pages        = {031021},
	doi          = {10.1103/PhysRevX.7.031021},
	url          = {https://link.aps.org/doi/10.1103/PhysRevX.7.031021},
	issue        = 3,
	numpages     = 22
}
@article{fritz2020synthetic,
	title        = {{A synthetic approach to Markov kernels, conditional independence and theorems on sufficient statistics}},
	author       = {Fritz, Tobias},
	year         = 2020,
	journal      = {Advances in Mathematics},
	publisher    = {Elsevier},
	volume       = 370,
	pages        = 107239,
	url          = {https://www.sciencedirect.com/science/article/abs/pii/S0001870820302656?via%3Dihub}
}
@article{furber2013towards,
	title        = {{Towards a categorical account of conditional probability}},
	author       = {Furber, Robert and Jacobs, Bart},
	year         = 2013,
	journal      = {arXiv:1306.0831},
	url          = {https://arxiv.org/abs/1306.0831}
}
@inproceedings{jacobs2019causal,
	title        = {{Causal inference by string diagram surgery}},
	author       = {Jacobs, Bart and Kissinger, Aleks and Zanasi, Fabio},
	year         = 2019,
	booktitle    = {International Conference on Foundations of Software Science and Computation Structures},
	pages        = {313--329},
	url          = {https://link.springer.com/chapter/10.1007/978-3-030-17127-8_18},
	organization = {Springer}
}
@article{coecke2012picturing,
	title        = {{Picturing classical and quantum Bayesian inference}},
	author       = {Coecke, Bob and Spekkens, Robert W},
	year         = 2012,
	journal      = {Synthese},
	publisher    = {Springer},
	volume       = 186,
	number       = 3,
	pages        = {651--696},
	url          = {https://www.jstor.org/stable/41494941}
}
@article{costa2016quantum,
	title        = {{Quantum causal modelling}},
	author       = {Costa, Fabio and Shrapnel, Sally},
	year         = 2016,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 18,
	number       = 6,
	pages        = {063032},
	url          = {https://iopscience.iop.org/article/10.1088/1367-2630/18/6/063032}
}
@article{shrapnel2019discovering,
	title        = {{Discovering quantum causal models}},
	author       = {Shrapnel, Sally},
	year         = 2019,
	journal      = {The British Journal for the Philosophy of Science},
	publisher    = {Oxford University Press},
	volume       = 70,
	number       = 1,
	pages        = {1--25},
	url          = {https://doi.org/10.1093/bjps/axx044}
}
@article{pienaar2020quantum,
	title        = {{Quantum causal models via quantum Bayesianism}},
	author       = {Pienaar, Jacques},
	year         = 2020,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 101,
	number       = 1,
	pages        = {012104},
	url          = {https://doi.org/10.1103/PhysRevA.101.012104}
}
@article{leifer2006quantum,
	title        = {{Quantum dynamics as an analog of conditional probability}},
	author       = {Leifer, Matthew S},
	year         = 2006,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 74,
	number       = 4,
	pages        = {042310},
	url          = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.74.042310}
}
@article{goyal2008information,
	title        = {{Information-geometric reconstruction of quantum theory}},
	author       = {Goyal, P.},
	year         = 2008,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 78,
	number       = 5,
	pages        = {052120},
	url          = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.78.052120}
}
@article{clifton2003characterizing,
	title        = {{Characterizing Quantum Theory in Terms of Information-Theoretic Constraints}},
	author       = {Clifton, Rob and Bub, Jeffrey and Halvorson, Hans},
	year         = 2003,
	month        = nov,
	day          = {01},
	journal      = {Foundations of Physics},
	volume       = 33,
	number       = 11,
	pages        = {1561--1591},
	doi          = {10.1023/A:1026056716397},
	issn         = {1572-9516},
	url          = {https://doi.org/10.1023/A:1026056716397}
}
@article{budiyono2017quantum,
	title        = {{Quantum mechanics as classical statistical mechanics with an ontic extension and an epistemic restriction}},
	author       = {Budiyono, A. and Rohrlich, D.},
	year         = 2017,
	journal      = {Nat. Commun.},
	publisher    = {Nature Publishing Group},
	volume       = 8,
	number       = 1,
	pages        = 1306,
	url          = {https://link.springer.com/article/10.1023/A:1026056716397}
}
@inproceedings{Royal-road,
	title        = {{A Royal Road to Quantum Theory (or Thereabouts), Extended Abstract}},
	author       = {Wilce, A.},
	year         = 2017,
	booktitle    = {{\rm Proceedings 13th International Conference on} Quantum Physics and Logic, {\rm Glasgow, Scotland, 6-10 June 2016}},
	publisher    = {Open Publishing Association},
	series       = {EPTCS},
	volume       = 236,
	pages        = {245--254},
	doi          = {10.4204/EPTCS.236.16},
	editor       = {Duncan, R. and Heunen, C.}
}
@article{hohn2017quantum,
	title        = {{Quantum theory from questions}},
	author       = {H{\"o}hn, P. A. and Wever, C. S. P.},
	year         = 2017,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 95,
	number       = 1,
	pages        = {012102},
	url          = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.95.012102}
}
@article{caves2002quantum,
	title        = {{Quantum probabilities as Bayesian probabilities}},
	author       = {Caves, Carlton M and Fuchs, Christopher A and Schack, R{\"u}diger},
	year         = 2002,
	journal      = {Physical review A},
	publisher    = {APS},
	volume       = 65,
	number       = 2,
	pages        = {022305},
	url          = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.65.022305}
}
@article{fuchs2013quantum,
	title        = {{Quantum-bayesian coherence}},
	author       = {Fuchs, Christopher A and Schack, R{\"u}diger},
	year         = 2013,
	journal      = {Reviews of modern physics},
	publisher    = {APS},
	volume       = 85,
	number       = 4,
	pages        = 1693,
	url          = {https://journals.aps.org/rmp/abstract/10.1103/RevModPhys.85.1693}
}
@book{hooker2012logico,
	title        = {{The Logico-Algebraic Approach to Quantum Mechanics: Volume I: Historical Evolution}},
	author       = {Hooker, Clifford Alan},
	year         = 2012,
	publisher    = {Springer Science \& Business Media},
	volume       = 5,
	url          = {https://www.springer.com/gp/book/9789027705679}
}
@book{hooker1979logico,
	title        = {{The Logico-Algebraic Approach to Quantum Mechanics: Vol. II: Contemporary Consolidation}},
	author       = {Hooker, Clifford Alan},
	year         = 1979,
	publisher    = {Springer Science \& Business Media},
	url          = {https://www.springer.com/gp/book/9789027707079}
}
@article{fuchs2010qbism,
	title        = {{QBism, the perimeter of quantum Bayesianism}},
	author       = {Fuchs, Christopher A},
	year         = 2010,
	journal      = {arXiv:1003.5209},
	url          = {https://arxiv.org/abs/1003.5209}
}
@inproceedings{leifer2007conditional,
	title        = {{Conditional density operators and the subjectivity of quantum operations}},
	author       = {Leifer, Matthew S},
	year         = 2007,
	booktitle    = {AIP Conference Proceedings},
	volume       = 889,
	number       = 1,
	pages        = {172--186},
	url          = {https://aip.scitation.org/doi/abs/10.1063/1.2713456},
	organization = {American Institute of Physics}
}
@article{barnum2014higher,
	title        = {Higher-order interference and single-system postulates characterizing quantum theory},
	author       = {Howard Barnum and Markus P M{\"u}ller and Cozmin Ududec},
	year         = 2014,
	month        = {dec},
	journal      = {New Journal of Physics},
	publisher    = {{IOP} Publishing},
	volume       = 16,
	number       = 12,
	pages        = 123029,
	doi          = {10.1088/1367-2630/16/12/123029},
	url          = {https://doi.org/10.1088%2F1367-2630%2F16%2F12%2F123029}
}
@book{duhem1991aim,
	title        = {{The aim and structure of physical theory}},
	author       = {Duhem, Pierre Maurice Marie},
	year         = 1991,
	publisher    = {Princeton University Press},
	volume       = 13,
	url          = {https://press.princeton.edu/books/paperback/9780691025247/the-aim-and-structure-of-physical-theory}
}
@incollection{van1976two,
	title        = {{Two dogmas of empiricism}},
	author       = {van Orman Quine, Willard},
	year         = 1976,
	booktitle    = {Can Theories be Refuted?},
	publisher    = {Springer},
	pages        = {41--64},
	url          = {https://www.jstor.org/stable/2181906}
}
@article{Chiribella2011,
	title        = {{Informational derivation of quantum theory}},
	author       = {Chiribella, Giulio and D'Ariano, Giacomo Mauro and Perinotti, Paolo},
	year         = 2011,
	month        = jul,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 84,
	pages        = {012311},
	doi          = {10.1103/PhysRevA.84.012311},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.84.012311},
	issue        = 1,
	numpages     = 39
}
@article{Masanes_2011,
	title        = {{A derivation of quantum theory from physical requirements}},
	author       = {Llu{\'{\i}}s Masanes and Markus P M{\"u}ller},
	year         = 2011,
	month        = jun,
	journal      = {New J. Phys.},
	publisher    = {{IOP} Publishing},
	volume       = 13,
	number       = 6,
	pages        = {063001},
	doi          = {10.1088/1367-2630/13/6/063001},
	url          = {https://doi.org/10.1088%2F1367-2630%2F13%2F6%2F063001}
}
@article{dakicbrukner,
	title        = {{Quantum Theory and Beyond: Is Entanglement Special?}},
	author       = {{Dakic}, Borivoje and {Brukner}, Caslav},
	year         = 2009,
	month        = nov,
	url          = {https://ui.adsabs.harvard.edu/abs/2009arXiv0911.0695D},
	archiveprefix = {arXiv},
	eprint       = {0911.0695}
}
@unpublished{GPTsAsCITheories,
	title        = {{Generalized probabilistic theories in the framework of causal-inferential theories}},
	author       = {David Schmid and John Selby and Robert W. Spekkens},
	note         = {Forthcoming}
}
@unpublished{DaleySpekkensToBePublished,
	title        = {{Experimentally adjudicating between different causal explanations of Bell inequality violations using standard model selection techniques}},
	author       = {Patrick Daley and Kevin Resch and Robert W. Spekkens},
	note         = {Forthcoming}
}
@article{chiribella2010probabilistic,
	title        = {{Probabilistic theories with purification}},
	author       = {Chiribella, Giulio and D'Ariano, Giacomo Mauro and Perinotti, Paolo},
	year         = 2010,
	month        = jun,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 81,
	number       = 6,
	pages        = {062348},
	doi          = {10.1103/PhysRevA.81.062348},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.81.062348},
	issue        = 6,
	numpages     = 40
}
@article{Chiribella2015QuantumTI,
	title        = {{Quantum Theory: Informational Foundations and Foils}},
	author       = {G. Chiribella and R. Spekkens},
	year         = 2015,
	journal      = {Springer Netherlands},
	url          = {https://www.springer.com/gp/book/9789401773027}
}
@article{mazurek2017experimentally,
	title        = {{Experimentally bounding deviations from quantum theory in the landscape of generalized probabilistic theories}},
	author       = {Mazurek, Michael D and Pusey, Matthew F and Resch, Kevin J and Spekkens, Robert W},
	year         = 2017,
	journal      = {arXiv:1710.05948},
	url          = {https://arxiv.org/abs/1710.05948}
}
@article{mazurek2021experimentally,
	title        = {{Experimentally Bounding Deviations From Quantum Theory in the Landscape of Generalized Probabilistic Theories}},
	author       = {Mazurek, Michael D. and Pusey, Matthew F. and Resch, Kevin J. and Spekkens, Robert W.},
	year         = 2021,
	month        = {Apr},
	journal      = {PRX Quantum},
	publisher    = {American Physical Society},
	volume       = 2,
	pages        = {020302},
	doi          = {10.1103/PRXQuantum.2.020302},
	url          = {https://link.aps.org/doi/10.1103/PRXQuantum.2.020302},
	issue        = 2,
	numpages     = 33
}
@inbook{spekkens2015paradigm,
	title        = {{The paradigm of kinematics and dynamics must yield to causal structure}},
	author       = {Spekkens, Robert W.},
	year         = 2015,
	booktitle    = {Questioning the Foundations of Physics: Which of Our Fundamental Assumptions Are Wrong?},
	publisher    = {Springer},
	pages        = {5--16},
	url          = {https://link.springer.com/chapter/10.1007/978-3-319-13045-3_2},
	editor       = {Aguirre, Anthony and Foster, Brendan and Merali, Zeeya}
}
@article{wood2015lesson,
	title        = {{The lesson of causal discovery algorithms for quantum correlations: Causal explanations of Bell-inequality violations require fine-tuning}},
	author       = {Wood, Christopher J and Spekkens, Robert W},
	year         = 2015,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 17,
	number       = 3,
	pages        = {033002},
	url          = {https://dx.doi.org/10.1088/1367-2630/17/3/033002}
}
@misc{Jaynesquote,
	note         = {E. T. Jaynes, in { Complexity, Entropy, and the Physics of Information}, edited by W. H. Zurek (Addison-Wesley, 1990) p. 381.}
}
@article{schmid2018contextual,
	title        = {{Contextual advantage for state discrimination}},
	author       = {Schmid, David and Spekkens, Robert W},
	year         = 2018,
	journal      = {Phys. Rev. X},
	publisher    = {APS},
	volume       = 8,
	number       = 1,
	pages        = {011015},
	url          = {https://journals.aps.org/prx/abstract/10.1103/PhysRevX.8.011015}
}
@article{ShahandehGPT,
	title        = {{Contextuality of General Probabilistic Theories}},
	author       = {Shahandeh, Farid},
	year         = 2021,
	month        = {Feb},
	journal      = {PRX Quantum},
	publisher    = {American Physical Society},
	volume       = 2,
	pages        = {010330},
	doi          = {10.1103/PRXQuantum.2.010330},
	url          = {https://link.aps.org/doi/10.1103/PRXQuantum.2.010330},
	issue        = 1,
	numpages     = 15
}
@incollection{chiribella2016quantum,
	title        = {{Quantum from Principles}},
	author       = {Giulio Chiribella and Giacomo Mauro D'Ariano and Paolo Perinotti},
	year         = 2015,
	month        = dec,
	booktitle    = {Fundamental Theories of Physics},
	publisher    = {Springer Netherlands},
	pages        = {171--221},
	doi          = {10.1007/978-94-017-7303-4_6},
	url          = {https://doi.org/10.1007/978-94-017-7303-4_6}
}
@article{SchmidGPT,
	title        = {{Characterization of Noncontextuality in the Framework of Generalized Probabilistic Theories}},
	author       = {Schmid, David and Selby, John H. and Wolfe, Elie and Kunjwal, Ravi and Spekkens, Robert W.},
	year         = 2021,
	month        = feb,
	journal      = {PRX Quantum},
	publisher    = {American Physical Society},
	volume       = 2,
	pages        = {010331},
	doi          = {10.1103/PRXQuantum.2.010331},
	url          = {https://link.aps.org/doi/10.1103/PRXQuantum.2.010331},
	issue        = 1,
	numpages     = 12
}
@article{leifer2014quantum,
	title        = {{Is the quantum state real? An extended review of psi-ontology theorems}},
	author       = {Leifer, Matthew Saul},
	year         = 2014,
	journal      = {arXiv:1409.1570},
	url          = {https://dx.doi.org/10.12743/quanta.v3i1.22}
}
@article{bartlett2012reconstruction,
	title        = {{Reconstruction of Gaussian quantum mechanics from Liouville mechanics with an epistemic restriction}},
	author       = {Bartlett, Stephen D and Rudolph, Terry and Spekkens, Robert W},
	year         = 2012,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 86,
	number       = 1,
	pages        = {012103},
	url          = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.86.012103}
}
@article{berksonparadox,
	title        = {{Limitations of the Application of Fourfold Table Analysis to Hospital Data}},
	author       = {Joseph Berkson},
	year         = 1946,
	journal      = {Biometrics Bulletin},
	publisher    = {[International Biometric Society, Wiley]},
	volume       = 2,
	number       = 3,
	pages        = {47--53},
	issn         = {00994987},
	url          = {http://www.jstor.org/stable/3002000}
}
@article{simpsonsparadox,
	title        = {{The Interpretation of Interaction in Contingency Tables}},
	author       = {Simpson, E. H.},
	year         = 1951,
	journal      = {Journal of the Royal Statistical Society: Series B (Methodological)},
	volume       = 13,
	number       = 2,
	pages        = {238--241},
	doi          = {10.1111/j.2517-6161.1951.tb00088.x}
}
@article{RAC2,
	title        = {{Parity oblivious d-level random access codes and class of noncontextuality inequalities}},
	author       = {Ambainis, Andris and Banik, Manik and Chaturvedi, Anubhav and Kravchenko, Dmitry and Rai, Ashutosh},
	year         = 2019,
	journal      = {Quantum Inf. Process.},
	publisher    = {Springer},
	volume       = 18,
	number       = 4,
	pages        = 111,
	url          = {https://link.springer.com/article/10.1007/s11128-019-2228-3}
}
@article{triangle,
	title        = {{Causal compatibility inequalities admitting quantum violations in the triangle structure}},
	author       = {Fraser, Thomas C. and Wolfe, Elie},
	year         = 2018,
	month        = aug,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 98,
	pages        = {022113},
	doi          = {10.1103/PhysRevA.98.022113},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.98.022113},
	issue        = 2,
	numpages     = 21
}
@article{Chaves2018,
	title        = {{Quantum violation of an instrumental test}},
	author       = {Chaves, Rafael and Carvacho, Gonzalo and Agresti, Iris and Di Giulio, Valerio and Aolita, Leandro and Giacomini, Sandro and Sciarrino, Fabio},
	year         = 2018,
	journal      = {Nature Physics},
	volume       = 14,
	number       = 3,
	pages        = {291--296},
	doi          = {10.1038/s41567-017-0008-5},
	issn         = {1745-2481},
	url          = {https://doi.org/10.1038/s41567-017-0008-5}
}
@article{Emersonthesis,
	title        = {{Quantum Chaos and Quantum-Classical Correspondence}},
	author       = {{Emerson}, Joseph},
	year         = 2002,
	month        = nov,
	archiveprefix = {arXiv},
	eprint       = {0211035},
	adsurl       = {https://ui.adsabs.harvard.edu/abs/2002quant.ph.11035E},
	adsnote      = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Lillystone2019,
	title        = {{Contextuality and the Single-Qubit Stabilizer Subtheory}},
	author       = {Lillystone, Piers and Wallman, Joel J. and Emerson, Joseph},
	year         = 2019,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 122,
	pages        = 140405,
	doi          = {10.1103/PhysRevLett.122.140405},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.122.140405},
	issue        = 14,
	numpages     = 5
}
@article{Lorenz2020,
	title        = {{Causal and compositional structure of unitary transformations}},
	author       = {{Lorenz}, Robin and {Barrett}, Jonathan},
	year         = 2020,
	month        = jan,
	url          = {https://ui.adsabs.harvard.edu/abs/2020arXiv200107774L},
	archiveprefix = {arXiv},
	eprint       = {2001.07774}
}
@article{leifer2008quantum,
	title        = {{Quantum graphical models and belief propagation}},
	author       = {Leifer, Matthew S and Poulin, David},
	year         = 2008,
	journal      = {Annals of Physics},
	publisher    = {Elsevier},
	volume       = 323,
	number       = 8,
	pages        = {1899--1946},
	url          = {https://www.sciencedirect.com/science/article/abs/pii/S0003491607001509?via%3Dihub}
}
@book{Mackey,
	title        = {{The mathematical foundations of quantum mechanics}},
	author       = {Mackey, G. W.},
	year         = 1963,
	publisher    = {W. A. Benjamin},
	address      = {New York},
	date-modified = {2014-03-10 18:36:51 +0000}
}
@article{Piron64,
	title        = {{Axiomatique Quantique}},
	author       = {C. Piron},
	year         = 1964,
	journal      = {Helvetia Physica Acta},
	volume       = 37,
	pages        = {439--468}
}
@book{Ludwig,
	title        = {{An Axiomatic Basis of Quantum Mechanics. 1. Derivation of Hilbert Space}},
	author       = {Ludwig, G.},
	year         = 1985,
	publisher    = {Springer-Verlag},
	date-modified = {2014-02-06 16:10:39 +0000}
}
@incollection{CMW,
	title        = {{Operational Quantum Logic: An Overview}},
	author       = {Coecke, B. and Moore, D. J. and Wilce, A.},
	year         = 2000,
	booktitle    = {Current Research in Operational Quantum Logic: Algebras, Categories and Languages},
	publisher    = {Springer-Verlag},
	series       = {Fundamental Theories of Physics},
	volume       = 111,
	pages        = {1--36},
	date-modified = {2014-02-05 23:44:20 +0000},
	editor       = {B. Coecke and D. J. Moore and A. Wilce}
}
@article{Soler,
	title        = {{Characterization of Hilbert spaces by orthomodular spaces}},
	author       = {M. P. Sol{\`e}r},
	year         = 1995,
	journal      = {Commun. Algebra},
	volume       = 23,
	number       = 1,
	pages        = {219--243}
}
@incollection{StubbeSteirt,
	title        = {{Propositional systems, Hilbert lattices and generalized Hilbert spaces}},
	author       = {I. Stubbe and B. van Steirteghem},
	year         = 2007,
	booktitle    = {Handbook Quantum Logic},
	publisher    = {Elsevier Publ.},
	pages        = {477--524},
	date-modified = {2014-02-06 16:11:58 +0000},
	editor       = {D. Gabbay, D. Lehmann and K. Engesser}
}
@article{Randall,
	title        = {{Operational statistics. II. Manuals of operations and their logics}},
	author       = {C. H. Randall and D. J. Foulis},
	year         = 1973,
	journal      = {Journal of Mathematical Physics},
	volume       = 14,
	number       = 10,
	pages        = {1472--1480}
}
@article{Harding2,
	title        = {{A link between quantum logic and categorical quantum mechanics}},
	author       = {J. Harding},
	year         = 2009,
	journal      = {International Journal of Theoretical Physics},
	volume       = 48,
	number       = 3,
	pages        = {769--802}
}
@book{CMWbook,
	title        = {{Current research in operational quantum logic: algebras, categories, languages}},
	author       = {Coecke, B. and Moore, D. J. and Wilce, A.},
	year         = 2000,
	publisher    = {Springer},
	volume       = 111,
	date-modified = {2014-02-05 23:44:26 +0000}
}
@article{BvN,
	title        = {{The logic of quantum mechanics}},
	author       = {G. Birkhoff and J. von Neumann},
	year         = 1936,
	journal      = {Annals of Mathematics},
	volume       = 37,
	pages        = {823--843}
}
@article{Barrett2019,
	title        = {{Quantum Causal Models}},
	author       = {{Barrett}, Jonathan and {Lorenz}, Robin and {Oreshkov}, Ognyan},
	year         = 2019,
	month        = jun,
	url          = {https://ui.adsabs.harvard.edu/abs/2019arXiv190610726B},
	archiveprefix = {arXiv},
	eprint       = {1906.10726},
	adsnote      = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{lewis2012distinct,
	title        = {{Distinct quantum states can be compatible with a single state of reality}},
	author       = {Lewis, Peter G and Jennings, David and Barrett, Jonathan and Rudolph, Terry},
	year         = 2012,
	journal      = {Physical Review Letters},
	publisher    = {APS},
	volume       = 109,
	number       = 15,
	pages        = 150404,
	url          = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.109.150404}
}
@article{Tsirelson,
	title        = {{Quantum generalizations of Bell's inequality}},
	author       = {{Cirel'Son}, B.~S.},
	year         = 1980,
	month        = mar,
	journal      = {Letters in Mathematical Physics},
	volume       = 4,
	number       = 2,
	pages        = {93--100},
	doi          = {10.1007/BF00417500},
	url          = {https://ui.adsabs.harvard.edu/abs/1980LMaPh...4...93C},
	adsnote      = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{SpePIRSA,
	title        = {{Why I Am Not a Psi-Ontologist}},
	author       = {Spekkens, Robert W},
	journal      = {PIRSA},
	url          = {http://pirsa.org/12050021/}
}
@article{SpePIRSA2,
	title        = {{Cause and Effect in a Quantum World}},
	author       = {Spekkens, Robert W},
	journal      = {PIRSA},
	url          = {http://pirsa.org/15060039/}
}
@article{Leifer_2014,
	title        = {{A Bayesian approach to compatibility, improvement, and pooling of quantum states}},
	author       = {M S Leifer and Robert W Spekkens},
	year         = 2014,
	month        = jun,
	journal      = {Journal of Physics A: Mathematical and Theoretical},
	publisher    = {{IOP} Publishing},
	volume       = 47,
	number       = 27,
	pages        = 275301,
	doi          = {10.1088/1751-8113/47/27/275301},
	url          = {https://doi.org/10.1088%2F1751-8113%2F47%2F27%2F275301}
}
@unpublished{lillystone2019contextual,
	title        = {{A Contextual $\psi$-Epistemic Model of the $n$-Qubit Stabilizer Formalism}},
	author       = {Lillystone, Piers and Emerson, Joseph},
	year         = 2019,
	url          = {https://arxiv.org/abs/1904.04268},
	eprint       = {1904.04268},
	archiveprefix = {arXiv}
}
@article{pooling2007,
	title        = {{Pooling quantum states obtained by indirect measurements}},
	author       = {Spekkens, Robert W. and Wiseman, H. M.},
	year         = 2007,
	month        = apr,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 75,
	pages        = {042104},
	doi          = {10.1103/PhysRevA.75.042104},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.75.042104},
	issue        = 4,
	numpages     = 5
}
@inbook{Wigner1995,
	title        = {{Remarks on the Mind-Body Question}},
	author       = {Wigner, E. P.},
	year         = 1995,
	booktitle    = {Philosophical Reflections and Syntheses},
	publisher    = {Springer Berlin Heidelberg},
	address      = {Berlin, Heidelberg},
	pages        = {247--260},
	doi          = {10.1007/978-3-642-78374-6_20},
	isbn         = {978-3-642-78374-6},
	url          = {https://doi.org/10.1007/978-3-642-78374-6_20},
	editor       = {Mehra, Jagdish}
}
@article{Frauchiger2018,
	title        = {{Quantum theory cannot consistently describe the use of itself}},
	author       = {Frauchiger, Daniela and Renner, Renato},
	year         = 2018,
	month        = sep,
	day          = 18,
	journal      = {Nat. Commun.},
	volume       = 9,
	number       = 1,
	pages        = 3711,
	doi          = {10.1038/s41467-018-05739-8},
	issn         = {2041-1723},
	url          = {https://doi.org/10.1038/s41467-018-05739-8}
}
@incollection{bell1995nouvelle,
	title        = {{La nouvelle cuisine}},
	author       = {Bell, John S},
	year         = 1995,
	booktitle    = {Quantum Mechanics, High Energy Physics And Accelerators: Selected Papers Of John S Bell (With Commentary)},
	publisher    = {World Scientific},
	pages        = {910--928},
	url          = {https://doi.org/10.1142/9789812386540_0022}
}
@book{pearl2009causality,
	title        = {{Causality}},
	author       = {Pearl, Judea},
	year         = 2009,
	publisher    = {Cambridge university press},
	url          = {https://doi.org/10.1017/CBO9780511803161}
}
@article{catani2017spekkens,
	title        = {{Spekkens' toy model in all dimensions and its relationship with stabiliser quantum mechanics}},
	author       = {Catani, Lorenzo and Browne, Dan E},
	year         = 2017,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 19,
	number       = 7,
	pages        = {073035},
	url          = {https://iopscience.iop.org/article/10.1088/1367-2630/aa781c}
}
@article{PhysRevA.98.052108,
	title        = {{State-injection schemes of quantum computation in Spekkens' toy theory}},
	author       = {Catani, Lorenzo and Browne, Dan E.},
	year         = 2018,
	month        = nov,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 98,
	pages        = {052108},
	doi          = {10.1103/PhysRevA.98.052108},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.98.052108},
	issue        = 5,
	numpages     = 12
}
@article{pusey2012stabilizer,
	title        = {{Stabilizer notation for Spekkens? toy theory}},
	author       = {Pusey, Matthew F},
	year         = 2012,
	journal      = {Foundations of Physics},
	publisher    = {Springer},
	volume       = 42,
	number       = 5,
	pages        = {688--708},
	url          = {https://link.springer.com/article/10.1007/s10701-012-9639-7}
}
@article{PhysRevLett.95.230504,
	title        = {{Stabilizer Formalism for Operator Quantum Error Correction}},
	author       = {Poulin, David},
	year         = 2005,
	month        = dec,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 95,
	pages        = 230504,
	doi          = {10.1103/PhysRevLett.95.230504},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.95.230504},
	issue        = 23,
	numpages     = 4
}
@article{PhysRevA.70.052328,
	title        = {{Improved simulation of stabilizer circuits}},
	author       = {Aaronson, Scott and Gottesman, Daniel},
	year         = 2004,
	month        = nov,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 70,
	pages        = {052328},
	doi          = {10.1103/PhysRevA.70.052328},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.70.052328},
	issue        = 5,
	numpages     = 14
}
@article{PhysRevA.83.020302,
	title        = {{Surface code quantum computing with error rates over 1%}},
	author       = {Wang, David S. and Fowler, Austin G. and Hollenberg, Lloyd C. L.},
	year         = 2011,
	month        = feb,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 83,
	pages        = {020302},
	doi          = {10.1103/PhysRevA.83.020302},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.83.020302},
	issue        = 2,
	numpages     = 4
}
@article{ashikhmin2001nonbinary,
	title        = {{Nonbinary quantum stabilizer codes}},
	author       = {Ashikhmin, Alexei and Knill, Emanuel},
	year         = 2001,
	journal      = {IEEE Transactions on Information Theory},
	publisher    = {IEEE},
	volume       = 47,
	number       = 7,
	pages        = {3065--3072},
	url          = {https://ieeexplore.ieee.org/abstract/document/959288?casa_token=KFuQspBlr5oAAAAA:Pr0hBSa4HSaSccu79EBMinuD63NCVOO8bmLYX19CsK5LdCHIDCA4MpsPc6FI1ZOjsU56QKHSSQ}
}
@article{Terhal2015,
	title        = {{Quantum error correction for quantum memories}},
	author       = {Terhal, Barbara M.},
	year         = 2015,
	month        = apr,
	journal      = {Rev. Mod. Phys.},
	publisher    = {American Physical Society},
	volume       = 87,
	pages        = {307--346},
	doi          = {10.1103/RevModPhys.87.307},
	url          = {https://link.aps.org/doi/10.1103/RevModPhys.87.307},
	issue        = 2,
	numpages     = 40
}
@article{riste2015detecting,
	title        = {{Detecting bit-flip errors in a logical qubit using stabilizer measurements}},
	author       = {Riste, Diego and Poletto, Stefano and Huang, M-Z and Bruno, Alessandro and Vesterinen, Visa and Saira, O-P and DiCarlo, Leonardo},
	year         = 2015,
	journal      = {Nat. Commun.},
	publisher    = {Nature Publishing Group},
	volume       = 6,
	number       = 1,
	pages        = {1--6},
	url          = {https://www.nature.com/articles/ncomms7983}
}
@article{nielsen2001quantum,
	title        = {{Quantum computation and quantum information}},
	author       = {Nielsen, Michael A and Chuang, Isaac L},
	year         = 2001,
	journal      = {Phys. Today},
	volume       = 54,
	number       = 2,
	pages        = 60,
	url          = {https://www.cambridge.org/core/books/quantum-computation-and-quantum-information/01E10196D0A682A6AEFFEA52D53BE9AE}
}
@article{LOSRvsLOCCentang,
	title        = {{Why standard entanglement theory is inappropriate for the study of Bell scenarios}},
	author       = {{Schmid}, David and {Fraser}, Thomas C. and {Kunjwal}, Ravi and {Sainz}, Ana Belen and {Wolfe}, Elie and {Spekkens}, Robert W.},
	year         = 2020,
	month        = apr,
	url          = {https://ui.adsabs.harvard.edu/abs/2020arXiv200409194S},
	archiveprefix = {arXiv},
	eprint       = {2004.09194},
	adsnote      = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{veitch2012negative,
	title        = {{Negative quasi-probability as a resource for quantum computation}},
	author       = {Veitch, Victor and Ferrie, Christopher and Gross, David and Emerson, Joseph},
	year         = 2012,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 14,
	number       = 11,
	pages        = 113011,
	url          = {https://iopscience.iop.org/article/10.1088/1367-2630/14/11/113011/meta}
}
@article{veitch2014resource,
	title        = {{The resource theory of stabilizer quantum computation}},
	author       = {Veitch, Victor and Mousavian, SA Hamed and Gottesman, Daniel and Emerson, Joseph},
	year         = 2014,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 16,
	number       = 1,
	pages        = {013009},
	url          = {https://iopscience.iop.org/article/10.1088/1367-2630/16/1/013009/meta}
}
@article{Schmid2020typeindependent,
	title        = {{The type-independent resource theory of local operations and shared randomness}},
	author       = {Schmid, David and Rosset, Denis and Buscemi, Francesco},
	year         = 2020,
	month        = apr,
	journal      = {{Quantum}},
	publisher    = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
	volume       = 4,
	pages        = 262,
	doi          = {10.22331/q-2020-04-30-262},
	issn         = {2521-327X},
	url          = {https://doi.org/10.22331/q-2020-04-30-262}
}
@article{Rossettype,
	title        = {{Type-Independent Characterization of Spacelike Separated Resources}},
	author       = {Rosset, Denis and Schmid, David and Buscemi, Francesco},
	year         = 2020,
	month        = nov,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 125,
	pages        = 210402,
	doi          = {10.1103/PhysRevLett.125.210402},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.125.210402},
	issue        = 21,
	numpages     = 7
}
@article{lee2018no,
	title        = {{A no-go theorem for theories that decohere to quantum mechanics}},
	author       = {Lee, Ciar{\'a}n M and Selby, John H},
	year         = 2018,
	journal      = {Proceedings of the Royal Society A: Mathematical, Physical and Engineering Sciences},
	publisher    = {The Royal Society Publishing},
	volume       = 474,
	number       = 2214,
	pages        = 20170732,
	url          = {https://royalsocietypublishing.org/doi/full/10.1098/rspa.2017.0732}
}
@article{sainz2015postquantum,
	title        = {{Postquantum steering}},
	author       = {Sainz, Ana Bel{\'e}n and Brunner, Nicolas and Cavalcanti, Daniel and Skrzypczyk, Paul and V{\'e}rtesi, Tam{\'a}s},
	year         = 2015,
	journal      = {Physical review letters},
	publisher    = {APS},
	volume       = 115,
	number       = 19,
	pages        = 190403,
	url          = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.115.190403}
}
@article{schmid2020postquantum,
	title        = {{Postquantum common-cause channels: the resource theory of local operations and shared entanglement}},
	author       = {Schmid, David and Du, Haoxing and Mudassar, Maryam and Wit, Ghi Coulter-de and Rosset, Denis and Hoban, Matty J},
	year         = 2020,
	journal      = {arXiv:2004.06133},
	url          = {https://arxiv.org/abs/2004.06133}
}
@article{zyczkowski2008quartic,
	title        = {{Quartic quantum theory: an extension of the standard quantum mechanics}},
	author       = {{\.Z}yczkowski, Karol},
	year         = 2008,
	journal      = {Journal of Physics A: Mathematical and Theoretical},
	publisher    = {IOP Publishing},
	volume       = 41,
	number       = 35,
	pages        = 355302,
	url          = {https://iopscience.iop.org/article/10.1088/1751-8113/41/35/355302}
}
@article{barnum2016composites,
	title        = {{Composites and categories of Euclidean Jordan algebras}},
	author       = {Barnum, Howard and Graydon, Matthew A and Wilce, Alexander},
	year         = 2016,
	journal      = {arXiv preprint arXiv:1606.09331},
	url          = {https://arxiv.org/abs/1606.09331},
	eprint       = {1606.09331},
	archiveprefix = {arXiv}
}
@article{Henson2015,
	title        = {{Macroscopic noncontextuality as a principle for almost-quantum correlations}},
	author       = {Henson, Joe and Sainz, Ana BelÃ©n},
	year         = 2015,
	month        = apr,
	journal      = {Phys. Rev. A},
	volume       = 91,
	number       = 4,
	pages        = {042114},
	doi          = {10.1103/PhysRevA.91.042114},
	url          = {http://link.aps.org/doi/10.1103/PhysRevA.91.042114},
	urldate      = {2016-11-15}
}
@inproceedings{riesz1914demonstration,
	title        = {{D\'emonstration nouvelle d'un th\'eor\`eme concernant les op\'erations fonctionnelles lin\'eaires}},
	author       = {Riesz, Fr{\'e}d{\'e}ric},
	year         = 1914,
	booktitle    = {Annales scientifiques de l'{\'E}cole Normale Sup{\'e}rieure},
	volume       = 31,
	pages        = {9--14}
}
@article{Pawlowski2009,
	title        = {{Information causality as a physical principle}},
	author       = {Paw{\l}owski, Marcin and Paterek, Tomasz and Kaszlikowski, Dagomir and Scarani, Valerio and Winter, Andreas and {\.Z}ukowski, Marek},
	year         = 2009,
	month        = oct,
	journal      = {Nature},
	volume       = 461,
	number       = 7267,
	pages        = {1101--1104},
	doi          = {10.1038/nature08400},
	issn         = {1476-4687},
	url          = {https://www.nature.com/articles/nature08400},
	urldate      = {2020-04-10},
	copyright    = {2009 Macmillan Publishers Limited. All rights reserved},
	note         = {Number: 7267 Publisher: Nature Publishing Group}
}
@article{Linden2007,
	title        = {{Quantum Nonlocality and Beyond: Limits from Nonlocal Computation}},
	shorttitle   = {Quantum {Nonlocality} and {Beyond}},
	author       = {Linden, Noah and Popescu, Sandu and Short, Anthony J. and Winter, Andreas},
	year         = 2007,
	month        = oct,
	journal      = {Physical Review Letters},
	volume       = 99,
	number       = 18,
	pages        = 180502,
	doi          = {10.1103/PhysRevLett.99.180502},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.99.180502},
	urldate      = {2020-04-10},
	note         = {Publisher: American Physical Society}
}
@article{Gonda2018almostquantum,
	title        = {{Almost Quantum Correlations are Inconsistent with Specker's Principle}},
	author       = {Gonda, Tom{\'{a}}{\v{s}} and Kunjwal, Ravi and Schmid, David and Wolfe, Elie and Sainz, Ana Bel{\'{e}}n},
	year         = 2018,
	month        = aug,
	journal      = {{Quantum}},
	publisher    = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
	volume       = 2,
	pages        = 87,
	doi          = {10.22331/q-2018-08-27-87},
	issn         = {2521-327X},
	url          = {https://doi.org/10.22331/q-2018-08-27-87}
}
@article{Cabello2012,
	title        = {{Specker's fundamental principle of quantum mechanics}},
	author       = {Cabello, Adan},
	year         = 2012,
	month        = dec,
	journal      = {arXiv:1212.1756 [physics, physics:quant-ph]},
	url          = {http://arxiv.org/abs/1212.1756},
	urldate      = {2020-04-10},
	note         = {arXiv: 1212.1756},
	annote       = {Comment: REVTeX4, 4 pages, 1 figure, 1 video}
}
@article{Fritz2013a,
	title        = {{Local orthogonality as a multipartite principle for quantum correlations}},
	author       = {Fritz, Tobias and Sainz, Ana Bel{\'e}n and Augusiak, Remigiusz and Brask, J Bohr and Chaves, Rafael and Leverrier, Anthony and Ac{\'\i}n, Antonio},
	year         = 2013,
	month        = aug,
	journal      = {Nat. Commun.},
	volume       = 4,
	number       = 1,
	pages        = {1--7},
	doi          = {10.1038/ncomms3263},
	issn         = {2041-1723},
	url          = {https://www.nature.com/articles/ncomms3263},
	urldate      = {2020-04-10},
	copyright    = {2013 Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved.},
	note         = {Number: 1 Publisher: Nature Publishing Group}
}
@article{brassardetal,
	title        = {{Limit on Nonlocality in Any World in Which Communication Complexity Is Not Trivial}},
	author       = {Brassard, Gilles and Buhrman, Harry and Linden, Noah and M\'ethot, Andr\'e Allan and Tapp, Alain and Unger , Falk},
	year         = 2006,
	month        = jun,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 96,
	pages        = 250401,
	doi          = {10.1103/PhysRevLett.96.250401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.96.250401},
	author.hide  = {G. {Brassard~$\textit{et~al.}$}},
	issue        = 25,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.96.250401}
}
@article{hostens,
	title        = {{Stabilizer states and Clifford operations for systems of arbitrary dimensions and modular arithmetic}},
	author       = {Hostens, Erik and Dehaene, Jeroen and De Moor, Bart},
	year         = 2005,
	month        = apr,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 71,
	pages        = {042315},
	doi          = {10.1103/PhysRevA.71.042315},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.71.042315},
	issue        = 4,
	numpages     = 9,
	eprint       = {quant-ph/0408190},
	archiveprefix = {arXiv}
}
@article{kunjwal2018from,
	title        = {{From statistical proofs of the Kochen-Specker theorem to noise-robust noncontextuality inequalities}},
	author       = {Kunjwal, Ravi and Spekkens, Robert W.},
	year         = 2018,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 97,
	pages        = {052110},
	doi          = {10.1103/PhysRevA.97.052110},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.97.052110},
	issue        = 5,
	numpages     = 13
}
@misc{schmid2020structure,
	title        = {{A structure theorem for generalized-noncontextual ontological models}},
	author       = {Schmid, David and Selby, John H and Pusey, Matthew F and Spekkens, Robert W},
	year         = 2020,
	journal      = {arXiv preprint arXiv:2005.07161},
	eprint       = {2005.07161},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{hardy2012limited,
	title        = {{Limited Holism and Real-Vector-Space Quantum Theory}},
	author       = {Hardy, Lucien and Wootters, William K},
	year         = 2012,
	journal      = {Found. Phys.},
	publisher    = {Springer},
	volume       = 42,
	number       = 3,
	pages        = {454--473},
	doi          = {10.1007/s10701-011-9616-6},
	url          = {https://link.springer.com/article/10.1007/s10701-011-9616-6}
}
@article{horsman2017can,
	title        = {{Can a quantum state over time resemble a quantum state at a single time?}},
	author       = {Horsman, Dominic and Heunen, Chris and Pusey, Matthew F and Barrett, Jonathan and Spekkens, Robert W},
	year         = 2017,
	journal      = {Proceedings of the Royal Society A: Mathematical, Physical and Engineering Sciences},
	publisher    = {The Royal Society Publishing},
	volume       = 473,
	number       = 2205,
	pages        = 20170395,
	url          = {https://royalsocietypublishing.org/doi/10.1098/rspa.2017.0395}
}
@article{norsen2006bell,
	title        = {{Bell locality and the nonlocal character of nature}},
	author       = {Norsen, Travis},
	year         = 2006,
	journal      = {quant-ph/0601205},
	url          = {https://arxiv.org/abs/quant-ph/0601205}
}
@article{werner2014comment,
	title        = {{Comment on What Bell did}},
	author       = {Werner, Reinhard F},
	year         = 2014,
	journal      = {J. Phys. A},
	publisher    = {IOP Publishing},
	volume       = 47,
	number       = 42,
	pages        = 424011,
	doi          = {10.1088/1751-8113/47/42/424011},
	url          = {https://doi.org/10.1088}
}
@article{Wolfe2020quantifyingbell,
	title        = {{Quantifying Bell: the Resource Theory of Nonclassicality of Common-Cause Boxes}},
	author       = {Wolfe, Elie and Schmid, David and Sainz, Ana Bel{\'{e}}n and Kunjwal, Ravi and Spekkens, Robert W.},
	year         = 2020,
	month        = jun,
	journal      = {{Quantum}},
	volume       = 4,
	pages        = 280,
	doi          = {10.22331/q-2020-06-08-280},
	issn         = {2521-327X},
	url          = {https://doi.org/10.22331/q-2020-06-08-280}
}
@article{Mayers2004,
	title        = {{Self Testing Quantum Apparatus}},
	author       = {Mayers, Dominic and Yao, Andrew},
	year         = 2004,
	journal      = {Quantum Information \& Computation},
	publisher    = {{Rinton Press, Incorporated}},
	volume       = 4,
	number       = 4,
	pages        = {273--286}
}
@article{Takagi-etal-2019,
	title        = {{Operational Advantage of Quantum Resources in Subchannel Discrimination}},
	author       = {Takagi, Ryuji and Regula, Bartosz and Bu, Kaifeng and Liu, Zi-Wen and Adesso, Gerardo},
	year         = 2019,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 122,
	pages        = 140402,
	doi          = {10.1103/PhysRevLett.122.140402},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.122.140402},
	issue        = 14,
	numpages     = 7
}
@article{hooft2017free,
	title        = {{Free Will in the Theory of Everything}},
	author       = {Hooft, Gerard't},
	year         = 2017,
	journal      = {arXiv:1709.02874},
	url          = {https://arxiv.org/pdf/1709.02874.pdf}
}
@article{Uola-etal-2019,
	title        = {{Quantifying Quantum Resources with Conic Programming}},
	author       = {Uola, Roope and Kraft, Tristan and Shang, Jiangwei and Yu, Xiao-Dong and G\"uhne, Otfried},
	year         = 2019,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 122,
	pages        = 130404,
	doi          = {10.1103/PhysRevLett.122.130404},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.122.130404},
	issue        = 13,
	numpages     = 6
}
@article{uola2019quantification,
	title        = {{Quantification of quantum dynamics with input-output games}},
	author       = {Uola, Roope and Kraft, Tristan and Abbott, Alastair A.},
	year         = 2020,
	month        = {May},
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 101,
	pages        = {052306},
	doi          = {10.1103/PhysRevA.101.052306},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.101.052306},
	issue        = 5,
	numpages     = 9
}
@article{Takagi-Regula-PRX,
	title        = {{General Resource Theories in Quantum Mechanics and Beyond: Operational Characterization via Discrimination Tasks}},
	author       = {Takagi, Ryuji and Regula, Bartosz},
	year         = 2019,
	month        = sep,
	journal      = {Phys. Rev. X},
	publisher    = {American Physical Society},
	volume       = 9,
	pages        = {031053},
	doi          = {10.1103/PhysRevX.9.031053},
	url          = {https://link.aps.org/doi/10.1103/PhysRevX.9.031053},
	issue        = 3,
	numpages     = 28
}
@article{Skr-Linden-2019,
	title        = {{Robustness of Measurement, Discrimination Games, and Accessible Information}},
	author       = {Skrzypczyk, Paul and Linden, Noah},
	year         = 2019,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 122,
	pages        = 140403,
	doi          = {10.1103/PhysRevLett.122.140403},
	issue        = 14,
	numpages     = 6
}
@article{Skr-Supic-Cavalcanti-2019,
	title        = {{All Sets of Incompatible Measurements give an Advantage in Quantum State Discrimination}},
	author       = {Skrzypczyk, Paul and Supic, Ivan and Cavalcanti, Daniel},
	year         = 2019,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 122,
	pages        = 130403,
	doi          = {10.1103/PhysRevLett.122.130403},
	issue        = 13,
	numpages     = 6
}
@article{Montanaro2016,
	title        = {{A Survey of Quantum Property Testing}},
	author       = {Montanaro, Ashley and {de Wolf}, Ronald},
	year         = 2016,
	month        = jul,
	journal      = {Theory of Computing},
	pages        = {1--81},
	doi          = {10.4086/toc.gs.2016.007},
	issn         = {1557-2862},
	language     = {EN}
}
@misc{gonda2019monotones,
	title        = {{Monotones in General Resource Theories}},
	author       = {Tom{\'{a}}{\v{s}} Gonda and Robert W. Spekkens},
	year         = 2021,
	eprint       = {1912.07085},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{Supic2019a,
	author       = {{\v S}upi{\'c}, Ivan and Bowles, Joseph},
	year         = 2019,
	month        = apr,
	archiveprefix = {arXiv},
	eprint       = {1904.10042}
}
@article{sq,
	title        = {{All Entangled Quantum States Are Nonlocal}},
	author       = {Buscemi, Francesco},
	year         = 2012,
	month        = may,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 108,
	pages        = 200401,
	doi          = {10.1103/PhysRevLett.108.200401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.108.200401},
	issue        = 20,
	numpages     = 5
}
@article{schrodinger_1935,
	title        = {{Discussion of Probability Relations between Separated Systems}},
	author       = {Schrodinger, E.},
	year         = 1935,
	journal      = {Mathematical Proceedings of the Cambridge Philosophical Society},
	publisher    = {Cambridge University Press},
	volume       = 31,
	number       = 4,
	pages        = {555--563},
	doi          = {10.1017/S0305004100013554}
}
@article{telep,
	title        = {{All Entangled States can Demonstrate Nonclassical Teleportation}},
	author       = {Cavalcanti, Daniel and Skrzypczyk, Paul and \ifmmode \check{S}\else \v{S}\fi{}upi\ifmmode \acute{c}\else \'{c}\fi{}, Ivan},
	year         = 2017,
	month        = sep,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 119,
	pages        = 110501,
	doi          = {10.1103/PhysRevLett.119.110501},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.119.110501},
	issue        = 11,
	numpages     = 5
}
@article{Bennett93,
	title        = {{Teleporting an unknown quantum state via dual classical and Einstein-Podolsky-Rosen channels}},
	author       = {Bennett, Charles H. and Brassard, Gilles and Cr\'epeau, Claude and Jozsa, Richard and Peres, Asher and Wootters, William K.},
	year         = 1993,
	month        = mar,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 70,
	pages        = {1895--1899},
	doi          = {10.1103/PhysRevLett.70.1895},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.70.1895},
	issue        = 13,
	numpages     = {0}
}
@article{Hoban_2018,
	title        = {{A channel-based framework for steering, non-locality and beyond}},
	author       = {Matty J Hoban and Ana Bel{\'{e}}n Sainz},
	year         = 2018,
	month        = may,
	journal      = {New Journal of Physics},
	publisher    = {{IOP} Publishing},
	volume       = 20,
	number       = 5,
	pages        = {053048},
	doi          = {10.1088/1367-2630/aabea8},
	url          = {https://doi.org/10.1088%2F1367-2630%2Faabea8}
}
@article{Supic2018,
	title        = {{Quantifying Non-Classical Teleportation}},
	author       = {{\v S}upi{\'c}, Ivan and Skrzypczyk, Paul and Cavalcanti, Daniel},
	year         = 2018,
	month        = apr,
	archiveprefix = {arXiv},
	eprint       = {1804.10612}
}
@article{Uola2019,
	title        = {{Quantum Steering}},
	author       = {Uola, Roope and Costa, Ana C. S. and Nguyen, H. Chau and G{\"u}hne, Otfried},
	year         = 2019,
	month        = mar,
	archiveprefix = {arXiv},
	eprint       = {1903.06663}
}
@misc{LipkaBartosik2019,
	title        = {{The Operational Advantages Provided by Non-Classical Teleportation}},
	author       = {{Lipka-Bartosik}, Patryk and Skrzypczyk, Paul},
	year         = 2019,
	month        = aug,
	note         = {arxiv Preprint arXiv:1908.05107 [quant-ph]}
}
@article{steer,
	title        = {{Entanglement verification and steering when Alice and Bob cannot be trusted}},
	author       = {Cavalcanti, Eric G. and Hall, Michael J. W. and Wiseman, Howard M.},
	year         = 2013,
	month        = mar,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 87,
	pages        = {032306},
	doi          = {10.1103/PhysRevA.87.032306},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.87.032306},
	issue        = 3,
	numpages     = 8
}
@article{Werner,
	title        = {{Quantum states with Einstein-Podolsky-Rosen correlations admitting a hidden-variable model}},
	author       = {Werner, Reinhard F.},
	year         = 1989,
	month        = oct,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 40,
	pages        = {4277--4281},
	doi          = {10.1103/PhysRevA.40.4277},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.40.4277},
	issue        = 8,
	numpages     = {0}
}
@article{Barrettlocal,
	title        = {{Nonsequential positive-operator-valued measurements on entangled mixed states do not always violate a Bell inequality}},
	author       = {Barrett, Jonathan},
	year         = 2002,
	month        = mar,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 65,
	pages        = {042302},
	doi          = {10.1103/PhysRevA.65.042302},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.65.042302},
	issue        = 4,
	numpages     = 4
}
@article{channelsteer,
	title        = {{Channel steering}},
	author       = {Marco Piani},
	year         = 2015,
	month        = apr,
	journal      = {J. Opt. Soc. Am. B},
	publisher    = {OSA},
	volume       = 32,
	number       = 4,
	pages        = {A1--A7},
	doi          = {10.1364/JOSAB.32.0000A1},
	url          = {http://josab.osa.org/abstract.cfm?URI=josab-32-4-A1}
}
@article{wisesteer,
	title        = {{Steering, Entanglement, Nonlocality, and the Einstein-Podolsky-Rosen Paradox}},
	author       = {Wiseman, H. M. and Jones, S. J. and Doherty, A. C.},
	year         = 2007,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 98,
	pages        = 140402,
	doi          = {10.1103/PhysRevLett.98.140402},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.98.140402},
	issue        = 14,
	numpages     = 4
}
@article{BobWI,
	title        = {{Bipartite post-quantum steering in generalised scenarios}},
	author       = {{Bel{\'e}n Sainz}, Ana and {Hoban}, Matty J. and {Skrzypczyk}, Paul and {Aolita}, Leandro},
	year         = 2019,
	month        = jul,
	archiveprefix = {arXiv},
	eprint       = {1907.03705},
	adsurl       = {https://ui.adsabs.harvard.edu/abs/2019arXiv190703705B},
	adsnote      = {Provided by the SAO/NASA Astrophysics Data System}
}
@book{Watrous,
	title        = {{The theory of quantum information}},
	author       = {Watrous, John},
	year         = 2018,
	publisher    = {Cambridge University Press},
	place        = {Cambridge, United Kingdom}
}
@article{causallocaliz,
	title        = {{Causal and localizable quantum operations}},
	author       = {Beckman, David and Gottesman, Daniel and Nielsen, M. A. and Preskill, John},
	year         = 2001,
	month        = oct,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 64,
	pages        = {052309},
	doi          = {10.1103/PhysRevA.64.052309},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.64.052309},
	issue        = 5,
	numpages     = 21
}
@article{Sperling2011,
	title        = {{The Schmidt Number as a Universal Entanglement Measure}},
	author       = {Sperling, J. and Vogel, W.},
	year         = 2011,
	journal      = {Physica Scripta},
	volume       = 83,
	number       = 4,
	pages        = {045002},
	doi          = {10.1088/0031-8949/83/04/045002},
	issn         = {1402-4896}
}
@article{resthry,
	title        = {{A mathematical theory of resources}},
	author       = {Bob Coecke and Tobias Fritz and Robert W. Spekkens},
	year         = 2016,
	journal      = {Information and Computation},
	volume       = 250,
	pages        = {59--86},
	doi          = {https://doi.org/10.1016/j.ic.2016.02.008},
	issn         = {0890-5401},
	url          = {http://www.sciencedirect.com/science/article/pii/S0890540116000353},
	note         = {{Q}uantum {P}hysics and {L}ogic}
}
@article{barrettgisin,
	title        = {{How Much Measurement Independence Is Needed to Demonstrate Nonlocality?}},
	author       = {Barrett, Jonathan and Gisin, Nicolas},
	year         = 2011,
	month        = mar,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 106,
	pages        = 100406,
	doi          = {10.1103/PhysRevLett.106.100406},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.106.100406},
	issue        = 10,
	numpages     = 4
}
@article{hall,
	title        = {{Local Deterministic Model of Singlet State Correlations Based on Relaxing Measurement Independence}},
	author       = {Hall, Michael J. W.},
	year         = 2010,
	month        = dec,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 105,
	pages        = 250404,
	doi          = {10.1103/PhysRevLett.105.250404},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.105.250404},
	issue        = 25,
	numpages     = 4
}
@article{kaur2018fundamental,
	title        = {{Fundamental limits on key rates in device-independent quantum key distribution}},
	author       = {Kaur, Eneet and Wilde, Mark M and Winter, Andreas},
	year         = 2018,
	url          = {https://arxiv.org/abs/1810.05627},
	eprinttype   = {arxiv},
	eprint       = {1810.05627}
}
@inproceedings{maudlin1992bell,
	title        = {{Bell's Inequality, Information Transmission, and Prism Models}},
	author       = {Maudlin, Tim},
	year         = 1992,
	booktitle    = {Philosophy of Science Association},
	number       = 1,
	pages        = {404--417},
	url          = {https://www.jstor.org/stable/192771},
	volume.hide  = 1992,
	organization.hide = {Philosophy of Science Association}
}
@article{Popescu1994,
	title        = {{Quantum Nonlocality as an Axiom}},
	author       = {Popescu, Sandu and Rohrlich, Daniel},
	year         = 1994,
	month        = mar,
	journal      = {Foundations of Physics},
	volume       = 24,
	number       = 3,
	pages        = {379--385},
	doi          = {10.1007/BF02058098},
	issn         = {0015-9018, 1572-9516},
	language     = {en}
}
@article{Barrett2005,
	title        = {{Nonlocal Correlations as an Information-Theoretic Resource}},
	author       = {Barrett, Jonathan and Linden, Noah and Massar, Serge and Pironio, Stefano and Popescu, Sandu and Roberts, David},
	year         = 2005,
	month        = feb,
	journal      = {Physical Review A},
	volume       = 71,
	number       = 2,
	pages        = {022101},
	doi          = {10.1103/PhysRevA.71.022101}
}
@misc{schmid2021only,
	title        = {{The only noncontextual model of the stabilizer subtheory is Gross's}},
	author       = {David Schmid and Haoxing Du and John H. Selby and Matthew F. Pusey},
	year         = 2021,
	eprint       = {2101.06263},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{Belltest1,
	title        = {{Loophole-free Bell inequality violation using electron spins separated by 1.3 kilometres}},
	author       = {B. {Hensen~$\textit{et~al.}$}},
	year         = 2015,
	month        = 10,
	day          = 21,
	journal      = {Nature},
	publisher    = {Nature Publishing Group},
	volume       = 526,
	pages        = {682 EP  -},
	doi          = {10.1038/nature15759},
	url          = {http://dx.doi.org/10.1038/nature15759},
	author.hide  = {Hensen, B. and Bernien, H. and Dr{\'e}au, A. E. and Reiserer, A. and Kalb, N. and Blok, M. S. and Ruitenberg, J. and Vermeulen, R. F. L. and Schouten, R. N. and Abell{\'a}n, C. and Amaya, W. and Pruneri, V. and Mitchell, M. W. and Markham, M. and Twitchen, D. J. and Elkouss, D. and Wehner, S. and Taminiau, T. H. and Hanson, R.},
	date         = {2015/10/21/online},
	l3           = {10.1038/nature15759; https://www.nature.com/articles/nature15759#supplementary-information},
	ty           = {JOUR}
}
@article{Belltest2,
	title        = {{Significant-Loophole-Free Test of Bell's Theorem with Entangled Photons}},
	author       = {M. {Giustina~$\textit{et~al.}$}},
	year         = 2015,
	month        = dec,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 115,
	pages        = 250401,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.115.250401},
	author.hide  = {Giustina, Marissa and Versteegh, Marijn A. M. and Wengerowsky, S\"oren and Handsteiner, Johannes and Hochrainer, Armin and Phelan, Kevin and Steinlechner, Fabian and Kofler, Johannes and Larsson, Jan-\AA{}ke and Abell\'an, Carlos and Amaya, Waldimar and Pruneri, Valerio and Mitchell, Morgan W. and Beyer, J\"orn and Gerrits, Thomas and Lita, Adriana E. and Shalm, Lynden K. and Nam, Sae Woo and Scheidl, Thomas and Ursin, Rupert and Wittmann, Bernhard and Zeilinger, Anton},
	issue        = 25,
	numpages     = 7,
	doi.hide     = {10.1103/PhysRevLett.115.250401}
}
@article{Belltest3,
	title        = {{Strong Loophole-Free Test of Local Realism}},
	author       = {L.K. {Shalm~$\textit{et~al.}$}},
	year         = 2015,
	month        = dec,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 115,
	pages        = 250402,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.115.250402},
	author.hide  = {Shalm, Lynden K. and Meyer-Scott, Evan and Christensen, Bradley G. and Bierhorst, Peter and Wayne, Michael A. and Stevens, Martin J. and Gerrits, Thomas and Glancy, Scott and Hamel, Deny R. and Allman, Michael S. and Coakley, Kevin J. and Dyer, Shellee D. and Hodge, Carson and Lita, Adriana E. and Verma, Varun B. and Lambrocco, Camilla and Tortorici, Edward and Migdall, Alan L. and Zhang, Yanbao and Kumor, Daniel R. and Farr, William H. and Marsili, Francesco and Shaw, Matthew D. and Stern, Jeffrey A. and Abell\'an, Carlos and Amaya, Waldimar and Pruneri, Valerio and Jennewein, Thomas and Mitchell, Morgan W. and Kwiat, Paul G. and Bienfang, Joshua C. and Mirin, Richard P. and Knill, Emanuel and Nam, Sae Woo},
	issue        = 25,
	numpages     = 10,
	doi.hide     = {10.1103/PhysRevLett.115.250402}
}
@article{Scarani2006QKD,
	title        = {{Secrecy extraction from no-signaling correlations}},
	author       = {Scarani, Valerio and Gisin, Nicolas and Brunner, Nicolas and Masanes, Llu{\'\i}s and Pino, Sergi and Ac\'{\i}n, Antonio},
	year         = 2006,
	month        = oct,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 74,
	pages        = {042339},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.74.042339},
	issue        = 4,
	numpages     = 21,
	doi.hide     = {10.1103/PhysRevA.74.042339}
}
@article{DIGME,
	title        = {{Device-Independent Witnesses of Genuine Multipartite Entanglement}},
	author       = {Bancal, Jean-Daniel and Gisin, Nicolas and Liang, Yeong-Cherng and Pironio, Stefano},
	year         = 2011,
	month        = jun,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 106,
	pages        = 250404,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.106.250404},
	issue        = 25,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.106.250404}
}
@article{selftesting,
	title        = {{Classical command of quantum systems}},
	author       = {Reichardt, Ben W. and Unger, Falk and Vazirani, Umesh},
	year         = 2013,
	month        = {04},
	day          = 24,
	journal      = {Nature},
	publisher    = {Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved. SN  -},
	volume       = 496,
	pages        = {456 EP  -},
	url          = {http://dx.doi.org/10.1038/nature12035},
	date         = {2013/04/24/online},
	date-added   = {2018-07-26 03:54:00 +0000},
	date-modified = {2018-07-26 03:54:00 +0000},
	l3           = {10.1038/nature12035; https://www.nature.com/articles/nature12035#supplementary-information},
	m3           = {Article},
	ty           = {JOUR},
	bdsk-url-1   = {http://dx.doi.org/10.1038/nature12035}
}
@article{colbeckamp,
	title        = {{Free randomness can be amplified}},
	author       = {Colbeck, Roger and Renner, Renato},
	year         = 2012,
	month        = {05},
	day          = {06},
	journal      = {Nat. Phys.},
	publisher    = {Nature Publishing Group SN  -},
	volume       = 8,
	pages        = {450 EP  -},
	url          = {http://dx.doi.org/10.1038/nphys2300},
	date         = {2012/05/06/online},
	date-added   = {2018-07-26 03:58:50 +0000},
	date-modified = {2018-07-26 03:58:50 +0000},
	l3           = {10.1038/nphys2300; https://www.nature.com/articles/nphys2300#supplementary-information},
	ty           = {JOUR},
	bdsk-url-1   = {http://dx.doi.org/10.1038/nphys2300}
}
@article{Pironio2010,
	title        = {{Random numbers certified by Bell's theorem}},
	author       = {Pironio, S. and Ac{\'\i}n, A. and Massar, S. and de la Giroday, A. Boyer and Matsukevich, D. N. and Maunz, P. and Olmschenk, S. and Hayes, D. and Luo, L. and Manning, T. A. and Monroe, C.},
	year         = 2010,
	month        = {04},
	day          = 15,
	journal      = {Nature},
	publisher    = {Macmillan Publishers Limited. All rights reserved SN  -},
	volume       = 464,
	pages        = {1021 EP  -},
	doi          = {10.1038/nature09008},
	url          = {http://dx.doi.org/10.1038/nature09008},
	author.hide  = {S. {Pironio~$\textit{et~al.}$}},
	date         = {2010/04/15/online},
	date-added   = {2018-07-26 04:04:02 +0000},
	date-modified = {2018-07-26 04:04:02 +0000},
	l3           = {10.1038/nature09008; https://www.nature.com/articles/nature09008#supplementary-information},
	ty           = {JOUR},
	bdsk-url-1   = {http://dx.doi.org/10.1038/nature09008}
}
@article{Pivoluska2015,
	title        = {{Device Independent Random Number Generation}},
	author       = {{Pivoluska}, Mataj and {Plesch}, Martin},
	year         = 2015,
	month        = feb,
	journal      = {Acta Physica Slovaca},
	volume       = 64,
	pages        = {600--663},
	url          = {https://arxiv.org/abs/1502.06393},
	issue        = 6,
	eprint.hide  = {1502.06393},
	primaryclass = {quant-ph}
}
@article{janotta2014,
	title        = {{Generalized probability theories: what determines the structure of quantum theory?}},
	author       = {Janotta, Peter and Hinrichsen, Haye},
	year         = 2014,
	journal      = {J. Phys. A},
	publisher    = {IOP Publishing},
	volume       = 47,
	number       = 32,
	pages        = 323001,
	doi          = {10.1088/1751-8113/47/32/323001}
}
@article{gallego2016nonlocality,
	title        = {{Nonlocality free wirings and the distinguishability between Bell boxes}},
	author       = {Gallego, Rodrigo and Aolita, Leandro},
	year         = 2017,
	month        = mar,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society ({APS})},
	volume       = 95,
	number       = 3,
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.95.032118},
	date         = {2016-11-21},
	doi.hide     = {10.1103/PhysRevA.95.032118}
}
@article{qcombs08,
	title        = {{Quantum Circuit Architecture}},
	author       = {Chiribella, G. and D'Ariano, G. M. and Perinotti, P.},
	year         = 2008,
	month        = aug,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 101,
	pages        = {060401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.101.060401},
	issue        = 6,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.101.060401}
}
@article{qcombs09,
	title        = {{Theoretical framework for quantum networks}},
	author       = {Chiribella, Giulio and D'Ariano, Giacomo Mauro and Perinotti, Paolo},
	year         = 2009,
	month        = aug,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 80,
	pages        = {022339},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.80.022339},
	issue        = 2,
	numpages     = 20,
	doi.hide     = {10.1103/PhysRevA.80.022339}
}
@article{WPICC,
	title        = {{Operational Framework for Nonlocality}},
	author       = {Gallego, Rodrigo and W\"urflinger, Lars Erik and Ac\'{\i}n, Antonio and Navascu\'es, Miguel},
	year         = 2012,
	month        = aug,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 109,
	pages        = {070401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.109.070401},
	issue        = 7,
	numpages     = 5,
	doi.hide     = {10.1103/PhysRevLett.109.070401}
}
@article{OCB12,
	title        = {{Quantum correlations with no causal order}},
	author       = {Oreshkov, Ognyan and Costa, Fabio and Brukner, {\v C}aslav},
	year         = 2012,
	month        = 10,
	day          = {02},
	journal      = {Nat. Comm.},
	publisher    = {The Author(s) SN  -},
	volume       = 3,
	pages        = {1092 EP  -},
	url          = {http://dx.doi.org/10.1038/ncomms2076},
	date         = {2012/10/02/online},
	date-added   = {2018-07-26 19:43:42 +0000},
	date-modified = {2018-07-26 19:43:42 +0000},
	l3           = {10.1038/ncomms2076; https://www.nature.com/articles/ncomms2076#supplementary-information},
	m3           = {Article},
	ty           = {JOUR},
	bdsk-url-1   = {http://dx.doi.org/10.1038/ncomms2076}
}
@article{Oreshkov2016,
	title        = {{Causal and causally separable processes}},
	author       = {Ognyan Oreshkov and Christina Giarmatzi},
	year         = 2016,
	month        = sep,
	journal      = {New J. Phys.},
	publisher    = {{IOP} Publishing},
	volume       = 18,
	number       = 9,
	pages        = {093020},
	doi          = {10.1088/1367-2630/18/9/093020},
	url          = {https://doi.org/10.1088/1367-2630/18/9/093020}
}
@article{beigi2015monotone,
	title        = {{Monotone Measures for Non-Local Correlations}},
	author       = {Beigi, Salman and Gohari, Amin},
	year         = 2015,
	month        = sep,
	journal      = {{IEEE} T. Inform. Theory},
	publisher    = {IEEE},
	volume       = 61,
	number       = 9,
	pages        = {5185--5208},
	doi          = {10.1109/tit.2015.2452253}
}
@article{de2014nonlocality,
	title        = {{On nonlocality as a resource theory and nonlocality measures}},
	author       = {{de} Vicente, Julio I},
	year         = 2014,
	month        = oct,
	journal      = {J. Phys. A},
	publisher    = {IOP Publishing},
	volume       = 47,
	number       = 42,
	pages        = 424017,
	doi          = {10.1088/1751-8113/47/42/424017}
}
@article{horodecki2015axiomatic,
	title        = {{Axiomatic approach to contextuality and nonlocality}},
	author       = {Karol Horodecki and Andrzej Grudka and Pankaj Joshi and Waldemar K{\l}obus and Justyna {\L}odyga},
	year         = 2015,
	month        = sep,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 92,
	number       = 3,
	pages        = {032104},
	doi          = {10.1103/physreva.92.032104}
}
@article{short2006entanglement,
	title        = {{Entanglement swapping for generalized nonlocal correlations}},
	author       = {Short, A.~J. and Popescu, Sandu and Gisin, Nicolas},
	year         = 2006,
	month        = jan,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 73,
	number       = 1,
	pages        = {012101},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.73.012101},
	doi.hide     = {10.1103/PhysRevA.73.012101}
}
@article{allcock2009closed,
	title        = {{Closed sets of nonlocal correlations}},
	author       = {Allcock, Jonathan and Brunner, Nicolas and Linden, Noah and Popescu, Sandu and Skrzypczyk, Paul and V{\'e}rtesi, Tam{\'a}s},
	year         = 2009,
	month        = dec,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 80,
	number       = 6,
	pages        = {062107},
	doi          = {10.1103/PhysRevA.80.062107},
	author.hide  = {J. {Allcock~$\textit{et~al.}$}}
}
@article{Acin2007QKD,
	title        = {{Device-Independent Security of Quantum Cryptography against Collective Attacks}},
	author       = {Ac\'{\i}n, Antonio and Brunner, Nicolas and Gisin, Nicolas and Massar, Serge and Pironio, Stefano and Scarani, Valerio},
	year         = 2007,
	month        = jun,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 98,
	pages        = 230501,
	doi          = {10.1103/PhysRevLett.98.230501},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.98.230501},
	author.hide  = {A. {Ac\'{\i}n~$\textit{et~al.}$}},
	issue        = 23,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.98.230501}
}
@article{vazirani14,
	title        = {{Fully Device-Independent Quantum Key Distribution}},
	author       = {Vazirani, Umesh and Vidick, Thomas},
	year         = 2014,
	month        = sep,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 113,
	pages        = 140501,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.113.140501},
	issue        = 14,
	numpages     = 6,
	doi.hide     = {10.1103/PhysRevLett.113.140501}
}
%%%%%%%%%%%%Old references
@article{Fritz2017asymptotic,
	title        = {{Resource convertibility and ordered commutative monoids}},
	author       = {Fritz, Tobias},
	year         = 2017,
	journal      = {Math. Struct. Comp. Sci.},
	publisher    = {Cambridge University Press},
	volume       = 27,
	number       = 6,
	pages        = {850â??938},
	doi          = {10.1017/S0960129515000444}
}
@article{Pusey2013,
	title        = {{Negativity and steering: A stronger Peres conjecture}},
	author       = {Pusey, Matthew F.},
	year         = 2013,
	month        = sep,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society ({APS})},
	volume       = 88,
	number       = 3,
	pages        = {032313},
	doi          = {10.1103/PhysRevA.88.032313},
	issn         = {1050-2947},
	url          = {http://link.aps.org/doi/10.1103/PhysRevA.88.032313}
}
@article{Gallego2014,
	title        = {{The resource theory of steering}},
	author       = {Gallego, Rodrigo and Aolita, Leandro},
	year         = 2015,
	month        = sep,
	journal      = {Phys. Rev. X},
	publisher    = {American Physical Society ({APS})},
	volume       = 5,
	number       = 4,
	pages        = 18,
	doi          = {10.1103/PhysRevX.5.041008},
	archiveprefix = {arXiv},
	arxivid      = {1409.5804},
	date         = {2014-09-19}
}
%%General resource theory references
@article{QuantLandauer,
	title        = {{The Minimal Work Cost of Information Processing}},
	author       = {Philippe Faist and FrÃ©dÃ©ric Dupuis and Jonathan Oppenheim and Renato Renner},
	year         = 2015,
	month        = jul,
	journal      = {Nat. Comm.},
	publisher    = {Springer Nature},
	volume       = 6,
	pages        = 7669,
	doi          = {10.1038/ncomms8669},
	date         = {2012-11-05},
	date-added   = {2013-09-17 16:52:44 +0000},
	date-modified = {2013-09-20 23:51:42 +0000},
	eprint.hide  = {arXiv:1211.1037},
	eprintclass  = {quant-ph},
	eprinttype   = {arXiv},
	file         = {online:http\://arxiv.org/pdf/1211.1037v2:PDF},
	journaltitle = {Nat. Commun. 6:7669 (2015)}
}
@article{AbergWork,
	title        = {{Truly work-like work extraction via a single-shot analysis}},
	author       = {Johan {\AA}berg},
	year         = 2013,
	month        = jun,
	journal      = {Nat. Commun.},
	publisher    = {Springer Nature},
	volume       = 4,
	pages        = 1925,
	doi          = {10.1038/ncomms2712},
	owner        = {nyungerhalpern},
	timestamp    = {2013.09.02}
}
@book{amato1968metodologia,
	title        = {{Metodologia statistica strutturale}},
	author       = {Amato, Vittorio},
	year         = 1968,
	publisher    = {F. Cacucci}
}
@book{Arnold87,
	title        = {{Majorization and the Lorenz Order: A Brief Introduction}},
	author       = {Barry C. Arnold},
	year         = 1987,
	publisher    = {Springer New York},
	doi          = {10.1007/978-1-4615-7379-1},
	date-modified = {2013-09-17 16:56:19 +0000},
	timestamp    = {2013.08.30}
}
@article{StochasticPpr,
	title        = {{Stochastic domination for iterated convolutions and catalytic majorization}},
	author       = {Aubrun, Guillaume and Nechita, Ion},
	year         = 2009,
	month        = aug,
	journal      = {Ann. Inst. H. Poincar{\'e} Probab. Statist},
	publisher    = {Institute of Mathematical Statistics},
	volume       = 45,
	number       = 3,
	pages        = {611--625},
	doi          = {10.1214/08-AIHP175}
}
@article{LPNorms,
	title        = {{Catalytic Majorization and \(\ell_p\) Norms}},
	author       = {Aubrun, Guillaume and Nechita, Ion},
	year         = 2008,
	journal      = {Comm. Math. Phys.},
	publisher    = {Springer},
	volume       = 278,
	number       = 1,
	pages        = {133--144},
	doi          = {10.1007/s00220-007-0382-4}
}
@article{Distinguish,
	title        = {{Discriminating States: The Quantum Chernoff Bound}},
	author       = {Audenaert, K. M. R. and Calsamiglia, J. and Mu\~noz-Tapia, R. and Bagan, E. and Masanes, Ll. and Acin, A. and Verstraete, F.},
	year         = 2007,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 98,
	pages        = 160501,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.98.160501},
	issue        = 16,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.98.160501}
}
@article{Asymy4,
	title        = {{Degradation of a quantum reference frame}},
	author       = {Bartlett, Stephen D and Rudolph, Terry and Spekkens, Robert W and Turner, Peter S},
	year         = 2006,
	month        = apr,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 8,
	number       = 4,
	pages        = 58,
	doi          = {10.1088/1367-2630/8/4/058}
}
@article{BennettComp,
	title        = {{The thermodynamics of computation\textemdasha review}},
	author       = {Bennett, Charles H},
	year         = 1982,
	month        = dec,
	journal      = {Int. J. Theor. Phys.},
	publisher    = {Springer},
	volume       = 21,
	number       = 12,
	pages        = {905--940},
	doi          = {10.1007/BF02084158}
}
@article{BennettLogical,
	title        = {{Logical reversibility of computation}},
	author       = {Bennett, Charles H.},
	year         = 1973,
	month        = nov,
	journal      = {IBM J. Res. Dev.},
	publisher    = {{IBM}},
	volume       = 17,
	number       = 6,
	pages        = {525--532},
	doi          = {10.1147/rd.176.0525},
	owner        = {nyungerhalpern},
	timestamp    = {2013.08.30}
}
@article{BBPS96,
	title        = {{Concentrating partial entanglement by local operations}},
	author       = {Bennett, Charles H and Bernstein, Herbert J and Popescu, Sandu and Schumacher, Benjamin},
	year         = 1996,
	month        = apr,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 53,
	number       = 4,
	pages        = {2046--2052},
	doi          = {10.1103/PhysRevA.53.2046}
}
@article{BBP+96,
	title        = {{Purification of noisy entanglement and faithful teleportation via noisy channels}},
	author       = {Bennett, Charles H and Brassard, Gilles and Popescu, Sandu and Schumacher, Benjamin and Smolin, John A and Wootters, William K},
	year         = 1996,
	month        = jan,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 76,
	number       = 5,
	pages        = {722--725},
	doi          = {10.1103/PhysRevLett.76.722}
}
@book{Bhatia,
	title        = {{Matrix analysis}},
	author       = {Bhatia, Rajendra},
	year         = 2013,
	publisher    = {Springer New York},
	volume       = 169,
	isbn         = {978-1-4612-0653-8},
	url          = {http://www.ebook.de/de/product/25252147/rajendra_bhatia_matrix_analysis.html},
	date         = {2013-12-01},
	ean          = 9781461206538
}
@article{Birkhoff,
	title        = {{Three observations on linear algebra}},
	author       = {Birkhoff, Garrett},
	year         = 1946,
	journal      = {Revi. Univ. Nac. Tucuman, ser A},
	volume       = 5,
	pages        = {147--151}
}
@article{1ShotAtherm2,
	title        = {{The second laws of quantum thermodynamics}},
	author       = {Brand{\~a}o, Fernando GSL and Horodecki, Micha{\l} and Ng, Nelly Huei Ying and Oppenheim, Jonathan and Wehner, Stephanie},
	year         = 2015,
	month        = feb,
	journal      = {Proceedings of the National Academy of Sciences},
	publisher    = {Proceedings of the National Academy of Sciences},
	volume       = 112,
	number       = 11,
	pages        = {3275--3279},
	doi          = {10.1073/pnas.1411728112},
	date         = {2013-05-22},
	date-modified = {2013-09-17 16:57:48 +0000},
	file         = {online:http\://arxiv.org/pdf/1305.5278v4:PDF},
	journaltitle = {PNAS 112, 3275 (2015)}
}
@article{AthermalityTheory,
	title        = {{The resource theory of quantum states out of thermal equilibrium}},
	author       = {Brand{\~a}o, Fernando GSL and Horodecki, Micha{\l} and Oppenheim, Jonathan and Renes, Joseph and Spekkens, Robert W},
	year         = 2011,
	journal      = {arXiv:1111.3882},
	date-modified = {2013-09-17 16:57:31 +0000}
}
@conference{Burg,
	title        = {{Maximum entropy spectral analysis}},
	author       = {Burg, J. P.},
	year         = 1967,
	booktitle    = {{Proceedings 37th Annual Meeting of the Society of Exploration Geophysicists}},
	date-modified = {2013-09-17 16:56:42 +0000},
	timestamp    = {2013.08.30}
}
@article{chefles2002quantum,
	title        = {{Quantum operations, state transformations and probabilities}},
	author       = {Chefles, Anthony},
	year         = 2002,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 65,
	number       = 5,
	pages        = {052314--052322}
}
@article{Asymy7,
	title        = {{Efficient Use of Quantum Resources for the Transmission of a Reference Frame}},
	author       = {Chiribella, G. and D'Ariano, G. M. and Perinotti, P. and Sacchi, M. F.},
	year         = 2004,
	month        = oct,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 93,
	pages        = 180503,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.93.180503},
	issue        = 18,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.93.180503}
}
@book{Clausius,
	title        = {{The mechanical theory of heat: With its applications to the steam-engine and to the physical properties of bodies}},
	author       = {Clausius, Rudolf},
	year         = 1867,
	publisher    = {J. van Voorst}
}
@book{CoverThomas,
	title        = {{Elements of Information Theory}},
	author       = {Cover, Thomas M. and Thomas, Joy A.},
	year         = 2006,
	publisher    = {John Wiley \& Sons},
	isbn         = {978-0-471-24195-9},
	url          = {http://www.ebook.de/de/product/4435631/thomas_m_cover_joy_a_thomas_elements_of_information_theory.html},
	date         = {2006-09-08},
	ean          = 9780471241959,
	pagetotal    = 776
}
@inproceedings{csiszar1974information,
	title        = {{Information measures: A critical survey}},
	author       = {Csisz{\'a}r, Imre},
	year         = 1974,
	booktitle    = {{Trans. 7th Prague Conf. on Information Theory}},
	pages        = {73--86}
}
@article{csisz1967information,
	title        = {{Information-type measures of difference of probability distributions and indirect observations}},
	author       = {Csisz{\'a}r, Imre},
	year         = 1967,
	journal      = {Studia Sci. Math. Hungar.},
	volume       = 2,
	pages        = {299--318}
}
@article{WorkValOfInfo,
	title        = {{The work value of information}},
	author       = {Dahlsten, Oscar CO and Renner, Renato and Rieper, Elisabeth and Vedral, Vlatko},
	year         = 2009,
	journal      = {arXiv:0908.0424},
	date-modified = {2013-09-17 16:58:01 +0000}
}
@misc{oscarPwrpt,
	title        = {{Maxwell's daemon in the 21st century}},
	author       = {Dahlsten, O. C. O.},
	year         = 2012,
	location     = {Grenoble},
	note         = {Presentation}
}
@article{InadequacyOfVonN,
	title        = {{Inadequacy of von Neumann entropy for characterizing extractable work}},
	author       = {Dahlsten, Oscar C. O. and Renner, Renato and Rieper, Elisabeth and Vedral, Vlatko},
	year         = 2011,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 13,
	number       = 5,
	pages        = {053015--1--053015--10}
}
@misc{DattaPItalk,
	title        = {{Generalized Relative Entropies, Entanglement Monotones and One-Shot Information Theory}},
	author       = {Datta, Nilanjana},
	year         = 2013,
	note         = {http://pirsa.org/13060003/}
}
@article{datta2009min,
	title        = {{Min-and max-relative entropies and a new entanglement monotone}},
	author       = {Datta, Nilanjana},
	year         = 2009,
	journal      = {IEEE T. Inform. Theory},
	publisher    = {IEEE},
	volume       = 55,
	number       = 6,
	pages        = {2816--2826},
	doi          = {10.1109/TIT.2009.2018325}
}
@article{ThermoMeaningNegEntropy,
	title        = {{The thermodynamic meaning of negative entropy}},
	author       = {{Del Rio}, Lidia and {\AA}berg, Johan and Renner, Renato and Dahlsten, Oscar and Vedral, Vlatko},
	year         = 2011,
	journal      = {Nature},
	publisher    = {Nature Publishing Group},
	volume       = 474,
	number       = 7349,
	pages        = {61--63}
}
@article{Donald2002,
	title        = {{The uniqueness theorem for entanglement measures}},
	author       = {Donald, Matthew J and Horodecki, Micha{\l} and Rudolph, Oliver},
	year         = 2002,
	journal      = {J. Mat. Phys.},
	volume       = 43,
	pages        = {4252--4273},
	doi          = {10.1063/1.1495917}
}
@inproceedings{GeneralizedHs,
	title        = {{Generalized Entropies}},
	author       = {Dupuis, Frederic and Kraemer, Lea and Faist, Philippe and Renes, Joseph M and Renner, Renato},
	year         = 2013,
	month        = oct,
	booktitle    = {{XVIIth} International Congress on Mathematical Physics},
	pages        = {134--153},
	doi          = {10.1142/9789814449243_0008},
	url          = {https://doi.org/10.1142/9789814449243_0008}
}
@article{LawsOfThermo,
	title        = {{A measure of majorization emerging from single-shot statistical mechanics}},
	author       = {Egloff, Dario and Dahlsten, Oscar C. O. and Renner, Renato and Vedral, Vlatko},
	year         = 2015,
	month        = jul,
	journal      = {New J. Phys.},
	publisher    = {{IOP} Publishing},
	volume       = 17,
	number       = 7,
	pages        = {073001},
	doi          = {10.1088/1367-2630/17/7/073001},
	url          = {https://doi.org/10.1088%2F1367-2630%2F17%2F7%2F073001},
	date-modified = {2013-09-17 16:55:56 +0000}
}
@inproceedings{vEH2010,
	title        = {{R\'enyi divergence and majorization}},
	author       = {van Erven, Tim and Harremo{\"e}s, Peter},
	year         = 2010,
	booktitle    = {{Information Theory Proceedings (ISIT), 2010 IEEE International Symposium on}},
	pages        = {1335--1339},
	organization.hide = {IEEE}
}
@article{RatchettExp,
	title        = {{Optical thermal ratchet}},
	author       = {Faucheux, LP and Bourdieu, LS and Kaplan, PD and Libchaber, AJ},
	year         = 1995,
	month        = feb,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society ({APS})},
	volume       = 74,
	number       = 9,
	pages        = {1504--1507},
	doi          = {10.1103/PhysRevLett.74.1504}
}
@article{EntnglmntWitness,
	title        = {{Entanglement detection}},
	author       = {G{\"u}hne, Otfried and Toth, Geza},
	year         = 2009,
	journal      = {Phys. Rep.},
	volume       = 474,
	pages        = {1--90},
	owner        = {nyungerhalpern},
	timestamp    = {2013.08.31}
}
@article{Scovil2,
	title        = {{Quantum equivalent of the Carnot cycle}},
	author       = {Geusic, JE and Schulz-DuBios, EO and Scovil, HED},
	year         = 1967,
	month        = apr,
	journal      = {Phys. Rev.},
	publisher    = {APS},
	volume       = 156,
	number       = 2,
	pages        = {343--351},
	doi          = {10.1103/PhysRev.156.343}
}
@article{gini1912variability,
	title        = {{Variability and Mutability, Contribution to The Study of Statistical Distribution and Relations}},
	author       = {Gini, CW},
	year         = 1912,
	journal      = {Studi Economico-Giuricici della R}
}
@article{Asymy6,
	title        = {{Spin Flips and Quantum Information for Antiparallel Spins}},
	author       = {Gisin, N. and Popescu, S.},
	year         = 1999,
	month        = jul,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 83,
	pages        = {432--435},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.83.432},
	issue        = 2,
	numpages     = {0},
	doi.hide     = {10.1103/PhysRevLett.83.432}
}
@article{gorban2010entropy,
	title        = {{Entropy: the Markov ordering approach}},
	author       = {Gorban, Alexander N and Gorban, Pavel A and Judge, George},
	year         = 2010,
	journal      = {Entropy},
	publisher    = {Molecular Diversity Preservation International},
	volume       = 12,
	number       = 5,
	pages        = {1145--1193}
}
@misc{GiladNotes,
	title        = {{Resource Theory of Nonuniformity}},
	author       = {Gour, Gilad},
	howpublished = {unpublished}
}
@article{Asymy1,
	title        = {{The resource theory of quantum reference frames: manipulations and monotones}},
	author       = {Gour, Gilad and Spekkens, Robert W},
	year         = 2008,
	journal      = {New J. Phys.},
	volume       = 10,
	number       = 3,
	pages        = {033023}
}
@article{GWYC06,
	title        = {{Atemporal diagrams for quantum circuits}},
	author       = {Griffiths, Robert B. and Wu, Shengjun and Yu, Li and Cohen, Scott M.},
	year         = 2006,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 73,
	pages        = {052309},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.73.052309},
	issue        = 5,
	numpages     = 17,
	doi.hide     = {10.1103/PhysRevA.73.052309}
}
@article{HaagerupMusat,
	title        = {{Factorization and dilation problems for completely positive maps on von Neumann algebras}},
	author       = {Haagerup, Uffe and Musat, Magdalena},
	year         = 2011,
	journal      = {Commun. Math. Phys.},
	publisher    = {Springer},
	volume       = 303,
	number       = 2,
	pages        = {555--594}
}
@book{hardy1952inequalities,
	title        = {{Inequalities}},
	author       = {Hardy, Godfrey Harold and Littlewood, John Edensor and Polya, George},
	year         = 1952,
	publisher    = {Cambridge university press}
}
@book{horn2012matrix,
	title        = {{Matrix Analysis}},
	author       = {Horn, Roger A and Johnson, Charles R},
	year         = 2012,
	publisher    = {Cambridge University Press},
	date-modified = {2013-09-20 23:45:35 +0000}
}
@article{Horodecki2001measures,
	title        = {{Entanglement measures}},
	author       = {Horodecki, Michal},
	year         = 2001,
	journal      = {Quantum Inf. Comput.},
	volume       = 1,
	number       = 1,
	pages        = {3--26},
	url          = {http://www.rintonpress.com/journals/qic-1-1/miarprz3.pdf},
	bibsource    = {DBLP, http://dblp.uni-trier.de},
	bdsk-url-1   = {http://www.rintonpress.com/journals/qic-1-1/miarprz3.pdf}
}
@article{HHH99b,
	title        = {{Limits for entanglement measures}},
	author       = {Horodecki, Micha{\l} and Horodecki, Pawe{\l} and Horodecki, Ryszard},
	year         = 2000,
	month        = feb,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 84,
	number       = 9,
	pages        = 2014,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.84.2014},
	doi.hide     = {10.1103/PhysRevLett.84.2014}
}
@article{HHH98,
	title        = {{Mixed-state entanglement and distillation: is there a ``bound'' entanglement in nature?}},
	author       = {Horodecki, Micha{\l} and Horodecki, Pawe{\l} and Horodecki, Ryszard},
	year         = 1998,
	month        = jun,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 80,
	number       = 24,
	pages        = {5239--5242},
	doi          = {10.1103/PhysRevLett.80.5239}
}
@article{HHOLong,
	title        = {{Reversible transformations from pure to mixed states and the unique measure of information}},
	author       = {Horodecki, Micha\l{} and Horodecki, Pawe\l{} and Oppenheim, Jonathan},
	year         = 2003,
	month        = jun,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 67,
	pages        = {062104},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.67.062104},
	issue        = 6,
	numpages     = 9,
	doi.hide     = {10.1103/PhysRevA.67.062104}
}
@article{FundLimitsNature,
	title        = {{Fundamental limitations for quantum and nanoscale thermodynamics}},
	author       = {Horodecki, Micha{\l} and Oppenheim, Jonathn},
	year         = 2013,
	month        = jun,
	journal      = {Nat. Commun.},
	publisher    = {Springer Nature},
	volume       = 4,
	pages        = {1--6},
	doi          = {10.1038/ncomms3059},
	owner        = {nyungerhalpern},
	timestamp    = {2013.08.31}
}
@article{HHH99c,
	title        = {{Bound Entanglement Can Be Activated}},
	author       = {Horodecki, Pawe\l{} and Horodecki, Micha\l{} and Horodecki, Ryszard},
	year         = 1999,
	month        = feb,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 82,
	pages        = {1056--1059},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.82.1056},
	issue        = 5,
	numpages     = {0},
	doi.hide     = {10.1103/PhysRevLett.82.1056}
}
@article{horodecki2009quantum,
	title        = {{Quantum entanglement}},
	author       = {Horodecki, Ryszard and Horodecki, Pawe{\l} and Horodecki, Micha{\l} and Horodecki, Karol},
	year         = 2009,
	journal      = {Rev. Mod. Phys.},
	volume       = 81,
	number       = 2,
	pages        = 865,
	owner        = {nyungerhalpern},
	timestamp    = {2013.08.31}
}
@article{HHOShort,
	title        = {{Local Information as a Resource in Distributed Quantum Systems}},
	author       = {Horodecki, Micha{\l} and Horodecki, Karol and Horodecki, Pawe{\l} and Horodecki, Ryszard and Oppenheim, Jonathan and Sen(De), Aditi and Sen, Ujjwal},
	year         = 2003,
	month        = mar,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society ({APS})},
	volume       = 90,
	number       = 10,
	pages        = {100402--1--100402--4},
	doi          = {10.1103/PhysRevLett.90.100402},
	author.hide  = {M. {Horodecki~$\textit{et~al.}$}},
	owner        = {nyungerhalpern},
	timestamp    = {2013.08.30}
}
@article{MolecMotors,
	title        = {{Molecular motors: structural adaptations to cellular functions}},
	author       = {Howard, Joe},
	year         = 1997,
	month        = oct,
	journal      = {Nature},
	publisher    = {Nature Publishing Group},
	volume       = 389,
	number       = 6651,
	pages        = {561--567},
	doi          = {10.1038/39247}
}
@article{janzing2000thermodynamic,
	title        = {{Thermodynamic cost of reliability and low temperatures: tightening Landauer's principle and the Second Law}},
	author       = {Janzing, Dominik and Wocjan, Pawel and Zeier, Robert and Geiss, Rubino and Beth, Th},
	year         = 2000,
	journal      = {Int. J. Theor. Phys.},
	publisher    = {Springer Nature},
	volume       = 39,
	number       = 12,
	pages        = {2717--2753},
	doi          = {10.1023/A:1026422630734}
}
@article{joe1990majorization,
	title        = {{Majorization and divergence}},
	author       = {Joe, Harry},
	year         = 1990,
	month        = may,
	journal      = {J. Math. Anal. Appl.},
	publisher    = {Elsevier},
	volume       = 148,
	number       = 2,
	pages        = {287--305},
	doi          = {10.1016/0022-247X(90)90002-W}
}
@article{JonathanPlenio,
	title        = {{Entanglement-Assisted Local Manipulation of Pure Quantum States}},
	author       = {Jonathan, Daniel and Plenio, Martin B.},
	year         = 1999,
	month        = oct,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 83,
	pages        = {3566--3569},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.83.3566},
	issue        = 17
}
@article{Pironio2016,
	title        = {{Focus on Device Independent Quantum Information}},
	author       = {Pironio, S. and Scarani, V. and Vidick, T.},
	year         = 2016,
	month        = oct,
	journal      = {New Journal of Physics},
	volume       = 18,
	number       = 10,
	pages        = 100202,
	doi          = {10.1088/1367-2630/18/10/100202},
	issn         = {1367-2630}
}
@article{Chruscinski2014,
	title        = {{Entanglement Witnesses: Construction, Analysis and Classification}},
	shorttitle   = {Entanglement Witnesses},
	author       = {Chru{\'s}ci{\'n}ski, Dariusz and Sarbicki, Gniewomir},
	year         = 2014,
	journal      = {Journal of Physics A: Mathematical and Theoretical},
	volume       = 47,
	number       = 48,
	pages        = 483001,
	doi          = {10.1088/1751-8113/47/48/483001},
	issn         = {1751-8121}
}
@article{Einstein1935,
	title        = {{Can Quantum-Mechanical Description of Physical Reality Be Considered Complete?}},
	author       = {Einstein, A. and Podolsky, B. and Rosen, N.},
	year         = 1935,
	month        = may,
	journal      = {Physical Review},
	volume       = 47,
	number       = 10,
	pages        = {777--780},
	doi          = {10.1103/PhysRev.47.777}
}
@article{Cavalcanti2017,
	title        = {{Quantum Steering: A Review with Focus on Semidefinite Programming}},
	shorttitle   = {Quantum Steering},
	author       = {Cavalcanti, D. and Skrzypczyk, P.},
	year         = 2017,
	journal      = {Reports on Progress in Physics},
	volume       = 80,
	number       = 2,
	pages        = {024001},
	doi          = {10.1088/1361-6633/80/2/024001},
	issn         = {0034-4885}
}
@article{JP99,
	title        = {{Minimal Conditions for Local Pure-State Entanglement Manipulation}},
	author       = {Jonathan, Daniel and Plenio, Martin B},
	year         = 1999,
	month        = aug,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 83,
	number       = 7,
	pages        = {1455--1458},
	doi          = {10.1103/PhysRevLett.83.1455}
}
@article{Jungetal08,
	title        = {{Amplitude damping for single-qubit system with single-qubit mixed-state environment}},
	author       = {Jung, Eylee and Hwang, Mi-Ra and Ju, You Hwan and Park, DK and Kim, Hungsoo and Kim, Min-Soo and Son, Jin-Woo},
	year         = 2008,
	journal      = {J. Phys. A: Math. Theor.},
	publisher    = {IOP Publishing},
	volume       = 41,
	number       = 4,
	pages        = {045306},
	author.hide  = {E. {Jung~$\textit{et~al.}$}}
}
@book{kakwani1980income,
	title        = {{Income Inequality and Poverty: Methods of Estimation and Policy Applications}},
	author       = {Kakwani, Nanak C},
	year         = 1980,
	publisher    = {Oxford University Press New York}
}
@article{Konig,
	title        = {{The operational meaning of min-and max-entropy}},
	author       = {Konig, R and Renner, Renato and Schaffner, Christian},
	year         = 2009,
	journal      = {IEEE T. Inform. Theory},
	publisher    = {IEEE},
	volume       = 55,
	number       = 9,
	pages        = {4337--4347},
	doi          = {10.1109/TIT.2009.2025545}
}
@article{kullback1951information,
	title        = {{On information and sufficiency}},
	author       = {Kullback, Solomon and Leibler, Richard A},
	year         = 1951,
	journal      = {{Ann. Math. Stat.}},
	volume       = 22,
	number       = 1,
	pages        = {79--86},
	url          = {https://projecteuclid.org/euclid.aoms/1177729694}
}
@article{Landauer,
	title        = {{Irreversibility and heat generation in the computing process}},
	author       = {Landauer, R.},
	year         = 1961,
	journal      = {IBM J. Res. Dev.},
	volume       = 5,
	pages        = {183--191},
	doi          = {10.1147/rd.53.0183},
	owner        = {nyungerhalpern},
	timestamp    = {2013.08.30}
}
@article{Lewenstein1998,
	title        = {{Separability and Entanglement of Composite Quantum Systems}},
	author       = {Lewenstein, M. and Sanpera, A.},
	year         = 1998,
	month        = mar,
	journal      = {Phys. Rev. Lett.},
	volume       = 80,
	number       = 11,
	pages        = {2261--2264},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.80.2261}
}
@article{SanduRefrig,
	title        = {{How Small Can Thermal Machines Be? The Smallest Possible Refrigerator}},
	author       = {Linden, Noah and Popescu, Sandu and Skrzypczyk, Paul},
	year         = 2010,
	month        = sep,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 105,
	pages        = 130401,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.105.130401},
	issue        = 13,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.105.130401}
}
@article{lorenz1905methods,
	title        = {{Methods of measuring the concentration of wealth}},
	author       = {Lorenz, Max O.},
	year         = 1905,
	journal      = {Publ. Am. Stat. Assoc.},
	publisher    = {Taylor \& Francis},
	volume       = 9,
	number       = 70,
	pages        = {209--219}
}
@book{MarshallOlkin,
	title        = {{Inequalities: theory of majorization and its applications}},
	author       = {Marshall, Albert W. and Olkin, Ingram and Arnold, Barry C.},
	year         = 2010,
	publisher    = {Springer}
}
@article{MaxDemonRev,
	title        = {{The physics of Maxwell's demon and information}},
	author       = {Maruyama, Koji and Nori, Franco and Vedral, Vlatko},
	year         = 2009,
	journal      = {Rev. Mod. Phys.},
	publisher    = {APS},
	volume       = 81,
	number       = 1,
	pages        = 1
}
@article{Asymy2,
	title        = {{The theory of manipulations of pure state asymmetry I: basic tools and equivalence classes of states under symmetric operations}},
	author       = {Marvian, Iman and Spekkens, Robert W.},
	year         = 2011,
	month        = mar,
	journal      = {arXiv:1104.0018},
	publisher    = {{IOP} Publishing},
	volume       = 15,
	number       = 3,
	pages        = {033001},
	doi          = {10.1088/1367-2630/15/3/033001},
	url          = {https://doi.org/10.1088/1367-2630/15/3/033001},
	date-modified = {2013-09-17 16:57:54 +0000}
}
@article{MendlWolf,
	title        = {{Unital quantum channels---convex structure and revivals of Birkhoff's Theorem}},
	author       = {Mendl, Christian B. and Wolf, Michael M.},
	year         = 2009,
	journal      = {Commun. Math. Phys.},
	publisher    = {Springer},
	volume       = 289,
	number       = 3,
	pages        = {1057--1086}
}
@article{morimoto1963markov,
	title        = {{Markov processes and the H-theorem}},
	author       = {Morimoto, Tetsuzo},
	year         = 1963,
	journal      = {J. Phys. Soc. Jap},
	volume       = 12,
	pages        = {328--331}
}
@article{Narang07,
	title        = {{Simulating a single-qubit channel using a mixed-state environment}},
	author       = {Narang, Geetu and Arvind},
	year         = 2007,
	month        = mar,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 75,
	pages        = {032305},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.75.032305},
	issue        = 3,
	numpages     = 7,
	doi.hide     = {10.1103/PhysRevA.75.032305}
}
@book{vonN,
	title        = {{Mathematical Foundations of Quantum Mechanics}},
	author       = {von Neumann, J.},
	year         = 1955,
	publisher    = {Princeton University Press}
}
@article{nielsen1999conditions,
	title        = {{Conditions for a Class of Entanglement Transformations}},
	author       = {Nielsen, Michael A.},
	year         = 1999,
	month        = jul,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 83,
	number       = 2,
	pages        = {436--439},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.83.436},
	doi.hide     = {10.1103/PhysRevLett.83.436}
}
@article{nielsen2001majorization,
	title        = {{Majorization and the interconversion of bipartite states.}},
	author       = {Nielsen, Michael A. and Vidal, Guifr{\'e}},
	year         = 2001,
	journal      = {Quantum Inf. Comput.},
	volume       = 1,
	number       = 1,
	pages        = {76--93},
	url          = {http://dl.acm.org/citation.cfm?id=2011326.2011331},
	acmid        = 2011331
}
@inproceedings{Renyi,
	title        = {{On measures of entropy and information}},
	author       = {R{\'e}nyi, Alfred},
	year         = 1961,
	booktitle    = {{Fourth Berkeley Symposium on Mathematical Statistics and Probability}},
	pages        = {547--561}
}
@book{Rao,
	title        = {{Chemical Engineering Thermodynamics}},
	author       = {Rao, Y. V. C.},
	year         = 1997,
	publisher    = {Orient Blackswan},
	isbn         = 8173710481,
	url          = {https://www.amazon.com/dp/8173710481}
}
@article{RennerThesis,
	title        = {{Security of quantum key distribution}},
	author       = {Renner, Renato},
	year         = 2008,
	journal      = {Int. J. Quantum Inf.},
	publisher    = {World Scientific},
	volume       = 6,
	number       = {01},
	pages        = {1--127},
	doi          = {10.1142/S0219749908003256}
}
@inproceedings{SmoothRenyiHAndApplns,
	title        = {{Smooth R\'enyi entropy and applications}},
	author       = {Renner, Renato and Wolf, Stefan},
	year         = 2004,
	booktitle    = {{ISIT Proceedings: International Symposium on Information Theory, 2004.}},
	pages        = 233,
	doi          = {10.1109/ISIT.2004.1365269},
	organization.hide = {IEEE},
	publisher.hide = {{IEEE}}
}
@article{ruch1975,
	title        = {{Theorie der Chiralittsfunktionen}},
	author       = {Ernst Ruch and Alfred Schnhofer},
	year         = 1970,
	journal      = {Theoretica Chimica Acta},
	publisher    = {Springer Nature},
	volume       = 19,
	number       = 3,
	pages        = {225--287},
	doi          = {10.1007/BF00532232}
}
@article{ruch1978information,
	title        = {{Information extent and information distance}},
	author       = {Ruch, Ernst and Lesche, Bernhard},
	year         = 1978,
	journal      = {J. Chem. Phys.},
	publisher    = {{AIP} Publishing},
	volume       = 69,
	number       = 1,
	pages        = 393,
	doi          = {10.1063/1.436365}
}
@article{RuchSchrannerSeligman,
	title        = {{The mixing distance}},
	author       = {Ruch, Ernst and Schranner, Rudolf and Seligman, Thomas H.},
	year         = 1978,
	journal      = {J. Chem. Phys.},
	publisher    = {{AIP} Publishing},
	volume       = 69,
	number       = 1,
	pages        = 386,
	doi          = {10.1063/1.436364}
}
@phdthesis{YuvalThesis,
	title        = {{Resource Theories in Quantum Information}},
	author       = {Sanders, Yuval Rishu},
	year         = 2012,
	doi          = {10.11575/PRISM/3875},
	url          = {http://hdl.handle.net/1880/104876},
	school       = {University of Calgary}
}
@article{Skrzypczyk2014,
	title        = {{Quantifying Einstein-Podolsky-Rosen Steering}},
	author       = {Skrzypczyk, Paul and Navascu{\'e}s, Miguel and Cavalcanti, Daniel},
	year         = 2014,
	month        = may,
	journal      = {Physical Review Letters},
	volume       = 112,
	number       = 18,
	pages        = 180404,
	doi          = {10.1103/PhysRevLett.112.180404}
}
@article{Piani2015a,
	title        = {{Necessary and Sufficient Quantum Information Characterization of Einstein-Podolsky-Rosen Steering}},
	author       = {Piani, Marco and Watrous, John},
	year         = 2015,
	month        = feb,
	journal      = {Physical Review Letters},
	volume       = 114,
	number       = 6,
	pages        = {060404},
	doi          = {10.1103/PhysRevLett.114.060404}
}
@article{gutoski2008properties,
	title        = {{Properties of local quantum operations with shared entanglement}},
	author       = {Gutoski, Gus},
	year         = 2008,
	journal      = {arXiv:0805.2209},
	url          = {https://arxiv.org/pdf/0805.2209.pdf}
}
@article{Gallego2015,
	title        = {{Resource Theory of Steering}},
	author       = {Gallego, Rodrigo and Aolita, Leandro},
	year         = 2015,
	month        = oct,
	journal      = {Physical Review X},
	volume       = 5,
	number       = 4,
	pages        = {041008},
	doi          = {10.1103/PhysRevX.5.041008}
}
@article{SandersGour,
	title        = {{Necessary conditions for entanglement catalysts}},
	author       = {Sanders, Yuval Rishu and Gour, Gilad},
	year         = 2009,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 79,
	pages        = {054302},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.79.054302},
	doi.hide     = {10.1103/PhysRevA.79.054302},
	issue        = 5,
	numpages     = 4
}
@inproceedings{RenyiEntropies,
	title        = {{Smooth R\'enyi entropy of ergodic quantum information sources}},
	author       = {Schoenmakers, Berry and Tjoelker, Jilles and Tuyls, Pim and Verbitskiy, Evgeny},
	year         = 2007,
	booktitle    = {{IEEE International Symposium on Information Theory}},
	pages        = {256--260},
	doi          = {10.1109/ISIT.2007.4557235},
	organization.hide = {IEEE}
}
@inproceedings{SchulmanVazirani,
	title        = {{Molecular scale heat engines and scalable quantum computation}},
	author       = {Schulman, Leonard J. and Vazirani, Umesh V.},
	year         = 1999,
	booktitle    = {{Proc. 31st annual ACM symposium on Theory of computing}},
	pages        = {322--329},
	url          = {http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.45.9719},
	organization.hide = {ACM}
}
@article{Schutz1951,
	title        = {{On the measurement of income inequality}},
	author       = {Schutz, R. R.},
	year         = 1951,
	journal      = {Amer. Econ. Rev.},
	volume       = 41,
	pages        = {107--122}
}
@article{Scovil1,
	title        = {{Three-Level Masers as Heat Engines}},
	author       = {Scovil, H. E. D. and Schulz-DuBois, E. O.},
	year         = 1959,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 2,
	number       = 6,
	pages        = 262,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.2.262}
}
@article{ScullyExp,
	title        = {{Quantum Afterburner: Improving the Efficiency of an Ideal Heat Engine}},
	author       = {Scully, Marlan O.},
	year         = 2002,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 88,
	number       = 5,
	pages        = {050602},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.88.050602},
	doi.hid      = {10.1103/PhysRevLett.88.050602}
}
@article{Shannon,
	title        = {{A Mathematical Theory of Communication}},
	author       = {Shannon, C. E.},
	year         = 1948,
	journal      = {Bell Syst. Tech. J.},
	volume       = 47,
	pages        = {379--423}
}
@misc{ShorTalk,
	title        = {{Structure of Unital Maps and the Asymptotic Quantum Birkhoff Conjecture}},
	author       = {Shor, Peter W.},
	year         = 2010,
	location     = {Cambridge, MA},
	url          = {http://science-visits.mccme.ru/doc/steklov-talk.pdf},
	note         = {Presentation}
}
@article{SSP1,
	title        = {{Extracting work from quantum systems}},
	author       = {Skrzypczyk, Paul and Short, Anthony J. and Popescu, Sandu},
	year         = 2013,
	journal      = {arXiv:1302.2811},
	url          = {https://arxiv.org/abs/1302.2811},
	date         = {2013-02-12},
	date-modified = {2013-09-17 16:54:27 +0000},
	eprint.hide  = {arXiv:1302.2811},
	eprintclass  = {quant-ph},
	eprinttype   = {arXiv},
	file         = {online:http\://arxiv.org/pdf/1302.2811v1:PDF}
}
@article{SSP2,
	title        = {{Thermodynamics for individual quantum systems}},
	author       = {Skrzypczyk, Paul and Short, Anthony J. and Popescu, Sandu},
	year         = 2014,
	month        = jun,
	journal      = {Nat. Comm},
	publisher    = {Springer Nature},
	volume       = 5,
	doi          = {10.1038/ncomms5185},
	date         = {2013-07-05},
	date-modified = {2013-09-17 16:58:08 +0000},
	file         = {online:http\://arxiv.org/pdf/1307.1558v2:PDF}
}
@misc{RobNotes,
	title        = {{Notes on the Resource Theory of Nonuniformity}},
	author       = {Spekkens, Robert W.},
	howpublished = {unpublished}
}
@article{Szilard,
	title        = {{\"Uber die Entropieverminderung in einem thermodynamischen System bei Eingriffen intelligenter Wesen}},
	author       = {Szilard, Leo},
	year         = 1929,
	journal      = {Zeitschrift f{\"u}r Physik},
	publisher    = {Springer},
	volume       = 53,
	number       = {11-12},
	pages        = {840--856},
	doi          = {10.1007/BF01341281},
	issn         = {0044-3328},
	url          = {https://doi.org/10.1007/BF01341281}
}
@article{Tomamichel,
	title        = {{A framework for non-asymptotic quantum information theory}},
	author       = {Tomamichel, Marco},
	year         = 2012,
	journal      = {arXiv:1203.2142},
	url          = {https://arxiv.org/abs/1203.2142},
	date-modified = {2013-09-17 16:51:14 +0000}
}
@article{LeftoverHashing,
	title        = {{Leftover hashing against quantum side information}},
	author       = {Tomamichel, Marco and Schaffner, Christian and Smith, Adam and Renner, Renato},
	year         = 2011,
	journal      = {IEEE T. Inform. Theory},
	publisher    = {IEEE},
	volume       = 57,
	number       = 8,
	pages        = {5524--5535},
	doi          = {10.1109/TIT.2011.2158473}
}
@article{ArticleAboutShannon,
	title        = {{Energy and information}},
	author       = {Tribus, Myron and McIrvine, Edward C.},
	year         = 1971,
	journal      = {Scientific American},
	volume       = 225,
	number       = 3,
	pages        = {179--188}
}
@article{TsallisRel,
	title        = {{Generalized entropy-based criterion for consistent testing}},
	author       = {Tsallis, Constantino},
	year         = 1998,
	month        = aug,
	journal      = {Phys. Rev. E},
	publisher    = {American Physical Society ({APS})},
	volume       = 58,
	number       = 2,
	pages        = {1442--1445},
	doi          = {10.1103/PhysRevE.58.1442},
	owner        = {nyungerhalpern},
	timestamp    = {2013.08.30}
}
@article{Tsallis,
	title        = {{Possible generalization of Boltzmann-Gibbs statistics}},
	author       = {Tsallis, Constantino},
	year         = 1988,
	journal      = {J. Stat. Phys.},
	volume       = 52,
	pages        = {479--487},
	doi          = {10.1007/BF01016429},
	owner        = {nyungerhalpern},
	timestamp    = {2013.08.30}
}
@article{Turgut,
	title        = {{Catalytic transformations for bipartite pure states}},
	author       = {Turgut, S.},
	year         = 2007,
	journal      = {J. Phys. A},
	publisher    = {IOP Publishing},
	volume       = 40,
	number       = 40,
	pages        = 12185,
	url          = {http://stacks.iop.org/1751-8121/40/i=40/a=012}
}
@article{Uhlmann,
	title        = {{Endlich-dimensionale Dichtematrizen. I}},
	author       = {Uhlmann, Armin},
	year         = 1972,
	journal      = {Wissenschaftliche Zeitschrift der Karl-Marx-Universit{\"a}t Leipzig. Mathematisch-Naturwissenschaftliche Reihe},
	volume       = 21,
	pages        = {421--452}
}
@article{uhlmann1970,
	title        = {{On the Shannon entropy and related functionals on convex sets}},
	author       = {Uhlmann, A.},
	year         = 1970,
	month        = oct,
	journal      = {Rep. Math. Phys.},
	publisher    = {Elsevier {BV}},
	volume       = 1,
	number       = 2,
	pages        = {147--159},
	doi          = {10.1016/0034-4877(70)90009-1}
}
@article{Asymy5,
	title        = {{Tradeoff between extractable mechanical work, accessible entanglement, and ability to act as a reference system, under arbitrary superselection rules}},
	author       = {Vaccaro, Joan Alfina and Anselmi, F. and Wiseman, Howard Mark and Jacobs, K.},
	year         = 2008,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 77,
	number       = 3,
	pages        = {032114}
}
@article{veinott1971,
	title        = {{Least d-majorized network flows with inventory and statistical applications}},
	author       = {Veinott, Arthur F.},
	year         = 1971,
	journal      = {Manage. Sci.},
	publisher    = {INFORMS},
	volume       = 17,
	number       = 9,
	pages        = {547--567},
	url          = {http://www.jstor.org/stable/2629040}
}
@article{veitch2013resource,
	title        = {{The resource theory of stabilizer computation}},
	author       = {Veitch, Victor and Mousavian, Seyed Ali Hamed and Gottesman, Daniel and Emerson, Joseph},
	year         = 2014,
	month        = jan,
	journal      = {New J. Phys.},
	publisher    = {{IOP} Publishing},
	volume       = 16,
	number       = 1,
	pages        = {013009},
	doi          = {10.1088/1367-2630/16/1/013009},
	date         = {2013-07-26},
	date-modified = {2013-09-17 16:57:40 +0000},
	file         = {online:http\://arxiv.org/pdf/1307.7171v1:PDF},
	timestamp    = {2013.08.31}
}
@article{vidal2000entanglement,
	title        = {{Entanglement monotones}},
	author       = {Vidal, Guifr{\'e}},
	year         = 2000,
	month        = feb,
	journal      = {J. Mod. Optic.},
	publisher    = {Taylor \& Francis},
	volume       = 47,
	number       = {2-3},
	pages        = {355--376},
	doi          = {10.1080/09500340008244048}
}
@book{ESP,
	title        = {{Algebra}},
	author       = {van der Waerden, Bartel Leendert},
	year         = 2004,
	publisher    = {Springer},
	volume       = 1,
	isbn         = {0387406247},
	url          = {http://www.ebook.de/de/product/2654446/bartel_leendert_van_der_waerden_algebra_1.html},
	date         = {2004-01-11},
	ean          = 9780387406244,
	owner        = {nyungerhalpern},
	timestamp    = {2013.08.30}
}
@article{wallace2013inferential,
	title        = {{Inferential vs. Dynamical Conceptions of Physics}},
	author       = {Wallace, David},
	year         = 2013,
	journal      = {arXiv:1306.4907},
	url          = {https://arxiv.org/abs/1306.4907},
	date         = {2013-06-20},
	date-modified = {2013-09-17 16:55:46 +0000},
	eprintclass  = {quant-ph},
	eprinttype   = {arXiv},
	file         = {online:http\://arxiv.org/pdf/1306.4907v1:PDF}
}
@book{LeffRex,
	title        = {{Maxwell's Demons 2}},
	year         = 2002,
	month        = dec,
	publisher    = {TAYLOR \& FRANCIS},
	isbn         = {0750307595},
	url          = {http://www.ebook.de/de/product/5493079/maxwell_s_demon_2_entropy_classical_and_quantum_information_computing.html},
	editor       = {Leff, Harvey and Rex, Andrew F.},
	date         = {2002-12-11},
	date-modified = {2013-09-17 16:56:35 +0000},
	ean          = 9780750307598,
	pagetotal    = 502,
	timestamp    = {2013.08.30}
}
@article{klimesh,
	title        = {{Inequalities that Collectively Completely Characterize the Catalytic Majorization Relation}},
	author       = {Klimesh, M.},
	year         = 2007,
	journal      = {arXiv:0709.3680},
	annote       = {http://arxiv.org/abs/0709.3680},
	date-modified = {2013-09-17 16:55:39 +0000}
}
@article{NielsenIntroduction,
	title        = {{An introduction to majorization and its applications to quantum mechanics}},
	author       = {Nielsen, M.},
	year         = 2002,
	journal      = {lecture notes (available online)},
	url          = {http://michaelnielsen.org/blog/talks/2002/maj/book.ps},
	bdsk-url-1   = {http://michaelnielsen.org/blog/talks/2002/maj/book.ps}
}
@article{vanDamHayden,
	title        = {{Universal entanglement transformations without communication}},
	author       = {van Dam, W. and Hayden, P.},
	year         = 2003,
	month        = jun,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 67,
	number       = 6,
	pages        = {060302(R)},
	bdsk-url-1   = {http://dx.doi.org/10.1103/PhysRevA.67.060302},
	doi.hide     = {10.1103/PhysRevA.67.060302}
}
@article{Fannes,
	title        = {{A continuity property of the entropy density for spin lattice systems}},
	author       = {Fannes, M.},
	year         = 1973,
	month        = dec,
	journal      = {Commun. Math. Phys.},
	publisher    = {Springer Nature},
	volume       = 31,
	number       = 4,
	pages        = {291--294},
	doi          = {10.1007/BF01646490}
}
@article{Audenaert,
	title        = {{A sharp continuity estimate for the von Neumann entropy}},
	author       = {Audenaert, K. M. R.},
	year         = 2007,
	journal      = {J. Phys. A: Math. Theor.},
	volume       = 40,
	pages        = 8127
}
@article{GConcurrence,
	title        = {{Family of Concurrence Monotones and its Applications}},
	author       = {Gour, Gilad},
	year         = 2005,
	month        = jan,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 71,
	pages        = {012318--1--012318--8},
	bdsk-url-1   = {https://link.aps.org/doi/10.1103/PhysRevA.71.012318},
	doi.hide     = {10.1103/PhysRevA.71.012318},
	issue        = 1,
	numpages     = 8,
	owner        = {nyungerhalpern},
	timestamp    = {2013.08.30}
}
@article{JaynesI,
	title        = {{Information Theory and Statistical Mechanics I}},
	author       = {Jaynes, E. T.},
	year         = 1957,
	journal      = {Phys. Rev.},
	volume       = 106,
	pages        = {620--630},
	owner        = {nyungerhalpern},
	timestamp    = {2013.08.30}
}
@article{RuchDiagrams,
	title        = {{The principle of increasing mixing character and some of its consequences}},
	author       = {Ruch, Ernst and Mead, Alden},
	year         = 1976,
	journal      = {Theoretica Chimica Acta},
	publisher    = {Springer},
	volume       = 41,
	number       = 2,
	pages        = {95--117},
	doi          = {10.1007/BF01178071}
}
@article{TCDGS99,
	title        = {{Simulating quantum operations with mixed environments}},
	author       = {Terhal, Barbara M. and Chuang, Isaac L. and DiVincenzo, David P. and Grassl, Markus and Smolin, John A.},
	year         = 1999,
	month        = aug,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 60,
	pages        = {881--885},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.60.881},
	issue        = 2,
	numpages     = {0},
	doi.hide     = {10.1103/PhysRevA.60.881}
}
@article{zalka2002quantum,
	title        = {{Quantum operations that cannot be implemented using a small mixed environment}},
	author       = {Zalka, Christof and Rieffel, Eleanor},
	year         = 2002,
	month        = sep,
	journal      = {J. Mat. Phys.},
	publisher    = {{AIP} Publishing},
	volume       = 43,
	number       = 9,
	pages        = {4376--4381},
	doi          = {10.1063/1.1499763},
	owner        = {nyungerhalpern},
	timestamp    = {2013.09.02}
}
@article{van2005implausible,
	title        = {{Implausible consequences of superstrong nonlocality}},
	author       = {Van Dam, Wim},
	year         = 2005,
	journal      = {arXiv:quant-ph/0501159},
	url          = {http://arxiv.org/abs/quant-ph/0501159}
}
@article{ML,
	title        = {{A glance beyond the quantum model}},
	author       = {Navascu{\'e}s, Miguel and Wunderlich, Harald},
	year         = 2009,
	journal      = {Proc. Roy. Soc. London A},
	issn         = {1364-5021},
	url          = {http://rspa.royalsocietypublishing.org/content/early/2009/11/07/rspa.2009.0453},
	doi.hide     = {10.1098/rspa.2009.0453},
	publisher.hide = {The Royal Society}
}
@article{Putz2014,
	title        = {{Arbitrarily Small Amount of Measurement Independence Is Sufficient to Manifest Quantum Nonlocality}},
	author       = {P{\"u}tz, Gilles and Rosset, Denis and Barnea, Tomer Jack and Liang, Yeong-Cherng and Gisin, Nicolas},
	year         = 2014,
	month        = nov,
	journal      = {Physical Review Letters},
	volume       = 113,
	number       = 19,
	pages        = 190402,
	doi          = {10.1103/PhysRevLett.113.190402}
}
@book{Bell2004,
	title        = {{Speakable and Unspeakable in Quantum Mechanics: Collected Papers on Quantum Philosophy}},
	shorttitle   = {Speakable and {{Unspeakable}} in {{Quantum Mechanics}}},
	author       = {Bell, J. S.},
	year         = 2004,
	month        = jun,
	publisher    = {{Cambridge University Press}},
	isbn         = {978-1-139-81106-4}
}
@article{Rosset2012a,
	title        = {{Imperfect Measurement Settings: Implications for Quantum State Tomography and Entanglement Witnesses}},
	shorttitle   = {Imperfect Measurement Settings},
	author       = {Rosset, Denis and {Ferretti-Sch{\"o}bitz}, Raphael and Bancal, Jean-Daniel and Gisin, Nicolas and Liang, Yeong-Cherng},
	year         = 2012,
	month        = dec,
	journal      = {Physical Review A},
	volume       = 86,
	number       = 6,
	pages        = {062325},
	doi          = {10.1103/PhysRevA.86.062325}
}
@article{Cavalcanti2015,
	title        = {{Detection of Entanglement in Asymmetric Quantum Networks and Multipartite Quantum Steering}},
	author       = {Cavalcanti, D. and Skrzypczyk, P. and Aguilar, G. H. and Nery, R. V. and Ribeiro, P. H. Souto and Walborn, S. P.},
	year         = 2015,
	month        = aug,
	journal      = {Nature Communications},
	volume       = 6,
	pages        = 7941,
	doi          = {10.1038/ncomms8941},
	issn         = {2041-1723},
	copyright    = {2015 Nature Publishing Group}
}
@article{girard2015witnesses,
	title        = {{Computable entanglement conversion witness that is better than the negativity}},
	author       = {Girard, M.~W. and Gour, Gilad},
	year         = 2015,
	journal      = {New J. Phys.},
	volume       = 17,
	number       = 9,
	pages        = {093013},
	doi          = {10.1088/1367-2630/17/9/093013},
	url          = {http://stacks.iop.org/1367-2630/17/i=9/a=093013}
}
@article{Cavalcanti2016Measures,
	title        = {{Quantitative relations between measurement incompatibility, quantum steering, and nonlocality}},
	author       = {Cavalcanti, D. and Skrzypczyk, P.},
	year         = 2016,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 93,
	pages        = {052112},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.93.052112},
	issue        = 5,
	numpages     = 12,
	doi.hide     = {10.1103/PhysRevA.93.052112}
}
@article{Aolita2012NLF,
	title        = {{Fully Nonlocal, Monogamous, and Random Genuinely Multipartite Quantum Correlations}},
	author       = {Aolita, Leandro and Gallego, Rodrigo and Cabello, Ad\'an and Ac\'{\i}n, Antonio},
	year         = 2012,
	month        = mar,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 108,
	pages        = 100401,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.108.100401},
	issue        = 10,
	numpages     = 5,
	doi.hide     = {10.1103/PhysRevLett.108.100401}
}
@article{Aolita2012NLFb,
	title        = {{Fully nonlocal quantum correlations}},
	author       = {Aolita, Leandro and Gallego, Rodrigo and Ac\'{\i}n, Antonio and Chiuri, Andrea and Vallone, Giuseppe and Mataloni, Paolo and Cabello, Ad\'an},
	year         = 2012,
	month        = mar,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 85,
	number       = 3,
	pages        = {032107},
	doi          = {10.1103/PhysRevA.85.032107},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.85.032107},
	author.hide  = {L. {Aolita~$\textit{et~al.}$}},
	issue        = 3,
	numpages     = 8,
	doi.hide     = {10.1103/PhysRevA.85.032107}
}
@article{geometry2018,
	title        = {{Geometry of the set of quantum correlations}},
	author       = {Goh, Koon Tong and Kaniewski, Jadrzej and Wolfe, Elie and Vertesi, Tamas and Wu, Xingyao and Cai, Yu and Liang, Yeong-Cherng and Scarani, Valerio},
	year         = 2018,
	month        = feb,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 97,
	pages        = {022104},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.97.022104},
	issue        = 2,
	numpages     = 20,
	doi.hide     = {10.1103/PhysRevA.97.022104}
}
@article{Wolfe2016inflation,
	title        = {{The Inflation Technique for Causal Inference with Latent Variables}},
	author       = {{Wolfe}, E. and {Spekkens}, R.~W. and {Fritz}, T.},
	year         = 2016,
	month        = sep,
	journal      = {arXiv:1609.00672},
	url          = {http://arxiv.org/abs/1609.00672},
	archiveprefix = {arXiv},
	eprint.hide  = {1609.00672},
	primaryclass = {quant-ph}
}
@article{Chaves2015relaxing,
	title        = {{Unifying Framework for Relaxations of the Causal Assumptions in Bell's Theorem}},
	author       = {Chaves, R. and Kueng, R. and Brask, J. B. and Gross, D.},
	year         = 2015,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 114,
	pages        = 140403,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.114.140403},
	issue        = 14,
	numpages     = 5,
	doi.hide     = {10.1103/PhysRevLett.114.140403}
}
@article{Chaves2017causalmultipartite,
	title        = {{Causal hierarchy of multipartite Bell nonlocality}},
	author       = {Rafael Chaves and Daniel Cavalcanti and Leandro Aolita},
	year         = 2017,
	month        = aug,
	journal      = {Quantum},
	publisher    = {Verein zur Forderung des Open Access Publizierens in den Quantenwissenschaften},
	volume       = 1,
	pages        = 23,
	doi          = {10.22331/q-2017-08-04-23},
	url          = {https://arxiv.org/abs/1607.07666}
}
@book{boyd2004convex,
	title        = {{Convex Optimization}},
	author       = {Boyd, Stephen},
	year         = 2004,
	publisher    = {Cambridge University Press},
	isbn         = 9780521833783,
	url          = {http://web.stanford.edu/~boyd/cvxbook/bv_cvxbook.pdf},
	address.hide = {Cambridge, UK New York}
}
@article{Beirhorst2016Bell,
	title        = {{Geometric decompositions of Bell polytopes with practical applications}},
	author       = {Peter Bierhorst},
	year         = 2016,
	journal      = {J. Phys. A},
	volume       = 49,
	number       = 21,
	pages        = 215301,
	url          = {http://stacks.iop.org/1751-8121/49/i=21/a=215301},
	doi.hide     = {10.1088/1751-8113/49/21/215301}
}
@article{Sekatski2018a,
	title        = {{Certifying the Building Blocks of Quantum Computers from Bell's Theorem}},
	author       = {Sekatski, Pavel and Bancal, Jean-Daniel and Wagner, Sebastian and Sangouard, Nicolas},
	year         = 2018,
	month        = nov,
	journal      = {Physical Review Letters},
	volume       = 121,
	number       = 18,
	pages        = 180505,
	doi          = {10.1103/PhysRevLett.121.180505},
	ids          = {Sekatski2018}
}
@article{Gheorghiu2015,
	title        = {{Robustness and Device Independence of Verifiable Blind Quantum Computing}},
	author       = {Gheorghiu, Alexandru and Kashefi, Elham and Wallden, Petros},
	year         = 2015,
	month        = aug,
	journal      = {New Journal of Physics},
	volume       = 17,
	number       = 8,
	pages        = {083040},
	doi          = {10.1088/1367-2630/17/8/083040},
	issn         = {1367-2630},
	language     = {en}
}
@article{Supic2016a,
	title        = {{Self-Testing through EPR-Steering}},
	author       = {{\v S}upi{\'c}, Ivan and Hoban, Matty J.},
	year         = 2016,
	month        = jul,
	journal      = {New Journal of Physics},
	volume       = 18,
	number       = 7,
	pages        = {075006},
	doi          = {10.1088/1367-2630/18/7/075006},
	issn         = {1367-2630},
	archiveprefix = {arXiv},
	eprinttype   = {arxiv},
	eprint       = {1601.01552},
	ids          = {Supic2016}
}
@article{Bancal2018a,
	title        = {{Noise-Resistant Device-Independent Certification of Bell State Measurements}},
	author       = {Bancal, Jean-Daniel and Sangouard, Nicolas and Sekatski, Pavel},
	year         = 2018,
	month        = dec,
	journal      = {Physical Review Letters},
	volume       = 121,
	number       = 25,
	pages        = 250506,
	doi          = {10.1103/PhysRevLett.121.250506}
}
@article{PhysRevResearch.2.013011,
	title        = {{Measurement incompatibility and steering are necessary and sufficient for operational contextuality}},
	author       = {Tavakoli, Armin and Uola, Roope},
	year         = 2020,
	month        = {Jan},
	journal      = {Phys. Rev. Research},
	publisher    = {American Physical Society},
	volume       = 2,
	pages        = {013011},
	doi          = {10.1103/PhysRevResearch.2.013011},
	url          = {https://link.aps.org/doi/10.1103/PhysRevResearch.2.013011},
	issue        = 1,
	numpages     = 7
}
@article{Tavakoli2018c,
	title        = {{Self-Testing Quantum States and Measurements in the Prepare-and-Measure Scenario}},
	author       = {Tavakoli, Armin and Kaniewski, Jedrzej and Vertesi, Tam{\'a}s and Rosset, Denis and Brunner, Nicolas},
	year         = 2018,
	month        = dec,
	journal      = {Physical Review A},
	volume       = 98,
	number       = 6,
	pages        = {062307},
	doi          = {10.1103/PhysRevA.98.062307}
}
@article{Renou2018,
	title        = {{Self-Testing Entangled Measurements in Quantum Networks}},
	author       = {Renou, Marc Olivier and Kaniewski, Jedrzej and Brunner, Nicolas},
	year         = 2018,
	month        = dec,
	journal      = {Physical Review Letters},
	volume       = 121,
	number       = 25,
	pages        = 250507,
	doi          = {10.1103/PhysRevLett.121.250507},
	issn         = {0031-9007, 1079-7114},
	archiveprefix = {arXiv},
	eprinttype   = {arxiv},
	eprint       = {1807.04956}
}
@article{Barrett2005PRunit,
	title        = {{Popescu-Rohrlich Correlations as a Unit of Nonlocality}},
	author       = {Barrett, Jonathan and Pironio, Stefano},
	year         = 2005,
	journal      = {prl},
	volume       = 95,
	number       = 14,
	pages        = 140401,
	url          = {http://link.aps.org/doi/10.1103/PhysRevLett.95.140401},
	type         = {Journal Article}
}
@article{Toner2003,
	title        = {{Communication Cost of Simulating Bell Correlations}},
	author       = {Toner, B. F. and Bacon, D.},
	year         = 2003,
	month        = oct,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 91,
	pages        = 187904,
	doi          = {10.1103/PhysRevLett.91.187904},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.91.187904},
	issue        = 18,
	numpages     = 4
}
Article{Brask2017,
  author  = {J. B. Brask and R. Chaves},
  title   = {{Bell scenarios with communication}},
  journal = {J. Phys. A},
  year    = {2017},
  volume  = {50},
  number  = {9},
  pages   = {094001},
  url     = {http://stacks.iop.org/1751-8121/50/i=9/a=094001},
}
@article{Norsen2009,
	title        = {{Local Causality and Completeness: Bell vs. Jarrett}},
	author       = {Norsen, Travis},
	year         = 2009,
	month        = mar,
	day          = {01},
	journal      = {Found. Phys.},
	volume       = 39,
	number       = 3,
	pages        = {273--294},
	doi          = {10.1007/s10701-009-9281-1},
	issn         = {1572-9516},
	url          = {https://doi.org/10.1007/s10701-009-9281-1}
}
@book{Maudlin2002quantum,
	title        = {{Quantum Non-Locality and Relativity : Metaphysical Intimations of Modern Physics}},
	author       = {Maudlin, Tim},
	year         = 2002,
	publisher    = {Blackwell Publishers},
	doi          = {10.1002/9780470752166},
	isbn         = 9780470752166
}
@article{Rosset2014classifying,
	title        = {{Classifying 50 years of Bell inequalities}},
	author       = {Denis Rosset and Jean-Daniel Bancal and Nicolas Gisin},
	year         = 2014,
	journal      = {J. Phys. A},
	volume       = 47,
	number       = 42,
	pages        = 424022,
	url          = {http://stacks.iop.org/1751-8121/47/i=42/a=424022}
}
@article{CGLMP2005,
	title        = {{Bell Inequalities for Arbitrarily High-Dimensional Systems}},
	author       = {Collins, Daniel and Gisin, Nicolas and Linden, Noah and Massar, Serge and Popescu, Sandu},
	year         = 2002,
	month        = jan,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 88,
	pages        = {040404},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.88.040404},
	issue        = 4,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.88.040404}
}
@article{Jones2005I3322NoSig,
	title        = {{Interconversion of nonlocal correlations}},
	author       = {Jones, Nick S. and Masanes, Llu\'{\i}s},
	year         = 2005,
	month        = nov,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 72,
	pages        = {052312},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.72.052312},
	issue        = 5,
	numpages     = 9,
	doi.hide     = {10.1103/PhysRevA.72.052312}
}
@article{Rai2018quantumvoids,
	title        = {{Into the Quantum Void: Geometry of the Quantum Set on No-Signaling Faces}},
	author       = {{Rai}, Ashutosh and {Duarte}, Cristhiano and {Brito}, Samurai and {Chaves}, Rafael},
	year         = 2018,
	month        = dec,
	journal      = {arXiv:1812.06057},
	url          = {https://arxiv.org/abs/1812.06057},
	eid.hide     = {arXiv:1812.06057},
	pages.hide   = {arXiv:1812.06057},
	archiveprefix.hide = {arXiv},
	eprint.hide  = {1812.06057},
	primaryclass = {quant-ph}
}
@article{Bamps2015selftesting,
	title        = {{Sum-of-squares decompositions for a family of Clauser-Horne-Shimony-Holt-like inequalities and their application to self-testing}},
	author       = {Bamps, C\'edric and Pironio, Stefano},
	year         = 2015,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 91,
	pages        = {052111},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.91.052111},
	issue        = 5,
	numpages     = 13,
	doi.hide     = {10.1103/PhysRevA.91.052111}
}
@article{Yang2013selftesting,
	title        = {{Robust self-testing of unknown quantum systems into any entangled two-qubit states}},
	author       = {Yang, Tzyh Haur and Navascu\'es, Miguel},
	year         = 2013,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 87,
	pages        = {050102(R)},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.87.050102},
	issue        = 5,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevA.87.050102}
}
@article{Acin2012randomnessvsnonlocality,
	title        = {{Randomness versus Nonlocality and Entanglement}},
	author       = {Ac\'{\i}n, Antonio and Massar, Serge and Pironio, Stefano},
	year         = 2012,
	month        = mar,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 108,
	pages        = 100402,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.108.100402},
	issue        = 10,
	numpages     = 5,
	doi.hide     = {10.1103/PhysRevLett.108.100402}
}
@article{BMP,
	title        = {{Device-independent randomness generation with sublinear shared quantum resources}},
	author       = {C{\'{e}}dric Bamps and Serge Massar and Stefano Pironio},
	year         = 2018,
	month        = aug,
	journal      = {Quantum},
	publisher    = {Verein zur Forderung des Open Access Publizierens in den Quantenwissenschaften},
	volume       = 2,
	pages        = 86,
	doi          = {10.22331/q-2018-08-22-86},
	url          = {https://arxiv.org/abs/1704.02130}
}
@article{Dhara2013DIRNG,
	title        = {{Maximal quantum randomness in Bell tests}},
	author       = {Dhara, Chirag and Prettico, Giuseppe and Ac\'{\i}n, Antonio},
	year         = 2013,
	month        = nov,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 88,
	pages        = {052116},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.88.052116},
	issue        = 5,
	numpages     = 5,
	doi.hide     = {10.1103/PhysRevA.88.052116}
}
@article{Kaniewski2016chsh,
	title        = {{Device-independent two-party cryptography secure against sequential attacks}},
	author       = {Jadrzej Kaniewski and Stephanie Wehner},
	year         = 2016,
	journal      = {New J. Phys.},
	volume       = 18,
	number       = 5,
	pages        = {055004},
	url          = {http://stacks.iop.org/1367-2630/18/i=5/a=055004}
}
@article{Wolfe2012quantumbounds,
	title        = {{Quantum bounds for inequalities involving marginal expectation values}},
	author       = {Wolfe, Elie and Yelin, S. F.},
	year         = 2012,
	month        = jul,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 86,
	pages        = {012123},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.86.012123},
	issue        = 1,
	numpages     = 6,
	doi.hide     = {10.1103/PhysRevA.86.012123}
}
@article{Brunner2005different,
	title        = {{Entanglement and non-locality are different resources}},
	author       = {Nicolas Brunner and Nicolas Gisin and Valerio Scarani},
	year         = 2005,
	journal      = {New J. Phys.},
	volume       = 7,
	number       = 1,
	pages        = 88,
	url          = {http://stacks.iop.org/1367-2630/7/i=1/a=088}
}
@article{Methot2006anomaly,
	title        = {{An anomaly of non-locality}},
	author       = {{Methot}, A.~A. and {Scarani}, V.},
	year         = 2006,
	month        = jan,
	journal      = {arXiv:quant-ph/0601210},
	url          = {https://arxiv.org/abs/quant-ph/0601210},
	eid.hide     = {quant-ph/0601210},
	pages.hide   = {quant-ph/0601210},
	archiveprefix.hide = {arXiv},
	eprint.hide  = {quant-ph/0601210},
	primaryclass = {quant-ph}
}
@article{Rabelo2012Hardy,
	title        = {{Device-Independent Bounds for Hardy's Experiment}},
	author       = {Rabelo, Rafael and Zhi, Law Yun and Scarani, Valerio},
	year         = 2012,
	month        = oct,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 109,
	pages        = 180401,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.109.180401},
	issue        = 18,
	numpages     = 5,
	doi.hide     = {10.1103/PhysRevLett.109.180401}
}
@article{Hardy1993paradox,
	title        = {{Nonlocality for two particles without inequalities for almost all entangled states}},
	author       = {Hardy, Lucien},
	year         = 1993,
	month        = sep,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 71,
	pages        = {1665--1668},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.71.1665},
	issue        = 11,
	numpages     = {0},
	doi.hide     = {10.1103/PhysRevLett.71.1665}
}
@article{Coladangelo2017,
	title        = {{All pure bipartite entangled states can be self-tested}},
	author       = {Andrea Coladangelo and Koon Tong Goh and Valerio Scarani},
	year         = 2017,
	month        = may,
	journal      = {Nat. Comm.},
	publisher    = {Springer Nature},
	volume       = 8,
	pages        = 15485,
	doi          = {10.1038/ncomms15485},
	url          = {https://doi.org/10.1038/ncomms15485}
}
@article{Buscemi-ProbInfTrans-2016,
	title        = {{Degradable channels, less noisy channels, and quantum statistical morphisms: An equivalence relation}},
	author       = {Buscemi, Francesco},
	year         = 2016,
	journal      = {Probl Inf Transm},
	volume       = 52,
	pages        = {201--213},
	doi          = {10.1134/S0032946016030017}
}
@article{Rosset-Buscemi-Liang-PRX,
	title        = {{Resource Theory of Quantum Memories and Their Faithful Verification with Minimal Assumptions}},
	author       = {Rosset, Denis and Buscemi, Francesco and Liang, Yeong-Cherng},
	year         = 2018,
	month        = may,
	journal      = {Phys. Rev. X},
	publisher    = {American Physical Society},
	volume       = 8,
	pages        = {021033},
	doi          = {10.1103/PhysRevX.8.021033},
	url          = {https://link.aps.org/doi/10.1103/PhysRevX.8.021033},
	issue        = 2,
	numpages     = 15
}
@article{Dur2000twoways,
	title        = {{Three qubits can be entangled in two inequivalent ways}},
	author       = {D\"ur, W. and Vidal, G. and Cirac, J. I.},
	year         = 2000,
	month        = nov,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 62,
	pages        = {062314},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.62.062314},
	issue        = 6,
	numpages     = 12,
	doi.hide     = {10.1103/PhysRevA.62.062314}
}
@article{Acin2001triclassify,
	title        = {{Classification of Mixed Three-Qubit States}},
	author       = {Ac\'{\i}n, A. and Bru\ss{}, D. and Lewenstein, M. and Sanpera, A.},
	year         = 2001,
	month        = jul,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 87,
	pages        = {040401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.87.040401},
	issue        = 4,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.87.040401}
}
@article{Guhne2009entanglement,
	title        = {{Entanglement detection}},
	author       = {Otfried GÃŒhne and GÃ©za TÃ³th},
	year         = 2009,
	journal      = {Phys. Rep.},
	volume       = 474,
	number       = 1,
	pages        = {1--75},
	issn         = {0370-1573},
	url          = {http://www.sciencedirect.com/science/article/pii/S0370157309000623},
	doi.hide     = {10.1016/j.physrep.2009.02.004}
}
@article{Pan2006,
	title        = {{Classification and Quantification of Entangled Bipartite Pure States}},
	author       = {Feng Pan and Guoying Lu and J.~P. Draayer},
	year         = 2006,
	month        = may,
	journal      = {IInt. J. Mod. Phys. B},
	publisher    = {World Scientific Pub Co Pte Lt},
	volume       = 20,
	number       = {11n13},
	pages        = {1333--1342},
	doi          = {10.1142/s0217979206033966},
	url          = {https://doi.org/10.1142/s0217979206033966}
}
@article{Masanes2003,
	title        = {{Necessary and sufficient condition for quantum-generated correlations}},
	author       = {{Masanes}, Ll.},
	year         = 2003,
	month        = sep,
	journal      = {quant-ph/0309137},
	url          = {https://arxiv.org/abs/quant-ph/0309137}
}
@article{Allcock2009,
	title        = {{Recovering part of the boundary between quantum and nonquantum correlations from information causality}},
	author       = {Allcock, Jonathan and Brunner, Nicolas and Pawlowski, Marcin and Scarani, Valerio},
	year         = 2009,
	month        = oct,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 80,
	pages        = {040103(R)},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.80.040103},
	issue        = 4,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevA.80.040103}
}
@article{Brito2018tracedistance,
	title        = {{Quantifying Bell nonlocality with the trace distance}},
	author       = {Brito, S. G. A. and Amaral, B. and Chaves, R.},
	year         = 2018,
	month        = feb,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 97,
	pages        = {022111},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.97.022111},
	issue        = 2,
	numpages     = 11,
	doi.hide     = {10.1103/PhysRevA.97.022111}
}
@article{Verstraete2003,
	title        = {{Normal forms and entanglement measures for multipartite quantum states}},
	author       = {Verstraete, Frank and Dehaene, Jeroen and De Moor, Bart},
	year         = 2003,
	month        = jul,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 68,
	pages        = {012103},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.68.012103},
	issue        = 1,
	numpages     = 7,
	doi.hide     = {10.1103/PhysRevA.68.012103}
}
@article{Barnum2001,
	title        = {{Monotones and invariants for multi-particle quantum states}},
	author       = {H Barnum and N Linden},
	year         = 2001,
	journal      = {J. Phys. A},
	volume       = 34,
	number       = 35,
	pages        = 6787,
	url          = {http://stacks.iop.org/0305-4470/34/i=35/a=305},
	doi.hide     = {10.1088/0305-4470/34/35/305}
}
@inproceedings{Pearl1995,
	title        = {{On the Testability of Causal Models with Latent and Instrumental Variables}},
	author       = {J. Pearl},
	year         = 1995,
	booktitle    = {Proc. 11th Conf. Uncertainty in Artificial Intelligence},
	pages        = {435--443},
	url          = {http://singapore.cs.ucla.edu/LECTURE/lecture_sec1.htm},
	address.hide = {San Francisco, CA},
	publisher.hide = {Morgan Kaufmann}
}
@inproceedings{Bonet2001,
	title        = {{Instrumentality Tests Revisited}},
	author       = {Blai Bonet},
	year         = 2001,
	booktitle    = {Proc. 17th Conf. Uncertainty in Artificial Intelligence},
	pages        = {48--55},
	url          = {https://pdfs.semanticscholar.org/e397/89b514f1a059e90fabada35aaaf7e6ef3bc9.pdf},
	publisher.hide = {Morgan Kaufmann}
}
@inproceedings{Evans2012,
	title        = {{Graphical methods for inequality constraints in marginalized DAGs}},
	author       = {Robin J. Evans},
	year         = 2012,
	month        = sep,
	booktitle    = {{{IEEE} International Workshop on Machine Learning for Signal Processing}},
	doi          = {10.1109/mlsp.2012.6349796},
	url          = {https://doi.org/10.1109/mlsp.2012.6349796},
	year.hide    = 2012,
	publisher.hide = {{IEEE}}
}
@article{Chaves2017instrumental,
	title        = {{Quantum violation of an instrumental test}},
	author       = {Rafael Chaves and Gonzalo Carvacho and Iris Agresti and Valerio Di Giulio and Leandro Aolita and Sandro Giacomini and Fabio Sciarrino},
	year         = 2017,
	month        = dec,
	journal      = {Nat. Phy.},
	publisher    = {Springer Nature},
	volume       = 14,
	number       = 3,
	pages        = {291--296},
	doi          = {10.1038/s41567-017-0008-5},
	author.hide  = {R. {Chaves~$\textit{et~al.}$}}
}
@article{Steudel2015,
	title        = {{Information-Theoretic Inference of Common Ancestors}},
	author       = {Steudel, Bastian and Ay, Nihat},
	year         = 2015,
	journal      = {Entropy},
	volume       = 17,
	number       = 4,
	pages        = {2304--2327},
	issn         = {1099-4300},
	url          = {http://www.mdpi.com/1099-4300/17/4/2304},
	doi.hide     = {10.3390/e17042304}
}
@article{Gisin2017triangle,
	title        = {{The Elegant Joint Quantum Measurement and some conjectures about N-locality in the Triangle and other Configurations}},
	author       = {{Gisin}, Nicolas},
	year         = 2017,
	month        = aug,
	journal      = {arXiv:1708.05556},
	url          = {https://arxiv.org/abs/1708.05556},
	eid.hide     = {arXiv:1708.05556},
	pages.hide   = {arXiv:1708.05556},
	archiveprefix.hide = {arXiv},
	eprint.hide  = {1708.05556},
	primaryclass = {quant-ph}
}
@article{Branciard2010,
	title        = {{Characterizing the Nonlocal Correlations Created via Entanglement Swapping}},
	author       = {Branciard, C. and Gisin, N. and Pironio, S.},
	year         = 2010,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 104,
	pages        = 170401,
	doi          = {10.1103/PhysRevLett.104.170401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.104.170401},
	issue        = 17,
	numpages     = 4
}
@article{BilocalCorrelations,
	title        = {{Bilocal versus nonbilocal correlations in entanglement-swapping experiments}},
	author       = {Branciard, Cyril and Rosset, Denis and Gisin, Nicolas and Pironio, Stefano},
	year         = 2012,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 85,
	number       = 3,
	pages        = {032119},
	url          = {http://link.aps.org/doi/10.1103/PhysRevA.85.032119}
}
@article{Chaves2017starnetworks,
	title        = {{Maximal violation of \(n\)-locality inequalities in a star-shaped quantum network}},
	author       = {Francesco Andreoli and Gonzalo Carvacho and Luca Santodonato and Rafael Chaves and Fabio Sciarrino},
	year         = 2017,
	journal      = {New J. Phys.},
	volume       = 19,
	number       = 11,
	pages        = 113020,
	url          = {http://stacks.iop.org/1367-2630/19/i=11/a=113020},
	doi.hide     = {10.1088/1367-2630/aa8b9b}
}
@article{TavakoliStarNetworks,
	title        = {{Nonlocal correlations in the star-network configuration}},
	author       = {Tavakoli, Armin and Skrzypczyk, Paul and Cavalcanti, Daniel and Ac\'{\i}n, Antonio},
	year         = 2014,
	month        = dec,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 90,
	pages        = {062109},
	url          = {http://link.aps.org/doi/10.1103/PhysRevA.90.062109},
	issue        = 6,
	numpages     = 12,
	doi.hide     = {10.1103/PhysRevA.90.062109}
}
@article{Branciard2013,
	title        = {{Measurement-Device-Independent Entanglement Witnesses for All Entangled Quantum States}},
	author       = {Branciard, Cyril and Rosset, Denis and Liang, Yeong-Cherng and Gisin, Nicolas},
	year         = 2013,
	month        = feb,
	journal      = {Physical Review Letters},
	volume       = 110,
	number       = 6,
	pages        = {060405},
	doi          = {10.1103/PhysRevLett.110.060405}
}
@article{Shahandeh2017,
	title        = {{Measurement-Device-Independent Approach to Entanglement Measures}},
	author       = {Shahandeh, Farid and Hall, Michael J. W. and Ralph, Timothy C.},
	year         = 2017,
	month        = apr,
	journal      = {Physical Review Letters},
	volume       = 118,
	number       = 15,
	pages        = 150505,
	doi          = {10.1103/PhysRevLett.118.150505}
}
@article{Supic2017,
	title        = {{Measurement-Device-Independent Entanglement and Randomness Estimation in Quantum Networks}},
	author       = {{\v S}upi{\'c}, Ivan and Skrzypczyk, Paul and Cavalcanti, Daniel},
	year         = 2017,
	month        = apr,
	journal      = {Physical Review A},
	volume       = 95,
	number       = 4,
	pages        = {042340},
	doi          = {10.1103/PhysRevA.95.042340}
}
@article{Rosset2018a,
	title        = {{Practical Measurement-Device-Independent Entanglement Quantification}},
	author       = {Rosset, Denis and Martin, Anthony and Verbanis, Ephanielle and Lim, Charles Ci Wen and Thew, Rob},
	year         = 2018,
	month        = nov,
	journal      = {Physical Review A},
	volume       = 98,
	number       = 5,
	pages        = {052332},
	doi          = {10.1103/PhysRevA.98.052332}
}
@article{Rosset2013a,
	title        = {{Entangled States Cannot Be Classically Simulated in Generalized Bell Experiments with Quantum Inputs}},
	author       = {Rosset, Denis and Branciard, Cyril and Gisin, Nicolas and Liang, Yeong-Cherng},
	year         = 2013,
	month        = may,
	journal      = {New Journal of Physics},
	volume       = 15,
	number       = 5,
	pages        = {053025},
	doi          = {10.1088/1367-2630/15/5/053025},
	issn         = {1367-2630}
}
@article{RossetNetworks,
	title        = {{Nonlinear Bell Inequalities Tailored for Quantum Networks}},
	author       = {Rosset, Denis and Branciard, Cyril and Barnea, Tomer Jack and P\"utz, Gilles and Brunner, Nicolas and Gisin, Nicolas},
	year         = 2016,
	month        = jan,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 116,
	pages        = {010403},
	doi          = {10.1103/PhysRevLett.116.010403},
	url          = {http://link.aps.org/doi/10.1103/PhysRevLett.116.010403},
	author.hide  = {D. {Rosset~$\textit{et~al.}$}},
	issue        = 1,
	numpages     = 5,
	doi.hide     = {10.1103/PhysRevLett.116.010403}
}
@article{tavakoli2016noncyclic,
	title        = {{Bell-type inequalities for arbitrary noncyclic networks}},
	author       = {Tavakoli, Armin},
	year         = 2016,
	month        = mar,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 93,
	pages        = {030101(R)},
	url          = {http://link.aps.org/doi/10.1103/PhysRevA.93.030101},
	issue        = 3,
	numpages     = 5,
	doi.hide     = {10.1103/PhysRevA.93.030101}
}
@article{Forster2009distillation,
	title        = {{Distilling Nonlocality}},
	author       = {Forster, Manuel and Winkler, Severin and Wolf, Stefan},
	year         = 2009,
	month        = mar,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 102,
	pages        = 120401,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.102.120401},
	issue        = 12,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.102.120401}
}
@article{Brunner2009distillation,
	title        = {{Nonlocality Distillation and Postquantum Theories with Trivial Communication Complexity}},
	author       = {Brunner, Nicolas and Skrzypczyk, Paul},
	year         = 2009,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 102,
	pages        = 160403,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.102.160403},
	issue        = 16,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.102.160403}
}
@article{Lang2014zoo,
	title        = {{Closed sets of correlations: answers from the zoo}},
	author       = {Ben Lang and TamÃ¡s VÃ©rtesi and Miguel NavascuÃ©s},
	year         = 2014,
	journal      = {J. Phys. A},
	volume       = 47,
	number       = 42,
	pages        = 424029,
	url          = {http://stacks.iop.org/1751-8121/47/i=42/a=424029}
}
@article{Gour2015thermo,
	title        = {{The resource theory of informational nonequilibrium in thermodynamics}},
	author       = {Gilad Gour and Markus P. M{\"u}ller and Varun Narasimhachar and Robert W. Spekkens and Nicole Yunger Halpern},
	year         = 2015,
	journal      = {Phys. Rep.},
	volume       = 583,
	pages        = {1--58},
	issn         = {0370-1573},
	url          = {http://www.sciencedirect.com/science/article/pii/S037015731500229X},
	doi.hide     = {10.1016/j.physrep.2015.04.003}
}
@book{BancalDIApproach,
	title        = {{On the Device-Independent Approach to Quantum Physics}},
	author       = {Bancal, Jean-Daniel},
	year         = 2014,
	journal      = {Springer Theses},
	publisher    = {Springer International Publishing},
	doi          = {10.1007/978-3-319-01183-7},
	isbn         = {http://id.crossref.org/isbn/978-3-319-01183-7},
	issn         = {2190-5061},
	url          = {http://dx.doi.org/10.1007/978-3-319-01183-7}
}
@article{Scarani2012device,
	title        = {{The Device-Independent Outlook on Quantum Physics}},
	author       = {Scarani, Valerio},
	year         = 2012,
	journal      = {Acta Physica Slovaca},
	publisher    = {SLOVAK ACAD SCIENCES INST PHYSICS DUBRAVSKA CESTA 9, 842 28 BRATISLAVA, SLOVAKIA},
	volume       = 62,
	number       = 4,
	pages        = 347,
	doi          = {10.2478/v10155-012-0003-4},
	url          = {http://www.physics.sk/aps/pub.php?y=2012&pub=aps-12-04}
}
@book{Seress2003,
	title        = {{Permutation Group Algorithms}},
	author       = {Seress, Akos},
	year         = 2003,
	publisher    = {Cambridge University Press},
	doi          = {10.1017/CBO9780511546549},
	place.hide   = {Cambridge},
	series.hide  = {Cambridge Tracts in Mathematics},
	collection.hide = {Cambridge Tracts in Mathematics}
}
@book{Bredon1972groups,
	title        = {{Introduction to Compact Transformation Groups}},
	author       = {Bredon, G.E.},
	year         = 1972,
	publisher    = {Elsevier Science},
	series       = {Pure and Applied Mathematics},
	isbn         = 9780080873596,
	url          = {https://books.google.co.uk/books?id=qXEl\_AIeSBUC}
}
@article{Linden1997,
	title        = {{On Multi-Particle Entanglement}},
	author       = {Linden, N. and Popescu, S. and Popescu, S.},
	year         = 1998,
	journal      = {Fortschritte der Physik},
	volume       = 46,
	number       = {4-5},
	pages        = {567--578},
	doi          = {10.1002/(SICI)1521-3978(199806)46:4/5<567::AID-PROP567>3.0.CO;2-H},
	url          = {https://onlinelibrary.wiley.com/doi/abs/10.1002/%28SICI%291521-3978%28199806%2946%3A4/5%3C567%3A%3AAID-PROP567%3E3.0.CO%3B2-H}
}
@article{Pironio2005,
	title        = {{Lifting Bell inequalities}},
	author       = {Stefano Pironio},
	year         = 2005,
	month        = jun,
	journal      = {J. Math. Phys.},
	publisher    = {{AIP} Publishing},
	volume       = 46,
	number       = 6,
	pages        = {062112},
	doi          = {10.1063/1.1928727}
}
@article{Wolfe2015nonconvexity,
	title        = {{Identifying nonconvexity in the sets of limited-dimension quantum correlations}},
	author       = {Donohue, John Matthew and Wolfe, Elie},
	year         = 2015,
	month        = dec,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 92,
	pages        = {062120},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.92.062120},
	issue        = 6,
	numpages     = 11,
	doi.hide     = {10.1103/PhysRevA.92.062120}
}
@thesis{Kabel2017,
	title        = {{Exploring the Interplay between Entanglement and Nonlocality: A novel perspective on the Peres Conjecture}},
	author       = {Kabel,  Victoria},
	url          = {http://hdl.handle.net/21.11116/0000-0001-3E8E-B},
	type         = {Bachelor's Thesis},
	school       = {Max Planck Institute of Quantum Optics}
}
@book{munkres2018topology,
	title        = {{Topology}},
	author       = {Munkres, James},
	year         = 2018,
	publisher    = {Pearson},
	address      = {New York, NY},
	isbn         = 9780134689517,
	url          = {}
}
@inproceedings{sep-bell-theorem,
	title        = {{Bell's Theorem}},
	author       = {Shimony, Abner},
	year         = 2017,
	booktitle    = {The Stanford Encyclopedia of Philosophy},
	url          = {https://plato.stanford.edu/archives/fall2017/entries/bell-theorem/},
	editor.hide  = {Edward N. Zalta},
	howpublished.hide = {\url{https://plato.stanford.edu/archives/fall2017/entries/bell-theorem/}},
	edition.hide = {Fall 2017},
	publisher.hide = {Metaphysics Research Lab, Stanford University}
}
@article{wiseman2014two,
	title        = {{The two Bell's theorems of John Bell}},
	author       = {Wiseman, Howard M},
	year         = 2014,
	journal      = {J. Phys. A},
	publisher    = {IOP Publishing},
	volume       = 47,
	number       = 42,
	pages        = 424001,
	doi          = {10.1088/1751-8113/47/42/424001},
	url          = {https://doi.org/10.1088%2F1751-8113%2F47%2F42%2F424001}
}
@article{d1979quantum,
	title        = {{The Quantum Theory and Reality}},
	author       = {d'Espagnat, Bernard},
	year         = 1979,
	journal      = {Scientific American},
	publisher    = {Scientific American},
	volume       = 241,
	number       = 5,
	pages        = {158--181},
	url          = {https://www.ifi.unicamp.br/~mtamash/f689_mecquant_i/sciam241_5_158.pdf}
}
@inbook{Pech2009minimalrep,
	title        = {{Enumerating Set Orbits}},
	author       = {Pech, Christian and Reichard, Sven},
	year         = 2009,
	booktitle    = {{Algorithmic Algebraic Combinatorics and Gr{\"o}bner Bases}},
	publisher    = {Springer Berlin Heidelberg},
	address      = {Berlin, Heidelberg},
	pages        = {137--150},
	doi          = {10.1007/978-3-642-01960-9_4},
	isbn         = {978-3-642-01960-9},
	url          = {https://doi.org/10.1007/978-3-642-01960-9_4},
	editor       = {Klin, Mikhail and Jones, Gareth A. and Juri{\v{s}}i{\'{c}}, Aleksandar and Muzychuk, Mikhail and Ponomarenko, Ilia}
}
@article{Jefferson2017canonicalrep,
	title        = {{Minimal and Canonical Images}},
	author       = {{Jefferson}, Christopher and {Jonauskyte}, Eliza and {Pfeiffer}, Markus and {Waldecker}, Rebecca},
	year         = 2017,
	month        = mar,
	journal      = {arXiv:1703.00197},
	url          = {https://arxiv.org/abs/1703.00197},
	eid.hide     = {arXiv:1703.00197},
	pages.hide   = {arXiv:1703.00197},
	archiveprefix = {arXiv},
	eprint.hide  = {1703.00197},
	primaryclass = {math.GR}
}
@article{Horodecki2015,
	title        = {{Axiomatic Approach to Contextuality and Nonlocality}},
	author       = {Horodecki, Karol and Grudka, Andrzej and Joshi, Pankaj and K{\l}obus, Waldemar and {\L}odyga, Justyna},
	year         = 2015,
	month        = sep,
	journal      = {Physical Review A},
	volume       = 92,
	number       = 3,
	pages        = {032104},
	doi          = {10.1103/PhysRevA.92.032104}
}
@misc{bellspaces,
	title        = {{Algebraic and geometric properties of local transformations}},
	author       = {Denis Rosset and {\"a}min Baumeler and Jean-Daniel Bancal and Nicolas Gisin and Anthony Martin and Marc-Olivier Renou and Elie Wolfe},
	year         = 2020,
	eprint       = {2004.09405},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@misc{Robnote,
	title        = {{Distinguishing inference from influence: reassessing how to formalize various causal notions appearing in the Bell literature}},
	author       = {Robert W. Spekkens},
	note         = {Forthcoming.}
}
@book{DimensionTheory,
	title        = {{Theory of dimensions, finite and infinite}},
	author       = {Ryszard Engelking},
	year         = 1995,
	series       = {Sigma series in pure mathematics},
	volume       = {},
	isbn         = {3885380102,9783885380108},
	url          = {http://gen.lib.rus.ec/book/index.php?md5=e3354d40ada5522a549950fa4118d136},
	publisher.hide = {Heldermann},
	edition      = {}
}
@book{Quotients1994,
	title        = {{Invariant Theory}},
	author       = {Vladimir Leonidovich Popov},
	year         = 1994,
	booktitle    = {Algebraic Geometry {IV}},
	publisher    = {Springer-Verlag},
	doi          = {10.1007/978-3-662-03073-8},
	url          = {https://doi.org/10.1007/978-3-662-03073-8},
	editor.hide  = {A. N. Parshin and I. R. Shafarevich},
	chapter      = {4: Quotients}
}
@article{Mcmillan1970,
	title        = {{On continuity conditions for functions.}},
	author       = {McMillan, Evelyn R.},
	year         = 1970,
	journal      = {Pacific J. Math.},
	publisher    = {Pacific Journal of Mathematics, A Non-profit Corporation},
	volume       = 32,
	number       = 2,
	pages        = {479--494},
	url          = {https://projecteuclid.org:443/euclid.pjm/1102977373},
	fjournal     = {Pacific Journal of Mathematics}
}
@book{croom2016principles,
	title        = {{Principles of Topology}},
	author       = {Croom, F.H.},
	year         = 2016,
	publisher    = {Dover Publications},
	isbn         = 9780486801544,
	url          = {https://books.google.ca/books?id=ZQFYCwAAQBAJ},
	lccn         = 2015030379,
	series.hide  = {Dover Books on Mathematics},
	chapter      = {6: Compactness}
}
@article{Schumacher2005,
	title        = {{Locality and Information Transfer in Quantum Operations}},
	author       = {Benjamin Schumacher and Michael D. Westmoreland},
	year         = 2005,
	month        = feb,
	journal      = {Quan. Info. Proc.},
	publisher    = {Springer Nature},
	volume       = 4,
	number       = 1,
	pages        = {13--34},
	doi          = {10.1007/s11128-004-3193-y},
	url          = {https://doi.org/10.1007/s11128-004-3193-y}
}
@article{PaviaLocalizable,
	title        = {{No Signaling, Entanglement Breaking, and Localizability in Bipartite Channels}},
	author       = {D'Ariano, Giacomo Mauro and Facchini, Stefano and Perinotti, Paolo},
	year         = 2011,
	month        = jan,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 106,
	pages        = {010501},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.106.010501},
	issue        = 1,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.106.010501}
}
@article{Bancal2012,
	title        = {{Quantum non-locality based on finite-speed causal influences leads to superluminal signalling}},
	author       = {J-D. Bancal and S. Pironio and A. Ac{\'{\i}}n and Y-C. Liang and V. Scarani and N. Gisin},
	year         = 2012,
	month        = oct,
	journal      = {Nat. Phys.},
	publisher    = {Springer Nature},
	volume       = 8,
	number       = 12,
	pages        = {867--870},
	doi          = {10.1038/nphys2460},
	url          = {https://doi.org/10.1038/nphys2460}
}
@article{GellerPiani,
	title        = {{Quantifying non-classical and beyond-quantum correlations in the unified operator formalism}},
	author       = {Joshua Geller and Marco Piani},
	year         = 2014,
	month        = oct,
	journal      = {J. Phys. A},
	publisher    = {{IOP} Publishing},
	volume       = 47,
	number       = 42,
	pages        = 424030,
	doi          = {10.1088/1751-8113/47/42/424030},
	url          = {https://doi.org/10.1088%2F1751-8113%2F47%2F42%2F424030}
}
@article{Short2013,
	title        = {{Simulating all Nonsignaling Correlations via Classical or Quantum Theory with Negative Probabilities}},
	author       = {Al-Safi, Sabri W. and Short, Anthony J.},
	year         = 2013,
	month        = oct,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 111,
	pages        = 170403,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.111.170403},
	issue        = 17,
	numpages     = 5,
	doi.hide     = {10.1103/PhysRevLett.111.170403}
}
@article{Acin2010Unified,
	title        = {{Unified Framework for Correlations in Terms of Local Quantum Observables}},
	author       = {Ac\'{\i}n, A. and Augusiak, R. and Cavalcanti, D. and Hadley, C. and Korbicz, J. K. and Lewenstein, M. and Masanes, Ll. and Piani, M.},
	year         = 2010,
	month        = apr,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 104,
	pages        = 140404,
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.104.140404},
	issue        = 14,
	numpages     = 4,
	doi.hide     = {10.1103/PhysRevLett.104.140404}
}
@article{Amaral2017NCW,
	title        = {{Noncontextual Wirings}},
	author       = {Amaral, Barbara and Cabello, Ad\'an and Cunha, Marcelo Terra and Aolita, Leandro},
	year         = 2018,
	month        = mar,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 120,
	pages        = 130403,
	doi          = {10.1103/PhysRevLett.120.130403},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.120.130403},
	issue        = 13,
	numpages     = 6
}
% Encoding: UTF-8
@control{apsrev41Control,
	title        = {{0}}
}
@article{marvian2016quantify,
	title        = {{How to quantify coherence: Distinguishing speakable and unspeakable notions}},
	author       = {Marvian, Iman and Spekkens, Robert W.},
	year         = 2016,
	month        = nov,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 94,
	pages        = {052324},
	doi          = {10.1103/PhysRevA.94.052324},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.94.052324},
	issue        = 5,
	numpages     = 23
}
@article{anshu2020communication,
	title        = {{From communication complexity to an entanglement spread area law in the ground state of gapped local Hamiltonians}},
	author       = {Anshu, Anurag and Harrow, Aram W and Soleimanifar, Mehdi},
	year         = 2020,
	journal      = {arXiv:2004.15009},
	url          = {https://arxiv.org/abs/2004.15009}
}
@article{Gutoski2008,
	author       = {{Gutoski}, Gus},
	year         = 2008,
	month        = may,
	archiveprefix = {arXiv},
	eprint       = {0805.2209}
}
@article{braunstein1992maximal,
	title        = {{Maximal violation of Bell inequalities for mixed states}},
	author       = {Braunstein, Samuel L. and Mann, A. and Revzen, M.},
	year         = 1992,
	month        = jun,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 68,
	pages        = {3259--3261},
	doi          = {10.1103/PhysRevLett.68.3259},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.68.3259},
	issue        = 22,
	numpages     = {0}
}
@article{Colbeckthesis,
	title        = {{Quantum And Relativistic Protocols For Secure Multi-Party Computation}},
	author       = {Roger Colbeck},
	year         = 2009,
	journal      = {arXiv:0911.3814},
	url          = {https://arxiv.org/abs/0911.3814}
}
@inproceedings{mayers1998quantum,
	title        = {{Quantum cryptography with imperfect apparatus}},
	author       = {Mayers, Dominic and Yao, Andrew},
	year         = 1998,
	booktitle    = {Proc. 39th Symp. Found. Comp. Sci.},
	pages        = {503--509},
	doi          = {10.1109/SFCS.1998.743501},
	organization = {IEEE}
}
@article{Franz2011SelfTestPrecursor,
	title        = {{Extremal Quantum Correlations and Cryptographic Security}},
	author       = {Franz, T. and Furrer, F. and Werner, R. F.},
	year         = 2011,
	month        = jun,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 106,
	pages        = 250502,
	doi          = {10.1103/PhysRevLett.106.250502},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.106.250502},
	issue        = 25,
	numpages     = 4
}
@article{ScaraniStateSelfTest2009,
	title        = {{Device-independent state estimation based on Bell's inequalities}},
	author       = {Bardyn, C.-E. and Liew, T. C. H. and Massar, S. and McKague, M. and Scarani, V.},
	year         = 2009,
	month        = dec,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 80,
	pages        = {062327},
	doi          = {10.1103/PhysRevA.80.062327},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.80.062327},
	issue        = 6,
	numpages     = 8
}
@article{McKague2012,
	title        = {{Robust self-testing of the singlet}},
	author       = {M McKague and T H Yang and V Scarani},
	year         = 2012,
	month        = oct,
	journal      = {J. Phys. A},
	publisher    = {{IOP} Publishing},
	volume       = 45,
	number       = 45,
	pages        = 455304,
	doi          = {10.1088/1751-8113/45/45/455304},
	url          = {https://doi.org/10.1088/1751-8113/45/45/455304}
}
@article{popescu1992states,
	title        = {{Which states violate Bell's inequality maximally?}},
	author       = {Popescu, Sandu and Rohrlich, Daniel},
	year         = 1992,
	journal      = {Phys. Lett. A},
	publisher    = {North-Holland},
	volume       = 169,
	number       = 6,
	pages        = {411--414},
	doi          = {10.1016/0375-9601(92)90819-8}
}
@inproceedings{mckague2010generalized,
	title        = {{Generalized Self-testing and the Security of the 6-State Protocol}},
	author       = {McKague, Matthew and Mosca, Michele},
	year         = 2010,
	booktitle    = {Conference on Quantum Computation, Communication, and Cryptography},
	pages        = {113--130},
	doi          = {10.1007/978-3-642-18073-6_10},
	organization = {Springer}
}
@unpublished{cutmotility,
	title        = {{Motility of the internal-external cut as a foundational principle}},
	author       = {Robert Spekkens},
	year         = 2018,
	url          = {http://pirsa.org/18040073/},
	note         = {{O}bservers in Quantum and Foil Theories, {PIRSA:18040073}}
}
@article{bennett2000exact,
	title        = {{Exact and asymptotic measures of multipartite pure-state entanglement}},
	author       = {Bennett, Charles H. and Popescu, Sandu and Rohrlich, Daniel and Smolin, John A. and Thapliyal, Ashish V.},
	year         = 2000,
	month        = dec,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 63,
	pages        = {012307},
	doi          = {10.1103/PhysRevA.63.012307},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.63.012307},
	issue        = 1,
	numpages     = 12
}
@article{gisin1996hidden,
	title        = {{Hidden quantum nonlocality revealed by local filters}},
	author       = {Gisin, Nicolas},
	year         = 1996,
	journal      = {Physics Letters A},
	publisher    = {Elsevier},
	volume       = 210,
	number       = 3,
	pages        = {151--156},
	url          = {https://www.sciencedirect.com/science/article/abs/pii/S0375960196800016}
}
@article{popescu1995bell,
	title        = {{Bell's inequalities and density matrices: revealing `hidden' nonlocality}},
	author       = {Popescu, Sandu},
	year         = 1995,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 74,
	number       = 14,
	pages        = 2619,
	url          = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.74.2619}
}
@article{gallego2014nonlocality,
	title        = {{Nonlocality in sequential correlation scenarios}},
	author       = {Gallego, Rodrigo and W{\"u}rflinger, Lars Erik and Chaves, Rafael and Ac{\'\i}n, Antonio and Navascu{\'e}s, Miguel},
	year         = 2014,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 16,
	number       = 3,
	pages        = {033037},
	url          = {https://iopscience.iop.org/article/10.1088/1367-2630/16/3/033037/meta}
}
@article{lo2001concentrating,
	title        = {{Concentrating entanglement by local actions: Beyond mean values}},
	author       = {Lo, Hoi-Kwong and Popescu, Sandu},
	year         = 2001,
	month        = jan,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 63,
	pages        = {022301},
	doi          = {10.1103/PhysRevA.63.022301},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.63.022301},
	issue        = 2,
	numpages     = 16
}
@article{regev2011bell,
	title        = {{Bell violations through independent bases games}},
	author       = {Regev, Oded},
	year         = 2011,
	journal      = {arXiv:1101.0576},
	url          = {https://arxiv.org/abs/1101.0576}
}
@article{eberhard1993background,
	title        = {{Background level and counter efficiencies required for a loophole-free Einstein-Podolsky-Rosen experiment}},
	author       = {Eberhard, Philippe H},
	year         = 1993,
	month        = feb,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 47,
	number       = 2,
	pages        = {R747},
	doi          = {10.1103/PhysRevA.47.R747}
}
@article{acin2005optimal,
	title        = {{Optimal Bell tests do not require maximally entangled states}},
	author       = {Ac{\'\i}n, Antonio and Gill, Richard and Gisin, Nicolas},
	year         = 2005,
	month        = nov,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 95,
	number       = 21,
	pages        = 210402,
	doi          = {10.1103/PhysRevLett.95.210402}
}
@article{vidick2011more,
	title        = {{More nonlocality with less entanglement}},
	author       = {Vidick, Thomas and Wehner, Stephanie},
	year         = 2011,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 83,
	number       = 5,
	pages        = {052310},
	doi          = {10.1103/PhysRevA.83.052310}
}
@article{cerf2004quantum,
	title        = {{Simulating Maximal Quantum Entanglement without Communication}},
	author       = {Cerf, N. J. and Gisin, N. and Massar, S. and Popescu, S.},
	year         = 2005,
	month        = jun,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 94,
	pages        = 220403,
	doi          = {10.1103/PhysRevLett.94.220403},
	issue        = 22,
	numpages     = 4
}
@article{liang2011semi,
	title        = {{Semi-device-independent bounds on entanglement}},
	author       = {Liang, Yeong-Cherng and V{\'e}rtesi, Tam{\'a}s and Brunner, Nicolas},
	year         = 2011,
	month        = feb,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 83,
	number       = 2,
	pages        = {022108},
	doi          = {10.1103/PhysRevA.83.022108}
}
@article{Acin2002,
	title        = {{Quantum nonlocality in two three-level systems}},
	author       = {Ac\'{\i}n, A. and Durt, T. and Gisin, N. and Latorre, J. I.},
	year         = 2002,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 65,
	pages        = {052325},
	doi          = {10.1103/PhysRevA.65.052325},
	issue        = 5,
	numpages     = 8
}
@article{Pironio2003,
	title        = {{Violations of Bell inequalities as lower bounds on the communication cost of nonlocal correlations}},
	author       = {Pironio, Stefano},
	year         = 2003,
	month        = dec,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 68,
	pages        = {062102},
	doi          = {10.1103/PhysRevA.68.062102},
	issue        = 6,
	numpages     = 9
}
%%%%%%%%%%%%Old references
%%General resource theory references
@article{PhysRevA.99.032334,
	title        = {{Methods to estimate entanglement in teleportation experiments}},
	author       = {\ifmmode \check{S}\else \v{S}\fi{}upi\ifmmode \acute{c}\else \'{c}\fi{}, Ivan and Skrzypczyk, Paul and Cavalcanti, Daniel},
	year         = 2019,
	month        = mar,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 99,
	pages        = {032334},
	doi          = {10.1103/PhysRevA.99.032334},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.99.032334},
	issue        = 3,
	numpages     = 13
}
@article{Palazuelos2012,
	title        = {{Superactivation of Quantum Nonlocality}},
	author       = {Palazuelos, Carlos},
	year         = 2012,
	month        = nov,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 109,
	pages        = 190401,
	doi          = {10.1103/PhysRevLett.109.190401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.109.190401},
	issue        = 19,
	numpages     = 5
}
@article{Navascues2011,
	title        = {{Activation of Nonlocal Quantum Resources}},
	author       = {Navascu\'es, Miguel and V\'ertesi, Tam\'as},
	year         = 2011,
	month        = feb,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 106,
	pages        = {060403},
	doi          = {10.1103/PhysRevLett.106.060403},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.106.060403},
	issue        = 6,
	numpages     = 4
}
@article{kraft2020quantum,
	title        = {{Quantum entanglement in the triangle network}},
	author       = {Kraft, Tristan and Designolle, S{\'e}bastien and Ritz, Christina and Brunner, Nicolas and G{\"u}hne, Otfried and Huber, Marcus},
	year         = 2020,
	journal      = {arXiv:2002.03970},
	url          = {https://arxiv.org/abs/2002.03970}
}
@article{WolfeNavascues,
	title        = {{The Inflation Technique Completely Solves the Causal Compatibility Problem}},
	author       = {Miguel Navascu{\'{e}}s and Elie Wolfe},
	year         = 2020,
	month        = sep,
	journal      = {J. Caus. Inf.},
	publisher    = {Walter de Gruyter {GmbH}},
	volume       = 8,
	number       = 1,
	pages        = {70--91},
	doi          = {10.1515/jci-2018-0008},
	url          = {https://doi.org/10.1515/jci-2018-0008}
}
Article{Brask2017,
  author  = {J. B. Brask and R. Chaves},
  title   = {{Bell scenarios with communication}},
  journal = {J. Phys. A},
  year    = {2017},
  volume  = {50},
  number  = {9},
  pages   = {094001},
  url     = {http://stacks.iop.org/1751-8121/50/i=9/a=094001},
}
@article{Barrett2005PRresource,
	title        = {{Nonlocal correlations as an information-theoretic resource}},
	author       = {J. {Barrett~$\textit{et~al.}$}},
	year         = 2005,
	month        = feb,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 71,
	pages        = {022101},
	doi          = {10.1103/PhysRevA.71.022101},
	author.hide  = {Barrett, Jonathan and Linden, Noah and Massar, Serge and Pironio, Stefano and Popescu, Sandu and Roberts, David},
	issue        = 2,
	numpages     = 11
}
@article{Jed2016Inequalities,
	title        = {{Analytic and Nearly Optimal Self-Testing Bounds for the Clauser-Horne-Shimony-Holt and Mermin Inequalities}},
	author       = {Kaniewski, Jadrzej},
	year         = 2016,
	month        = aug,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 117,
	pages        = {070402},
	doi          = {10.1103/PhysRevLett.117.070402},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.117.070402},
	issue        = 7,
	numpages     = 6
}
@article{vsupic2019self,
	title        = {{Self-testing of quantum systems: a review}},
	author       = {{\v{S}}upi{\'c}, Ivan and Bowles, Joseph},
	year         = 2019,
	journal      = {arXiv:1904.10042},
	url          = {https://arxiv.org/abs/1904.10042}
}
@article{JedWeak2020,
	title        = {{Weak form of self-testing}},
	author       = {Kaniewski, Jadrzej},
	year         = 2020,
	month        = sep,
	journal      = {Phys. Rev. Research},
	publisher    = {American Physical Society},
	volume       = 2,
	pages        = {033420},
	doi          = {10.1103/PhysRevResearch.2.033420},
	url          = {https://link.aps.org/doi/10.1103/PhysRevResearch.2.033420},
	issue        = 3,
	numpages     = 12
}
@article{Baccari2020,
	title        = {{Device-Independent Certification of Genuinely Entangled Subspaces}},
	author       = {Baccari, Flavio and Augusiak, Remigiusz and \ifmmode \check{S}\else \v{S}\fi{}upi\ifmmode \acute{c}\else \'{c}\fi{}, Ivan and Ac\'{\i}n, Antonio},
	year         = 2020,
	month        = dec,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 125,
	pages        = 260507,
	doi          = {10.1103/PhysRevLett.125.260507},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.125.260507},
	issue        = 26,
	numpages     = 6
}
@article{Wang2016,
	title        = {{All the self-testings of the singlet for two binary measurements}},
	author       = {Yukun Wang and Xingyao Wu and Valerio Scarani},
	year         = 2016,
	month        = feb,
	journal      = {New J. Phys.},
	publisher    = {{IOP} Publishing},
	volume       = 18,
	number       = 2,
	pages        = {025021},
	doi          = {10.1088/1367-2630/18/2/025021},
	url          = {https://doi.org/10.1088/1367-2630/18/2/025021}
}
@article{schmidallinequalities,
	title        = {{All the noncontextuality inequalities for arbitrary prepare-and-measure experiments with respect to any fixed set of operational equivalences}},
	author       = {Schmid, David and Spekkens, Robert W. and Wolfe, Elie},
	year         = 2018,
	month        = {Jun},
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 97,
	pages        = {062103},
	doi          = {10.1103/PhysRevA.97.062103},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.97.062103},
	issue        = 6,
	numpages     = 12
}
@article{PhysRevLett.115.110403,
	title        = {{From the Kochen-Specker Theorem to Noncontextuality Inequalities without Assuming Determinism}},
	author       = {Kunjwal, Ravi and Spekkens, Robert W.},
	year         = 2015,
	month        = {Sep},
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 115,
	pages        = 110403,
	doi          = {10.1103/PhysRevLett.115.110403},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.115.110403},
	issue        = 11,
	numpages     = 5
}
@article{mazurek2016experimental,
	title        = {{An experimental test of noncontextuality without unphysical idealizations}},
	author       = {Mazurek, Michael D and Pusey, Matthew F and Kunjwal, Ravi and Resch, Kevin J and Spekkens, Robert W},
	year         = 2016,
	journal      = {Nature communications},
	publisher    = {Nature Publishing Group},
	volume       = 7,
	number       = 1,
	pages        = {1--7},
	doi          = {10.1038/ncomms11780},
	url          = {https://www.nature.com/articles/ncomms11780}
}
@misc{schmid2020unscrambling,
	title        = {{Unscrambling the omelette of causation and inference: The framework of causal-inferential theories}},
	author       = {David Schmid and John H. Selby and Robert W. Spekkens},
	year         = 2021,
	eprint       = {2009.03297},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{Acin2000triclassify,
	title        = {{Generalized Schmidt Decomposition and Classification of Three-Quantum-Bit States}},
	author       = {Ac\'{\i}n, A. and Andrianov, A. and Costa, L. and Jan\'e, E. and Latorre, J. I. and Tarrach, R.},
	year         = 2000,
	month        = aug,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 85,
	pages        = {1560--1563},
	doi          = {10.1103/PhysRevLett.85.1560},
	issue        = 7,
	numpages     = {0}
}
@article{Acin2001puretriclassify,
	title        = {{Three-qubit pure-state canonical forms}},
	author       = {A Ac{\'{\i}}n and A Andrianov and E Jan{\'{e}} and R Tarrach},
	year         = 2001,
	month        = aug,
	journal      = {J. Phys. A},
	publisher    = {{IOP} Publishing},
	volume       = 34,
	number       = 35,
	pages        = {6725--6739},
	doi          = {10.1088/0305-4470/34/35/301}
}
@article{Cadney2014,
	title        = {{Inequalities for the ranks of multipartite quantum states}},
	author       = {Josh Cadney and Marcus Huber and Noah Linden and Andreas Winter},
	year         = 2014,
	journal      = {Linear Algebra and its Applications},
	volume       = 452,
	pages        = {153--171},
	doi          = {10.1016/j.laa.2014.03.035},
	issn         = {0024-3795},
	url          = {http://www.sciencedirect.com/science/article/pii/S0024379514001797}
}
@article{Supi2018Mutliselftest,
	title        = {{Self-testing multipartite entangled states through projections onto two systems}},
	author       = {I {\v{S}}upi{\'{c}} and A Coladangelo and R Augusiak and A Ac{\'{\i}}n},
	year         = 2018,
	month        = aug,
	journal      = {New J. Phys.},
	publisher    = {{IOP} Publishing},
	volume       = 20,
	number       = 8,
	pages        = {083041},
	doi          = {10.1088/1367-2630/aad89b}
}
@article{Bancal2015SelfTesting,
	title        = {{Physical characterization of quantum devices from nonlocal correlations}},
	author       = {Bancal, Jean-Daniel and Navascu\'es, Miguel and Scarani, Valerio and V\'ertesi, Tam\'as and Yang, Tzyh Haur},
	year         = 2015,
	month        = feb,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 91,
	pages        = {022115},
	doi          = {10.1103/PhysRevA.91.022115},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.91.022115},
	issue        = 2,
	numpages     = 16
}
@article{rosset2019characterizing,
	title        = {{Characterizing nonclassicality of arbitrary distributed devices}},
	author       = {Denis Rosset and David Schmid and Francesco Buscemi},
	year         = 2019,
	journal      = {arXiv:1911.12462},
	url          = {https://arxiv.org/abs/1911.12462}
}
@article{Himbeeck2018instrumental,
	title        = {{Quantum violations in the Instrumental scenario and their relations to the Bell scenario}},
	author       = {T. {Van~Himbeeck~$\textit{et~al.}$}},
	year         = 2018,
	month        = apr,
	journal      = {arXiv:1804.04119},
	url          = {https://arxiv.org/abs/1804.04119},
	author.hide  = {{Van Himbeeck}, Thomas and {Bohr Brask}, Jonatan and {Pironio}, Stefano and {Ramanathan}, Ravishankar and {Bel{\'e}n Sainz}, Ana and {Wolfe}, Elie},
	eid.hide     = {arXiv:1804.04119},
	pages.hide   = {arXiv:1804.04119},
	archiveprefix.hide = {arXiv},
	eprint.hide  = {1804.04119},
	primaryclass = {quant-ph}
}
@article{Vertesi2014,
	title        = {{Disproving the Peres conjecture by showing Bell nonlocality from bound entanglement}},
	author       = {Vertesi, Tamas and Brunner, Nicolas},
	year         = 2014,
	journal      = {Nat. Comm.},
	volume       = 5,
	number       = 1,
	pages        = 5297,
	doi          = {10.1038/ncomms6297},
	issn         = {2041-1723},
	url          = {https://doi.org/10.1038/ncomms6297}
}
@article{Peres1999,
	title        = {{All the Bell Inequalities}},
	author       = {Peres, Asher},
	year         = 1999,
	month        = apr,
	day          = {01},
	journal      = {Found. Phys.},
	volume       = 29,
	number       = 4,
	pages        = {589--614},
	doi          = {10.1023/A:1018816310000},
	issn         = {1572-9516}
}
@article{PeresConjDisproof,
	title        = {{Quantum Nonlocality Does Not Imply Entanglement Distillability}},
	author       = {V\'ertesi, Tam\'as and Brunner, Nicolas},
	year         = 2012,
	month        = jan,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 108,
	pages        = {030403},
	doi          = {10.1103/PhysRevLett.108.030403},
	issue        = 3,
	numpages     = 4
}
@article{densecoding,
	title        = {{Communication via one- and two-particle operators on Einstein-Podolsky-Rosen states}},
	author       = {Bennett, Charles H. and Wiesner, Stephen J.},
	year         = 1992,
	month        = nov,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 69,
	pages        = {2881--2884},
	doi          = {10.1103/PhysRevLett.69.2881},
	issue        = 20,
	numpages     = {0}
}
@article{Huber2018,
	title        = {{High-Dimensional Entanglement in States with Positive Partial Transposition}},
	author       = {Huber, Marcus and Lami, Ludovico and Lancien, C{\'e}cilia and M{\"u}ller-Hermes, Alexander},
	year         = 2018,
	month        = nov,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 121,
	pages        = 200503,
	doi          = {10.1103/PhysRevLett.121.200503},
	issue        = 20,
	numpages     = 7
}
@article{Terhal2000,
	title        = {{Schmidt number for density matrices}},
	author       = {Terhal, Barbara M. and Horodecki, Pawe\l{}},
	year         = 2000,
	month        = mar,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 61,
	pages        = {040301},
	doi          = {10.1103/PhysRevA.61.040301},
	issue        = 4,
	numpages     = 4
}
@article{Swapan2013,
	title        = {{Negative eigenvalues of partial transposition of arbitrary bipartite states}},
	author       = {Rana, Swapan},
	year         = 2013,
	month        = may,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 87,
	pages        = {054301},
	doi          = {10.1103/PhysRevA.87.054301},
	issue        = 5,
	numpages     = 4
}
@article{Yu2012,
	title        = {{All Entangled Pure States Violate a Single Bell's Inequality}},
	author       = {Yu, Sixia and Chen, Qing and Zhang, Chengjie and Lai, C. H. and Oh, C. H.},
	year         = 2012,
	month        = sep,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 109,
	pages        = 120402,
	doi          = {10.1103/PhysRevLett.109.120402},
	issue        = 12,
	numpages     = 5
}
@article{GisinsTheorem,
	title        = {{Bell's inequality holds for all non-product states}},
	author       = {N. Gisin},
	year         = 1991,
	journal      = {Phys. Lett. A},
	volume       = 154,
	number       = 5,
	pages        = {201--202},
	doi          = {10.1016/0375-9601(91)90805-I},
	issn         = {0375-9601},
	url          = {http://www.sciencedirect.com/science/article/pii/037596019190805I}
}
@article{Kunkri2005,
	title        = {{Nonlocality without inequality for spin-$s$ systems}},
	author       = {Kunkri, Samir and Choudhary, Sujit K.},
	year         = 2005,
	month        = aug,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 72,
	pages        = {022348},
	doi          = {10.1103/PhysRevA.72.022348},
	issue        = 2,
	numpages     = 3
}
@article{Kunkri2006,
	title        = {{Nonlocality without inequality for almost all two-qubit entangled states based on Cabello's nonlocality argument}},
	author       = {Kunkri, Samir and Choudhary, Sujit K. and Ahanj, Ali and Joag, Pramod},
	year         = 2006,
	month        = feb,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 73,
	pages        = {022346},
	doi          = {10.1103/PhysRevA.73.022346},
	issue        = 2,
	numpages     = 6
}
@article{Hardy1992,
	title        = {{Quantum mechanics, local realistic theories, and Lorentz-invariant realistic theories}},
	author       = {Hardy, Lucien},
	year         = 1992,
	month        = may,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 68,
	pages        = {2981--2984},
	doi          = {10.1103/PhysRevLett.68.2981},
	issue        = 20,
	numpages     = {0}
}
@article{Cabello2002,
	title        = {{Bell's theorem with and without inequalities for the three-qubit Greenberger-Horne-Zeilinger and W states}},
	author       = {Cabello, Ad\'an},
	year         = 2002,
	month        = feb,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 65,
	pages        = {032108},
	doi          = {10.1103/PhysRevA.65.032108},
	issue        = 3,
	numpages     = 4
}
@article{Liang2005,
	title        = {{Nonlocality without inequalities for two-qubit mixed states based on Cabello's nonlocality}},
	author       = {Lin-mei Liang and Cheng-zu Li},
	year         = 2005,
	journal      = {Phys. Lett. A},
	volume       = 335,
	number       = 5,
	pages        = {371--373},
	doi          = {10.1016/j.physleta.2004.12.046},
	issn         = {0375-9601},
	url          = {http://www.sciencedirect.com/science/article/pii/S0375960104017591}
}
@article{Buml2015,
	title        = {{Limitations on quantum key repeaters}},
	author       = {Stefan B\"{a}uml and Matthias Christandl and Karol Horodecki and Andreas Winter},
	year         = 2015,
	month        = apr,
	journal      = {Nat. Comm.},
	publisher    = {Springer Science and Business Media {LLC}},
	volume       = 6,
	number       = 1,
	doi          = {10.1038/ncomms7908}
}
@article{Cereceda2004,
	title        = {{Hardy's nonlocality for generalized n-particle GHZ states}},
	author       = {JosÃ© L Cereceda},
	year         = 2004,
	journal      = {Phys. Lett. A},
	volume       = 327,
	number       = 5,
	pages        = {433--437},
	doi          = {10.1016/j.physleta.2004.06.004},
	issn         = {0375-9601},
	url          = {http://www.sciencedirect.com/science/article/pii/S0375960104007777}
}
@article{Horodecki2015PPT,
	title        = {{Bounds on quantum nonlocality via partial transposition}},
	author       = {Horodecki, Karol and Murta, Gl\'aucia},
	year         = 2015,
	month        = jul,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 92,
	pages        = {010301},
	doi          = {10.1103/PhysRevA.92.010301},
	issue        = 1,
	numpages     = 5
}
@article{RandomnessViaHardy2015,
	title        = {{Device- and semi--device-independent random numbers based on noninequality paradox}},
	author       = {Li, Hong-Wei and Paw\l{}owski, Marcin and Rahaman, Ramij and Guo, Guang-Can and Han, Zheng-Fu},
	year         = 2015,
	month        = aug,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 92,
	pages        = {022327},
	doi          = {10.1103/PhysRevA.92.022327},
	issue        = 2,
	numpages     = 6
}
@article{RandomnessViaHardy2018,
	title        = {{Generic randomness amplification schemes using Hardy paradoxes}},
	author       = {{Ramanathan}, Ravishankar and {Horodecki}, Micha{\l} and {Pironio}, Stefano and {Horodecki}, Karol and {Horodecki}, Pawe{\l}},
	year         = 2018,
	month        = oct,
	journal      = {arXiv:1810.11648},
	url          = {https://arxiv.org/abs/1810.11648},
	eid.hide     = {arXiv:1810.11648},
	pages.hide   = {arXiv:1810.11648},
	archiveprefix = {arXiv},
	eprint.hide  = {1810.11648},
	primaryclass = {quant-ph}
}
@article{Liu2012Local,
	title        = {{Local Unitary Classification of Arbitrary Dimensional Multipartite Pure States}},
	author       = {Liu, Bin and Li, Jun-Li and Li, Xikun and Qiao, Cong-Feng},
	year         = 2012,
	month        = jan,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 108,
	pages        = {050501},
	doi          = {10.1103/PhysRevLett.108.050501},
	issue        = 5,
	numpages     = 4
}
@article{Li2013Classification,
	title        = {{Classification of arbitrary multipartite entangled states under local unitary equivalence}},
	author       = {Li, Jun-Li and Qiao, Cong-Feng},
	year         = 2013,
	month        = jan,
	journal      = {Jo. Phys. A},
	publisher    = {{IOP} Publishing},
	volume       = 46,
	number       = 7,
	pages        = {075301},
	doi          = {10.1088/1751-8113/46/7/075301}
}
@article{Kraus2010Local,
	title        = {{Local unitary equivalence and entanglement of multipartite pure states}},
	author       = {Kraus, B.},
	year         = 2010,
	month        = sep,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 82,
	pages        = {032121},
	doi          = {10.1103/PhysRevA.82.032121},
	issue        = 3,
	numpages     = 14
}
@article{walter2013entanglement,
	title        = {{Entanglement Polytopes: Multiparticle Entanglement from Single-Particle Information}},
	author       = {Walter, Michael and Doran, Brent and Gross, David and Christandl, Matthias},
	year         = 2013,
	journal      = {Science},
	publisher    = {American Association for the Advancement of Science},
	volume       = 340,
	number       = 6137,
	pages        = {1205--1208},
	doi          = {10.1126/science.1232957}
}
@article{Mermin1990,
	title        = {{Quantum mysteries revisited}},
	author       = {N. David Mermin},
	year         = 1990,
	month        = aug,
	journal      = {Amer. J. Phys.},
	publisher    = {American Association of Physics Teachers ({AAPT})},
	volume       = 58,
	number       = 8,
	pages        = {731--734},
	doi          = {10.1119/1.16503}
}
@article{Brassard2005,
	title        = {{Recasting Mermin's Multi-player Game into the Framework of Pseudo-telepathy}},
	author       = {Brassard, Gilles and Broadbent, Anne and Tapp, Alain},
	year         = 2005,
	month        = nov,
	journal      = {Quantum Info. Comput.},
	volume       = 5,
	number       = 7,
	pages        = {538--550},
	issn         = {1533-7146},
	url          = {https://arxiv.org/abs/quant-ph/0408052},
	issue_date   = {November 2005},
	numpages     = 13
}
@article{Svetlichny,
	title        = {{Distinguishing three-body from two-body nonseparability by a Bell-type inequality}},
	author       = {Svetlichny, George},
	year         = 1987,
	month        = may,
	journal      = {Phys. Rev. D},
	publisher    = {American Physical Society},
	volume       = 35,
	pages        = {3066--3069},
	doi          = {10.1103/PhysRevD.35.3066},
	issue        = 10,
	numpages     = {0}
}
@article{kProducibleEntanglement,
	title        = {{Multipartite entanglement in spin chains}},
	author       = {G\"uhne, Otfried  and T\'oth, G\'eza  and Briegel, Hans J},
	year         = 2005,
	journal      = {New J. Phys.},
	volume       = 7,
	number       = 1,
	pages        = 229,
	url          = {http://stacks.iop.org/1367-2630/7/i=1/a=229},
	doi.hide     = {10.1088/1367-2630/7/1/229}
}
@article{EntanglementManyBody,
	title        = {{Entanglement in many-body systems}},
	author       = {Amico, Luigi and Fazio, Rosario and Osterloh, Andreas and Vedral, Vlatko},
	year         = 2008,
	month        = may,
	journal      = {Rev. Mod. Phys.},
	publisher    = {American Physical Society},
	volume       = 80,
	pages        = {517--576},
	doi          = {10.1103/RevModPhys.80.517},
	issue        = 2,
	numpages     = {0}
}
@article{Broadbent2006,
	title        = {{On the power of non-local boxes}},
	author       = {Anne Broadbent and Andr{\'{e}} Allan M{\'{e}}thot},
	year         = 2006,
	journal      = {Theo. Comp. Sci.},
	volume       = 358,
	number       = 1,
	pages        = {3--14},
	doi          = {10.1016/j.tcs.2005.08.035},
	issn         = {0304-3975},
	url          = {http://www.sciencedirect.com/science/article/pii/S0304397505005864}
}
@article{Palazuelos2016,
	title        = {{Survey on nonlocal games and operator space theory}},
	author       = {Carlos Palazuelos and Thomas Vidick},
	year         = 2016,
	month        = jan,
	journal      = {J. Math. Phys.},
	publisher    = {{AIP} Publishing},
	volume       = 57,
	number       = 1,
	pages        = {015220},
	doi          = {10.1063/1.4938052}
}
@article{Johnston2016,
	title        = {{Extended non-local games and monogamy-of-entanglement games}},
	author       = {Nathaniel Johnston and Rajat Mittal and Vincent Russo and John Watrous},
	year         = 2016,
	month        = may,
	journal      = {Proc. Roy. Soc. A},
	publisher    = {The Royal Society},
	volume       = 472,
	number       = 2189,
	pages        = 20160003,
	doi          = {10.1098/rspa.2016.0003}
}
@book{shafarevich2012linear,
	title        = {{Linear algebra and geometry}},
	author       = {Shafarevich, I. R.},
	year         = 2013,
	publisher    = {Springer},
	isbn         = 3642309933,
	url          = {https://books.google.com/books/about/Linear_Algebra_and_Geometry.html?id=6Pp2-DTOKWIC&redir_esc=y},
	address.hide = {Berlin New York}
}
@article{navascues2020genuine,
	title        = {{Genuine Network Multipartite Entanglement}},
	author       = {Navascu\'es, Miguel and Wolfe, Elie and Rosset, Denis and Pozas-Kerstjens, Alejandro},
	year         = 2020,
	month        = dec,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 125,
	pages        = 240505,
	doi          = {10.1103/PhysRevLett.125.240505},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.125.240505},
	issue        = 24,
	numpages     = 6
}
@article{wolfe2019quantum,
	title        = {{Quantum Inflation: A General Approach to Quantum Causal Compatibility}},
	author       = {Elie Wolfe and Alejandro Pozas-Kerstjens and Matan Grinberg and Denis Rosset and Antonio Ac\'in and Miguel Navascues},
	year         = 2019,
	journal      = {arXiv:1909.10519},
	url          = {https://arxiv.org/abs/1909.10519}
}
@article{bowles2018device,
	title        = {{Device-independent entanglement certification of all entangled states}},
	author       = {Bowles, Joseph and {\v{S}}upi{\'c}, Ivan and Cavalcanti, Daniel and Ac{\'\i}n, Antonio},
	year         = 2018,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 121,
	number       = 18,
	pages        = 180503,
	url          = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.121.180503}
}
@article{contreras2020any,
	title        = {{Genuine multipartite nonlocality is intrinsic to quantum networks}},
	author       = {Contreras-Tejada, Patricia and Palazuelos, Carlos and de Vicente, Julio I},
	year         = 2020,
	journal      = {arXiv:2004.01722},
	url          = {https://arxiv.org/abs/2004.01722}
}
@article{Hiraxh2020PPT,
	title        = {{The Schmidt number of a quantum state cannot always be device-independently certified }},
	author       = {Flavien Hirsch and Marcus Huber},
	year         = 2020,
	journal      = {arXiv:2003.14189},
	url          = {https://arxiv.org/abs/2003.14189},
	eprint.hide  = {2003.14189},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{biamonte2013tensor,
	title        = {{Tensor network methods for invariant theory}},
	author       = {Biamonte, Jacob and Bergholm, Ville and Lanzagorta, Marco},
	year         = 2013,
	journal      = {J. Phys. A},
	publisher    = {IOP Publishing},
	volume       = 46,
	number       = 47,
	pages        = 475301,
	doi          = {10.1088/1751-8113/46/47/475301}
}
@article{klyachko2006quantum,
	title        = {{Quantum marginal problem and N-representability}},
	author       = {Klyachko, Alexander A},
	year         = 2006,
	journal      = {J. Phys.: Conference Series},
	volume       = 36,
	number       = 1,
	pages        = 72,
	doi          = {10.1088/1742-6596/36/1/014},
	organization = {IOP Publishing}
}
@article{Stinespring1955,
	title        = {{Positive functions on \(\textitC^\ast\)-algebras}},
	author       = {W. Forrest Stinespring},
	year         = 1955,
	month        = feb,
	journal      = {Proc. Am. Math. Soc.},
	publisher    = {American Mathematical Society ({AMS})},
	volume       = 6,
	number       = 2,
	pages        = {211--211},
	doi          = {10.1090/s0002-9939-1955-0069403-4},
	url          = {https://doi.org/10.1090/s0002-9939-1955-0069403-4}
}
@book{Paulsen2003Apr,
	title        = {{Completely Bounded Maps and Operator Algebras}},
	author       = {Paulsen, Vern},
	year         = 2003,
	month        = apr,
	publisher    = {Cambridge University Press},
	isbn         = {978-052181669-4},
	url          = {https://www.cambridge.org/ca/academic/subjects/mathematics/abstract-analysis/completely-bounded-maps-and-operator-algebras?format=HB&isbn=9780521816694}
}
@article{AnomalyExtra2008Brunner,
	title        = {{Simulation of partial entanglement with nonsignaling resources}},
	author       = {Brunner, Nicolas and Gisin, Nicolas and Popescu, Sandu and Scarani, Valerio},
	year         = 2008,
	month        = nov,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 78,
	pages        = {052111},
	doi          = {10.1103/PhysRevA.78.052111},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.78.052111},
	issue        = 5,
	numpages     = 5
}
@article{AnomalyExtra2011Junge,
	title        = {{Large Violation of Bell Inequalities with Low Entanglement}},
	author       = {M. Junge and C. Palazuelos},
	year         = 2011,
	month        = jul,
	journal      = {Comm. Math. Phys.},
	publisher    = {Springer Science and Business Media {LLC}},
	volume       = 306,
	number       = 3,
	pages        = {695--746},
	doi          = {10.1007/s00220-011-1296-8},
	url          = {https://doi.org/10.1007/s00220-011-1296-8}
}
@article{AnomalyExtra2014Tan,
	title        = {{The Essence of More Nonlocality with Less Entanglement in Bell Tests}},
	author       = {Yong-Gang Tan and Qiang Liu and Yao-Hua Hu and Hua Lu},
	year         = 2014,
	month        = jan,
	journal      = {Comm. Theo. Phys.},
	publisher    = {{IOP} Publishing},
	volume       = 61,
	number       = 1,
	pages        = {40--44},
	doi          = {10.1088/0253-6102/61/1/07},
	url          = {https://doi.org/10.1088%2F0253-6102%2F61%2F1%2F07}
}
@article{AnomalyExtra2015Augusiak,
	title        = {{Entanglement and Nonlocality are Inequivalent for Any Number of Parties}},
	author       = {Augusiak, R. and Demianowicz, M. and Tura, J. and Ac\'{\i}n, A.},
	year         = 2015,
	month        = jul,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 115,
	pages        = {030404},
	doi          = {10.1103/PhysRevLett.115.030404},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.115.030404},
	issue        = 3,
	numpages     = 5
}
@article{AnomalyExtra2015Fonseca,
	title        = {{Measure of nonlocality which is maximal for maximally entangled qutrits}},
	author       = {Fonseca, E. A. and Parisio, Fernando},
	year         = 2015,
	month        = sep,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 92,
	pages        = {030101},
	doi          = {10.1103/PhysRevA.92.030101},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.92.030101},
	issue        = 3,
	numpages     = 5
}
@article{AnomalyExtra2016Bowles,
	title        = {{Genuinely Multipartite Entangled Quantum States with Fully Local Hidden Variable Models and Hidden Multipartite Nonlocality}},
	author       = {Bowles, Joseph and Francfort, J\'er\'emie and Fillettaz, Mathieu and Hirsch, Flavien and Brunner, Nicolas},
	year         = 2016,
	month        = mar,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physal Society},
	volume       = 116,
	pages        = 130401,
	doi          = {10.1103/PhysRevLett.116.130401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.116.130401},
	issue        = 13,
	numpages     = 5
}
@phdthesis{AnomalyExtra2018Curchod,
	title        = {{Nonlocal resources for quantum information tasks}},
	author       = {Curchod, Florian John},
	year         = 2018,
	url          = {http://hdl.handle.net/2117/123515},
	school       = {Universitat PolitÃšcnica de Catalunya. Institut de CiÃšncies FotÃ²niques}
}
@article{AnomalyExtra2018Chitambar,
	title        = {{More nonlocality with less entanglement in Clauser-Horne-Shimony-Holt experiments using inefficient detectors}},
	author       = {Dilley, Daniel and Chitambar, Eric},
	year         = 2018,
	month        = jun,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 97,
	pages        = {062313},
	doi          = {10.1103/PhysRevA.97.062313},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.97.062313},
	issue        = 6,
	numpages     = 5
}
@article{AnomalyExtra2018Lipinska,
	title        = {{Towards an equivalence between maximal entanglement and maximal quantum nonlocality}},
	author       = {Victoria Lipinska and Florian J. Curchod and Alejandro M{\'{a}}ttar and Antonio Ac{\'{\i}}n},
	year         = 2018,
	month        = jun,
	journal      = {New J. Phys.},
	publisher    = {{IOP} Publishing},
	volume       = 20,
	number       = 6,
	pages        = {063043},
	doi          = {10.1088/1367-2630/aaca22},
	url          = {https://doi.org/10.1088%2F1367-2630%2Faaca22}
}
@article{AnomalyExtra2018Barasinski,
	title        = {{Volume of violation of Bell-type inequalities as a measure of nonlocality}},
	author       = {Barasi\ifmmode \acute{n}\else \'{n}\fi{}ski, Artur and Nowotarski, Mateusz},
	year         = 2018,
	month        = aug,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 98,
	pages        = {022132},
	doi          = {10.1103/PhysRevA.98.022132},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.98.022132},
	issue        = 2,
	numpages     = 9
}
@incollection{Scarani2019,
	title        = {{Device-Independent Self-Testing}},
	author       = {Valerio Scarani},
	year         = 2019,
	month        = aug,
	booktitle    = {{Bell Nonlocality}},
	publisher    = {Oxford University Press},
	pages        = {86--97},
	doi          = {10.1093/oso/9780198788416.003.0007},
	url          = {https://doi.org/10.1093/oso/9780198788416.003.0007},
	chapter      = 7
}
@article{MultipartiteProblem2020Luo,
	title        = {{New Genuine Multipartite Entanglement}},
	author       = {Ming-Xing Luo},
	year         = 2020,
	journal      = {arXiv:2003.07153},
	url          = {https://arxiv.org/abs/2003.07153}
}
@article{Hayden2003,
	title        = {{Communication cost of entanglement transformations}},
	author       = {Hayden, Patrick and Winter, Andreas},
	year         = 2003,
	month        = jan,
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 67,
	pages        = {012326},
	doi          = {10.1103/PhysRevA.67.012326},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.67.012326},
	issue        = 1,
	numpages     = 8
}
@inproceedings{Harrow2010,
	title        = {{Entanglement spread and clean resource inequalities}},
	author       = {Aram~W. Harrow},
	year         = 2010,
	month        = mar,
	booktitle    = {{XVIth} Int. Cong. Math. Phys.},
	doi          = {10.1142/9789814304634_0046},
	url          = {https://doi.org/10.1142/9789814304634_0046}
}
@misc{Gour2020RT,
	title        = {{Quantum Bell Nonlocality is Entanglement}},
	author       = {Kuntal Sengupta and Rana Zibakhsh and Eric Chitambar and Gilad Gour},
	year         = 2020,
	eprint       = {2012.06918},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
%**********ADDED*********************
@article{pal2021experimental,
	title        = {{Experimental localisation of quantum entanglement through monitored classical mediator}},
	author       = {Pal, Soham and Batra, Priya and Krisnanda, Tanjung and Paterek, Tomasz and Mahesh, TS},
	year         = 2021,
	journal      = {Quantum},
	publisher    = {Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften},
	volume       = 5,
	pages        = 478
}
@article{d2014fermionic,
	title        = {{Fermionic computation is non-local tomographic and violates monogamy of entanglement}},
	author       = {D'Ariano, Giacomo Mauro and Manessi, Franco and Perinotti, Paolo and Tosini, Alessandro},
	year         = 2014,
	journal      = {EPL (Europhysics Letters)},
	publisher    = {IOP Publishing},
	volume       = 107,
	number       = 2,
	pages        = 20009
}
@book{coecke_kissinger_2017,
	title        = {{Picturing Quantum Processes: A First Course in Quantum Theory and Diagrammatic Reasoning}},
	author       = {Coecke, Bob and Kissinger, Aleks},
	year         = 2017,
	publisher    = {Cambridge University Press},
	doi          = {10.1017/9781316219317},
	place        = {Cambridge}
}
@article{coecke2016terminality,
	title        = {{Terminality implies no-signalling... and much more than that}},
	author       = {Coecke, Bob},
	year         = 2016,
	journal      = {New Generation Computing},
	publisher    = {Springer},
	volume       = 34,
	number       = {1-2},
	pages        = {69--85}
}
@article{d2020classical,
	title        = {{Classical theories with entanglement}},
	author       = {D'Ariano, Giacomo Mauro and Erba, Marco and Perinotti, Paolo},
	year         = 2020,
	journal      = {Physical Review A},
	publisher    = {APS},
	volume       = 101,
	number       = 4,
	pages        = {042118}
}
@article{cavalcanti2021witworld,
	title        = {{Witworld: A generalised probabilistic theory featuring post-quantum steering}},
	author       = {Cavalcanti, Paulo J and Selby, John H and Sikora, Jamie and Galley, Thomas D and Sainz, Ana Bel{\'e}n},
	year         = 2021,
	journal      = {arXiv preprint arXiv:2102.06581}
}
@article{coecke2009group,
	title        = {{Phase groups and the origin of non-locality for qubits}},
	author       = {Coecke, Bob and Edwards, Bill and Spekkens, Robert W},
	year         = 2011,
	journal      = {Electronic Notes in Theoretical Computer Science},
	publisher    = {Elsevier},
	volume       = 270,
	number       = 2,
	pages        = {15--36}
}
@article{KaroubiEnvelope,
	title        = {{Cauchy completion in category theory}},
	author       = {Borceux, Francis and Dejean, Dominique},
	year         = 1986,
	journal      = {Cahiers de Topologie et G\'eom\'etrie Diff\'erentielle Cat\'egoriques},
	publisher    = {Dunod \'editeur, publi\'e avec le concours du CNRS},
	volume       = 27,
	number       = 2,
	pages        = {133--146},
	url          = {www.numdam.org/item/CTGDC_1986__27_2_133_0/},
	zbl          = {0595.18001},
	mrnumber     = 850528,
	language     = {en}
}
@article{spekkens2005contextuality,
	title        = {{Contextuality for preparations, transformations, and unsharp measurements}},
	author       = {Spekkens, Robert W},
	year         = 2005,
	journal      = {Physical Review A},
	publisher    = {APS},
	volume       = 71,
	number       = 5,
	pages        = {052108}
}
@book{holevo2011probabilistic,
	title        = {{Probabilistic and statistical aspects of quantum theory}},
	author       = {Holevo, Alexander S},
	year         = 2011,
	publisher    = {Springer Science \& Business Media},
	volume       = 1
}
@article{janotta2014generalized,
	title        = {{Generalized probability theories: what determines the structure of quantum theory?}},
	author       = {Janotta, Peter and Hinrichsen, Haye},
	year         = 2014,
	journal      = {Journal of Physics A: Mathematical and Theoretical},
	publisher    = {IOP Publishing},
	volume       = 47,
	number       = 32,
	pages        = 323001
}
@article{spekkens2019ontological,
	title        = {{The ontological identity of empirical indiscernibles: Leibniz's methodological principle and its significance in the work of Einstein}},
	author       = {Spekkens, Robert W},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1909.04628}
}
@article{dakic2009quantum,
	title        = {{Quantum theory and beyond: Is entanglement special?}},
	author       = {Dakic, Borivoje and Brukner, Caslav},
	year         = 2009,
	journal      = {arXiv preprint arXiv:0911.0695}
}
@article{mueller2020probabilistic,
	title        = {Probabilistic theories and reconstructions of quantum theory},
	author       = {Markus M\"{u}ller},
	year         = 2021,
	month        = mar,
	journal      = {{SciPost} Physics Lecture Notes},
	publisher    = {Stichting {SciPost}},
	doi          = {10.21468/scipostphyslectnotes.28},
	url          = {https://doi.org/10.21468/scipostphyslectnotes.28}
}
@article{mauro2020classicality,
	title        = {{Classicality without local discriminability: Decoupling entanglement and complementarity}},
	author       = {D'Ariano, Giacomo Mauro and Erba, Marco and Perinotti, Paolo},
	year         = 2020,
	journal      = {Physical Review A},
	publisher    = {APS},
	volume       = 102,
	number       = 5,
	pages        = {052216}
}
@article{heinosaari2019no,
	title        = {No-free-information principle in general probabilistic theories},
	author       = {Teiko Heinosaari and Leevi Lepp{\"a}j{\"a}rvi and Martin Pl{\'{a} }vala},
	year         = 2019,
	month        = {jul},
	journal      = {Quantum},
	publisher    = {Verein zur Forderung des Open Access Publizierens in den Quantenwissenschaften},
	volume       = 3,
	pages        = 157,
	doi          = {10.22331/q-2019-07-08-157},
	url          = {https://doi.org/10.22331%2Fq-2019-07-08-157}
}
@article{richens2017entanglement,
	title        = {{Entanglement is necessary for emergent classicality in all physical theories}},
	author       = {Richens, Jonathan G and Selby, John H and Al-Safi, Sabri W},
	year         = 2017,
	journal      = {Physical Review Letters},
	publisher    = {APS},
	volume       = 119,
	number       = 8,
	pages        = {080503}
}
@article{d2019information,
	title        = {{Information and disturbance in operational probabilistic theories}},
	author       = {D'Ariano, Giacomo Mauro and Perinotti, Paolo and Tosini, Alessandro},
	year         = 2019,
	journal      = {arXiv preprint arXiv:1907.07043}
}
@article{coecke2017two,
	title        = {{Two roads to classicality}},
	author       = {Coecke, Bob and Selby, John and Tull, Sean},
	year         = 2017,
	journal      = {arXiv preprint arXiv:1701.07400}
}
@article{hardy2001quantum,
	title        = {{Quantum theory from five reasonable axioms}},
	author       = {Hardy, Lucien},
	year         = 2001,
	journal      = {arXiv preprint quant-ph/0101012}
}
@article{barrett2007information,
	title        = {{Information processing in generalized probabilistic theories}},
	author       = {Barrett, Jonathan},
	year         = 2007,
	journal      = {Physical Review A},
	publisher    = {APS},
	volume       = 75,
	number       = 3,
	pages        = {032304}
}
@article{cavalcanti2021,
	title        = {{Extended boxworld: a generalised probabilistic theory for type independent common cause resources}},
	author       = {Selby, John H. and Cavalcanti, Paulo and Sainz, Ana Bel\'en},
	year         = {forthcoming}
}
@article{hossenfelder2010experimental,
	title        = {{Experimental search for quantum gravity}},
	author       = {Hossenfelder, Sabine},
	year         = 2010,
	journal      = {Classical and quantum gravity: Theory, Analysis and Applications},
	publisher    = {Springer},
	volume       = 5
}
@article{penrose2014gravitization,
	title        = {{On the gravitization of quantum mechanics 1: Quantum state reduction}},
	author       = {Penrose, Roger},
	year         = 2014,
	journal      = {Foundations of Physics},
	publisher    = {Springer},
	volume       = 44,
	number       = 5,
	pages        = {557--575}
}
@article{diosi1987universal,
	title        = {{A universal master equation for the gravitational violation of quantum mechanics}},
	author       = {Diosi, Lajos},
	year         = 1987,
	journal      = {Physics Letters A},
	publisher    = {Elsevier},
	volume       = 120,
	number       = 8,
	pages        = {377--381}
}
@article{bronstein2012republication,
	title        = {{Republication of: Quantum theory of weak gravitational fields}},
	author       = {Bronstein, Matvei},
	year         = 2012,
	journal      = {General Relativity and Gravitation},
	publisher    = {Springer},
	volume       = 44,
	number       = 1,
	pages        = {267--283}
}
@article{pagegeilker,
	title        = {{Indirect Evidence for Quantum Gravity}},
	author       = {Page, Don N. and Geilker, C. D.},
	year         = 1981,
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 47,
	pages        = {979--982},
	doi          = {10.1103/PhysRevLett.47.979},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.47.979},
	issue        = 14,
	numpages     = {0}
}
@article{Eppley1977,
	title        = {{The necessity of quantizing the gravitational field}},
	author       = {Eppley, Kenneth and Hannah, Eric},
	year         = 1977,
	day          = {01},
	journal      = {Foundations of Physics},
	volume       = 7,
	number       = 1,
	pages        = {51--68},
	doi          = {10.1007/BF00715241},
	issn         = {1572-9516},
	url          = {https://doi.org/10.1007/BF00715241}
}
@article{mattinglygravityquantum,
	title        = {{Why Eppley and Hannah's thought experiment fails}},
	author       = {Mattingly, James},
	year         = 2006,
	journal      = {Phys. Rev. D},
	publisher    = {American Physical Society},
	volume       = 73,
	pages        = {064025},
	doi          = {10.1103/PhysRevD.73.064025},
	url          = {https://link.aps.org/doi/10.1103/PhysRevD.73.064025},
	issue        = 6,
	numpages     = 8
}
@article{carlipnecessity,
	title        = {{Is quantum gravity necessary?}},
	author       = {S Carlip},
	year         = 2008,
	journal      = {Class. Quant. Grav.},
	volume       = 25,
	number       = 15,
	pages        = 154010,
	url          = {http://stacks.iop.org/0264-9381/25/i=15/a=154010}
}
@article{Giampaolo:2018yql,
	title        = {{Entanglement, holonomic constraints, and the quantization of fundamental interactions}},
	author       = {Giampaolo, Salvatore M and Macr{\`\i}, Tommaso},
	year         = 2018,
	journal      = {arXiv preprint arXiv:1806.08383}
}
@book{cecile2011role,
	title        = {{The role of gravitation in physics: Report from the 1957 Chapel Hill Conference}},
	author       = {C{\'e}cile M. DeWitt and Dean Rickles},
	year         = 2011,
	publisher    = {epubli},
	volume       = 5
}
@article{zeh2011feynman,
	title        = {{Feynman's interpretation of quantum theory}},
	author       = {Zeh, H Dieter},
	year         = 2011,
	journal      = {The European Physical Journal H},
	publisher    = {Springer},
	volume       = 36,
	number       = 1,
	pages        = {63--74}
}
@article{anastopoulos2015probing,
	title        = {{Probing a gravitational cat state}},
	author       = {Anastopoulos, Charis and Hu, Bei-Lok},
	year         = 2015,
	journal      = {Classical and Quantum Gravity},
	publisher    = {IOP Publishing},
	volume       = 32,
	number       = 16,
	pages        = 165022
}
@article{anastopoulos2020quantum,
	title        = {{Quantum superposition of two gravitational cat states}},
	author       = {Anastopoulos, Charis and Hu, Bei-Lok},
	year         = 2020,
	journal      = {Classical and Quantum Gravity},
	publisher    = {IOP Publishing},
	volume       = 37,
	number       = 23,
	pages        = 235012
}
@article{carlesso2017cavendish,
	title        = {{When Cavendish meets Feynman: A quantum torsion balance for testing the quantumness of gravity}},
	author       = {Carlesso, Matteo and Paternostro, Mauro and Ulbricht, Hendrik and Bassi, Angelo},
	year         = 2017,
	journal      = {arXiv preprint arXiv:1710.08695}
}
@article{bahrami2015gravity,
	title        = {{Is gravity quantum?}},
	author       = {Bahrami, M and Bassi, A and McMillen, S and Paternostro, M and Ulbricht, H},
	year         = 2015,
	journal      = {arXiv preprint arXiv:1507.05733}
}
@article{lindner2005testing,
	title        = {{Testing quantum superpositions of the gravitational field with Bose-Einstein condensates}},
	author       = {Lindner, Netanel H and Peres, Asher},
	year         = 2005,
	journal      = {Physical Review A},
	publisher    = {APS},
	volume       = 71,
	number       = 2,
	pages        = {024101}
}
@article{ford1982gravitational,
	title        = {{Gravitational radiation by quantum systems}},
	author       = {Ford, LH},
	year         = 1982,
	journal      = {Annals of Physics},
	publisher    = {Elsevier},
	volume       = 144,
	number       = 2,
	pages        = {238--248}
}
@article{kafri2013noise,
	title        = {{A noise inequality for classical forces}},
	author       = {Kafri, Dvir and Taylor, JM},
	year         = 2013,
	journal      = {arXiv preprint arXiv:1311.4558}
}
@article{kafri2014classical,
	title        = {{A classical channel model for gravitational decoherence}},
	author       = {Kafri, D and Taylor, JM and Milburn, GJ},
	year         = 2014,
	journal      = {New Journal of Physics},
	publisher    = {IOP Publishing},
	volume       = 16,
	number       = 6,
	pages        = {065020}
}
@article{altamirano2018gravity,
	title        = {{Gravity is not a pairwise local classical channel}},
	author       = {Altamirano, Natacha and Corona-Ugalde, Paulina and Mann, Robert B and Zych, Magdalena},
	year         = 2018,
	journal      = {Classical and Quantum Gravity},
	publisher    = {IOP Publishing},
	volume       = 35,
	number       = 14,
	pages        = 145005
}
@article{belenchia2018quantum,
	title        = {{Quantum superposition of massive objects and the quantization of gravity}},
	author       = {Belenchia, Alessio and Wald, Robert M and Giacomini, Flaminia and Castro-Ruiz, Esteban and Brukner, {\v{C}}aslav and Aspelmeyer, Markus},
	year         = 2018,
	journal      = {Physical Review D},
	publisher    = {APS},
	volume       = 98,
	number       = 12,
	pages        = 126009
}
@article{belenchia2019information,
	title        = {{Information content of the gravitational field of a quantum superposition}},
	author       = {Belenchia, Alessio and Wald, Robert M and Giacomini, Flaminia and Castro-Ruiz, Esteban and Brukner, {\v{C}}aslav and Aspelmeyer, Markus},
	year         = 2019,
	journal      = {International Journal of Modern Physics D},
	publisher    = {World Scientific},
	volume       = 28,
	number       = 14,
	pages        = 1943001
}
@article{christodoulou2019possibility,
	title        = {{On the possibility of laboratory evidence for quantum superposition of geometries}},
	author       = {Christodoulou, Marios and Rovelli, Carlo},
	year         = 2019,
	journal      = {Physics Letters B},
	publisher    = {Elsevier},
	volume       = 792,
	pages        = {64--68}
}
@article{howl2020testing,
	title        = {{Testing Quantum Gravity with a Single Quantum System}},
	author       = {Howl, Richard and Vedral, Vlatko and Christodoulou, Marios and Rovelli, Carlo and Naik, Devang and Iyer, Aditya},
	year         = 2020,
	journal      = {arXiv preprint arXiv:2004.01189}
}
@article{krisnanda2020observable,
	title        = {{Observable quantum entanglement due to gravity}},
	author       = {Krisnanda, Tanjung and Tham, Guo Yao and Paternostro, Mauro and Paterek, Tomasz},
	year         = 2020,
	journal      = {npj Quantum Information},
	publisher    = {Nature Publishing Group},
	volume       = 6,
	number       = 1,
	pages        = {1--6}
}
@article{bose2017spin,
	title        = {{Spin entanglement witness for quantum gravity}},
	author       = {Bose, Sougato and Mazumdar, Anupam and Morley, Gavin W and Ulbricht, Hendrik and Toro{\v{s}}, Marko and Paternostro, Mauro and Geraci, Andrew A and Barker, Peter F and Kim, MS and Milburn, Gerard},
	year         = 2017,
	journal      = {Physical Review Letters},
	publisher    = {APS},
	volume       = 119,
	number       = 24,
	pages        = 240401
}
@article{marletto2017gravitationally,
	title        = {{Gravitationally induced entanglement between two massive particles is sufficient evidence of quantum effects in gravity}},
	author       = {Marletto, Chiara and Vedral, Vlatko},
	year         = 2017,
	journal      = {Physical Review Letters},
	publisher    = {APS},
	volume       = 119,
	number       = 24,
	pages        = 240402
}
@article{hall2018two,
	title        = {{On two recent proposals for witnessing nonclassical gravity}},
	author       = {Hall, Michael JW and Reginatto, Marcel},
	year         = 2018,
	journal      = {Journal of Physics A: Mathematical and Theoretical},
	publisher    = {IOP Publishing},
	volume       = 51,
	number       = 8,
	pages        = {085303}
}
@article{anastopoulos2018comment,
	title        = {{Comment on “a spin entanglement witness for quantum gravity” and on “gravitationally induced entanglement between two massive particles is sufficient evidence of quantum effects in gravity”}},
	author       = {Anastopoulos, C and Hu, Bei-Lok},
	year         = 2018,
	journal      = {arXiv preprint arXiv:1804.11315}
}
@article{mari2016experiments,
	title        = {{Experiments testing macroscopic quantum superpositions must be slow}},
	author       = {Mari, Andrea and De Palma, Giacomo and Giovannetti, Vittorio},
	year         = 2016,
	journal      = {Scientific reports},
	publisher    = {Nature Publishing Group},
	volume       = 6,
	pages        = 22777
}
@article{baym2009two,
	title        = {{Two-slit diffraction with highly charged particles: Niels Bohr's consistency argument that the electromagnetic field must be quantized}},
	author       = {Baym, Gordon and Ozawa, Tomoki},
	year         = 2009,
	journal      = {Proceedings of the National Academy of Sciences},
	publisher    = {National Acad Sciences},
	volume       = 106,
	number       = 9,
	pages        = {3035--3040}
}
@article{bennett1993teleporting,
	title        = {{Teleporting an unknown quantum state via dual classical and Einstein-Podolsky-Rosen channels}},
	author       = {Bennett, Charles H and Brassard, Gilles and Cr{\'e}peau, Claude and Jozsa, Richard and Peres, Asher and Wootters, William K},
	year         = 1993,
	journal      = {Physical Review Letters},
	publisher    = {APS},
	volume       = 70,
	number       = 13,
	pages        = 1895
}
@article{marletto2020witnessing,
	title        = {{Witnessing non-classicality beyond quantum theory}},
	author       = {Marletto, Chiara and Vedral, Vlatko},
	year         = 2020,
	journal      = {arXiv preprint arXiv:2003.07974}
}
@article{marletto2017we,
	title        = {{Why we need to quantise everything, including gravity}},
	author       = {Marletto, Chiara and Vedral, Vlatko},
	year         = 2017,
	journal      = {npj Quantum Information},
	publisher    = {Nature Publishing Group},
	volume       = 3,
	number       = 1,
	pages        = {1--5}
}
@article{deutsch2013constructor,
	title        = {{Constructor theory}},
	author       = {Deutsch, David},
	year         = 2013,
	journal      = {Synthese},
	publisher    = {Springer},
	volume       = 190,
	number       = 18,
	pages        = {4331--4359}
}
@incollection{unruh2000false,
	title        = {{False loss of coherence}},
	author       = {Unruh, William G},
	year         = 2000,
	booktitle    = {Relativistic quantum measurement and decoherence},
	publisher    = {Springer},
	pages        = {125--140}
}
@article{sikora2018simple,
	title        = {{Simple proof of the impossibility of bit commitment in generalized probabilistic theories using cone programming}},
	author       = {Sikora, Jamie and Selby, John},
	year         = 2018,
	journal      = {Physical Review A},
	publisher    = {APS},
	volume       = 97,
	number       = 4,
	pages        = {042302}
}
@article{selby2018make,
	title        = {How to make unforgeable money in generalised probabilistic theories},
	author       = {John H. Selby and Jamie Sikora},
	year         = 2018,
	month        = {nov},
	journal      = {Quantum},
	publisher    = {Verein zur Forderung des Open Access Publizierens in den Quantenwissenschaften},
	volume       = 2,
	pages        = 103,
	doi          = {10.22331/q-2018-11-02-103},
	url          = {https://doi.org/10.22331%2Fq-2018-11-02-103}
}
@article{sikora2019impossibility,
	title        = {Impossibility of coin flipping in generalized probabilistic theories via discretizations of semi-infinite programs},
	author       = {Sikora, Jamie and Selby, John H.},
	year         = 2020,
	month        = {Oct},
	journal      = {Phys. Rev. Research},
	publisher    = {American Physical Society},
	volume       = 2,
	pages        = {043128},
	doi          = {10.1103/PhysRevResearch.2.043128},
	url          = {https://link.aps.org/doi/10.1103/PhysRevResearch.2.043128},
	issue        = 4,
	numpages     = 7
}
@article{bae2016structure,
	title        = {{Structure of Optimal State Discrimination in Generalized Probabilistic Theories}},
	author       = {Bae, Joonwoo and Kim, Dai-Gyoung and Kwek, Leong-Chuan},
	year         = 2016,
	journal      = {Entropy},
	publisher    = {Multidisciplinary Digital Publishing Institute},
	volume       = 18,
	number       = 2,
	pages        = 39,
	doi          = {10.3390/e18020039},
	bdsk-url-1   = {https://doi.org/10.3390/e18020039}
}
@article{lee2016bounds,
	title        = {Bounds on the power of proofs and advice in general physical theories},
	author       = {Ciar{\'{a} }n M. Lee and Matty J. Hoban},
	year         = 2016,
	month        = {jun},
	journal      = {Proc. Roy. Soc. A},
	publisher    = {The Royal Society},
	volume       = 472,
	number       = 2190,
	pages        = 20160076,
	doi          = {10.1098/rspa.2016.0076},
	url          = {https://doi.org/10.1098%2Frspa.2016.0076}
}
@inproceedings{barnum2008nonclassicality,
	title        = {Nonclassicality without entanglement enables bit commitment},
	author       = {Howard Barnum and Oscar C.O. Dahlsten and Matthew Leifer and Ben Toner},
	year         = 2008,
	month        = {may},
	booktitle    = {2008 {IEEE} Information Theory Workshop},
	publisher    = {{IEEE}},
	doi          = {10.1109/itw.2008.4578692},
	url          = {https://doi.org/10.1109%2Fitw.2008.4578692}
}
@article{lami2018ultimate,
	title        = {Ultimate Data Hiding in Quantum Mechanics and Beyond},
	author       = {Ludovico Lami and Carlos Palazuelos and Andreas Winter},
	year         = 2018,
	month        = {jun},
	journal      = {Communications in Mathematical Physics},
	publisher    = {Springer Science and Business Media {LLC}},
	volume       = 361,
	number       = 2,
	pages        = {661--708},
	doi          = {10.1007/s00220-018-3154-4},
	url          = {https://doi.org/10.1007%2Fs00220-018-3154-4}
}
@article{barrett2005no,
	title        = {No Signaling and Quantum Key Distribution},
	author       = {Jonathan Barrett and Lucien Hardy and Adrian Kent},
	year         = 2005,
	month        = {jun},
	journal      = {Physical Review Letters},
	publisher    = {American Physical Society ({APS})},
	volume       = 95,
	number       = 1,
	doi          = {10.1103/physrevlett.95.010503},
	url          = {https://doi.org/10.1103%2Fphysrevlett.95.010503}
}
@article{barrett2017computational,
	title        = {The computational landscape of general physical theories},
	author       = {Jonathan Barrett and Niel de Beaudrap and Matty J. Hoban and Ciar{\'{a}}n M. Lee},
	year         = 2019,
	month        = {may},
	journal      = {npj Quantum Information},
	publisher    = {Springer Science and Business Media {LLC}},
	volume       = 5,
	number       = 1,
	doi          = {10.1038/s41534-019-0156-9},
	url          = {https://doi.org/10.1038%2Fs41534-019-0156-9}
}
@article{krumm2018quantum,
	title        = {Quantum computation is the unique reversible circuit model for which bits are balls},
	author       = {Marius Krumm and Markus P. M{\"u}ller},
	year         = 2019,
	month        = {jan},
	journal      = {npj Quantum Information},
	publisher    = {Springer Science and Business Media {LLC}},
	volume       = 5,
	number       = 1,
	doi          = {10.1038/s41534-018-0123-x},
	url          = {https://doi.org/10.1038%2Fs41534-018-0123-x}
}
@article{lee2016generalised,
	title        = {Generalised phase kick-back: the structure of computational algorithms from physical principles},
	author       = {Ciar{\'{a} }n M Lee and John H Selby},
	year         = 2016,
	month        = {mar},
	journal      = {New Journal of Physics},
	publisher    = {{IOP} Publishing},
	volume       = 18,
	number       = 3,
	pages        = {033023},
	doi          = {10.1088/1367-2630/18/3/033023},
	url          = {https://doi.org/10.1088%2F1367-2630%2F18%2F3%2F033023}
}
@article{lee2016deriving,
	title        = {Deriving Grover{\textquotesingle}s lower bound from simple physical principles},
	author       = {Ciar{\'{a} }n M Lee and John H Selby},
	year         = 2016,
	month        = {sep},
	journal      = {New Journal of Physics},
	publisher    = {{IOP} Publishing},
	volume       = 18,
	number       = 9,
	pages        = {093047},
	doi          = {10.1088/1367-2630/18/9/093047},
	url          = {https://doi.org/10.1088%2F1367-2630%2F18%2F9%2F093047}
}
@article{JP17,
	title        = {{Conditions on the existence of maximally incompatible two-outcome measurements in general Probabilistic Theory}},
	author       = {Anna Jen\v{c}ov\'{a} and Martin Pl\'{a}vala},
	year         = 2017,
	journal      = {Physical Review A},
	volume       = 96,
	pages        = {022113},
	doi          = {10.1103/PhysRevA.96.022113},
	date-added   = {2017-11-30 20:08:31 +0000},
	date-modified = {2017-11-30 20:09:47 +0000},
	bdsk-url-1   = {https://doi.org/10.1103/PhysRevA.96.022113}
}
@article{czekaj2018bell,
	title        = {{Bell measurement ruling out supraquantum correlations}},
	author       = {Czekaj, \L. and Horodecki, M. and Tylec, T.},
	year         = 2018,
	month        = {Sep},
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 98,
	pages        = {032117},
	doi          = {10.1103/PhysRevA.98.032117},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.98.032117},
	issue        = 3,
	numpages     = 7
}
@article{schmid2019characterization,
	title        = {Characterization of Noncontextuality in the Framework of Generalized Probabilistic Theories},
	author       = {David Schmid and John H. Selby and Elie Wolfe and Ravi Kunjwal and Robert W. Spekkens},
	year         = 2021,
	month        = {feb},
	journal      = {{PRX} Quantum},
	publisher    = {American Physical Society ({APS})},
	volume       = 2,
	number       = 1,
	doi          = {10.1103/prxquantum.2.010331},
	url          = {https://doi.org/10.1103%2Fprxquantum.2.010331}
}
@article{shahandeh2019contextuality,
	title        = {Contextuality of General Probabilistic Theories},
	author       = {Farid Shahandeh},
	year         = 2021,
	month        = {feb},
	journal      = {{PRX} Quantum},
	publisher    = {American Physical Society ({APS})},
	volume       = 2,
	number       = 1,
	doi          = {10.1103/prxquantum.2.010330},
	url          = {https://doi.org/10.1103%2Fprxquantum.2.010330}
}
@article{masanes2019measurement,
	title        = {The measurement postulates of quantum mechanics are operationally redundant},
	author       = {Llu{\'{\i}}s Masanes and Thomas D. Galley and Markus P. M{\"u}ller},
	year         = 2019,
	month        = {mar},
	journal      = {Nature Communications},
	publisher    = {Springer Science and Business Media {LLC}},
	volume       = 10,
	number       = 1,
	doi          = {10.1038/s41467-019-09348-x},
	url          = {https://doi.org/10.1038%2Fs41467-019-09348-x}
}
@article{galley2017classification,
	title        = {Classification of all alternatives to the Born rule in terms of informational properties},
	author       = {Thomas D. Galley and Llu{\'\i}s Masanes},
	year         = 2017,
	month        = {jul},
	journal      = {Quantum},
	publisher    = {Verein zur Forderung des Open Access Publizierens in den Quantenwissenschaften},
	volume       = 1,
	pages        = 15,
	doi          = {10.22331/q-2017-07-14-15},
	url          = {https://doi.org/10.22331%2Fq-2017-07-14-15}
}
@article{galley2018any,
	title        = {Any modification of the Born rule leads to a violation of the purification and local tomography principles},
	author       = {Thomas D. Galley and Llu{\'\i}s Masanes},
	year         = 2018,
	month        = {nov},
	journal      = {Quantum},
	publisher    = {Verein zur Forderung des Open Access Publizierens in den Quantenwissenschaften},
	volume       = 2,
	pages        = 104,
	doi          = {10.22331/q-2018-11-06-104},
	url          = {https://doi.org/10.22331%2Fq-2018-11-06-104}
}
@article{galley2020dynamics,
	title        = {How dynamics constrains probabilities in general probabilistic theories},
	author       = {Thomas D. Galley and Llu{\'\i}s Masanes},
	year         = 2021,
	month        = {may},
	journal      = {Quantum},
	publisher    = {Verein zur Forderung des Open Access Publizierens in den Quantenwissenschaften},
	volume       = 5,
	pages        = 457,
	doi          = {10.22331/q-2021-05-21-457},
	url          = {https://doi.org/10.22331%2Fq-2021-05-21-457}
}
@article{dakic2014density,
	title        = {Density cubes and higher-order interference theories},
	author       = {B Daki{\'{c} } and T Paterek and {\v{C}} Brukner},
	year         = 2014,
	month        = {feb},
	journal      = {New Journal of Physics},
	publisher    = {{IOP} Publishing},
	volume       = 16,
	number       = 2,
	pages        = {023028},
	doi          = {10.1088/1367-2630/16/2/023028},
	url          = {https://doi.org/10.1088%2F1367-2630%2F16%2F2%2F023028}
}
@article{lee2017higher,
	title        = {Higher-Order Interference in Extensions of Quantum Theory},
	author       = {Ciar{\'{a}}n M. Lee and John H. Selby},
	year         = 2016,
	month        = oct,
	journal      = {Foundations of Physics},
	publisher    = {Springer Science and Business Media {LLC}},
	volume       = 47,
	number       = 1,
	pages        = {89--112},
	doi          = {10.1007/s10701-016-0045-4},
	url          = {https://doi.org/10.1007/s10701-016-0045-4}
}
@article{barnum2017ruling,
	title        = {Ruling out Higher-Order Interference from Purity Principles},
	author       = {Howard Barnum and Ciar{\'{a}}n Lee and Carlo Scandolo and John Selby},
	year         = 2017,
	month        = {jun},
	journal      = {Entropy},
	publisher    = {{MDPI} {AG}},
	volume       = 19,
	number       = 6,
	pages        = 253,
	doi          = {10.3390/e19060253},
	url          = {https://doi.org/10.3390%2Fe19060253}
}
@article{horvat2020interference,
	title        = {Interference as an information-theoretic game},
	author       = {Sebastian Horvat and Borivoje Daki{\'{c} }},
	year         = 2021,
	month        = {mar},
	journal      = {Quantum},
	publisher    = {Verein zur Forderung des Open Access Publizierens in den Quantenwissenschaften},
	volume       = 5,
	pages        = 404,
	doi          = {10.22331/q-2021-03-08-404},
	url          = {https://doi.org/10.22331%2Fq-2021-03-08-404}
}
@article{barnum2007generalized,
	title        = {Generalized No-Broadcasting Theorem},
	author       = {Howard Barnum and Jonathan Barrett and Matthew Leifer and Alexander Wilce},
	year         = 2007,
	month        = {dec},
	journal      = {Physical Review Letters},
	publisher    = {American Physical Society ({APS})},
	volume       = 99,
	number       = 24,
	doi          = {10.1103/physrevlett.99.240501},
	url          = {https://doi.org/10.1103%2Fphysrevlett.99.240501}
}
@inproceedings{barnum2012teleportation,
	title        = {{Teleportation in general probabilistic theories}},
	author       = {Barnum, Howard and Barrett, Jonathan and Leifer, Matthew and Wilce, Alexander},
	year         = 2012,
	booktitle    = {Proceedings of Symposia in Applied Mathematics},
	volume       = 71,
	pages        = {25--48},
	doi          = {10.48550/ARXIV.0805.3553},
	url          = {https://arxiv.org/abs/0805.3553}
}
@article{chiribella2011informational,
	title        = {Informational derivation of quantum theory},
	author       = {Giulio Chiribella and Giacomo Mauro D'Ariano and Paolo Perinotti},
	year         = 2011,
	month        = {jul},
	journal      = {Physical Review A},
	publisher    = {American Physical Society ({APS})},
	volume       = 84,
	number       = 1,
	doi          = {10.1103/physreva.84.012311},
	url          = {https://doi.org/10.1103%2Fphysreva.84.012311}
}
@article{chiribella2017microcanonical,
	title        = {Microcanonical thermodynamics in general physical theories},
	author       = {Giulio Chiribella and Carlo Maria Scandolo},
	year         = 2017,
	month        = {dec},
	journal      = {New Journal of Physics},
	publisher    = {{IOP} Publishing},
	volume       = 19,
	number       = 12,
	pages        = 123043,
	doi          = {10.1088/1367-2630/aa91c7},
	url          = {https://doi.org/10.1088%2F1367-2630%2Faa91c7}
}
@article{chiribella2014distinguishability,
	title        = {{Distinguishability and copiability of programs in general process theories}},
	author       = {Chiribella, Giulio},
	year         = 2014,
	journal      = {arXiv preprint arXiv:1411.3035}
}
@misc{czekaj2020correlations,
	title        = {Correlations constrained by composite measurements},
	author       = {Czekaj, Lukasz and Sainz, Ana Belén and Selby, John and Horodecki, Michal},
	year         = 2020,
	publisher    = {arXiv},
	doi          = {10.48550/ARXIV.2009.04994},
	url          = {https://arxiv.org/abs/2009.04994},
	copyright    = {arXiv.org perpetual, non-exclusive license},
}
@article{muller2012structure,
	title        = {Structure of Reversible Computation Determines the Self-Duality of Quantum Theory},
	author       = {M{\"u}ller, Markus P. and Ududec, Cozmin},
	year         = 2012,
	month        = {Mar},
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 108,
	pages        = 130401,
	doi          = {10.1103/PhysRevLett.108.130401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.108.130401},
	issue        = 13,
	numpages     = 5
}
@article{masanes2011derivation,
	title        = {{A derivation of quantum theory from physical requirements}},
	author       = {Masanes, Llu{\'\i}s and M{\"u}ller, Markus P},
	year         = 2011,
	journal      = {New Journal of Physics},
	publisher    = {IOP Publishing},
	volume       = 13,
	number       = 6,
	pages        = {063001}
}
@article{wilce2011symmetry,
	title        = {{Symmetry and composition in probabilistic theories}},
	author       = {Wilce, Alexander},
	year         = 2011,
	journal      = {Electronic Notes in Theoretical Computer Science},
	publisher    = {Elsevier},
	volume       = 270,
	number       = 2,
	pages        = {191--207}
}
@article{barnum2013symmetry,
	title        = {{Symmetry, compact closure and dagger compactness for categories of convex operational models}},
	author       = {Barnum, Howard and Duncan, Ross and Wilce, Alexander},
	year         = 2013,
	journal      = {Journal of Philosophical Logic},
	publisher    = {Springer},
	volume       = 42,
	number       = 3,
	pages        = {501--523}
}
@article{wilce2018royal,
	title        = {{A royal road to quantum theory (or thereabouts)}},
	author       = {Wilce, Alexander},
	year         = 2018,
	journal      = {Entropy},
	publisher    = {Multidisciplinary Digital Publishing Institute},
	volume       = 20,
	number       = 4,
	pages        = 227
}
@article{wilce2009four,
	title        = {{Four and a half axioms for finite dimensional quantum mechanics}},
	author       = {Wilce, Alexander},
	year         = 2009,
	journal      = {arXiv preprint arXiv:0912.5530}
}
@article{barnum2014local,
	title        = {{Local tomography and the Jordan structure of quantum theory}},
	author       = {Barnum, Howard and Wilce, Alexander},
	year         = 2014,
	journal      = {Foundations of Physics},
	publisher    = {Springer},
	volume       = 44,
	number       = 2,
	pages        = {192--212}
}
@article{weilenmann2020analysing,
	title        = {Analysing causal structures in generalised probabilistic theories},
	author       = {Mirjam Weilenmann and Roger Colbeck},
	year         = 2020,
	month        = {feb},
	journal      = {Quantum},
	publisher    = {Verein zur Forderung des Open Access Publizierens in den Quantenwissenschaften},
	volume       = 4,
	pages        = 236,
	doi          = {10.22331/q-2020-02-27-236},
	url          = {https://doi.org/10.22331%2Fq-2020-02-27-236}
}
@article{scandolo2018possible,
	title        = {Universal structure of objective states in all fundamental causal theories},
	author       = {Carlo Maria Scandolo and Roberto Salazar and Jaros{\l}aw K. Korbicz and Pawe{\l} Horodecki},
	year         = 2021,
	month        = {aug},
	journal      = {Physical Review Research},
	publisher    = {American Physical Society ({APS})},
	volume       = 3,
	number       = 3,
	doi          = {10.1103/physrevresearch.3.033148},
	url          = {https://doi.org/10.1103%2Fphysrevresearch.3.033148}
}
@article{chiribella2014dilation,
	title        = {{Dilation of states and processes in operational-probabilistic theories}},
	author       = {Chiribella, Giulio},
	year         = 2014,
	journal      = {arXiv preprint arXiv:1412.8539}
}
@article{chiribella2014measurement,
	title        = {{Measurement sharpness cuts nonlocality and contextuality in every physical theory}},
	author       = {Chiribella, Giulio and Yuan, Xiao},
	year         = 2014,
	journal      = {arXiv preprint arXiv:1404.3348}
}
@article{chiribella2015entanglement,
	title        = {{Entanglement and thermodynamics in general probabilistic theories}},
	author       = {Chiribella, Giulio and Scandolo, Carlo Maria},
	year         = 2015,
	journal      = {New Journal of Physics},
	publisher    = {IOP Publishing},
	volume       = 17,
	number       = 10,
	pages        = 103027
}
@article{barnum2013ensemble,
	title        = {{Ensemble Steering, Weak Self-Duality, and the Structure of Probabilistic Theories}},
	author       = {Barnum, Howard and Gaebler, Carl Philipp and Wilce, Alexander},
	year         = 2013,
	month        = dec,
	journal      = {Found. Phys.},
	publisher    = {Springer US},
	volume       = 43,
	number       = 12,
	pages        = {1411--1427},
	doi          = {10.1007/s10701-013-9752-2},
	issn         = {1572-9516}
}
@article{barnum2010local,
	title        = {Local Quantum Measurement and No-Signaling Imply Quantum Correlations},
	author       = {Barnum, H. and Beigi, S. and Boixo, S. and Elliott, M. B. and Wehner, S.},
	year         = 2010,
	month        = {Apr},
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society},
	volume       = 104,
	pages        = 140401,
	doi          = {10.1103/PhysRevLett.104.140401},
	url          = {https://link.aps.org/doi/10.1103/PhysRevLett.104.140401},
	issue        = 14,
	numpages     = 4
}
@article{barnum2010entropy,
	title        = {Entropy and information causality in general probabilistic theories},
	author       = {Howard Barnum and Jonathan Barrett and Lisa Orloff Clark and Matthew Leifer and Robert Spekkens and Nicholas Stepanik and Alex Wilce and Robin Wilke},
	year         = 2010,
	month        = {mar},
	journal      = {New Journal of Physics},
	publisher    = {{IOP} Publishing},
	volume       = 12,
	number       = 3,
	pages        = {033024},
	doi          = {10.1088/1367-2630/12/3/033024},
	url          = {https://doi.org/10.1088%2F1367-2630%2F12%2F3%2F033024}
}
@article{masanes2013existence,
	title        = {{Existence of an information unit as a postulate of quantum theory}},
	author       = {Masanes, Llu{\'\i}s and M{\"u}ller, Markus P and Augusiak, Remigiusz and P{\'e}rez-Garc{\'\i}a, David},
	year         = 2013,
	journal      = {Proceedings of the National Academy of Sciences},
	publisher    = {National Acad Sciences},
	volume       = 110,
	number       = 41,
	pages        = {16373--16377}
}
@article{barnum2015entropy,
	title        = {Entropy, majorization and thermodynamics in general probabilistic theories},
	author       = {Howard Barnum and Jonathan Barrett and Marius Krumm and Markus P. M{\"u}ller},
	year         = 2015,
	month        = {nov},
	journal      = {Electronic Proceedings in Theoretical Computer Science},
	publisher    = {Open Publishing Association},
	volume       = 195,
	pages        = {43--58},
	doi          = {10.4204/eptcs.195.4},
	url          = {https://doi.org/10.4204%2Feptcs.195.4}
}
@article{mueller2013three,
	title        = {{Three-dimensionality of space and the quantum bit: an information-theoretic approach}},
	author       = {M{\"u}ller , Markus P and Masanes, Llu{\'\i}s},
	year         = 2013,
	journal      = {New Journal of Physics},
	publisher    = {IOP Publishing},
	volume       = 15,
	number       = 5,
	pages        = {053040}
}
@article{goldin1995nonlinear,
	title        = {{Nonlinear Schr\"odinger Equations and the Separation Property}},
	author       = {Gerald   A.   Goldin  and  George   Svetlichny},
	year         = 1995,
	journal      = {Journal of Nonlinear Mathematical Physics},
	publisher    = {Taylor & Francis},
	volume       = 2,
	number       = 2,
	pages        = {120--132},
	doi          = {10.2991/jnmp.1995.2.2.3},
	url          = {https://doi.org/10.2991/jnmp.1995.2.2.3},
	eprint       = {https://doi.org/10.2991/jnmp.1995.2.2.3}
}
@article{gisin_1990_weinberg,
	title        = {{Weinberg's non-linear quantum mechanics and supraluminal communications}},
	author       = {N. Gisin},
	year         = 1990,
	journal      = {Physics Letters A},
	volume       = 143,
	number       = 1,
	pages        = {1--2},
	doi          = {https://doi.org/10.1016/0375-9601(90)90786-N},
	issn         = {0375-9601},
	url          = {http://www.sciencedirect.com/science/article/pii/037596019090786N}
}
@article{helou_2017_extensions,
	title        = {{Extensions of Born's rule to non-linear quantum mechanics, some of which do not imply superluminal communication}},
	author       = {Bassam Helou and Yanbei Chen},
	year         = 2017,
	month        = {aug},
	journal      = {Journal of Physics: Conference Series},
	publisher    = {{IOP} Publishing},
	volume       = 880,
	pages        = {012021},
	doi          = {10.1088/1742-6596/880/1/012021},
	url          = {https://doi.org/10.1088%2F1742-6596%2F880%2F1%2F012021}
}
@article{weinberg_1989_testing,
	title        = {{Testing quantum mechanics}},
	author       = {Steven Weinberg},
	year         = 1989,
	journal      = {Annals of Physics},
	volume       = 194,
	number       = 2,
	pages        = {336--386},
	doi          = {https://doi.org/10.1016/0003-4916(89)90276-5},
	issn         = {0003-4916},
	url          = {http://www.sciencedirect.com/science/article/pii/0003491689902765}
}
@article{beltrametti1995classical,
	title        = {{A classical extension of quantum mechanics}},
	author       = {E G Beltrametti and S Bugajski},
	year         = 1995,
	month        = {jun},
	journal      = {Journal of Physics A: Mathematical and General},
	publisher    = {{IOP} Publishing},
	volume       = 28,
	number       = 12,
	pages        = {3329--3343},
	doi          = {10.1088/0305-4470/28/12/007},
	url          = {https://doi.org/10.1088%2F0305-4470%2F28%2F12%2F007}
}
@article{hall2012nonlocal,
	title        = {{Nonlocal signaling in the configuration space model of quantum-classical interactions}},
	author       = {Hall, Michael J. W. and Reginatto, Marcel and Savage, C. M.},
	year         = 2012,
	month        = {Nov},
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 86,
	pages        = {054101},
	doi          = {10.1103/PhysRevA.86.054101},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.86.054101},
	issue        = 5,
	numpages     = 3
}
@article{reginatto2009quantum,
	title        = {{Quantum-classical interactions and measurement: a consistent description using statistical ensembles on configuration space}},
	author       = {M Reginatto and M J W Hall},
	year         = 2009,
	month        = {jun},
	journal      = {Journal of Physics: Conference Series},
	publisher    = {{IOP} Publishing},
	volume       = 174,
	pages        = {012038},
	doi          = {10.1088/1742-6596/174/1/012038},
	url          = {https://doi.org/10.1088%2F1742-6596%2F174%2F1%2F012038}
}
@book{hall2016ensembles,
	title        = {{Ensembles on Configuration Space: Classical, Quantum, and Beyond}},
	author       = {Hall, M.J.W. and Reginatto, M.},
	year         = 2016,
	publisher    = {Springer International Publishing},
	series       = {Fundamental Theories of Physics},
	isbn         = 9783319341668,
	url          = {https://books.google.ca/books?id=NQxkDAAAQBAJ}
}
@article{bialynicki1976nonlinear,
	title        = {{Nonlinear wave mechanics}},
	author       = {I Bialynicki-Birula and J Mycielski},
	year         = 1976,
	journal      = {Ann. Phys. (NY)},
	volume       = 100,
	pages        = {62–93}
}
@article{mielnik1974,
	title        = {{Generalized quantum mechanics}},
	author       = {Mielnik, Bogdan},
	year         = 1974,
	journal      = {Comm. Math. Phys.},
	publisher    = {Springer},
	volume       = 37,
	number       = 3,
	pages        = {221--256},
	url          = {https://projecteuclid.org:443/euclid.cmp/1103859881},
	fjournal     = {Communications in Mathematical Physics}
}
@article{marshman2020locality,
	title        = {{Locality and entanglement in table-top testing of the quantum nature of linearized gravity}},
	author       = {Marshman, Ryan J and Mazumdar, Anupam and Bose, Sougato},
	year         = 2020,
	journal      = {Physical Review A},
	publisher    = {APS},
	volume       = 101,
	number       = 5,
	pages        = {052110}
}
@article{posiewnik_category_1985,
	title        = {{Category theoretical construction of the figure of states}},
	author       = {Posiewnik, Andrzej},
	year         = 1985,
	month        = feb,
	journal      = {International Journal of Theoretical Physics},
	volume       = 24,
	number       = 2,
	pages        = {193--200},
	doi          = {10.1007/BF00672653},
	issn         = {0020-7748, 1572-9575},
	url          = {http://link.springer.com/10.1007/BF00672653},
	urldate      = {2021-07-28},
	language     = {en}
}
@article{mielnik_mobility_1980,
	title        = {{Mobility of nonlinear systems}},
	author       = {Mielnik, Bogdan},
	year         = 1980,
	month        = jan,
	journal      = {Journal of Mathematical Physics},
	volume       = 21,
	number       = 1,
	pages        = {44--54},
	doi          = {10.1063/1.524331},
	issn         = {0022-2488, 1089-7658},
	url          = {http://aip.scitation.org/doi/10.1063/1.524331},
	urldate      = {2021-07-28},
	language     = {en}
}
@article{haag_comments_1978,
	title        = {{Comments on Mielnik's generalized (non linear) quantum mechanics}},
	author       = {Haag, Rudolf and Bannier, Ulrich},
	year         = 1978,
	month        = feb,
	journal      = {Communications in Mathematical Physics},
	volume       = 60,
	number       = 1,
	pages        = {1--6},
	doi          = {10.1007/BF01609470},
	issn         = {0010-3616, 1432-0916},
	url          = {http://link.springer.com/10.1007/BF01609470},
	urldate      = {2021-07-22},
	language     = {en}
}
@article{diosi1984gravitation,
	title        = {{Gravitation and quantum-mechanical localization of macro-objects}},
	author       = {L. Diósi},
	year         = 1984,
	journal      = {Physics Letters A},
	volume       = 105,
	number       = 4,
	pages        = {199--202},
	doi          = {https://doi.org/10.1016/0375-9601(84)90397-9},
	issn         = {0375-9601},
	url          = {https://www.sciencedirect.com/science/article/pii/0375960184903979}
}
@article{diosi1989models,
	title        = {{Models for universal reduction of macroscopic quantum fluctuations}},
	author       = {Di{\'o}si, Lajos},
	year         = 1989,
	journal      = {Phys. Rev. A},
	publisher    = {APS},
	volume       = 40,
	number       = 3,
	pages        = 1165
}
@article{penrose1996gravity,
	title        = {{On gravity's role in quantum state reduction}},
	author       = {Penrose, Roger},
	year         = 1996,
	journal      = {Gen. Rel. Grav.},
	publisher    = {Springer},
	volume       = 28,
	number       = 5,
	pages        = {581--600}
}
@article{ghirardi1986unified,
	title        = {{Unified dynamics for microscopic and macroscopic systems}},
	author       = {Ghirardi, G. C. and Rimini, A. and Weber, T.},
	year         = 1986,
	month        = {Jul},
	journal      = {Phys. Rev. D},
	publisher    = {American Physical Society},
	volume       = 34,
	pages        = {470--491},
	doi          = {10.1103/PhysRevD.34.470},
	url          = {https://link.aps.org/doi/10.1103/PhysRevD.34.470},
	issue        = 2,
	numpages     = {0}
}
@article{ghirardi1990Markov,
	title        = {{Markov processes in Hilbert space and continuous spontaneous localization of systems of identical particles}},
	author       = {Ghirardi, Gian Carlo and Pearle, Philip and Rimini, Alberto},
	year         = 1990,
	month        = {Jul},
	journal      = {Phys. Rev. A},
	publisher    = {American Physical Society},
	volume       = 42,
	pages        = {78--89},
	doi          = {10.1103/PhysRevA.42.78},
	url          = {https://link.aps.org/doi/10.1103/PhysRevA.42.78},
	issue        = 1,
	numpages     = {0}
}
@article{Adler_2007,
	title        = {{Collapse models with non-white noises}},
	author       = {Stephen L Adler and Angelo Bassi},
	year         = 2007,
	month        = {nov},
	journal      = {J Phys A},
	publisher    = {{IOP} Publishing},
	volume       = 40,
	number       = 50,
	pages        = {15083--15098},
	doi          = {10.1088/1751-8113/40/50/012},
	url          = {https://doi.org/10.1088/1751-8113/40/50/012}
}
@article{Adler275,
	title        = {{Is Quantum Theory Exact?}},
	author       = {Adler, Stephen L. and Bassi, Angelo},
	year         = 2009,
	journal      = {Science},
	publisher    = {American Association for the Advancement of Science},
	volume       = 325,
	number       = 5938,
	pages        = {275--276},
	doi          = {10.1126/science.1176858},
	issn         = {0036-8075},
	url          = {https://science.sciencemag.org/content/325/5938/275},
	eprint       = {https://science.sciencemag.org/content/325/5938/275.full.pdf}
}
@article{bassi2003dynamical,
	title        = {{Dynamical reduction models}},
	author       = {Angelo Bassi and GianCarlo Ghirardi},
	year         = 2003,
	journal      = {Physics Reports},
	volume       = 379,
	number       = 5,
	pages        = {257--426},
	doi          = {https://doi.org/10.1016/S0370-1573(03)00103-0},
	issn         = {0370-1573},
	url          = {https://www.sciencedirect.com/science/article/pii/S0370157303001030}
}
@article{simon2001no,
	title        = {{No-signaling condition and quantum dynamics}},
	author       = {Simon, Christoph and Bu{\v{z}}ek, Vladim{\'\i}r and Gisin, Nicolas},
	year         = 2001,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 87,
	number       = 17,
	pages        = 170405
}
@article{vanMeter:2011xr,
	title        = {{Schrodinger-Newton 'collapse' of the wave function}},
	author       = {van Meter, J. R.},
	year         = 2011,
	journal      = {Class. Quant. Grav.},
	volume       = 28,
	pages        = 215013,
	doi          = {10.1088/0264-9381/28/21/215013},
	eprint       = {1105.1579},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{Anastopoulos:2013zya,
	title        = {{A Master Equation for Gravitational Decoherence: Probing the Textures of Spacetime}},
	author       = {Anastopoulos, C. and Hu, B. L.},
	year         = 2013,
	journal      = {Class. Quant. Grav.},
	volume       = 30,
	pages        = 165007,
	doi          = {10.1088/0264-9381/30/16/165007},
	eprint       = {1305.5231},
	archiveprefix = {arXiv},
	primaryclass = {gr-qc}
}
@article{blencowe2013effective,
	title        = {{Effective field theory approach to gravitationally induced decoherence}},
	author       = {Blencowe, MP},
	year         = 2013,
	journal      = {Phys. Rev. Lett.},
	publisher    = {APS},
	volume       = 111,
	number       = 2,
	pages        = {021302}
}
@article{anastopoulos2014problems,
	title        = {{Problems with the Newton--Schr\"odinger equations}},
	author       = {Anastopoulos, C and Hu, BL},
	year         = 2014,
	journal      = {New J. Phys.},
	publisher    = {IOP Publishing},
	volume       = 16,
	number       = 8,
	pages        = {085007}
}
@article{bassi2017gravitational,
	title        = {{Gravitational decoherence}},
	author       = {Bassi, Angelo and Gro{\ss}ardt, Andr{\'e} and Ulbricht, Hendrik},
	year         = 2017,
	journal      = {Class. Quant. Grav.},
	publisher    = {IOP Publishing},
	volume       = 34,
	number       = 19,
	pages        = 193002
}
@misc{palmer2020discretisation,
	title        = {{Discretisation of the Bloch Sphere, Fractal Invariant Sets and Bell's Theorem}},
	author       = {T. N. Palmer},
	year         = 2020,
	journal      = {arXiv preprint arXiv:1804.01734},
	eprint       = {1804.01734},
	archiveprefix = {arXiv},
	primaryclass = {quant-ph}
}
@article{Janotta_2011,
	title        = {{Limits on nonlocal correlations from the structure of the local state space}},
	author       = {Janotta, Peter and Gogolin, Christian and Barrett, Jonathan and Brunner, Nicolas},
	year         = 2011,
	month        = {Jun},
	journal      = {New Journal of Physics},
	publisher    = {IOP Publishing},
	volume       = 13,
	number       = 6,
	pages        = {063024},
	doi          = {10.1088/1367-2630/13/6/063024},
	issn         = {1367-2630},
	url          = {http://dx.doi.org/10.1088/1367-2630/13/6/063024}
}
@article{Buniy_2005,
	title        = {{Is Hilbert space discrete?}},
	author       = {Buniy, Roman V. and Hsu, Stephen D.H. and Zee, A.},
	year         = 2005,
	month        = {Dec},
	journal      = {Physics Letters B},
	publisher    = {Elsevier BV},
	volume       = 630,
	number       = {1-2},
	pages        = {68–72},
	doi          = {10.1016/j.physletb.2005.09.084},
	issn         = {0370-2693},
	url          = {http://dx.doi.org/10.1016/j.physletb.2005.09.084}
}
@article{Muller_2009,
	title        = {{Does probability become fuzzy in small regions of spacetime?}},
	author       = {M{\"u}ller, Markus},
	year         = 2009,
	month        = {Mar},
	journal      = {Physics Letters B},
	publisher    = {Elsevier BV},
	volume       = 673,
	number       = 2,
	pages        = {166–167},
	doi          = {10.1016/j.physletb.2009.02.017},
	issn         = {0370-2693},
	url          = {http://dx.doi.org/10.1016/j.physletb.2009.02.017}
}
@article{Muller_2012,
	title        = {{The black hole information problem beyond quantum theory}},
	author       = {M{\"u}ller, Markus P. and Oppenheim, Jonathan and Dahlsten, Oscar C.O.},
	year         = 2012,
	month        = {Sep},
	journal      = {Journal of High Energy Physics},
	publisher    = {Springer Science and Business Media LLC},
	volume       = 2012,
	number       = 9,
	doi          = {10.1007/jhep09(2012)116},
	issn         = {1029-8479},
	url          = {http://dx.doi.org/10.1007/JHEP09(2012)116}
}
@misc{masanes_communication,
	author       = {Masanes, Llu{\'\i}s},
	howpublished = {personal communication}
}
@article{Donoghue:2017pgk,
	title        = {{EPFL Lectures on General Relativity as a Quantum Field Theory}},
	author       = {Donoghue, John F. and Ivanov, Mikhail M. and Shkerin, Andrey},
	year         = 2017,
	journal      = {arXiv preprint arXiv:1702.00319},
	archiveprefix = {arXiv},
	primaryclass = {hep-th},
	reportnumber = {INR-TH-2017-001}
}
@article{gross_2010,
	title        = {{All Reversible Dynamics in Maximally Nonlocal Theories are Trivial}},
	author       = {Gross, David and M{\"u}ller, Markus and Colbeck, Roger and Dahlsten, Oscar C. O.},
	year         = 2010,
	month        = {Feb},
	journal      = {Physical Review Letters},
	publisher    = {American Physical Society (APS)},
	volume       = 104,
	number       = 8,
	doi          = {10.1103/physrevlett.104.080402},
	issn         = {1079-7114},
	url          = {http://dx.doi.org/10.1103/PhysRevLett.104.080402}
}
@article{aubrun2021entanglement,
	title        = {Entanglement and Superposition Are Equivalent Concepts in Any Physical Theory},
	author       = {Guillaume Aubrun and Ludovico Lami and Carlos Palazuelos and Martin Pl{\'{a} }vala},
	year         = 2022,
	month        = {apr},
	journal      = {Phys. Rev. Lett.},
	publisher    = {American Physical Society ({APS})},
	volume       = 128,
	number       = 16,
	doi          = {10.1103/physrevlett.128.160402},
	url          = {https://doi.org/10.1103%2Fphysrevlett.128.160402}
}
@article{alsafi_2014,
	title        = {{Reversible dynamics in strongly non-local Boxworld systems}},
	author       = {Al-Safi, Sabri W and Short, Anthony J},
	year         = 2014,
	month        = {Jul},
	journal      = {Journal of Physics A: Mathematical and Theoretical},
	publisher    = {IOP Publishing},
	volume       = 47,
	number       = 32,
	pages        = 325303,
	doi          = {10.1088/1751-8113/47/32/325303},
	issn         = {1751-8121},
	url          = {http://dx.doi.org/10.1088/1751-8113/47/32/325303}
}
@misc{giacomini2020einstein,
	title        = {Einstein's Equivalence principle for superpositions of gravitational fields and quantum reference frames},
	author       = {Giacomini, Flaminia and Brukner, Caslav},
	year         = 2020,
	publisher    = {arXiv},
	doi          = {10.48550/ARXIV.2012.13754},
	url          = {https://arxiv.org/abs/2012.13754},
	copyright    = {arXiv.org perpetual, non-exclusive license}
}


==> preamble.tex <==
\RequirePackage{etex}
%\RequirePackage{doi}
\usepackage{rotating}
\usepackage{floatpag}
\rotfloatpagestyle{empty}
%\renewcommand{\theenumi}{\arabic{enumi}}
%\setcounter{tocdepth}{4}

%\newcommand{\showoptional}{1}
%\newcommand{\ismain}{0}

%\usepackage{hyperref}
%\font\omding=omding
\usepackage{dsfont}
%\usepackage{amsmath,amsthm,amssymb}
\usepackage{xspace,enumerate,epsfig}%color,
\usepackage{graphicx}
\graphicspath{{.}{./figures/}}
%\usepackage{marvosym}

\usepackage{tikzfig}
\usepackage{stmaryrd}
\usepackage{docmute}
\usepackage{keycommand}

\pgfplotsset{compat=newest}

\input{defs.tex}
\input{tikzstyles.tex}
%\input{tikzfigures.tex}

%\newcommand{\alert}[1]{{\color{red}#1}}
%\let\olddagger\dagger
%\renewcommand{\dagger}{\ensuremath{\oldd%agger}\xspace}

% indexes
% uncomment the relevant set of commands

% for a single index
%\usepackage{makeidx}
%\makeindex

% for multiple indexes using multind.sty
  % \usepackage{multind}\ProvidesPackage{multind}
  % \makeindex{authors}
  % \makeindex{subject}

% for multiple indexes using index.sty
% \usepackage{index}
% \newindex{aut}{adx}{and}{Author index}
% \makeindex

%\newcommand\cambridge{cambridge6A}




\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}\par\noindent}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}\par\noindent}
%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}\par\noindent}
\newcommand{\beqa}{\begin{eqnarray*}}
\newcommand{\eeqa}{\end{eqnarray*}\par\noindent}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}\par\noindent}
%end Bob's

\definecolor{quantumviolet}{RGB}{79, 4, 134}
\definecolor{quantumgray}{RGB}{134,79,4}
\definecolor{higherorderred}{RGB}{134,0,0}
\definecolor{higherordergreen}{RGB}{0,134,0}

% hide certain colours

% \def\bR{\begin{color}{black}}
% \def\bB{\begin{color}{black}}
% \def\bM{\begin{color}{black}}
% \def\bC{\begin{color}{black}}
% \def\bW{\begin{color}{black}}
% \def\bG{\begin{color}{black}}
% \def\bY{\begin{color}{black}}
    
    % \def\jR{\begin{color}{DarkRed}}
    % \def\jB{\begin{color}{MidnightBlue}}
    % \def\jM{\begin{color}{magenta}}
    % \def\jC{\begin{color}{cyan}}
    % \def\jW{\begin{color}{white}}
    % \def\jBl{\begin{color}{black}}
    % \def\jG{\begin{color}{green}}
    % \def\jY{\begin{color}{yellow}}
    
    % \def\cR{\begin{color}{Crimson}}
    % \def\cB{\begin{color}{cyan}}
    % \def\cM{\begin{color}{magenta}}
    % \def\cC{\begin{color}{cyan}}
    % \def\cW{\begin{color}{white}}
    % \def\cBl{\begin{color}{black}}
    % \def\cG{\begin{color}{green}}
    % \def\cY{\begin{color}{yellow}}
    % % hide certain colours

% \def\jR{\begin{color}{black}}
% \def\jB{\begin{color}{black}}
% \def\jM{\begin{color}{black}}
% \def\jC{\begin{color}{black}}
% \def\jW{\begin{color}{black}}
% \def\jG{\begin{color}{black}}
% \def\jY{\begin{color}{black}}


==> tikzstyles.tex <==
\usetikzlibrary{shapes.multipart}

\tikzstyle{bwSpider}=[
       rectangle split,
       rectangle split parts=2,
       rectangle split part fill={black,white},
 minimum size=3.6 mm, inner sep=-2mm, draw=black,scale=0.5,rounded corners=0.8 mm
       ]
 \tikzstyle{wbSpider}=[
       rectangle split,
       rectangle split parts=2,
       rectangle split part fill={white,black},
 minimum size=3.6 mm, inner sep=-2mm, draw=black,scale=0.5,rounded corners=0.8 mm
       ]
\tikzstyle{qWire}=[line width = 1pt, color=quantumviolet]
\tikzstyle{hWire}=[line width = 1.5pt, color=higherorderred]
\tikzstyle{sWire}=[line width = 2pt, color=higherordergreen]
\tikzstyle{cWire}=[color=quantumgray,thin]
\tikzstyle{rWire}=[color=black,thin]%[densely dotted, thick]

%MY GROUND:
\tikzstyle{env}=[copoint,regular polygon rotate=0,minimum width=0.2cm, fill=black]

\tikzstyle{probs}=[shape=semicircle,fill=white,draw=black,shape border rotate=180,minimum width=1.2cm]

%SIMON'S GROUND:
%
%\newcommand{\ground}[2]{
%\node[inner sep=0mm] (#1) at (#2) {};
%\draw[thick]  ($(#2)+(0.3,-0.01)$) -- ($(#2)+(-0.3,-0.01)$);
%\draw[thick]  ($(#2)+(0.23,0.069)$) -- ($(#2)+(-0.22,0.069)$);se
%\draw[thick]  ($(#2)+(0.16,0.139)$) -- ($(#2)+(-0.16,0.139)$);
%\draw[thick]  ($(#2)+(0.09,0.209)$) -- ($(#2)+(-0.09,0.209)$);
%\draw[thick]  ($(#2)+(0.02,0.279)$) -- ($(#2)+(-0.02,0.279)$);
%}
%
%\newcommand{\sground}[2]{
%\node[inner sep=0mm] (#1) at (#2) {};
%\draw[thick]  ($(#2)+(0.2,-0.01)$) -- ($(#2)+(-0.2,-0.01)$);
%\draw[thick]  ($(#2)+(0.12,0.069)$) -- ($(#2)+(-0.12,0.069)$);
%\draw[thick]  ($(#2)+(0.04,0.139)$) -- ($(#2)+(-0.04,0.139)$);
%}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzstyle{every picture}=[baseline=-0.25em,scale=.5]
\tikzstyle{dotpic}=[] % for backwards-compatibility
\tikzstyle{diredges}=[every to/.style={diredge}]
\tikzstyle{math matrix}=[matrix of math nodes,left delimiter=(,right delimiter=),inner sep=2pt,column sep=1em,row sep=0.5em,nodes={inner sep=0pt},text height=1.5ex, text depth=0.25ex]

% ==========
% = LABELS =
% ==========

\tikzstyle{inline text}=[text height=1.5ex, text depth=0.25ex,yshift=0.5mm]
\tikzstyle{label}=[font=\scriptsize,text height=1.5ex, text depth=0.25ex,yshift=0.0mm]%font=\footnotesize,yshift=0.5mm
\tikzstyle{left label}=[label,anchor=east,xshift=1.5mm]
\tikzstyle{right label}=[label,anchor=west,xshift=-1mm]

% create a white box of the given tikz size
%\newcommand{\phantombox}[1]{\tikz[baseline=(current bounding box).east]{\path [use as bounding box] (0,0) rectangle #1;}}
\tikzstyle{braceedge}=[decorate,decoration={brace,amplitude=2mm,raise=-1mm}]
\tikzstyle{small braceedge}=[decorate,decoration={brace,amplitude=1mm,raise=-1mm}]

\tikzstyle{doubled}=[line width=1.6pt] % set the line width for all doubled (quantum) maps/wires
\tikzstyle{boldedge}=[doubled,shorten <=-0.17mm,shorten >=-0.17mm]
\tikzstyle{boldedgegray}=[doubled,gray,shorten <=-0.17mm,shorten >=-0.17mm]
\tikzstyle{singleedgegray}=[gray]%,shorten <=-0.1mm,shorten >=-0.1mm]

\tikzstyle{semidoubled}=[line width=1.4pt] % set the line width for all doubled (quantum) maps/wires
\tikzstyle{semiboldedgegray}=[semidoubled,gray,shorten <=-0.17mm,shorten >=-0.17mm]

\tikzstyle{boxedge}=[semiboldedgegray]

\tikzstyle{boldedgedashed}=[very thick,dashed,shorten <=-0.17mm,shorten >=-0.17mm]
\tikzstyle{vboldedgedashed}=[doubled,dashed,shorten <=-0.17mm,shorten >=-0.17mm]
\tikzstyle{left hook arrow}=[left hook-latex]
\tikzstyle{right hook arrow}=[right hook-latex]
\tikzstyle{sembracket}=[line width=0.5pt,shorten <=-0.07mm,shorten >=-0.07mm]

\tikzstyle{causal edge}=[->,thick,gray]
\tikzstyle{causal nondir}=[thick,gray]
\tikzstyle{timeline}=[thick,gray, dashed]

% edges for (symmetric) correspondences/correlations
\tikzstyle{cedge}=[<->,thick,gray!70!white]

\tikzstyle{empty diagram}=[draw=gray!40!white,dashed,shape=rectangle,minimum width=1cm,minimum height=1cm]
\tikzstyle{empty diagram small}=[draw=gray!50!white,dashed,shape=rectangle,minimum width=0.6cm,minimum height=0.5cm]

\newcommand{\measurement}{\tikz[scale=0.6]{ \draw [use as bounding box,draw=none] (0,-0.1) rectangle (1,0.7); \draw [fill=white] (1,0) arc (0:180:5mm); \draw (0,0) -- (1,0) (0.5,0) -- +(60:7mm);}}

% ================
% = VARIOUS DOTS =
% ================

\tikzstyle{dot}=[inner sep=0mm,minimum width=2mm,minimum height=2mm,draw,shape=circle]
\tikzstyle{proj}=[trapezium, trapezium angle=67.5, draw, inner sep=1pt, outer sep=0pt, minimum height=6pt, minimum width=2pt,rotate=0,trapezium stretches=true]
\tikzstyle{inc}=[trapezium, trapezium angle=-67.5, draw, inner sep=1pt, outer sep=0pt, minimum height=6pt, minimum width=2pt,rotate=0,trapezium stretches=true]
\tikzstyle{coproj}=[trapezium, trapezium angle=-67.5, draw, inner sep=1pt, outer sep=0pt, minimum height=6pt, minimum width=2pt,rotate=0,trapezium stretches=true]
\tikzstyle{coinc}=[trapezium, trapezium angle=67.5, draw, inner sep=1pt, outer sep=0pt, minimum height=6pt, minimum width=2pt,rotate=0,trapezium stretches=true]
\tikzstyle{leak}=[white dot, shape=regular polygon, minimum size=3.3 mm, regular polygon sides=3, outer sep=-0.2mm, regular polygon rotate=270]
%\tikzstyle{proj}=[white dot, shape=regular polygon, minimum size=3.3 mm, regular polygon sides=4, outer sep=-0.2mm,rotate=45]
%\tikzstyle{proj}=[draw,fill=white,chamfered rectangle,chamfered rectangle angle=30, minimum width=2mm, minimum height= 1mm,scale=0.5, outer sep=-0.2mm]
\tikzstyle{wide proj}=[draw,fill=white,chamfered rectangle,chamfered rectangle angle=30, minimum width=15mm,minimum height=1mm,scale=0.5, outer sep=-0.2mm]
\tikzstyle{very wide proj}=[draw,fill=white,chamfered rectangle,chamfered rectangle angle=30, minimum width=25mm,minimum height=1mm,scale=0.5, outer sep=-0.2mm]
\tikzstyle{very very wide proj}=[draw,fill=white,chamfered rectangle,chamfered rectangle angle=30, minimum width=35mm,minimum height=1mm,scale=0.5, outer sep=-0.2mm]
\tikzstyle{preleak}=[proj]


\tikzstyle{split proj out}=[regular polygon,regular polygon sides=3,draw,scale=0.75,inner sep=-0.5pt,minimum width=3.3mm,fill=white,regular polygon rotate=180]
\tikzstyle{split proj in}=[regular polygon,regular polygon sides=3,draw,scale=0.75,inner sep=-0.5pt,minimum width=3.3mm,fill=white]
\tikzstyle{Vleak}=[white dot, shape=regular polygon, minimum size=3.3 mm, regular polygon sides=3, outer sep=-0.2mm, regular polygon rotate=90]
\tikzstyle{dleak}=[white dot, line width=1.6pt, shape=regular polygon, minimum size=3.3 mm, regular polygon sides=3, outer sep=-0.2mm, regular polygon rotate=270]

\tikzstyle{Wsquare}=[white dot, shape=regular polygon, rounded corners=0.8 mm, minimum size=3.3 mm, regular polygon sides=3, outer sep=-0.2mm]
\tikzstyle{Wsquareadj}=[white dot, shape=regular polygon, rounded corners=0.8 mm, minimum size=3.3 mm, regular polygon sides=3, outer sep=-0.2mm, regular polygon rotate=180]
% \tikzstyle{ddot}=[inner sep=0.6mm, double=white, very thick, double distance=1pt, minimum width=2.5mm,minimum height=2.5mm,draw,shape=circle]
\tikzstyle{ddot}=[inner sep=0mm, doubled, minimum width=2.5mm,minimum height=2.5mm,draw,shape=circle]

\tikzstyle{black dot}=[dot,fill=black]
\tikzstyle{white dot}=[dot,fill=white,,text depth=-0.2mm]
\tikzstyle{white Wsquare}=[Wsquare,fill=gray,,text depth=-0.2mm]
\tikzstyle{white Wsquareadj}=[Wsquareadj,fill=white,,text depth=-0.2mm]
\tikzstyle{green dot}=[white dot] % for backwards-compatibility
\tikzstyle{gray dot}=[dot,fill=gray!40!white,,text depth=-0.2mm]
\tikzstyle{red dot}=[gray dot] % for backwards-compatibility

% \tikzstyle{red point}=[point,fill=red,font=\color{white}]
% \tikzstyle{red dpoint}=[dpoint,fill=red,font=\color{white}]
% \tikzstyle{red dot}=[dot,fill=red,font=\color{white}]
% \tikzstyle{red ddot}=[ddot,fill=red,font=\color{white}]

\tikzstyle{black ddot}=[ddot,fill=black]
\tikzstyle{white ddot}=[ddot,fill=white]
\tikzstyle{gray ddot}=[ddot,fill=gray!40!white]


\tikzstyle{gray edge}=[gray!60!white]


\tikzstyle{small dot}=[inner sep=0.5mm,minimum width=0pt,minimum height=0pt,draw,shape=circle]

\tikzstyle{small black dot}=[small dot,fill=black]
\tikzstyle{small white dot}=[small dot,fill=white]
\tikzstyle{small gray dot}=[small dot,fill=gray!40!white]

\tikzstyle{causal dot}=[inner sep=0.4mm,minimum width=0pt,minimum height=0pt,draw=white,shape=circle,fill=gray!40!white]

%\tikzstyle{phase dimensions}=[font=\footnotesize,inner sep=0.5pt,minimum width=5mm,minimum height=5mm]

\tikzstyle{phase dimensions}=[minimum size=5mm,font=\footnotesize,rectangle,rounded corners=2.5mm,inner sep=0.2mm,outer sep=-2mm]
%,outer sep=-2mm,text height=1ex, text depth=0.25ex,
\tikzstyle{dphase dimensions}=[minimum size=5mm,font=\footnotesize,rectangle,rounded corners=2.5mm,inner sep=0.2mm,outer sep=-2mm]
%\tikzstyle{dphase dimensions}=[minimum size=5mm,font=\footnotesize,rectangle,rounded corners=2.5mm,inner sep=0.2mm,outer sep=-2mm]

\tikzstyle{white phase dot}=[dot,fill=white,phase dimensions]
\tikzstyle{white phase ddot}=[ddot,fill=white,dphase dimensions]

\tikzstyle{white rect ddot}=[draw=black,fill=white,doubled,minimum size=5mm,font=\footnotesize,rectangle,rounded corners=2.5mm,inner sep=0.2mm]
\tikzstyle{gray rect ddot}=[draw=black,fill=gray!40!white,doubled,minimum size=6mm,font=\footnotesize,rectangle,rounded corners=3mm]

\tikzstyle{gray phase dot}=[dot,fill=gray!40!white,phase dimensions]
\tikzstyle{gray phase ddot}=[ddot,fill=gray!40!white,dphase dimensions]
\tikzstyle{grey phase dot}=[gray phase dot]
\tikzstyle{grey phase ddot}=[gray phase ddot]

\tikzstyle{small phase dimensions}=[minimum size=4mm,font=\tiny,rectangle,rounded corners=2mm,inner sep=0.2mm,outer sep=-2mm]
\tikzstyle{small dphase dimensions}=[minimum size=4mm,font=\tiny,rectangle,rounded corners=2mm,inner sep=0.2mm,outer sep=-2mm]

\tikzstyle{small gray phase dot}=[dot,fill=gray!40!white,small phase dimensions]
\tikzstyle{small gray phase ddot}=[ddot,fill=gray!40!white,small dphase dimensions]

% =======================
% = OTHER KINDS OF MAPS =
% =======================

\tikzstyle{small map}=[draw,shape=rectangle,minimum height=4mm,minimum width=4mm,fill=white]

\tikzstyle{cnot}=[fill=white,shape=circle,inner sep=-1.4pt]

\tikzstyle{asym hadamard}=[fill=white,draw,shape=NEbox,inner sep=0.6mm,font=\footnotesize,minimum height=4mm]
\tikzstyle{asym hadamard conj}=[fill=white,draw,shape=NWbox,inner sep=0.6mm,font=\footnotesize,minimum height=4mm]
\tikzstyle{asym hadamard dag}=[fill=white,draw,shape=SEbox,inner sep=0.6mm,font=\footnotesize,minimum height=4mm]


\tikzstyle{hadamard}=[fill=white,draw,inner sep=0.6mm,font=\footnotesize,minimum height=4mm,minimum width=4mm]
\tikzstyle{small hadamard}=[fill=white,draw,inner sep=0.6mm,minimum height=1.5mm,minimum width=1.5mm]
\tikzstyle{small hadamard rotate}=[small hadamard,rotate=45]
\tikzstyle{dhadamard}=[hadamard,doubled]
\tikzstyle{small dhadamard}=[small hadamard,doubled]
\tikzstyle{small dhadamard rotate}=[small hadamard rotate,doubled]
\tikzstyle{antipode}=[white dot,inner sep=0.3mm,font=\footnotesize]

\tikzstyle{scalar}=[diamond,draw,inner sep=0.5pt,font=\small]
\tikzstyle{dscalar}=[diamond,doubled, draw,inner sep=0.5pt,font=\small]

\tikzstyle{small box}=[rectangle,inline text,fill=white,draw,minimum height=5mm,yshift=-0.5mm,minimum width=5mm,font=\small]
\tikzstyle{small gray box}=[small box,fill=gray!30]
\tikzstyle{medium box}=[rectangle,inline text,fill=white,draw,minimum height=5mm,yshift=-0.5mm,minimum width=10mm,font=\small]
\tikzstyle{square box}=[small box] % for backwards-compatibility
\tikzstyle{medium gray box}=[small box,fill=gray!30]
\tikzstyle{semilarge box}=[rectangle,inline text,fill=white,draw,minimum height=5mm,yshift=-0.5mm,minimum width=12.5mm,font=\small]
\tikzstyle{large box}=[rectangle,inline text,fill=white,draw,minimum height=5mm,yshift=-0.5mm,minimum width=15mm,font=\small]
\tikzstyle{large gray box}=[small box,fill=gray!30]

\tikzstyle{Bayes box}=[rectangle,fill=black,draw, minimum height=3mm, minimum width=3mm]

\tikzstyle{gray square point}=[small box,fill=gray!50]

\tikzstyle{dphase box white}=[dhadamard]
\tikzstyle{dphase box gray}=[dhadamard,fill=gray!50!white]
\tikzstyle{phase box white}=[hadamard]
\tikzstyle{phase box gray}=[hadamard,fill=gray!50!white]

% \tikzstyle{point}=[regular polygon,regular polygon sides=3,draw,inner sep=-0.65pt,minimum width=8mm,fill=white,regular polygon rotate=180]
% \tikzstyle{copoint}=[regular polygon,regular polygon sides=3,draw,inner sep=-0.65pt,minimum width=8mm,fill=white]
\tikzstyle{point}=[regular polygon,regular polygon sides=3,draw,scale=0.75,inner sep=-0.5pt,minimum width=9mm,fill=white,regular polygon rotate=180]
\tikzstyle{point nosep}=[regular polygon,regular polygon sides=3,draw,scale=0.75,inner sep=-2pt,minimum width=9mm,fill=white,regular polygon rotate=180]
\tikzstyle{copoint}=[regular polygon,regular polygon sides=3,draw,scale=0.75,inner sep=-0.5pt,minimum width=9mm,fill=white]
\tikzstyle{dpoint}=[point,doubled]
\tikzstyle{dcopoint}=[copoint,doubled]

\tikzstyle{pointgrow}=[shape=cornerpoint,kpoint common,scale=0.75,inner sep=3pt]
\tikzstyle{pointgrow dag}=[shape=cornercopoint,kpoint common,scale=0.75,inner sep=3pt]

\tikzstyle{wide copoint}=[fill=white,draw,shape=isosceles triangle,shape border rotate=90,isosceles triangle stretches=true,inner sep=0pt,minimum width=1.5cm,minimum height=6.12mm]
\tikzstyle{wide point}=[fill=white,draw,shape=isosceles triangle,shape border rotate=-90,isosceles triangle stretches=true,inner sep=0pt,minimum width=1.5cm,minimum height=6.12mm,yshift=-0.0mm]
\tikzstyle{wide point plus}=[fill=white,draw,shape=isosceles triangle,shape border rotate=-90,isosceles triangle stretches=true,inner sep=0pt,minimum width=1.74cm,minimum height=7mm,yshift=-0.0mm]

\tikzstyle{wide dpoint}=[fill=white,doubled,draw,shape=isosceles triangle,shape border rotate=-90,isosceles triangle stretches=true,inner sep=0pt,minimum width=1.5cm,minimum height=6.12mm,yshift=-0.0mm]

\tikzstyle{tinypoint}=[regular polygon,regular polygon sides=3,draw,scale=0.55,inner sep=-0.15pt,minimum width=6mm,fill=white,regular polygon rotate=180]

\tikzstyle{white point}=[point]
\tikzstyle{white dpoint}=[dpoint]
\tikzstyle{green point}=[white point] % for backwards-compatibility
\tikzstyle{white copoint}=[copoint]
\tikzstyle{gray point}=[point,fill=gray!40!white]
\tikzstyle{gray dpoint}=[gray point,doubled]
\tikzstyle{red point}=[gray point] % for backwards-compatibility
\tikzstyle{gray copoint}=[copoint,fill=gray!40!white]
\tikzstyle{gray dcopoint}=[gray copoint,doubled]

\tikzstyle{white point guide}=[regular polygon,regular polygon sides=3,font=\scriptsize,draw,scale=0.65,inner sep=-0.5pt,minimum width=9mm,fill=white,regular polygon rotate=180]

\tikzstyle{black point}=[point,fill=black,font=\color{white}]
\tikzstyle{black copoint}=[copoint,fill=black,font=\color{white}]

\tikzstyle{tiny gray point}=[tinypoint,fill=gray!40!white]

\tikzstyle{diredge}=[->]
\tikzstyle{ddiredge}=[<->]
\tikzstyle{rdiredge}=[<-]
\tikzstyle{thickdiredge}=[->, very thick]
\tikzstyle{pointer edge}=[->,very thick,gray]
\tikzstyle{pointer edge part}=[very thick,gray]
\tikzstyle{dashed edge}=[dashed]
\tikzstyle{thick dashed edge}=[very thick,dashed]
\tikzstyle{thick gray dashed edge}=[thick dashed edge,gray!40]
\tikzstyle{thick map edge}=[very thick,|->]

% =======================
% = PARALLELAGRAM BOXES =
% =======================

\makeatletter
\newcommand{\boxshape}[3]{%
\pgfdeclareshape{#1}{
\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{east}
% ... and possibly more
\backgroundpath{% this is new
% store lower right in xa/ya and upper right in xb/yb
\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y

\@tempdima=#2
\@tempdimb=#3

\pgfpathmoveto{\pgfpoint{\pgf@xa - 5pt + \@tempdima}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xa - 5pt - \@tempdima}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb + 5pt + \@tempdimb}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb + 5pt - \@tempdimb}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xa - 5pt + \@tempdima}{\pgf@ya}}
\pgfpathclose
}
}}

%\boxshape{NEbox}{0pt}{5pt}
\boxshape{NEbox}{0pt}{3pt}
%\boxshape{SEbox}{0pt}{-5pt}
\boxshape{SEbox}{0pt}{-3pt}
\boxshape{NWbox}{5pt}{0pt}
\boxshape{SWbox}{-5pt}{0pt}
\boxshape{EBox}{-3pt}{3pt}
\boxshape{WBox}{3pt}{-3pt}
\makeatother

\tikzstyle{cloud}=[shape=cloud,draw,minimum width=1.5cm,minimum height=1.5cm]

%\tikzstyle{map}=[draw,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{map}=[draw,shape=NEbox,inner sep=1pt,minimum height=4mm,fill=white]
\tikzstyle{dashedmap}=[draw,dashed,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white]
%\tikzstyle{mapdag}=[draw,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{mapdag}=[draw,shape=SEbox,inner sep=1pt,minimum height=4mm,fill=white]
\tikzstyle{mapadj}=[draw,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{maptrans}=[draw,shape=SWbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{mapconj}=[draw,shape=NWbox,inner sep=2pt,minimum height=6mm,fill=white]

\tikzstyle{medium map}=[draw,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=7mm]
\tikzstyle{medium map dag}=[draw,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=7mm]
\tikzstyle{medium map adj}=[draw,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=7mm]
\tikzstyle{medium map trans}=[draw,shape=SWbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=7mm]
\tikzstyle{medium map conj}=[draw,shape=NWbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=7mm]
\tikzstyle{semilarge map}=[draw,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=9.5mm]
\tikzstyle{semilarge map trans}=[draw,shape=SWbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=9.5mm]
\tikzstyle{semilarge map adj}=[draw,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=9.5mm]
\tikzstyle{semilarge map dag}=[draw,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=9.5mm]
\tikzstyle{semilarge map conj}=[draw,shape=NWbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=9.5mm]
\tikzstyle{large map}=[draw,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=12mm]
\tikzstyle{large map conj}=[draw,shape=NWbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=12mm]
\tikzstyle{very large map}=[draw,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=17mm]

\tikzstyle{medium dmap}=[draw,doubled,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=7mm]
\tikzstyle{medium dmap dag}=[draw,doubled,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=7mm]
\tikzstyle{medium dmap adj}=[draw,doubled,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=7mm]
\tikzstyle{medium dmap trans}=[draw,doubled,shape=SWbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=7mm]
\tikzstyle{medium dmap conj}=[draw,doubled,shape=NWbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=7mm]
\tikzstyle{semilarge dmap}=[draw,doubled,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=9.5mm]
\tikzstyle{semilarge dmap trans}=[draw,doubled,shape=SWbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=9.5mm]
\tikzstyle{semilarge dmap adj}=[draw,doubled,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=9.5mm]
\tikzstyle{semilarge dmap dag}=[draw,doubled,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=9.5mm]
\tikzstyle{semilarge dmap conj}=[draw,doubled,shape=NWbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=9.5mm]
\tikzstyle{large dmap}=[draw,doubled,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=12mm]
\tikzstyle{large dmap conj}=[draw,doubled,shape=NWbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=12mm]
\tikzstyle{large dmap trans}=[draw,doubled,shape=SWbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=12mm]
\tikzstyle{large dmap adj}=[draw,doubled,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=12mm]
\tikzstyle{large dmap dag}=[draw,doubled,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=12mm]
\tikzstyle{very large dmap}=[draw,doubled,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white,minimum width=19.5mm]

\tikzstyle{muxbox}=[draw,shape=rectangle,minimum height=3mm,minimum width=3mm,fill=white]
\tikzstyle{dmuxbox}=[muxbox,doubled]

\tikzstyle{box}=[draw,shape=rectangle,inner sep=2pt,minimum height=6mm,minimum width=6mm,fill=white]
\tikzstyle{dbox}=[draw,doubled,shape=rectangle,inner sep=2pt,minimum height=6mm,minimum width=6mm,fill=white]
\tikzstyle{dmap}=[draw,doubled,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{dmapdag}=[draw,doubled,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{dmapadj}=[draw,doubled,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{dmaptrans}=[draw,doubled,shape=SWbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{dmapconj}=[draw,doubled,shape=NWbox,inner sep=2pt,minimum height=6mm,fill=white]

\tikzstyle{ddmap}=[draw,doubled,dashed,shape=NEbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{ddmapdag}=[draw,doubled,dashed,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{ddmapadj}=[draw,doubled,dashed,shape=SEbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{ddmaptrans}=[draw,doubled,dashed,shape=SWbox,inner sep=2pt,minimum height=6mm,fill=white]
\tikzstyle{ddmapconj}=[draw,doubled,dashed,shape=NWbox,inner sep=2pt,minimum height=6mm,fill=white]

\boxshape{sNEbox}{0pt}{3pt}
\boxshape{sSEbox}{0pt}{-3pt}
\boxshape{sNWbox}{3pt}{0pt}
\boxshape{sSWbox}{-3pt}{0pt}
\tikzstyle{smap}=[draw,shape=sNEbox,fill=white]
\tikzstyle{smapdag}=[draw,shape=sSEbox,fill=white]
\tikzstyle{smapadj}=[draw,shape=sSEbox,fill=white]
\tikzstyle{smaptrans}=[draw,shape=sSWbox,fill=white]
\tikzstyle{smapconj}=[draw,shape=sNWbox,fill=white]

\tikzstyle{dsmap}=[draw,dashed,shape=sNEbox,fill=white]
\tikzstyle{dsmapdag}=[draw,dashed,shape=sSEbox,fill=white]
\tikzstyle{dsmaptrans}=[draw,dashed,shape=sSWbox,fill=white]
\tikzstyle{dsmapconj}=[draw,dashed,shape=sNWbox,fill=white]

\boxshape{mNEbox}{0pt}{10pt}
\boxshape{mSEbox}{0pt}{-10pt}
\boxshape{mNWbox}{10pt}{0pt}
\boxshape{mSWbox}{-10pt}{0pt}
\tikzstyle{mmap}=[draw,shape=mNEbox]
\tikzstyle{mmapdag}=[draw,shape=mSEbox]
\tikzstyle{mmaptrans}=[draw,shape=mSWbox]
\tikzstyle{mmapconj}=[draw,shape=mNWbox]

\tikzstyle{mmapgray}=[draw,fill=gray!40!white,shape=mNEbox]
\tikzstyle{smapgray}=[draw,fill=gray!40!white,shape=sNEbox]



\makeatletter

\pgfdeclareshape{cornerpoint}{
\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{east}
% ... and possibly more
\backgroundpath{% this is new
% store lower right in xa/ya and upper right in xb/yb
\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y

\pgfmathsetmacro{\pgf@shorten@left}{\pgfkeysvalueof{/tikz/shorten left}}
\pgfmathsetmacro{\pgf@shorten@right}{\pgfkeysvalueof{/tikz/shorten right}}

\pgfpathmoveto{\pgfpoint{0.5 * (\pgf@xa + \pgf@xb)}{\pgf@ya - 5pt}}
\pgfpathlineto{\pgfpoint{\pgf@xa - 8pt + \pgf@shorten@left}{\pgf@yb - 1.5 * \pgf@shorten@left}}
\pgfpathlineto{\pgfpoint{\pgf@xa - 8pt + \pgf@shorten@left}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb + 8pt - \pgf@shorten@right}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb + 8pt - \pgf@shorten@right}{\pgf@yb - 1.5 * \pgf@shorten@right}}
\pgfpathclose
}
}

\pgfdeclareshape{cornercopoint}{
\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{east}
% ... and possibly more
\backgroundpath{% this is new
% store lower right in xa/ya and upper right in xb/yb
\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y

\pgfmathsetmacro{\pgf@shorten@left}{\pgfkeysvalueof{/tikz/shorten left}}
\pgfmathsetmacro{\pgf@shorten@right}{\pgfkeysvalueof{/tikz/shorten right}}

\pgfpathmoveto{\pgfpoint{0.5 * (\pgf@xa + \pgf@xb)}{\pgf@yb + 5pt}}
\pgfpathlineto{\pgfpoint{\pgf@xa - 8pt + \pgf@shorten@left}{\pgf@ya + 1.5 * \pgf@shorten@left}}
\pgfpathlineto{\pgfpoint{\pgf@xa - 8pt + \pgf@shorten@left}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xb + 8pt - \pgf@shorten@right}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xb + 8pt - \pgf@shorten@right}{\pgf@ya + 1.5 * \pgf@shorten@right}}
\pgfpathclose
}
}

\makeatother

\pgfkeyssetvalue{/tikz/shorten left}{0pt}
\pgfkeyssetvalue{/tikz/shorten right}{0pt}



\tikzstyle{kpoint common}=[draw,fill=white,inner sep=1pt,minimum height=4mm]
\tikzstyle{kpoint sc}=[shape=cornerpoint,kpoint common]
\tikzstyle{kpoint adjoint sc}=[shape=cornercopoint,kpoint common]
\tikzstyle{kpoint}=[shape=cornerpoint,shorten left=5pt,kpoint common]
\tikzstyle{kpoint adjoint}=[shape=cornercopoint,shorten left=5pt,kpoint common]
\tikzstyle{kpoint conjugate}=[shape=cornerpoint,shorten right=5pt,kpoint common]
\tikzstyle{kpoint transpose}=[shape=cornercopoint,shorten right=5pt,kpoint common]
\tikzstyle{kpoint symm}=[shape=cornerpoint,shorten left=5pt,shorten right=5pt,kpoint common]

\tikzstyle{wide kpoint sc}=[shape=cornerpoint,kpoint common, minimum width=1 cm]
\tikzstyle{wide kpointdag sc}=[shape=cornercopoint,kpoint common, minimum width=1 cm]

\tikzstyle{black kpoint}=[shape=cornerpoint,shorten left=5pt,kpoint common,fill=black,font=\color{white}]

\tikzstyle{black kpoint sm}=[shape=cornerpoint,shorten left=5pt,kpoint common,fill=black,font=\color{white},scale=0.75]

\tikzstyle{black kpoint adjoint}=[shape=cornercopoint,shorten left=5pt,kpoint common,fill=black,font=\color{white}]
\tikzstyle{black kpointadj}=[shape=cornercopoint,shorten left=5pt,kpoint common,fill=black,font=\color{white}]

\tikzstyle{black kpointadj sm}=[shape=cornercopoint,shorten left=5pt,kpoint common,fill=black,font=\color{white},scale=0.75]

\tikzstyle{black dkpoint}=[shape=cornerpoint,shorten left=5pt,kpoint common,fill=black, doubled,font=\color{white}]
\tikzstyle{black dkpoint adjoint}=[shape=cornercopoint,shorten left=5pt,kpoint common,fill=black, doubled,font=\color{white}]
\tikzstyle{black dkpointadj}=[shape=cornercopoint,shorten left=5pt,kpoint common,fill=black, doubled,font=\color{white}]

\tikzstyle{black dkpoint sm}=[shape=cornerpoint,shorten left=5pt,kpoint common,fill=black, doubled,font=\color{white},scale=0.75]
\tikzstyle{black dkpointadj sm}=[shape=cornercopoint,shorten left=5pt,kpoint common,fill=black, doubled,font=\color{white},scale=0.75]

\tikzstyle{kpointdag}=[kpoint adjoint]
\tikzstyle{kpointadj}=[kpoint adjoint]
\tikzstyle{kpointconj}=[kpoint conjugate]
\tikzstyle{kpointtrans}=[kpoint transpose]

\tikzstyle{big kpoint}=[kpoint, minimum width=1.2 cm, minimum height=8mm, inner sep=4pt, text depth=3mm]

\tikzstyle{wide kpoint}=[kpoint, minimum width=1 cm, inner sep=2pt]%, text depth=-0.7 mm]
\tikzstyle{wide kpointdag}=[kpointdag, minimum width=1 cm, inner sep=2pt]%, text depth=0.7 mm]
\tikzstyle{wide kpointconj}=[kpointconj, minimum width=1 cm, inner sep=2pt]%, text depth=-0.7 mm]
\tikzstyle{wide kpointtrans}=[kpointtrans, minimum width=1 cm, inner sep=2pt]%, text depth=0.7 mm]

\tikzstyle{wider kpoint}=[kpoint, minimum width=1.25 cm, inner sep=2pt]%, text depth=-0.7 mm]
\tikzstyle{wider kpointdag}=[kpointdag, minimum width=1.25 cm, inner sep=2pt]%, text depth=0.7 mm]
\tikzstyle{wider kpointconj}=[kpointconj, minimum width=1.25 cm, inner sep=2pt]%, text depth=-0.7 mm]
\tikzstyle{wider kpointtrans}=[kpointtrans, minimum width=1.25 cm, inner sep=2pt]%, text depth=0.7 mm]

\tikzstyle{gray kpoint}=[kpoint,fill=gray!50!white]
\tikzstyle{gray kpointdag}=[kpointdag,fill=gray!50!white]
\tikzstyle{gray kpointadj}=[kpointadj,fill=gray!50!white]
\tikzstyle{gray kpointconj}=[kpointconj,fill=gray!50!white]
\tikzstyle{gray kpointtrans}=[kpointtrans,fill=gray!50!white]

\tikzstyle{gray dkpoint}=[kpoint,fill=gray!50!white,doubled]
\tikzstyle{gray dkpointdag}=[kpointdag,fill=gray!50!white,doubled]
\tikzstyle{gray dkpointadj}=[kpointadj,fill=gray!50!white,doubled]
\tikzstyle{gray dkpointconj}=[kpointconj,fill=gray!50!white,doubled]
\tikzstyle{gray dkpointtrans}=[kpointtrans,fill=gray!50!white,doubled]

\tikzstyle{white label}=[draw,fill=white,rectangle,inner sep=0.7 mm]
\tikzstyle{gray label}=[draw,fill=gray!50!white,rectangle,inner sep=0.7 mm]
\tikzstyle{black label}=[draw,fill=black,rectangle,inner sep=0.7 mm]

\tikzstyle{dkpoint}=[kpoint,doubled]
\tikzstyle{wide dkpoint}=[wide kpoint,doubled]
\tikzstyle{dkpointdag}=[kpoint adjoint,doubled]
\tikzstyle{wide dkpointdag}=[wide kpointdag,doubled]
\tikzstyle{dkcopoint}=[kpoint adjoint,doubled]
\tikzstyle{dkpointadj}=[kpoint adjoint,doubled]
\tikzstyle{dkpointconj}=[kpoint conjugate,doubled]
\tikzstyle{dkpointtrans}=[kpoint transpose,doubled]

\tikzstyle{kscalar}=[kpoint common, shape=EBox, inner xsep=-1pt, inner ysep=3pt,font=\small]
\tikzstyle{kscalarconj}=[kpoint common, shape=WBox, inner xsep=-1pt, inner ysep=3pt,font=\small]

\tikzstyle{spekpoint}=[kpoint sc,minimum height=5mm,inner sep=3pt]
\tikzstyle{spekcopoint}=[kpoint adjoint sc,minimum height=5mm,inner sep=3pt]

\tikzstyle{dspekpoint}=[spekpoint,doubled]
\tikzstyle{dspekcopoint}=[spekcopoint,doubled]

% ========================
% = GROUND =
% ========================


 \tikzstyle{upground}=[circuit ee IEC,thick,ground,rotate=90,scale=2.5]
 \tikzstyle{downground}=[circuit ee IEC,thick,ground,rotate=-90,scale=2.5]
 %\tikzstyle{ground}=[regular polygon,regular polygon sides=3,draw=gray,scale=0.50,inner sep=-0.5pt,minimum width=5mm,fill=gray]
 \tikzstyle{bigground}=[regular polygon,regular polygon sides=3,draw=gray,scale=0.50,inner sep=-0.5pt,minimum width=10mm,fill=gray]
 %\tikzstyle{grounddag}=[regular polygon,regular polygon sides=3,draw=gray,scale=0.50,inner sep=-0.5pt,minimum width=5mm,fill=gray,regular polygon rotate=180]

% ========================
% = COMMUTATIVE DIAGRAMS =
% ========================

\tikzstyle{arrs}=[-latex,font=\small,auto]
\tikzstyle{arrow plain}=[arrs]
\tikzstyle{arrow dashed}=[dashed,arrs]
\tikzstyle{arrow bold}=[very thick,arrs]
\tikzstyle{arrow hide}=[draw=white!0,-]
\tikzstyle{arrow reverse}=[latex-]
\tikzstyle{cdnode}=[]




